Nezha: Deployable and High-Performance Consensus Using Synchronized Clocks

This paper presents a high-performance consensus protocol, Nezha, which can be deployed by cloud tenants without any support from their cloud provider. Nezha bridges the gap between protocols such as Multi-Paxos and Raft, which can be readily deployed and protocols such as NOPaxos and Speculative Paxos, that provide better performance, but require access to technologies such as programmable switches and in-network prioritization, which cloud tenants do not have. Nezha uses a new multicast primitive called deadline-ordered multicast (DOM). DOM uses high-accuracy software clock synchronization to synchronize sender and receiver clocks. Senders tag messages with deadlines in synchronized time; receivers process messages in deadline order, on or after their deadline. We compare Nezha with Multi-Paxos, Fast Paxos, Raft, a NOPaxos version we optimized for the cloud, and 2 recent protocols, Domino and TOQ-EPaxos, that use synchronized clocks. In throughput, Nezha outperforms all baselines by a median of 5.4x (range: 1.9-20.9x). In latency, Nezha outperforms five baselines by a median of 2.3x (range: 1.3-4.0x), with one exception: it sacrifices 33% latency compared with our optimized NOPaxos in one test. We also prototype two applications, a key-value store and a fair-access stock exchange, on top of Nezha to show that Nezha only modestly reduces their performance relative to an unreplicated system. Nezha is available at https://github.com/Steamgjk/Nezha.

==> ablation_study.tex <==
\section{Ablation Study}
\label{sec-ablation-study}
As mentioned in \S\ref{sec-latency-throughput},
\sysname's outperformance comes from three main components. We conduct an ablation study to evaluate the effectiveness of each one. To be more specific, we remove one component from the full protocol each time, and yield three variants, shown as No-DOM, No-QC-Offloading, No-Commutativity in Figure~\ref{fig-ablation}. No-DOM variant removes the DOM primitive from \sysname, and \sysname essentially becomes Multi-Paxos with proxies doing the quorum check. No-QC-Offloading variant relies on the leader replica to do the quorum check, and it still relies on DOM for uniform ordering (the proxies with DOM-Ses conduct request mutlicast). No-Commutativity variant disables \sysname's commutativity optimization.

We run all protocols under the same setting, i.e. using 10 open-loop clients and 3 replicas, under the workload with read ratio of 50\% and skew factor of 0.5. 

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/exp/ablation-v2.pdf}
    \caption{Ablation study of \primname, quorum check offloading, and commutativity}
    \label{fig-ablation}
\end{figure}

Figure~\ref{fig-ablation} shows that, removing any of the three components can degrade the performance (i.e., throughput and/or latency). 

\begin{enumerate}[wide,label=(\arabic*)]
    \item The No-DOM variant makes the fast path meaningless, because uniform ordering is no longer guaranteed and set equality (i.e. reply messages with consistent hash) no longer indicates the state consistency among replicas. In this case, the NO-DOM variant actually becomes the Multi-Paxos protocol with quorum check offloading, and the leader replica still takes the responsibility of ordering and request multicast,  which makes No-DOM variant only yields a much lower throughput and higher latency. 

\item The No-QC-Offloading variant still uses DOM for ordering and request multicast, but it relies on the leader to do quorum check for every request. Therefore, the leader's burden becomes much heavier than the full protocol, and the heavy bottleneck at the leader replica degrades the throughput and latency performance.

\item The No-Commutativity variant degrades the fast commit ratio and causes more requests to commit via the slow path. It does not cause distinct impact on the throughput. However, compared with the full protocol,  the lack of commutativity optimization degrades the latency performance by up to \SI{32}{\percent}. Besides, we also evaluate the effectiveness of our commutativity optimization across different workloads, as presented in \S\ref{sec:extensive-eval}, which further proves that the commutativity optimization remains effective across different workloads.
\end{enumerate}





% \textbf{Effect of DOM.}

% \textbf{Effect of quorum check offloading.}


% \textbf{Effect of commutativity optimization.}

==> bk.tex <==
\section{Illustration of Message Delays in Different Protocols}
\label{sec-protocol-message-delay}
We illustrate the workflow for each of the protocols we listed in Table~\ref{tab:cmp}.


% \subsection{Multi-Paxos/Raft}
Multi-Paxos/Raft requires 4 message delays to commit a request (Figure~\ref{fig:mp-md}).
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/mp.pdf}
    \caption{Message Delay of Multi-Paxos}
    \label{fig:mp-md}
\end{figure}


% \subsection{Fast Paxos}
Fast Paxos requires 3 message delays to commit a request in the fast path (Figure~\ref{fig:fp-fast-md}) and 5 message delays in the slow path (Figure~\ref{fig:fp-slow-md}).
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/fp-fast.pdf}
    \caption{Message Delay of Fast Paxos (Fast Path)}
    \label{fig:fp-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/fp-slow.pdf}
    \caption{Message Delay of Fast Paxos (Slow Path)}
    \label{fig:fp-slow-md}
\end{figure}



% \subsection{Speculative Paxos}
Speculative Paxos requires 2 message delays to commit a request in the fast path (Figure~\ref{fig:spec-fast-md}) and 6 message delays in the slow path (Figure~\ref{fig:spec-slow-md}).
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/spec-fast.pdf}
    \caption{Message Delay of Speculative Paxos (Fast Path)}
    \label{fig:spec-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/spec-slow.pdf}
    \caption{Message Delay of Speculative Paxos (Slow Path)}
    \label{fig:spec-slow-md}
\end{figure}





% \subsection{NOPaxos}
NOPaxos requires 2 message delays to commit a request in the fast path (Figure~\ref{fig:nopaxos-fast-md}) and 4 message delays in the slow path (Figure~\ref{fig:nopaxos-slow-md}). Note that when the sequencer is a software sequencer (e.g., a standalone VM) instead of a hardware sequencer (e.g, programmable switch), there will be one extra message delay added to both the fast path and the slow path.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/message-delay-figs/nopaxos-fast.pdf}
    \caption{Message Delay of NOPaxos (Fast Path)}
    \label{fig:nopaxos-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/message-delay-figs/nopaxos-slow.pdf}
    \caption{Message Delay of NOPaxos (Slow Path)}
    \label{fig:nopaxos-slow-md}
\end{figure}



% \subsection{Mencius}
Mencius requires 4 message delays to commit a request in the fast path (Figure~\ref{fig:mencius-fast-md}) and 6 message delays in the slow path (Figure~\ref{fig:mencius-slow-md}), because the leader who is responsible to commit the request needs to take one extra round (2 message delays) to coordinate with the other leader replicas.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/mencius-fast.pdf}
    \caption{Message Delay of Mencius (Fast Path)}
    \label{fig:mencius-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/mencius-slow.pdf}
    \caption{Message Delay of Mencius (Slow Path)}
    \label{fig:mencius-slow-md}
\end{figure}


% \subsection{EPaxos}
EPaxos requires 4 message delays to commit a request in the fast path (Figure~\ref{fig:epaxos-fast-md}) and 6 message delays in the slow path (Figure~\ref{fig:epaxos-slow-md}).

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/epaxos-fast.pdf}
    \caption{Message Delay of EPaxos (Fast Path)}
    \label{fig:epaxos-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/epaxos-slow.pdf}
    \caption{Message Delay of EPaxos (Slow Path)}
    \label{fig:epaxos-slow-md}
\end{figure}



% \subsection{CURP}
CURP requires 2 message delays to commit a request in the fast path (Figure~\ref{fig:curp-fast-md}) and 4 message delays in the slow path (Figure~\ref{fig:curp-slow-md}).


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/curp-fast.pdf}
    \caption{Message Delay of CURP (Fast Path)}
    \label{fig:curp-fast-md}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=6cm]{figures/message-delay-figs/curp-slow.pdf}
    \caption{Message Delay of CURP (Slow Path)}
    \label{fig:curp-slow-md}
\end{figure}

==> brief-desciption.tex <==
\section{Comparative Description of Typical Consensus Protocols}
\label{sec-cmp-protocol}
In the following subsections, we aim to compare the protocols in a unified way, so we illustrate each protocol with 5 replicas, denoted as R1$\sim$R5, and 2 clients, denoted as C1 and C2. Except Multi-Paxos/Raft, the other protocols have both fast path and slow path. We distinguish the quorum of the two paths as fast quorum and slow quorum. Besides, for simplicity, we omit messages less relevant to the workflow and keeps the minimal set of messages (e.g. to satisfy the quorum) in the figure. 

\subsection{Multi-Paxos/Raft}
\label{sec-paxos-background}
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/Paxos-Normal.pdf}
    \caption{Multi-Paxos/Raft workflow}
    \label{Paxos-Normal}
\end{figure}
In Multi-Paxos/Raft, the workflow (shown in Figure~\ref{Paxos-Normal}) can be summarized as\\
\centerline{definitive ordering$\xrightarrow{}$replication$\xrightarrow{}$quorum check$\xrightarrow{}$execution}
The message flow follows\\ 
\centerline{client $\xrightarrow{}$ leader $\xrightarrow{}$ follower $\xrightarrow{}$ leader $\xrightarrow{}$ client}

The leader takes all the responsibility and makes itself a potential performance bottleneck, and it also costs more message delays (4 message delays) for the client to know the committed result. However, because of the centralized control from the leader, Multi-Paxos/Raft suffers from much less inconsistency penalty compared with the other protocols described below. Each replica follows the \emph{definitive ordering} to append and execute the requests. There is no concept of fast path and slow path in the design of Multi-Paxos/Raft.  
%So long as the leader is alive, the ordering decided by the leader is always correct and cannot be reverted. 


\subsection{NOPaxos}
\label{sec-nopaxos-background}

In NOPaxos, the workflow of the fast path (shown in Figure~\ref{NOPaxos-Fast}) can be summarized as\\
\centerline{definitive ordering$\xrightarrow{}$replication$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
The message flow follows \\
\centerline{client $\xrightarrow{}$ sequencer  $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client}
\begin{figure}[H]
    \centering
    \includegraphics[width=8cm]{figures/NoPaxos-Fast.pdf}
    \caption{NOPaxos workflow (fast path)}
    \label{NOPaxos-Fast}
\end{figure}


Unlike Multi-Paxos/Raft, NOPaxos offloads the ordering responsibility to an independent sequencer, which is implemented by either hardware (e.g. programmable switch) or software (e.g. a standalone server). Besides, it also offloads the responsibility of replication and quorum check (of the fast path) to the clients. The leader only does the quorum check (i.e. gap agreement) for the slow path. To keep correctness, NOPaxos enforces the constraints during quorum check: the client considers the request as committed after it receives the reply from a fast/slow quorum (3 replicas), and the quorum must include the leader. 

The design of NOPaxos much relieves the leader bottleneck, but brings more risk of inconsistency. Though each replica also uses the \emph{definitive ordering} like Multi-Paxos/Raft, the request reordering/drop from sequencer to the replicas can make replica states become inconsistent. Fortunately, the sequencer tags each request with a sequential number, which enables the replica to detect the inconsistency early when they receive requests with nonconsecutive sequential numbers.



\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/NoPaxos-Slow.pdf}
    \caption{NOPaxos workflow (slow path)}
    \label{NOPaxos-Slow}
\end{figure}
In Figure~\ref{NOPaxos-Slow}, we show a case when the leader (R3) experiences the reordering of C1's request and C2's request. To ensure consistency, the leader needs to take an extra round-trip time (2 message delays) to resolve the inconsistency (which is called gap agreement in NOPaxos design~\cite{osdi16-nopaxos}). The gap agreement subprotocol erases C1's request from the follower replicas and ensure that at least a slow quorum (3 replicas including leader) have consistent states. After resolving the inconsistency, the leader can move on to execute the request and reply to the client. In the case of Figure~\ref{NOPaxos-Slow}, C2's request is eventually committed, whereas C1's request is uncommitted, because it misses the reply from the leader.

\subsection{Fast Paxos}
\label{sec-fast-paxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/FastPaxos-Fast.pdf}
    \caption{Fast Paxos workflow (fast path)}
    \label{Fast-Paxos-Fast}
\end{figure}
In Fast Paxos, the workflow of the fast path (shown in Figure~\ref{Fast-Paxos-Fast}) can be summarized as\\
\centerline{replication$\xrightarrow{}$approx ordering$\xrightarrow{}$quorum check$\xrightarrow{}$execution}
The message flow follows \\
\centerline{client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ leader $\xrightarrow{}$ client}


Similar to NOPaxos, Fast Paxos also relies on clients to do the replication (i.e. the client broadcasts its request to every replica), but each replica uses \emph{approximate ordering} temporarily decided by itself to to append the request to its log list (according to the receiving order of requests). However, the \emph{approximate ordering} decided by each replica may be inconsistent, so they need to contact the leader to confirm the ordering consistency. Normally, each replica maintains the consistent ordering of the requests. After the leader ensures the consistency of a fast quorum (4 replicas including the leader itself), it executes the request and replies the result to the client. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/FastPaxos-Slow.pdf}
    \caption{Fast Paxos workflow (slow path)}
    \label{Fast-Paxos-Slow}
\end{figure}
The design of Fast Paxos is more aggressive than NOPaxos, since it does replication even before ordering. On the other hand, the inconsistency can only be detected later after the followers have appended the request and contacted the leader. In Figure~\ref{Fast-Paxos-Slow}, we show a case when 2 replicas (R4 and R5) have inconsistent states from the others, due to the reordering of C1's and C2's requests. After appending the requests, followers contact the leader (R3) for consistency confirmation, then R3 detects the inconsistency. Similar to NOPaxos, the leader needs to take an extra RTT to resolve the inconsistency and ensure consistency among at least a slow quorum (3 replicas including itself), before executing the request and replying to the client. 

\subsection{Speculative Paxos}
\label{sec-speculative-paxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/SpecPaxos-Fast.pdf}
    \caption{Speculative Paxos workflow (fast path)}
    \label{SpecPaxos-Fast}
\end{figure}
In Speculative Paxos, the  workflow of the fast path (shown in Figure~\ref{SpecPaxos-Fast}) can be summarized as\\
\centerline{replication$\xrightarrow{}$approx ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
The message flow follows \\
\centerline{client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client}
Speculative Paxos also relies on clients to do the replication. Similar to Fast Paxos, each replica in Speculative Paxos also uses \emph{approximate ordering} decided by each replica. But unlike Fast Paxos, Speculative Paxos takes more aggressive (and risky) actions and makes each replica immediately execute the request and reply to the client. In the reply, the replica includes the execution result of the request, as well as a hash value indicating the system state of the replica. In the fast path, the client considers the request as committed after receiving a fast quorum (4 replicas) of replies with the same hash value.

The design of Speculative Paxos can achieve the optimal latency in the fast path, but it suffers from very costly penalty in the slow path. Unlike Fast Paxos, the fast path of NOPaxos runs in a leaderless way essentially: all the replicas have executed request even if the execution order proves to be inconsistent later. When inconsistency occurs, it takes much longer time for the leader to detect that, either by the notification from the client (as shown in Figure~\ref{SpecPaxos-Slow}), or by the leader's periodical synchronization. Even after the inconsistency has already been detected, it still costs much to resolve the inconsistency. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/SpecPaxos-Slow.pdf}
    \caption{Speculative Paxos workflow (slow path)}
    \label{SpecPaxos-Slow}
\end{figure}
In Figure~\ref{SpecPaxos-Slow}, we showcase how Speculative Paxos resolves the inconsistency. R4 and R5 have inconsistent states from the other replicas because they have executed C2's request before executing C1's request. Such inconsistency is first noticed by C1 while doing the quorum check and finding it impossible to form a fast quorum (4 replicas) of replies with the same hash, so C1 broadcasts a reconciliation request to every replica, notifying them of the inconsistency. After receiving the reconciliation request, the leader coordinates a slow quorum of replicas (3 replicas including itself) to decide a definitive execution order of the requests. Then the leader broadcasts the new order to all replicas. The problematic replicas, either executing requests in an inconsistent order (e.g. R4 and R5), or missing the execution of some requests (e.g. R1, R2 and R3), need to rollback and/or re-execute the requests in the correct order. The rollback mechanism requires the support from application, which can be very costly and even impossible in practical cases~\footnote{The rollback requires the application have checkpointing mechanism to record the system state periodically~\cite{vldb14-fast-recovery}. Since checkpointing can be costly, it is not conducted for every execution of requests. Suppose the application has executed 1 million requests and it records checkpoints for every 1000 requests. When the Speculative Consensus Protocol encounters conflict, it needs to rollback 1000 requests and re-execute them in the definitive and consistent order. Even worse, if the application is not equipped with checkpoint mechanism, the rollback essentially means re-executing all the requests from scratch, which is unbearable in practice.}.

\subsection{Nezha}
\label{sec-nezha-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/Nezha-Fast.pdf}
    \caption{\sysname workflow (fast path)}
    \label{Nezha-Fast}
\end{figure}
In \sysname, the  workflow of the fast path (shown in Figure~\ref{Nezha-Fast}) can be summarized as\\
\centerline{replication$\xrightarrow{}$definite ordering$\xrightarrow{}$leader execution$\xrightarrow{}$quorum check}
The message flow follows \\
\centerline{client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client}
Different from the other protocols, \sysname relies on clock synchronization to achieve the approximate consensus. Given that replica clocks are well synchronized and each request arrives before its deadline, \sysname can release and then append/execute the message simultaneously.  \sysname also costs 2 message delays to commit the request in the fast path. But it involves extra buffering time at replicas to help rectify requests which are reordered in the network. 

Similar to Speculative Paxos, \sysname also includes a hash value in the reply of the fast path, we call the reply message \emph{fast-reply} (defined in \S\ref{sec-fast-quorum-check}). But \sysname adopts incremental hash, which can be rapidly updated according to the modification of the replica \emph{log}s. By contrast, Speculative Paxos uses iterative hash. When some log entries are inserted into or deleted from the middle of the replica \emph{log}, the final hash can only be computed from the that point iteratively. 


\sysname also relies on clients to do the replication, which is similar to Speculative Paxos and Fast Paxos. But the advantage of \sysname over Speculative Paxos/Fast Paxos is that, the request ordering of \sysname is decided when it reaches the leader, i.e., the leader's order of requests serves as the reference for replicas. Such a strong leadership avoids the costly coordination overheads (as in Fast Paxos/Speculative Paxos) when inconsistency happens.  


\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/Nezha-Slow.pdf}
    \caption{\sysname workflow (slow path)}
    \label{Nezha-Slow}
\end{figure}
In Figure~\ref{Nezha-Slow}, we showcase how \sysname resolves the inconsistency. 
In Figure~\ref{Nezha-Slow}, C2's request has a smaller deadline than C1's request, so it is expected to be appended/executed ahead of C1's request. R3 and R4 receive the two requests in the correct order (i.e., the ascending order of their deadlines). By contrast, the two requests are reordered during the transmission from the clients to R1 and R2, and these two replicas receive C1's request ahead of C2's request. For R2, though the requests are reordered, C1's request is still buffered by \primname, which offers the opportunities to rectify the reordering effect, so C2's request is still released and appended/executed before C1's request. On the other hand, however, \primname is unable to rectify the reordering on R1, because C2's request arrives too late, even after C1's request has been released. In this case, \sysname makes the leader (C3) take an active role. After the leader has appended the request, the log position (ordering) has been decided, so the leader broadcast the \emph{sync} message (\S\ref{sec-fix-set-inequality}) to all followers, and C1 can modify its \emph{log} after receiving the \emph{sync} message, so as to keep consistent with the leader.



==> design_overview-old.tex <==

\section{\sysname Overview}
\label{sec:design}
\Para{Fast path/slow path division.} In order to commit requests more efficiently, a common design principle in several consensus protocols~\cite{fastpaxos, lamport2005generalized, sosp13-epaxos, nsdi15-specpaxos, osdi16-nopaxos} is to involve two different paths to commit requests: a fast and a slow path. While the fast path commits requests more quickly, it may not always succeed and needs to fall back to the slow path when it fails. \sysname uses the same principle: the fast path opportunistically commits requests that arrive in the same order at all replicas, and the slow path is a remedy.


%\rv{Multi-Paxos/Raft put disproportionally heavy workload on the leader replica, which sequences and multicasts all requests, and then conducts quorum check for the replies. Such a design causes throughput bottleneck and long commit/execution latency.} To address that, a common design principle in several consensus protocols~\cite{fastpaxos, lamport2005generalized, sosp13-epaxos, nsdi15-specpaxos, osdi16-nopaxos} is to involve two different paths to commit requests: a fast and a slow path. While the fast path commits requests more quickly, it may not always succeed and needs to fall back to the slow path when it fails. \sysname uses the same principle: the fast path opportunistically commits requests that arrive in the same order at all replicas, and the slow path is a remedy.

\Para{Primitive/protocol decoupling.}
The underlying assumption behind the fast path/slow path division is that the fast path is the common case. To increase the fraction of client requests that take the fast path, Speculative Paxos~\cite{nsdi15-specpaxos} and NOPaxos~\cite{osdi16-nopaxos} decouple the responsibility of consensus between 2 components: a {\em primitive} and a {\em replication protocol}. The primitive cannot guarantee consensus, but increases the likelihood that requests are received in the same order across all replicas. This allows requests to take the fast path frequently. The replication protocol is responsible for consensus and achieves consensus more quickly on the fast path. Inspired by this primitive-protocol decoupling, we build a primitive called Deadline-Ordered Multicast (DOM), for \sysname to achieve high-performance consensus. DOM uses clock synchronization in lieu of in-network functionality to order client-to-replica requests in the common case.

% Move to appendix
%Concretely, the mostly ordered multicast (MOM) primitive~\cite{nsdi15-specpaxos} used by Speculative Paxos creates a network environment to make most requests arrive at all replicas in the same order. The ordered unreliable multicast (OUM) primitive~\cite{osdi16-nopaxos} used by NOPaxos ensures ordered delivery of requests without a reliability guarantee using a programmable switch as a request sequencer. Both primitives are essential for high performance. Inspired by this primitive-protocol decoupling, we build a primitive called Deadline-Ordered Multicast (\primname), for \sysname to achieve high-performance consensus. DOM uses clock synchronization in lieu of in-network functionality to order client-to-replica requests in the common case.

%For instance, such protocols, when deployed in highly-engineered networks~\cite{nsdi15-specpaxos, osdi16-nopaxos}, can yield good latency and throughput. By contrast, when they are deployed in public cloud environments, their performance degrades drastically, as observed in~\cite{conext20-domino} and our evaluation (\S\ref{sec:evaluation}).

\rv{
\Para{Stateless proxies.} \sysname is still a leader-based consensus protocol, but \sysname delegates proxies to undertake the two most heavy tasks: request multicast and quorum check. Therefore, \sysname's leader is much more lightweight than Multi-Paxos/Raft. \sysname's proxy design is different from the offloading strategy adopted by some existing works (e.g., Speculative Paxos, NOPaxos, CURP~\cite{nsdi19-curp}): they let clients undertake these tasks, which is intrusive to the client-side logic and constrains the performance of individual clients (\S\ref{sec:proxy}). Besides, unlike the proxies employed by the other works (e.g., PigPaxos~\cite{sigmod21-pigpaxos} and Compartmentalized Paxos~\cite{vldb21-compartmentalized-paxos}), \sysname's proxies are stateless, so they enjoy much better scalability and their failure causes no harm to \sysname's correctness, thus incurring no extra complexity to the recovery protocol.}

==> dom_primitive.tex <==

\section{Deadline-Ordered Multicast (DOM)}
\label{sec-dom}

% add/delete logs to simple
%remove "log" in sec 4
% figure 1 arrow from rp to dom client, and from dom client to rp



To describe DOM, we first specify the {\em safety} requirements for consensus. Given two replicas $R_1$ and $R_2$, we say their states are consistent if the following 2 requirements are met.
%\footnote{NOPaxos~\cite{osdi16-nopaxos} calls these 2 requirements ordering and reliable delivery.}
\begin{itemize}[wide, labelwidth=!,nosep]
    \item \textbf{Consistent ordering.} If $R_1$ processes request $a$ before request $b$, then $R_2$ cannot process request $b$ before request $a$, and vice versa.
    \item \textbf{Set equality.} If $R_1$ processes request $a$, then $R_2$ also processes request $a$, and vice versa~.
\end{itemize}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/DOM-v2.pdf}
    \caption{\primname design}
    \label{dom-design}
\end{figure}

% . \primname-Ses broadcast the  requests. On \primname-Rs, every request is destined to either \circleincap{1}\emph{early-buffer} or \circleincap{2}\emph{late-buffer}, and the requests in the \emph{early-buffer} are released with consistent ordering.

A vacuous solution to both safety requirements is to drop all requests, but that would not provide \emph{liveness}. Besides, guaranteeing both safety properties and providing liveness is equivalent to building an atomic broadcast primitive, which is as hard as consensus itself~\cite{weakestfd}. Similar to MOM (used by Speculative Paxos) and OUM (used by NOPaxos), DOM's goal is to judiciously move some responsibility for both safety and liveness to the DOM primitive, giving the protocol a leg up in the process. Unlike MOM/OUM, DOM does this without relying on in-network functionality. As shown in Figure~\ref{dom-design}, DOM consists of two roles, DOM-S (sender) and DOM-R (receiver). DOM's key idea is to use clock synchronization between DOM-Ses and DOM-Rs to provide each request with a deadline specified in synchronized wall-clock time. DOM-Rs release requests in deadline order. This provides consistent ordering in the common case. We describe details below.



%\todo{Should we give an example in footnote? A very long footnote}
%~\footnote{Consider two request \emph{req-1} and \emph{req-2} and two replicas \emph{replica-1} and \emph{replica-2}. \emph{req-1} has a smaller deadline. Both requests arrive before their deadlines on \emph{replica-1} and are processed according their deadline order, but \emph{req-1} arrives very late on \emph{replica-2} even after the replica has processed \emph{req-2}. In such cases, if \emph{replica-2} immediately processes \emph{req-1}, it will have a different processing order from \emph{replica-1}, thus violating consistent ordering. }.
\rv{Every DOM-S can multicast its requests to all DOM-Rs. DOM-Rs will release the received requests, and the sequence of the requests later becomes the state of the replicas. DOM aims to create favorable conditions for consensus protocol, so it wants the sequences released by each DOM-R \emph{close to} state consistency, if \emph{consistent ordering} and \emph{set equality} cannot be both fulfilled. More specifically, DOM prioritizes consistent ordering over set equality if it cannot achieve both. To make that, DOM synchronizes the clocks for DOM-Ses and DOM-Rs. DOM-Ses and DOM-Rs leverage the synchronized clocks to achieve consistent ordering, and (possibly) set equality.}


\rv{\Para{DOM-S.} 
Each DOM-S estimates the one-way delay (OWD) to each DOM-R (the estimation approach is explained later). When DOM-S multicasts its request to DOM-Rs, it chooses the maximum among the estimated OWDs across all DOM-Rs. The maximum provides a latency bound: an estimate for how long it takes for the request to reach all replicas. DOM-S attaches the sending time and the latency bound to the request. Adding this latency bound to the sending time provides a deadline by when the request should have reached all DOM-Rs.}


\rv{\Para{DOM-R.} 
Each DOM-R maintains two buffers to hold the incoming requests, namely, \emph{early-buffer} and \emph{late-buffer}. \emph{early-buffer} is a priority queue sorted by request deadlines, whereas \emph{late-buffer} is a map which can be searched by the request index~\footnote{We concatenate the \emph{client-id} to \emph{request-id} as the index for the request.}. Requests which enter the \emph{early-buffer} will be eventually released according to their deadline order, whereas the others will be kept in the \emph{late-buffer}.} 


When DOM-R receives a request, DOM-R first considers whether it is eligible to enter the \emph{early-buffer}. Not all requests can be accepted by the \emph{early-buffer} because consistent ordering must be guaranteed for all requests released from \emph{early-buffer}. The simplest eligibility check to enter the \emph{early-buffer} is to compare the request's deadline with the DOM-R's local clock time at request arrival, and only accept the request if it arrives before its deadline. However, this entrance condition is unnecessarily strict, \rv{and will damage consistent ordering if DOM-R's clock does not satisfy monotonously increasing property}. Instead, DOM-R uses a more relaxed condition that ensures the consistent ordering \rv{regardless of clock skew}: if the deadline of the incoming request exceeds that of the last released one, it enters the \emph{early-buffer}. Otherwise, DOM places this request into the \emph{late-buffer} with no further actions. These requests will be further handled by \sysname protocol, to reach state consistency finally (\S\ref{sec-fix-set-inequality}). 



% Request delays have 2 components: the processing delay of the request at the replica and the transmission delay from the client to the replica. For DOM to be effective, request delays must be predictable: replicas must not be overloaded and there should not be significant network congestion. These are reasonable assumptions because consensus is not network-capacity-bound and replicas typically run on well-provisioned VMs. DOM first synchronizes the clocks of the clients and replicas. Then, each client maintains a moving median of its one-way delays to each replica. Each client computes the maximum of these median one-way delays across all replicas. This maximum provides a latency bound: an estimate for how long it will take for a client's request to reach all replicas. Adding this latency bound to the timestamp at which the client generated its request provides a deadline by when the request should have been reached all replicas. Clients puts this deadline into a request header. Replicas do not process the requests until their deadlines. After that, requests are processed in ascending deadline order.

% So, if requests arrive before their deadlines, they will be processed in the same order across all replicas in the fast path (i.e., consistent ordering). However, some requests may arrive late. These late requests cannot be immediately processed because doing so may violate the consistent ordering among replicas. Therefore, \primname divides incoming requests into two separate buffers for fast path and slow path processing: the \emph{early-buffer} and \emph{late-buffer} (Figure~\ref{dom-design}). The \emph{early-buffer} is a priority queue sorted by request deadlines. The \emph{late-buffer} is a map that can be searched with the key obtained by concatenating \emph{client-id} to \emph{request-id}. At each replica, \primname releases a request from the \emph{early-buffer} when the replica's local clock time has passed the request deadline; this request is then passed to the replication protocol for consensus. 

%, but a request might arrive later than its deadline
% However, not all requests can be sent to the \emph{early-buffer}, because \primname ensures consistent ordering for the requests released from the \emph{early-buffer}. Hence, when a request arrives, \primname first considers whether it is eligible to enter the \emph{early-buffer}. The simplest eligibility check to enter the \emph{early-buffer} is to compare the request's deadline with the replica's local clock time at request arrival, and only accept the request if it arrives before its deadline. However, this entrance condition is unnecessarily strict to ensure consistent ordering. Instead, DOM uses a more relaxed condition that still ensures the consistent ordering: if the deadline of the incoming request exceeds that of the last released one, it is sent to the \emph{early-buffer}. Otherwise, \primname places this request into the \emph{late-buffer}. 
%TODO: "because appending it to the replica log would violate ..." can be made a bit clearer. Not sure how though. Let's discuss.


\Para{\rv{Adaptive latency bound.}}
\label{mov-avg-bound}
During the interaction between DOM-Ses and DOM-Rs, the latency bound becomes the key factor to the effectiveness of DOM. A good latency bound should just cover the request delays from DOM-S to all DOM-Rs, so that the request can be accepted by their \emph{early-buffers} but suffers little additional delay. The latency bound accounts for the variance of request delays, which mainly consists of two components: the processing delay of the request at DOM-R and the transmission delay from DOM-S to DOM-R. {Though the public cloud is inherently more variable than bare-metal clusters, we empirically find that \sysname's latency bound can still handle this variability and outperform the baselines (\S\ref{sec-latency-throughput}), likely because of the inter-tenant performance isolation and rate limiting enforced by cloud operators~\cite{gcp-isolation,azure-isolation, aws-isolation}.}  

%For DOM to be effective, the latency bound should be predictable for \emph{most} requests: replicas  cannot be overloaded and there should not be significant network congestion. These are reasonable assumptions because consensus traffic is not network-capacity-bound~\cite{nsdi15-specpaxos} and replicas typically run on well-provisioned VMs. 
% Besides, cloud providers also offer multiple isolation options~\cite{gcp-vpc,aws-isolation} to protect \sysname's replicas/proxies from external interference.}

% Besides, virtual private cloud (VPC) clusters are also available to provide better network isolation for replicas/proxies of \sysname.

DOM fully utilizes the synchronized clocks on DOM-S and DOM-R to estimate the request delay (i.e. OWD) as follows.
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.2cm}
    \widetilde{OWD} = 
    \begin{cases}
        M + \beta (\sigma_{S}+\sigma_{R}), \quad 0<OWD<D \\
        D
    \end{cases}
\end{equation*}

\rv{DOM-R maintains a sliding window for each DOM-S, and records the OWD samples by subtracting the attached sending time with its receiving time. Then DOM-R picks the median value from the samples in the sliding window as $M$. We previously tried moving average but found that just a few outliers (i.e. the tail latency samples) can inflate the estimated value. Therefore, we choose the moving median instead for robustness. Besides $M$, DOM-R also obtains from Huygens the standard deviation  for the sending time and receiving time, denoted as $\sigma_{S}$ and $\sigma_{R}$~\footnote{$\sigma_{S}$ and $\sigma_{R}$ are calculated based on the method in Appendix A of~\cite{yilong-spn}.}. $\sigma_{S}$ and $\sigma_{R}$ provide an \emph{approximate} error bound for the synchronized clock time, so we add the error bound with a factor $\beta$ to $M$ and obtain the final estimated OWD. The involvement of $\beta (\sigma_{S}+\sigma_{R})$ enables an adaptive increase of the estimated value, leading to a graceful degradation of \sysname as the clock synchronization performs worse.} 

\rv{Even after we have considered the robustness and graceful degradation, the possibility still exists that clock synchronization goes wrong and provides invalid OWD values (i.e. very large or even negative OWDs). To tackle this, we further adopt a clamping operation: If the estimated OWD goes out of a predefined scope $[0, D]$, we will use $D$ as the estimated OWD.} 

\rv{The estimation runs as a separate routine on DOM-Rs. Periodically, DOM-Rs piggyback the estimated OWDs to DOM-Ses, and DOM-Ses choose the maximum OWDs across DOM-Rs as their latency bound for the following request multicast.} 


%DOM first synchronizes the clocks of the clients and replicas. Then, each client maintains a moving median of its one-way delays to each replica. Each client computes the maximum of these median one-way delays across all replicas. This maximum provides a latency bound: an estimate for how long it will take for a client's request to reach all replicas. Adding this latency bound to the timestamp at which the client generated its request provides a deadline by when the request should have been reached all replicas. Clients puts this deadline into a request header. Replicas do not process the requests until their deadlines. After that, requests are processed in ascending deadline order.


%that decides whether the request can enter the \emph{early-buffer}s and eventually be released by DOM-Rs. As a special case, with sufficiently large latency bounds, all requests can arrive before their deadlines and be accepted by the \emph{early-buffer}s, then the request sequences released by DOM-Rs are consistent. However, the large latency bounds also causes long pending delay for requests and further prolongs their commit/execution latency. On the opposite side, with too small latency bounds, requests are more likely to enter the \emph{late-buffer}s, thus requiring further processing from \sysname protocol, which undermines the effectiveness of \primname. 



% To maintain consistent ordering, \primname does not release requests from \emph{late-buffer} to the protocol. However, liveness is impacted if replicas leave requests in the \emph{late-buffer} indefinitely. For liveness, the replication protocol takes a lightweight approach (\S\ref{sec-fix-set-inequality}) to handling requests in the \emph{late-buffer}: all replicas, except the leader replica, simply ignore them, and only process the requests from their \emph{early-buffer}s, which are released in the ascending order of their deadlines. The leader alone fetches requests from its \emph{late-buffer} and overwrites their deadlines to be larger than the deadline of the last released request. Having just become eligible, these requests now enter the leader's \emph{early-buffer} and are processed by the leader replica. These requests will be appended to the leader's log and applied to the leader's state machine. Once the requests become log entries of the leader, the leader broadcasts the indices of log entries to follower replicas. The follower replicas refer to the log indices and modify their logs, so as to maintain set equality with the leader.


%%%


\Para{Comparison to other primitives.} \jk{There are three other primitives closely related to DOM, namely, MOM~\cite{nsdi15-specpaxos}, OUM~\cite{osdi16-nopaxos} and TOQ~\cite{nsdi21-epaxos}. From the perspective of deployability, DOM and TOQ are both based on software clock synchronization whereas MOM and OUM rely on highly engineered network. This gives DOM and TOQ an advantage over MOM/OUM in an environment like public cloud. On the other hand, MOM and TOQ only provide best-effort ordering, i.e.,  requests output from MOM and TOQ can still contain out-of-order cases. By contrast, DOM and OUM guarantees consistent ordering of requests. Regarding the comparison between DOM and OUM, OUM's gap detection mechanism is more sensitive to packet reordering/drop than the deadline-based holding mechanism of DOM. Whenever the incoming sequential numbers become non-consecutive, OUM triggers gap agreement even if consistent ordering is not violated, causing performance degradation of NOPaxos (\S\ref{sec-latency-throughput}). We also include a more formal comparison in \S\ref{appendix-formulation}.}




%In effect, \primname intends to add a small delay to all requests (by waiting until their deadlines) to save delay overall (by creating more chances to commit requests in fast path). The additional delay allows \primname to rectify requests' order even if they have been reordered by the network. This gives \primname an advantage over MOM/OUM in an environment like public cloud. A cloud tenant's network is not highly-engineered, causing frequent packet reordering, forcing MOM/OUM to trigger the slow path of their protocols. By contrast, most reordering can be rectified by \primname at the replica, as long as clocks are well synced and the deadlines account for variability in transmission and processing delays. A more formal comparison is included in ~\cite{nezha-tech-report} (\S\ref{appendix-formulation}). 

% Highlight: MOM only provides best-effort ordering, OUM/DOM both provide consistent ordering, and OUM also provides gap detection. TOQ can be considered as a deployable MOM. 

==> error-domino-old.tex <==

\section{Error Traces of Domino}
\label{error-trace-domino}
Domino~\cite{conext20-domino} is a recently proposed solution to achieve consensus with clock synchronization. Unfortunately, its improper use of synchronized clocks in Fast Paxos completely damage the correctness of the protocol. We analyze in more details as below.

%its improper adaption of the original Fast Paxos damages the protocol correctness. We point out and explain two main mistakes of Domino.

\subsection{Durability/Consistency Violation}
\label{durability-violation-domino}

Domino does not guarantee durability property, and further cannot guarantee consistency and linearizability properties. The reason for the Domino's violation comes from the misunderstanding of Fast Paxos. To be more specific, Domino has made two serious mistakes, namely, weak leadership and stray reply messages. Any one of them can cause Domino to violate the durability property, i.e. losing committed requests permanently. We explain more details below.

\subsubsection{Weak leadership}
Fast Paxos is still a leader-based protocol, and the leader (which is termed as ``coordinator'' in the original paper of Fast Paxos~\cite{fastpaxos}) plays a crucial role for its durability/consistency, but is overlooked by Domino during its adaption. 


As explained in \S4.4 of~\cite{nsdi15-specpaxos}, Fast Paxos  requires 1.5 RTTs to commit the request and reply the execution result to clients. The message flow can be described as below:

Client$\xrightarrow[]{}$Replicas$\xrightarrow[]{}$Leader$\xrightarrow[]{}$Client.


As an optimization, when commit and execution are decoupled, it is possible for Fast Paxos to commit in 1 RTT, without the execution result (as explained in \S B3.3 of~\cite{nsdi19-curp}). Domino tries to use this optimization to reduce commit latency. However, the difference between the proper Fast Paxos optimization and Domino design is, even if the request is committed in the fast path (1 RTT), Fast Paxos can only decide the log position for the request until the leader receives a super quorum of consistent Replicas$\xrightarrow[]{}$Leader messages. By contrast, Domino client takes the leadership from the replica and has already decided the log position of the request during its submission (i.e. predefined arrival time). \emph{The early decision of log positions for fast-committed request eventually damages Domino's correctness}, because its slow path allows the leader (or any other replicas working as DM leader) to assign log positions for requests to be committed in the slow path (refer to para. 4 of \S5.5 in \cite{conext20-domino}). When the log position of the slow-committed request collides with that of the fast-committed request, one of them will be overwritten by the other, causing permanent loss. Below we use a specific error trace (Error Trace 1) to illustrate it. 



% The message delay follower$\xrightarrow{}$ leader is necessary for the durability and consistency property. A super quorum without including the leader may lead to the loss of requests after recovery, which can violate the durability and consistency property, as shown in Error Trace 1.


% \textbf{Error Trace 1:} There are 5 replicas in Domino, i.e. 1 leader and 4 followers. 
% \begin{enumerate}
%     \item The client submits the request to the replicas, and it is received the 4 followers but lost to the leader. 
%     \item The 4 followers reply to the client and Domino considers a super quorum formed. Therefore, the client considers the request as committed.
%     \item  Then two followers crash, which is allowed by the failure model, and they are relaunched immediately. 
%     \item After the relaunch, the two followers recovery their logs by copying from the leader, which do not contain the request.
%     \item  After the two followers have recovered, the other two followers also crash and are relaunched. Similarly, they also copy the leader's logs for recovery, which do not contain the request.
%     \item After all replicas are recovered, the request, which is considered as committed, is lost forever. 
% \end{enumerate}

% It is possible to confirm the commit of requests with a super quorum in 1 RTT. However, it requires some additional constraints of the super quorum, i.e., the super quorum needs to include the leader replica. Such a requirement is involved in the design of \sysname and NOPaxos~\cite{osdi16-nopaxos}. Unfortunately, it is missing in the design of Domino. Therefore, Domino cannot guarantee durability, as shown in Error Trace 1. Besides, if the execution results of the following requests have dependency on the lost request, then the execution results will also become inconsistent after recovery, so Domino does not guarantee
% consistency either. 



\textbf{Error Trace 1:} There are 5 replicas in Domino, and we denote them as R0-R4. There are two requests included in the trace, denoted as request-1 and request-2.
\begin{enumerate}
    \item The client submits request-1 to the replicas, and it is received by R3 and R4, but lost to R0-R2. request-1 occupies a log position in the logs of R3 and R4, and the log position is its predefined-arrival time. 
    \item Another client chooses Domino's Mencius (DM) to handle request-2, so it submits request-2 to a DM leader (R0), and the DM leader decides a log position for request-2, and also asks other replicas to accept it (refer to para. 4 of \S 5.5 in \cite{conext20-domino}). However, this log position happens to be the same as that of request-1, which have been accepted by R3 and R4. 
    \item R1 and R2 accept request-2 and replies to R0. R3 and R4 fail to receive the request from R0 because the messages have been delayed in the network.
    \item R0 realizes the majority has established including itself, R1 and R2, so R0 considers request-2 as committed and replies to the client.
    \item R1 and R2 crash and are immediately relaunched. When they try to recover the log state, they notice that, among the 3 remaining replicas (i.e. R0, R3, and R4), R3 and R4 have request-1 on the log position whereas R0 has request-2 on the same log position. Then R1 and R2 follow the majority and also put request-1 in their recovered log. 
    \item R0 crashes and is relaunched. Then R0 notices every one of the 4 remaining replicas only have request-1 in the log, so R0 also takes request-1 into its recovered logs. 
    \item So far, request-2, which has been committed in the slow path, is permanently lost. 
\end{enumerate}



% \textbf{Error Trace 2:} There are 5 replicas in Domino, and we denote them as R0-R4. 
% \begin{enumerate}
%     \item The client submits request-1 to the replicas, and it is received by R3 and R4, but lost to R0, and delayed to R1 and R2. 
    
%     \item R3 and R4 send reply to the client immediately after receiving the request. Then they crash.
    
%     \item R3 and R4 are relaunched, and they contact the other 3 replicas (R0, R1 and R2) for recovery. All of them have empty log lists, so R3 and R4 recover with empty log lists.
    
%     \item The delayed request-1 arrives at R1 and R2, so R1 and R2 also immediately send replies to the client. 
    
%     \item So far, the client now has received the replies from the super-majority, so the client considers request-1 as committed (though R3 and R4 have forgotten request-1). 
    
%     \item R1 and R2 crash and are relaunched. Then they contact the other 3 replicas (R0, R3 and R4) for recovery. But all the 3 replicas  
% \end{enumerate}


% let request-1 committed in the fast path first, and make R3 and R4 crash and be relaunched immediately to accept request-2, and finally make R1 and R2 crash and recover request-2 into their logs. In this way, we create another error trace showing that request-1, which have been committed in the fast path, is lost.

The error trace is caused by the collision of log positions from concurrent proposers (i.e. clients and DM leaders). Both Fast Paxos and Mencius have no such errors. 

\begin{itemize}
    \item Fast Paxos. In terms of the original paper of Fast Paxos~\cite{fastpaxos}, the consensus algorithm is executed in multiple rounds, each with a round number. The coordinator (leader) can only launch new rounds with larger number than those already started, and the acceptors (followers) can only participate the rounds with incremental number (refer to Phase 1(b) of \S2.2.1 and Observation 1 of \S2.2.2 in \cite{fastpaxos}). This rule prevents two requests from being committed in the same log position (the term ``round'' in \cite{fastpaxos} can be mapped to the log position here), because only one request can get the super majority. Besides, the description of Fast Paxos included in NOPaxos paper~\cite{osdi16-nopaxos} is a bit different from the original paper~\cite{fastpaxos}, but it also implicitly indicates the requirement of monotonically increasing property of round number. Regarding the implementation of Fast Paxos in NOPaxos repository~\cite{nopaxos-code}, each replica assigns an \emph{opnum} for every incoming request, and \emph{opnum} maintains the monotonically increasing property. The leader needs to ensure the consistency of \emph{opnum} during quorum check. Therefore, two different requests cannot be committed with the same \emph{opnum}.  
    
    \item Mencius. Mencius~\cite{osdi08-mencius} also avoids the error of Domino, because Mencius has partitioned the log positions in advance with no overlap. Even if multiple leaders propose requests concurrently, the requests are only committed in the log positions belonging to the corresponding leaders.   
\end{itemize}

Although Fast Paxos and Mencius both avoid the error cases shown in Error Trace 1, Domino makes an incorrect mix of them: its improper use of  time ordering in the fast path weakens the leadership of Fast Paxos and fails to guarantee the monotonically increasing property of rounds (i.e. log positions), whereas its employment of Mencius in the slow path leads to log position collision and eventually violates the durability property. 

Note that the collision discussed here is different from the collision mentioned in \S5.3.2 of Domino paper~\cite{conext20-domino}. The collision in \S5.3.2 is detectable by the Domino replicas and thus can be resolved to prevent it from affecting correctness, because the collision are caused by clients and the dedicated \emph{proposer} (which can be considered as a special client in essence). However, the collision discussed here is caused by the replicas (i.e. the DFP replicas and the DM leaders). It results from the flaws of Domino design and is not detectable by replicas themselves. Such error cases can easily occur in the scenario with frequent bursts, where a large number of concurrent requests are issued in a small interval and has high probability to be assigned with the same log position by the clients (and then accepted by DFP replicas) and DM leaders.


\sysname suffers no such error cases. The reason lies in the elaborate design of its quorum check in the fast path and the strong leadership in the slow path. The quorum check in the fast path checks the consistency of the entire sequence of requests so far, rather than a single one (which Domino does). The quorum check in the slow path happens after the majority has confirmed their consistency with the single leader (i.e. it is still the single leader which decides the log positions of the requests). Therefore, after a request is considered as committed by the quorum check in the slow path, it indicates the leader also agrees with the log position for the request, so the single leader would not commit a different request in the same log position. The only concern about correctness violation for \sysname comes from the collision of the hash included in the \emph{fast-reply} messages. However, such hash collision is equivalent to breaking the security of cryptography, which we assume impractical~\footnote{Although \sysname is using SHA1 in the current implementation, \sysname is compatible to any hash algorithm, and the design of collision-resistant hash algorithm is out of the scope of \sysname}. 



\subsubsection{Stray Reply Messages}
\label{sec-stray-reply-domino}
Domino is also a diskless implementation~\cite{domino-repo}, so replicas can lose their memory after they fail and recover, which causes the violation of durability. Below we use a specific error trace (Error Trace 2) to illustrate it. 



\textbf{Error Trace 2:} There are 5 replicas in Domino, and we denote them as R0-R4. 
\begin{enumerate}
    \item The client submits a request to the replicas, and it is received by R3 and R4, but delayed in the network while transmitting to R1 and R2, and is lost to R0.  
    \item R3 and R4 accept the request and immediately reply to the client.
    \item R3 and R4 crash and are relaunched. They contact the other replicas to recover their states, but notice that all of the 3 replicas (R0-R2) have empty logs, so R3 and R4 also recover an empty log list. 
    \item The delayed request finally arrives at R1 and R2, so R1 and R2 also reply to the client immediately. 
    \item So far, the client has received the reply messages from a super majority (R1-R4), so it considers the request as committed in the fast path, although R3 and R4 no longer have the request and have forgotten they have sent replies before. 
    \item R1 and R2 crash and are relaunched, they contact the other replicas to recover their states, but notice that all of the 3 replicas (R0, R3, R4) have empty logs, so R1 and R2 also recover an empty log list. 
    \item So far, the request, which has been committed in the fast path, is permanently lost. 
\end{enumerate}

The error trace of Domino is caused by the stray reply messages and the lack of coordination among replicas in the fast path. Fast Paxos have no such errors. In the original description of Fast Paxos, replicas are assumed to be equipped with stable storage, and recovers the state from the stable storage before resume the service, so that the failure of the replica becomes ``indistinguishable from its simply pausing''~\cite{fastpaxos}. When Fast Paxos runs in diskless mode, Fast Paxos can employ \emph{crash-vector}s~\cite{disc17-dcr,disc17-dcr-techreport} to avoid stray messages. However, Domino lacks both the stable storage and \emph{crash-vector} mechanism, therefore, it has no way to avoid the effect of \emph{stray messages}.

\sysname suffers no such error cases. The reason lies in the use of \emph{crash-vector}s. As described in \S\ref{sec-fast-quorum-check}, the $hash$ in \emph{fast-replies} include the information of \emph{crash-vector}s. When some replicas fail and are relaunched, they rejoin as followers (\S\ref{replica-rejoin}). These \textsc{recovering} replicas broadcast a new \emph{crash-vector},~\footnote{The new \emph{crash-vector} is different from that before their crash, because the \textsc{recovering} followers increment their own counters.} (Algorithm~\ref{algo-replica-rejoin}), which leads to the update of the leader's, as well as other remaining replicas', \emph{crash-vector}s after the state transfer. The leader and other replicas will include the hash of the new \emph{crash-vector} in the subsequent \emph{fast-replies}. Therefore, the stray \emph{fast-replies} and the fresh \emph{fast-replies} have inconsistent hash and cannot form the superquorum during the quorum check in the fast path. The slow path of \sysname does not suffer from such \emph{stray message} effect, because there is a causal order between the leader and followers: leader's state update always precedes followers' sending \emph{slow-replies}. Therefore, the followers' state before crash is no \emph{fresher} than their recovered state. When the relaunched followers recover their state from the leader, they will not forget the \emph{slow-replies} sent before their crash.



The durability property is a necessary condition for the consistency and linearizability properties: 
\begin{itemize}
    \item Because one committed request affects the execution result of the subsequent requests, the loss of it will lead to different execution results for the subsequent requests, thus violating consistency. 
    \item Because the committed request can be observed by clients, the loss of it causes contrary observation afterwards, thus violating linearizability.
\end{itemize}
 
Error Trace 1 and Error Trace 2 have shown that Domino can violate durability in both the fast path and the slow path. Therefore, the consistency and linearizability properties of Domino are also damaged in both paths. In \S\ref{linearizability-violation-domino} we will continue to show that, even without considering the violation of durability/consistency property, Domino still violates linearizability. 



\subsection{Linearizability Violation}
\label{linearizability-violation-domino}
Domino does not guarantee linearizability~\cite{linearizability}, or even a weaker form, sequential consistency~\cite{lamport-sequential-consistency,sequential-consistency-vs-linearizability}. Domino uses the pre-estimated arrival time to order requests, but it lets the replicas \textbf{immediately} reply to the clients once receiving the request, so as not to increase the commit latency (Para. 6 of \S5.4 in Domino paper ~\cite{conext20-domino}). However, such a design violates the linearizability property, as shown in Error Trace 3.

\textbf{Error Trace 3:} There are 5 replicas in Domino, i.e. 1 leader and 4 followers. There are two clients, namely C1 and C2, submitting requests to replicas. The requests are not commutative. 
\begin{enumerate}
    \item When $t=0$, C1 submits its request to all replicas, with a pre-estimated arrival time $t_1 = 10$ (invocation). 
    \item When $t=1$, all replicas receive C1's request and reply to C1.
    \item When $t=2$, C1 receives the reply messages from all replicas, and the request is committed (response). 
    \item When $t=3$, C2 submits its request to all replicas, with a pre-estimated arrival time $t_2 = 9$.
    \item  When $t=4$, all replicas receive C2's request and reply to C2.
    \item When $t=5$, C2 receives the reply messages from all replicas, and the request is committed (response).
    \item When $t=11$, every replica has executed the two requests, with C2's request executed first and C1's request executed second. 
\end{enumerate}

It can be easily checked that Error Trace 3 violates linearizability based on the definition of "Execution Linearizability" described in ~\cite{sosp13-epaxos, epaxos-proof}: if two interfering commands $\gamma$ and $\delta$ are serialized by clients (i.e., $\delta$  is
proposed only after $\gamma$ is committed by any replica), then every replica will execute $\gamma$ before $\delta$). However, Error Trace 3 just goes to the opposite way: the early committed request is executed later. 

More formally, the linearizability violation can be derived as follows: consider the two commit events, the event sequence can be summarized as: Invocation(C1)$\xrightarrow{}$Response(C1)$\xrightarrow{}$Invoke(C2)$\xrightarrow{}$Response(C2), and there is no overlap. According to the definition of linearizability~\cite{linearizability}: each operation appears to take effect instantaneously and exactly once at some point between its invocation and its response. Therefore, C1's request should take effect before C2's request, which is opposite to the execution order conducted by Domino. 

%In other words, linearizability requires the request should be responded if it is guaranteed to be executed before a later started (invoked) request, but Domino violates this requirement. 

Furthermore, if we consider C1 and C2 as the same client in Error Trace 3, we can find that the error trace even violates sequential consistency~\cite{lamport-sequential-consistency}, which is a weaker correctness condition than linearizability (as mentioned in~\cite{linearizability,sequential-consistency-vs-linearizability}). According to the description from \cite{sequential-consistency-vs-linearizability}, ``sequential consistency requires that all of the data operations appear to have executed atomically, in some sequential order that is consistent with the order seen at individual process". Obviously, if C1 and C2 are the same client, this individual client sees an order which is opposite of the execution order of its two requests. Therefore, Domino's design also violates sequential consistency.  


The root cause for the violation of linearizability and sequential consistency of Domino comes from its improper decoupling of commit and execution. Given a sequence of committed requests, the execution order of these requests can be arbitrary in Domino because they may be assigned with different arrival-time and lead to arbitrary execution order. Decoupling commit and execution is possible for consensus protocols, such as Fast Paxos and EPaxos. However, the consistency between commit order and execution order must be guaranteed: Fast Paxos relies on its leader to achieve this, whereas EPaxos relies on the dependency chain, which is persisted together with the committed request. By contrast, Domino does not have any mechanism to maintain such consistency, so it violates linearizability and sequential consistency.  

\sysname uses the \emph{deadline}, which is similar to the concept of \emph{expected arrival time} in Domino, to decide the execution order of requests, but \sysname does not violate linearizability thanks to two design principles.
\begin{itemize}

\item  First, \sysname appends/executes requests released from the \emph{early-buffer} of \primname, which preserves the ascending order of \emph{deadline}s. If Step 1 and Step 2 of the error trace happen to any replica, Step 5 cannot happen to that replica, because \primname has put C2's request to the \emph{late-buffer}. If the replica is leader, the leader will modify the \emph{deadline} of C2's request, and it will be eventually executed after C1's request. 

\item Second, contrary to Domino, replicas in \sysname do not immediately reply to clients after they receive the request. Instead, replicas in \sysname reply to clients after the replica's local clock time has passed the \emph{deadline} of the request. In Error Trace 2, if C1's request arrives before $t=10$, it will be held until $t=10$. Meanwhile, if C2's request arrives before $t=9$, it will be replied before C1's request. In this way, linearizability is still preserved (i.e. the two commit events overlap and they appear to take effect instantaneously with C2's request first and C1's request second). It is true that the \emph{early-buffer} can cause additional pending time for some requests if the latency bound is too large, and that is why we choose moving median as the latency bound, whereas Domino chooses the 95th tail latency as the estimation. Besides, we also conduct commutativity optimization (rather than rely on a very large latency bound) to improve fast commit/execution ratio and reduce commit/execution latency (details in \S\ref{commutativity-optimization}).

\end{itemize}

==> error-trace-nopaxos.tex <==


\section{Error Trace of NOPaxos}
\label{error-trace-nopaxos}
Michael et al~\cite{disc17-dcr, disc17-dcr-techreport} discover the incorrectness in the diskless recovery of viewstamped replication~\cite{viewstamp} and present an error trace in \S B.1 of \cite{disc17-dcr-techreport}. The cause for the incorrectness is later defined as \emph{stray message} in \cite{tdsn21-recovery}. We are inspired by the error trace of viewstamped replication and find that, the similar bugs also exist in the recovery of Speculative Paxos~\cite{nsdi15-specpaxos} and NOPaxos~\cite{osdi16-nopaxos}. It can appear during both view change process (due to \emph{stray messages} between replicas) and the fast path (due to \emph{stray messages} between replicas and clients). We use two error traces to illustrate them respectively.

\subsection{Stray Messages During View Change}
\label{sec-nopaxos-stray-view-change}
In the terminology of NOPaxos protocol (refer to \S5.2.3 in \cite{osdi16-nopaxos}), we describe an error trace to illustrate how \emph{stray messages} can damage the correctness of NOPaxos. Such errors commonly exist in all protocols that inherit the diskless recovery of viewstamped replication whereas \sysname avoids the problem by using \emph{crash-vector}~\cite{disc17-dcr,disc17-dcr-techreport} during the recovery process (\S\ref{recovery-algo}). 

\textbf{Error Trace 1:} There are 3 replicas in NOPaxos, denoted as R0, R1, and R2.

\begin{enumerate}
    \item Initially, the view is 0, and R0 is the leader. We assume the sequencer does not fail during the following process, and the \emph{session-num} is always 0.
    \item R1 suspects R0 fails, so R1 initiates a view change: it sets its \emph{status} to \textsc{viewchange}, increments its \emph{view-id} from 0 to 1. Then it broadcasts <\textsc{view-change-req}, \emph{view-id}> to all the other replicas. After that, R1 crashes, and the messages are delayed in the network.
    
    \item R1 is relaunched and contacts R0 and R2 for recovery (R0 and R2 forms a majority). R0 and R2 have not received the \textsc{view-change-req} messages sent by R1 before crash, so R0 and R2 are still \textsc{normal} in view 0 with R0 as the leader. Then, R1 is recovered as a follower, with \emph{view-id}=0.
    
    
    \item R2 receives the \textsc{view-change-req} message (this is a \emph{stray message} and the recovered R1 has forgotten it!) from R1, so it sets \emph{status} as \textsc{viewchange}. Then, it also broadcasts \textsc{view-change-req} messages to all the other replicas,
    and sends a \textsc{view-change} message to the leader in the new view (R1). After sending the messages, R2 crashes. The messages are delayed in the network.
    
    \item R2 is relaunched and contacts R0 and R1 for recovery (R0 and R1 forms a majority). R0 and R1 have not received the \textsc{view-change-req} messages sent by R2 before crash, so R0 and R1 are still \textsc{normal} in view 0. Then, R2 is recovered as a follower, with \emph{view-id}=0.
    
    \item The \textsc{view-change-req} message is lost to R0, but both the \textsc{view-change-req} message and \textsc{view-change} message arrives at R1 (this is another \emph{stray messages}, and the recovered R2 has forgotten it!). R1 then initiates the view change: incrementing \emph{view-id} from 0 to 1, broadcasting \textsc{view-change-req} messages and sending a \textsc{view-change} message to the new leader. It notices itself is the new leader, so it collects \textsc{view-change} from itself and R2, thus forming a majority. 
    
    \item R1 thinks it has got the \textsc{view-change} messages from the majority (though R2 has forgotten it has sent that), so it
    merges the logs from the two \textsc{view-change} messages, resets its \emph{status} to \textsc{normal}, and becomes the leader in view 1. Meantime, R0 and R2 are both in view 0 and R2 still believes R0 is the leader.
    
    \item A request is multicast to all replicas but is lost to R1. Both R0 and R2 receive the request and reply to the client. The client gets replies from a majority of replicas with matching \emph{view-id}s (0), and the leader (R0) is also included, so the client considers it as committed. 
    
    \item R0 crashes and is relaunched. It contacts R1 and R2 for recovery, and notice the highest \emph{view-id} is 1, so it does a state transfer with the leader (R1) in view 1, and copies R1's state, which does not include the committed request. 
    
    \item R2 also crashes after R0 is recovered. It follows the same workflow to recover and also copies the state from R1, and finally becomes a follower in view 1. Then, the committed request is lost forever. 
\end{enumerate}

During the whole process, there is no violation of NOPaxos assumptions, i.e. at most $f=1$ replicas fail at the same time. However, the final result does not guarantee durability of committed request, and can further damage consistency and linearizability.


\subsection{Stray Messages During Quorum Check}
\label{sec-nopaxos-stray-quorum-check}

The stray reply messages can also affect client's quorum check and cause permanent loss of committed requests. We use the following error trace to illustrate this. 

\textbf{Error Trace 2:} There are 3 replicas in NOPaxos, denoted as R0, R1, and R2, and R0 is the leader. 

\begin{enumerate}
\item The client submits a request to the replicas, and the request is tagged with the sequential number of 1 at the sequencer, and then multicast to all replicas.

\item The request is received by R1, and is lost to R2, and is delayed in the network while transmitting to R0.  
\item R1 sends a reply to the client. After that, R1 crashes and is relaunched. It requests the state transfer from the leader, R0. Since R0 has an empty log list, R1 also has an empty log list. 

\item The delayed request finally arrives at R0, so R0 sends a reply to the client, then the client has got replies in  matching \emph{view-id}s and \emph{log-slot-num}s from $f+1$ replicas, including the leader, so the client considers the request as committed.

\item R0 crashes, then R1 and R2 launch the view change process and finally elects R1 as leader. Both R1 and R2 have empty log lists.

\item R0 is relaunched, and requests state transfer from R1, so R0 also gets an empty log list.

\item A new request is multicast by the sequencer (with the sequential number of 2) and arrives at all replicas. Then every replica notices there is a gap occurring. Therefore, the leader starts gap agreement and fill a NOOP in the first slot.

\item So far, the request with sequential number of 1, which has been committed, is lost permanently. 
\end{enumerate}

Error Trace 2 shows that, even if the view change process is executed correctly, the stray messages between replicas and clients can still violate the durability property. Compared with Error Trace 1, Error Trace 2 is even more common and can happen for many diskless protocols which conduct client-side quorum check. The general pattern for such error cases can be summarized as follows:

\textbf{General Error Pattern}. Imagine a request is delayed in the network, whenever it arrives at one replica, that replica sends a reply and immediately crashes afterwards, then the crashed replica recover from the others and gets an empty log list (because the other replicas have not received the request). After each replica completes such behavior, the client gets replies from all the replicas but actually none of them is holding the request. Such a pattern does not violate the failure model, but causes permanent loss of committed requests. 


Reviewing the existing protocols,  
Speculative Paxos, NOPaxos and Domino all suffer from such cases. CURP~\cite{nsdi19-curp} can avoid the \emph{stray message} effect by assuming the existence of a configuration manager, which never produces stray messages (e.g., by using stable storage). Whenever the witnesses crash and are relaunched, the configuration manager need to refresh the information for the master replica as well as the clients, so that clients can detect the stray messages during quorum check and avoid incorrectness.  

\sysname avoids such error cases by including the information of \emph{crash-vector} in the hash of \emph{fast-replies}, which prevent stray reply messages from forming the superquorum in the fast path and creating an \emph{illusion} to the proxies/clients. We analyze in more details below. 


Regarding the general pattern above, 

\begin{enumerate}[wide,label=(\arabic*)]
    \item When the follower(s) fail, they need to contact the leader and complete the state transfer before their recovery (Algorithm~\ref{algo-replica-rejoin}). 
\begin{itemize}
    \item If the leader has already received the request before the state transfer, then after the follower's recovery, it can remember the \emph{fast-reply} that it has sent before crash, and can replay it. In this case, the \emph{fast-reply} is not a stray message.
    \item If the leader has not received the request before the state transfer, then the leader's \emph{crash-vector} will be updated after receiving the follower's \textsc{state-transfer-req} (line 74-75 in Algorithm~\ref{algo-replica-rejoin}), which includes a different \emph{crash-vector} (the follower has incremented its own counter). Therefore, the \emph{hash} of the leader's \emph{fast-reply} is computed with the aggregated \emph{crash-vector}, and will be different from that included in the \emph{fast-reply} (stray message) sent by the follower before crash, i.e. the leader's \emph{fast-reply} and the followers' stray \emph{fast-replies} cannot form a superquorum. 
\end{itemize}
    \item When the leader fails, based on Algorithm~\ref{algo-leader-change}, the view change will elect a new leader. \emph{crash-vectors} ensure the view change process is not affected by \emph{stray messages}. After the view change is completed, the \emph{view-id} is incremented. At least $f+1$  replicas after the view change will send \emph{fast-replies} with higher \emph{view-id}s. Because the quorum check requires reply messages have matching \emph{view-id}s, the \emph{stray fast-replies} (sent by the old leader) can not form a super-quorum together with the \emph{fast-replies} sent by the replicas after the view change.
 
\end{enumerate}

\sysname's slow path does not suffer from \emph{stray message} effect, because there is causal relation between leader's state update (advancing its \emph{sync-point}) and followers' sending \emph{slow-replies}. 
\begin{enumerate}[wide,label=(\arabic*)]
    \item When followers crash and recover, they copy the state from the leader. The followers' state before crash is no fresher than their recovered state, so the followers have no \emph{stray slow-replies}, i.e. the followers can remember the \emph{slow-replies} they have sent before crash and can replay them.
    \item When the leader crashes and recovers, it can only rejoin as a follower replica after the new leader has been elected (\S\ref{replica-rejoin}), so the old leader's reply messages before crash have smaller \emph{view-id}s, compared with the \emph{slow-replies} of replicas after the view change. With matching \emph{view-id}s, these reply messages cannot form a quorum together in the slow path. 
\end{enumerate}
 

% Besides, \sysname explicitly assume a small fraction of stable storage can survive the crash and can be accessed by the recovering replicas (\S\ref{sec:recovery}). The stable storage enables the correct recovery of replicas and the update of \emph{crash-vectors}, which further prevents the \emph{stray message} effect in normal processing.

==> error-trace-raft.tex <==
\section{Why is Stable Storage Necessary for Raft?}
\label{error-trace-raft}

Paxos and Viewstamped Replication (VR) have developed diskless version in~\cite{podc07_diskless_paxos} and ~\cite{viewstamp}, respectively, and the internal bugs of both diskless protocols can be fixed using crash vectors~\cite{disc17-dcr,disc17-dcr-techreport}. In contrast, Raft, since it was invented~\cite{atc14-raft}, has not developed a diskless version so far. Its correctness has more dependency on the stable storage than the other two protocols. In other words, Raft will no longer be correct if stable storage is removed from the protocol. Here we provide an error trace of Raft without stable storage.

There are 5 replicas in Raft, denoted as R0-R4. R0 is the leader.
\begin{enumerate}
\item R0 receives a request from the client, and appends it to the other replicas.

\item R1 and R2 reply to the AppendEntries RPC from R0. Before replying, R1 and R2 should have persisted the request to its stable storage. In this error trace, we will see how Raft goes incorrect if it does not have stable storage for log persistence.

\item The AppendEntries RPC is lost to R3 and R4.

\item R0 receives the replies from R1 and R2. It forms a quorum including R1, R2 and itself, so it replies to the client, notifying it of the commit result.

\item The client considers the request as committed. 

\item \label{key-1} R1 fails, and recovers immediately. Since there is no stable storage, its recovered log is empty. Note that Raft does not have a state transfer mechanism like Paxos and VR, so R1 does not ask logs from the other replicas during recovery. It just recovers with an empty log list, forgetting it has once appended the request and replied to R0. 

\item R0 is network partitioned or fails. The other replicas fail to hear from R0 for sufficiently long time, so they decide to elect a new leader.

\item R3 (with an empty log list) becomes a candidate and sends RequestVote RPC to the others.

\item \label{key-2} R4 and R1 give their votes to R3, so R3 gets the votes from the majority including itself, and becomes the new leader.

\item R3 overwrites the logs of all the other replicas, then the committed request is lost forever.

\end{enumerate}

The root cause for this error trace comes from Raft's leader election mechanism, which takes log persistence as a necessity. Unlike VR, which takes a round-robin way to decide the leader (so that the leader is deterministic in every new view), Raft gives more freedom for replicas to compete for the leadership in each term. The voters decide whether the candidate is qualified by checking whether the candidate's {log} is more \emph{up-to-date} than itself. 

In the error trace, R1 forgets its log in Step~\ref{key-1} without stable storage. Therefore, it mistakenly considers R3 is qualified to become the new leader in Step~\ref{key-2}. By contrast, if it had stable storage and remembered its log after recovery, R1 should have rejected the RequestVote RPC from R3, because R3's log is not as \emph{up-to-date} as its log. In that way, R3 could not become the new leader in Step~\ref{key-2}. 




==> eval-failure-recovery.tex <==

% \subsection{Evaluation of Recovery}
% \label{eval-failure-recovery}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=8cm]{figures/exp/failure-recovery/vc-cost.pdf}
%     \caption{Time cost of view change}
%     \label{fig-vc-cost}
% \end{figure}


% \begin{figure*}[!t]
%     \begin{minipage}{1\linewidth}
%     \centering
%     \subcaptionbox{Total submission rate of 20K reqs/sec}
%       {
%       \includegraphics[width=0.32\linewidth]{figures/exp/failure-recovery/20K-failure-recovery.pdf}
%     \label{recovery-20K}
%       }
%     \subcaptionbox{Total submission rate of 100K reqs/sec}
%       {\includegraphics[width=0.32\linewidth]{figures/exp/failure-recovery/100K-failure-recovery.pdf}
%         \label{recovery-100K}
%      }
%     \subcaptionbox{Total submission rate of 200K reqs/sec}
%       {\includegraphics[width=0.32\linewidth]{figures/exp/failure-recovery/200K-failure-recovery.pdf}
%         \label{recovery-200K}
%      }
%   \caption{Recover to the same throughput level under different load}
%   \label{fig-recovery-time}
%   \end{minipage}
% \end{figure*}



% We evaluate the failure recovery as shown in Figure~\ref{fig-vc-cost} and Figure~\ref{fig-recovery-time}. Since follower's crash and recovery do not affect the availability of \sysname, we mainly focus on the evaluation of the leader's crash and recovery. We study two aspects: (1) How long does it take for the remaining replicas to complete a view change with the new leader elected? (2) How long does it take to recover the throughput to the same level before crash?


% We maintain 3 replicas and 10 open-loop clients, and vary the client submission rate from 1K reqs/sec to 20K reqs/sec, so the total submission rate varies from 10K reqs/sec to 200K reqs/sec. Under different submission rates, we kill the leader and measure the time cost of view change, as shown in Figure~\ref{fig-vc-cost}. To mitigate the noise effect, we also run each case for 5 times and average them as the reported value. We can see from Figure~\ref{fig-vc-cost}, the time cost of view change grows as the submission rate increases, because there is an increasing amount of state (log) transfer to complete the view change. In general, the view change takes about \SI{150}{\milli\second}-\SI{300}{\milli\second}.

% The time cost to recover the same throughout level is larger than the time cost of view change, because there are other necessary works to do after the replicas enter the new view. For example, replicas need to relaunch the working threads and reinitialize the contexts; replicas need to notify proxies and further the clients to continue submitting requests; replicas need to handle clients' retried requests, which fail to be responded before crash; followers may need additional state transfer due to lagging too far behind, etc. 

% In Figure~\ref{fig-recovery-time}, we plot three recovery cases with different throughput levels. Based on the measured trace, we calculate the throughput every \SI{10}{\milli\second}, and plot the data points in Figure~\ref{fig-recovery-time}. Figure~\ref{fig-recovery-time} implies that the recovery time is related to the throughput level to recover. A lower throughput level takes a shorter time to recover, and vice versa. Figure~\ref{fig-recovery-time} shows three different throughput levels: it takes approximately \SI{0.7}{\second}, \SI{1.9}{\second}, \SI{4.0}{\second}, to recover to the same throughput level under the load of 20K reqs/sec, 100K reqs/sec, 200K reqs/sec, respectively. As a reference to compare, Figure 3.20 in \cite{feiran-craft} evaluates the recovery time for an industrial Raft implementation~\cite{hashicorp-raft}, which takes about 6 seconds to recover to 18K reqs/sec.  

==> microbench.tex <==

\begin{figure*}[!t]
    \centering
    \begin{minipage}{0.3\textwidth}
   \includegraphics[width=1\linewidth]{figures/exp/microbench/reorder-client.pdf}
   \caption{Packet reordering vs. number of senders}
   \label{fig-micro-vary-client}
    \end{minipage}
    \hspace{0.5cm}
    \begin{minipage}{0.3\textwidth}
       \includegraphics[width=1\linewidth]{figures/exp/microbench/reorder-rate.pdf}
       \caption{Packet reordering vs. submission rate}
       \label{fig-micro-vary-rate}
    \end{minipage}
    \hspace{0.5cm}
    \begin{minipage}{0.3\textwidth}
      \includegraphics[width=1\linewidth]{figures/exp/microbench/reorder-dom.pdf}
      \caption{Effectiveness of DOM on packet reordering}
      \label{fig-micro-dom-effectiveness}
    \end{minipage}
\end{figure*}

\section{Micro Benchmark of Reordering in Public Cloud}
\label{sec-microbench}

\subsection{Measurement of Packet Reordering and Evaluation of DOM Effectiveness}

% \begin{figure}[!htbp]
%     \centering
%   \includegraphics[width=6cm]{figures/exp/microbench/reorder-client.pdf}
%   \caption{Packet reordering vs. number of senders}
%   \label{fig-micro-vary-client}
% \end{figure}
% \begin{figure}[!htbp]
%     \centering
%   \includegraphics[width=6cm]{figures/exp/microbench/reorder-rate.pdf}
%   \caption{Packet reordering vs. submission rate}
%   \label{fig-micro-vary-rate}
% \end{figure}

% \begin{figure}[!htbp]
%     \centering
%   \includegraphics[width=6cm]{figures/exp/microbench/reorder-dom.pdf}
%   \caption{Effectiveness of DOM on packet reordering}
%   \label{fig-micro-dom-effectiveness}
% \end{figure}




To evaluate the packet reordering in public cloud, we made a micro benchmark as follows. We launch two receivers (denoted as Receiver-0 and Receiver-1) and multiple senders. After the receivers complete receiving the requests, we take Receiver-0's sequence of requests as the reference, so we get the sequence number of each request based on Receiver-0's sequence. Then, we use these sequence numbers to check how much reordering has occurred on Receiver-1. We count the request received by Receiver-1 as ``reordered request'' if (1) its sequential number is smaller than th1e sequential number of its previous request, or (2) the request does not exist in Receiver-0's sequence (due to packet drop). 

We evaluate in two settings. First, we make each sender send at the rate of 10K reqs/sec (following the Poisson distribution), and vary the number of senders. Second, we only use 2 clients, and varying their submission rates. Each case is run for 5 times and we average the value of the reported number. Figure~\ref{fig-micro-vary-client} and Figure~\ref{fig-micro-vary-rate} show the reordering rate in both settings. Figure~\ref{fig-micro-vary-client} shows that, the reordering rate becomes higher as more senders are involved. Even 2 senders (with 10K reqs/sec each) yield the reordering rate of 8.1\%. Figure~\ref{fig-micro-vary-rate} shows the increase of reordering rate as the submission rate increases from 20K reqs/sec to 40K reqs/sec. Although there is not a continuous trend of reordering rate increase, we can see the reordering rate maintains more than 20\% when the submission rate varies from 40K reqs/sec to 100K reqs/sec.


After the measurement of packet reordering in public cloud, as shown in Figure~\ref{fig-micro-vary-rate}  and Figure~\ref{fig-micro-vary-client}, we would like to study the effectiveness of DOM to reduce packet reordering. We use 10 open-loop clients with each submitting at 10K reqs/sec, so the total submission rate is 100K reqs/sec. Recall that DOM is using a sliding window to estimate the OWD (i.e., $M$ in the OWD estimation formula in \S\ref{sec-dom}). We evaluate the effectiveness of DOM using different percentiles of OWD estimation. In Figure~\ref{fig-micro-vary-client} we already measured that the reordering rate in this setting can reach 36\%. Then, after we have installed DOM~\footnote{Note that in this experiment, both receivers are following the same way as the \sysname leaders, that is to say, when the packet comes late and cannot enter the \emph{early-buffer}, the receiver will modify its deadline to make it eligible to enter the \emph{early-buffer}, instead of leaving it in the \emph{late-buffer} forever.}, we can see from Figure~\ref{fig-micro-dom-effectiveness} that DOM can effectively reduce the reordering rate. Since a larger percentile will leads to a larger estimated value of OWD and further a longer holding delay of the \emph{early-buffer}, it can enable DOM to rectify more reordering cases. On the other hand, the longer holding delay will be added to the latency to commit the requests. 

In order to avoid using a large percentile, \sysname seeks commutativity as an optimization, which has been described in \S\ref{commutativity-optimization}. Given a fixed latency bound, the reordering cases occur more frequently as the throughput grows. But when commutativity is considered, reordering cases does not matter for commutative requests, which essentially makes DOM handle a ``downsampled'' throughput. Therefore, DOM does not need the high percentile estimation and DOM-50p is already sufficient for \sysname to achieve a high fast commit ratio (\SI{80}{\percent}-\SI{97}{\percent}).  


\subsection{Discussion on OWD Variance and Latency Bound Estimation}
\label{discussion-owd-variance}

% \sysname aims to use an estimated latency bound to accommodate the variance of the request one-way delay (OWD), which comes from two aspects as described in \S\ref{sec-dom}: (1) the processing delay of the request at DOM-R (2) the transmission delay from DOM-S to DOM-R. 

% \sysname does not build its correctness on bounded request delay, but a small variance of request delay can benefit \sysname's performance, which enables \sysname to use a small latency bound and suffer less pending delay. Indeed the delay variance in public cloud is more distinct than the bare-metal cluster. However, the isolation provided by today's public cloud~\cite{aws-isolation,gcp-isolation,azure-isolation} is sufficient for \sysname to sacrifice an affordable latency bound and outperform the other baselines, as shown in our evaluation (\S\ref{sec-latency-throughput}). 

%Although we have not experienced a high variance within a single GCP/AWS zone, it is worthwhile to make some extensive discussion on scenarios with highly various one-way delays (OWD). When the OWD measurement shows high variance, in order to commit more requests in the fast path, we need to increase the latency bound, but increasing the latency bound also undermines the latency benefit of the fast path. 

Essentially, the estimation of latency bound is a trade-off  between overall commit/execution latency and the fast commit ratio. A proper latency bound aims to accommodating the variance for \emph{most} conflicting (non-commutative) requests so that they  can achieve a low latency overall. The latency bound does not target at cover the latency variance for \emph{all} request (in that case, the latency bound will be determined by the heavy tail of OWD samples). Thus setting the latency bound is essentially an open question of hyper-parameter tuning, which aims to find the sweet spot between improving fast commit ratio and reducing pending delay in \emph{early-buffer}s. In general, we have considered two turning approaches.

\Para{Approach 1: Target-based tuning.} We pre-define a target of fast commit ratio, and then we let the proxies monitor the change of the fast commit ratio. When the fast commit ratio becomes lower than the target, the proxies increase the latency bound by a step size. Otherwise, it reduces the latency bound by a step size.

\Para{Approach 2: Measurement-based tuning.} We let the replicas collect the OWD samples from proxies, and then the replicas piggyback an estimation of OWD to the proxies (e.g., by using the sliding window mechanism), so that proxies can decide the latency bound based on the estimated OWDs from each replica (e.g., by taking the maximum as the decided latency bound).

Neither approaches can bypass the tuning of some hyper-parameters. Approach 1 needs to tune the target fast commit ratio and the step size whereas Approach 2 needs to decide the proper percentile used for estimation. In the current implementation of \sysname, we choose Approach 2 because its estimation of latency bound is more intuitive and only includes one hyper-parameter. However, just like the other hyper-parameter tuning problems, there is no ``one-size-fits-all'' approach to decide a proper latency bound for every scenario. For instance, when commutativity is unavailable and the submission rate is very high (e.g., more than 100K reqs/sec), DOM-50p may be not the best choice for OWD estimation, and choosing a larger percentile (DOM-75p) may be desirable. \sysname is also compatible to any other intelligent tuning algorithms for \emph{adaptive latency bound}, and we leave the study of better tuning algorithms in our future work.


%In our case,  we choose the moving median to estimate OWD (refer to the formula of \emph{adaptive latency bound} in \S\ref{sec-dom}), because it is robust to the outlier OWD samples caused by the congested request messages, clock skew, etc. When the OWD exhibits more variance than our scenario, it is possible that the other percentiles (e.g. 75th percentile) can achieve better latency than the moving median (50th percentile) used by us.


%Recall that the performance of Speculative Paxos is degraded by 10x with the reordering rate of 1\% (Figure 9 in~\cite{nsdi15-specpaxos}). Figure~\ref{fig-micro-vary-client} and Figure~\ref{fig-micro-vary-rate} indicate that, the public cloud causes more reordering than Speculative Paxos can undertake. Speculative Paxos can hardly work in public cloud, so we do not include it in our comparative evaluation. On the other hand, NOPaxos can work in public cloud and achieves better performance than other baselines such as Multi-Paxos, because its sequencer aggregates the incast traffic from multiple senders, which reduces the reordering effect. However, the software sequencer is not as powerful as a hardware sequencer: a single-thread software sequencer is insufficient to forward the large volume of requests when clients are submitting at high rates, or when there are many replicas. Therefore, we use multi-threading for the sequencer to alleviate its bottleneck. But in that case, the sequencer is equivalent to multiple senders and causes more reordering. 


%Besides, for both Speculative Paxos and NOPaxos, the effect of request reordering/drop is long-lasting. For example, in NOPaxos, when the request with non-consecutive sequential number arrives at the replicas, it triggers the gap handling procedure. The subsequent requests still suffer from the gap handling even if they all arrive in order: they cannot be processed before the gap handling is complete. The long-lasting effect is more distinct to the open-loop tests than the close-loop tests. During the closed-loop test, clients will not continue to submit new requests when the replicas are conducting gap handling. Therefore, the latency measurement of newly submitted requests does not count the gap handling time. By contrast, open-loop clients can have multiple outstanding requests. Even when replicas are undertaking gap handling, the clients still submit new requests, which adds more burden to the replicas and continues to cause reordering/drop (leading to more gap handling work). Meanwhile, the replicas will also hold more pending requests and the latency measurement of all these requests will count the gap handling time. Therefore, NOPaxos yields a worse performance in the open-loop test, compared with the closed-loop test. 



==> nezha_proxy.tex <==
\subsection{{Stateless Proxy Design}}
\label{nezha-proxy}

\rv{Since DOM-R has been installed on each replica, the follow-up consideration is where to install DOM-S, and furthermore, where to check the quorum of the replies corresponding to those requests multicast by DOM-Ses.} 

Mulit-Paxos/Raft rely on the single leader to conduct request multicast and quorum check, which leads to the throughput bottleneck. An alternative design (e.g. Speculative Paxos, NOPaxos, CURP) is to offload the two tasks to the clients. It seems attractive because the offloading can mitigate the workload of the leader and also cut down the commit/execution latency. However, we note that such offloading design is not generally favorable. The reasons come from two aspects: (1) Deployment. Multi-Paxos/Raft are the \emph{de facto} standard protocols widely applied in practice. Protocols with such offloading can hardly be deployed as a direct replacement of Multi-Paxos/Raft due to more intrusiveness to client logic. Even worse, the client VMs may be beyond control in many scenarios and clients do not allow installing extra libraries on their machines, thus making such protocols not deployable. (2) Throughput (of individual clients). Although the offloading design reduces the leader replica's burden, it can cause new bottlenecks to the client. As the number of replicas grows, the client needs to undertake more work to commit every request, and can easily become CPU-intensive, thus constraining its individual throughput (\S\ref{sec:proxy}).
 
 
\rv{Considering the two main drawbacks, we introduce stateless proxies (shown in Figure~\ref{fig-workflow-fast}-\ref{fig-workflow-slow}) between replicas and clients which take over the 2 responsibilities instead of clients/replicas: (1) DOM-S, which includes clock synchronization and request multicast, (2) quorum check.} 

\rv{The proxy design allows the client to be unchanged from Multi-Paxos/Raft. To commit one request, the client just sends and receives one message regardless of the number of replicas. The proxy is a similar on-path device to the NOPaxos sequencer, but there are key differences. First, the stateless nature makes the proxy's failure cause no effect on the protocol correctness; a proxy failure is like a dropped request. By contrast, the NOPaxos sequencer is stateful and requires external entities (e.g., SDN controller) to guarantee its correct state (e.g., session number) after crashes. Second, since our proxy is stateless, its scalability and availability can both be easily improved by adding extra proxies. In contrast, because the sequencer is stateful, it is much harder to add multiple sequencers, hindering both scalability and availability.}

Note that request multicast and quorum check can both be concurrently executed. Therefore, we can employ a flexible number of proxies. Clients can choose any proxy and delegate that proxy to do the multicast and the corresponding quorum check. Different proxies work concurrently without mutual interference. The proper number of proxies depends on the real workload and can be dynamically adjusted by an auto-scaling entity~\cite{google-gke,eurosys20-autopilot,amazon-eks,microsoft-aks}, which is outside the design scope of \sysname.  

\rv{We are aware that the introduction of proxies unavoidably adds two additional message delays to commit requests. However, we believe the benefits (i.e. easy deployment and high throughput of individual client) outweigh the latency sacrifice. Besides, \sysname is also compatible to non-proxy design (i.e. co-locating the proxy with the client): If clients have abundant CPU resource and allow code modification, the non-proxy design is favored for better latency (as shown in \S\ref{sec-latency-throughput}).}

Based on the proxy design, we next describe how proxies interact with replicas to commit requests in fast/slow path. 
% either fast path (\S\ref{sec-fast-quorum-check} and \S\ref{commutativity-optimization}) or slow path (\S\ref{sec-fix-set-inequality} and \S\ref{sec-slow-quorum-check}).



==> notes-worth-thinking.tex <==
1. DOM can be enhanced. For now we only let client set a deadline to cover the OWD variance.
As an enhanced version, DOM can also maintain a tunable parameter (denoted as P) at each replica, i.e.
when replicas previously intend to hold the request up to its deadline, now the replica holds
it until deadline+P. These two tunable parameters (deadline and P) give more power for DOM
to adapt to more delay-varying environment (e.g. WAN)


1.1. In concurrency control, the pending delay (P) can be per-tuple based instead of per-replica based. Because different tuples (keys) may have different popularity

2. A defending note for Nezha against traditional batching:  Some readers may think the high throughput can be easily achieved so long as we do some batching. But, if we do batching, the latency can become much higher (up to ms-level). Although Nezha also suffers from some latency degradation after introducing proxies, we should highlight that, its latency is still good (~300us). If the readers wants high throughput as well as such good latency, Nezha is the best choice. If someone says "I do not care about latency at all and only wants high throughput", of course, you just need to do large-sized batching and that is sufficient, no need to invent new protocols.


==> old/a-protocol-bk.tex <==


\section{Decomposing Ordering Agreement}

While committing requests from concurrent clients, the consensus protocol takes two-fold responsibility.
\begin{itemize}
    \item \textbf{Ordering agreement.} The consensus protocol needs to establish a definitive order for all requests, so that every replica can process the requests following the consistent order.
    \item \textbf{Replication.} The consensus protocol needs to replicate the requests to at least a majority of replicas, so that the requests can be recovered after failure.  
\end{itemize}

Ordering agreement is essential for consistency and lineaizability whereas replication is necessary for durability. 

Reaching ordering agreement is expensive, but an early ordering agreement can avoid heavy penalty when inconsistency really happens later. The typical consensus protocols makes different trade-off between the cost of ordering agreement and the potential penalty of resolving inconsistency. 

(1) Multi-Paxos and NOPaxos chooses to prioritize ordering agreement over replication. Multi-Paxos/Raft and relies on the leader replica as the centralized serialization point to reach the agreement, which suffers from the worst throughput/latency performance. NOPaxos relies on a standalone sequencer as the serlization point, which relieves the throughput bottleneck, but also incurs longer or extra message delay~\footnote{The software sequencer costs 1 extra message delay for NOPaxos. The hardware sequencer does not add extra message delays but requires every request message detour the root switch, thus prolonging the message delay. }. Besides, it also imposes stringent networking requirement, making it hard to deploy in public cloud. 

(2) Fast Paxos and Speculative Paxos choose to prioritize replication over ordering agreement. Such approaches can save some latency and/or throughput overheads in fast path. But when inconsistency really happens, it takes longer time for the leader to detect it and costs more overheads to resolve it. 


\sysname shares the same principle with the later category, i.e. \sysname also prioritizes replication over  ordering agreement. But more importantly, \sysname also avoids heavy penalty to resolve the (possible) inconsistency. The key idea of \sysname is to decompose the ordering agreement and achieve it in two phases: \emph{eliminating ordering ambiguity} during replication and \emph{fixing set equality} during reconciliation. 

Though it is expensive to achieve ordering agreement completely, we notice the ordering agreement can be further decomposed into two main tasks. 
\begin{enumerate}
    \item \textbf{Eliminate ordering ambiguity.} If one replica orders request $a$ ahead of request $b$, no other replicas can order them in a reverse way.   
    \item \textbf{Maintain set equality.} All the replicas should have exactly the same orders (i.e. the sets of orders are equal).
\end{enumerate}
Without introducing the centralized serialization point or inter-replica communication, it is quite challenging to achieve ordering agreement among replicas. However, by using clock synchronization, it is fairly easy to eliminate ordering ambiguity first, and we can postpone the requirement of set equality later. 
% \section{Main Assumptions of Nezha}
% The design of Nezha is built atop two main assumptions. However, it is worth noting the two assumptions do not affect the safety of the protocol, and they only affect the liveness of \sysname. 
% \begin{enumerate}
%     \item \textbf{Mostly-Bounded Latency}. Nezha assumes that the latency between VMs (both clients and replicas) are mostly bounded ((i.e. not necessarily always bounded).
%     \item \textbf{Mostly-Synchronized Clocks}. Nezha assumes that the clocks on VMs (both clients and replicas) are mostly synchronized with a small error bound (i.e. not necessarily always synchronized)
% \end{enumerate}


% The key idea of \sysname is to initially use an \emph{approximate ordering} (which is probably consistent among the majority), and then pay trivial cost to upgrade \emph{approximate ordering} to \emph{consistent ordering} (which is truly consistent among the majority).

% A consistent state is achieved if every replica maintains the same ordering for the same requests. Such consistent ordering is expensive to performance, which requires a centralized serialization point such as the leader (e.g. Multi-Paxos/Raft) or a standalone sequencer (e.g. NOPaxos). 

% Incomplete but correct ordering. 




% Without a centralized serialization point, each replica needs to decide the ordering rank of its received requests. However, considering request reordering/drop, it is not guaranteed for the same request to be assigned with exactly the same ordering rank on each replica. \sysname does not intend to achieve this during the replication process, however, it is possible for the replicas to eliminate ordering ambiguity for the requests . 

% the replicas to agree with the consistent ordering rank for each request. However, it is possible for each replica to eliminate the ordering ambiguity 

% Although unable to decide the consistent ordering rank for each request without a centralized serialization point, \sysname can eliminate the ambiguity of requests at each 

% Ordering agreement can be expensive

% However, if ordering agreement is not reached early, it is possible to face significant penalty later when inconsistency occurs. 

%  \sysname is not doing order agreement at the beginning, but it eliminates ordering ambiguity, so as to avoid heavy penalty even when inconsistency happens later. 
 

% Protocols, such as Multi-Paxos/Raft and NOPaxos, uses a centralized serialization point (the leader replica or the sequencer) to erase the ordering ambiguity. 


% An always-correct ordering agreement is expensive to maintain, and it requires a centralized serialization point to 

% A consistent ordering is necessary for any consensus protocols. However, the consistent ordering is expensive  

% \begin{enumerate}
%     \item Consistent (but Possibly Incomplete) Ordering
%     \item Set equality.
% \end{enumerate}

\section{\sysname Protocol Design}
\sysname is a new consensus protocol that allows the client to complete linear updates in 1 RTT (2 message delays) in normal cases. To ensure the durability, the client broadcasts the request to every replica. Different from previous protocols (e.g. Fast Paxos, Speculative Paxos, NOPaxos, etc), the client itself decides the ordering rank of the request by tagging synchronized clock time in the request. Each replica \textbf{selectively} accepts the requests and \textbf{independently} sorts them according to the ordering rank. Since the ordering rank of requests has been pre-assigned during submission, the inter-replica consistency problem is simplified to the set equality. When the follower's set of requests becomes unequal to the leaders' set of requests, the leader takes the responsibility to fix set equality by adding/deleting requests to/from follower's set.


\subsection{Architecture and Model}
\sysname assumes a fail-stop model and does not handle byzantine failure. As in typical consens protocols, it uses $2f+1$ replicas, including 1 leader and $2f$ followers. In addition to that, \sysname makes two assumption of the system. 

\begin{enumerate}
    \item \textbf{Mostly-Bounded Latency}. Nezha assumes that the latency between clients and replicas are mostly bounded (i.e. not necessarily always bounded).
    \item \textbf{Mostly-Synchronized Clocks}. Nezha assumes that the clocks on VMs (both clients and replicas) are mostly synchronized with a small error bound (i.e. not necessarily always synchronized)
\end{enumerate}

Although \sysname makes assumptions about latency bound and clock synchronization, it does not rely on these assumptions for correctness. It remains correct under the same assumptions as Multi-Paxos/Raft. 

The workflow of \sysname can be divided into fast path and slow path. Normally, clients commit their requests through fast path, which can be completed in 1 RTT. When inconsistency happens between leader and followers, the request is committed through slow path, which can be completed in 2 RTTs or up to 3 RTTs. Among the $2f+1$ replicas, only the leader executes the request and replies the execution result. The other $2f$ followers mainly stores the requests to survive crash.





% For each request, the client needs to replicate the submission to all replicas. After receiving the request, replicas may reply with
% \begin{enumerate}
%     \item \emph{acceptance}, together with a hashed value, which is calculated with all the entries in its log. If the replica is the leader, it also includes the execution result of the request in the reply.
%     \item \emph{rejection}.
% \end{enumerate}
% Since there are 2 types of reply (\emph{acceptance} and \emph{rejection}),
% the format of the replies are as follows.
% \begin{equation*}
%     acceptance = <\texttt{ACCEPT}, clientID, reqID, h, result, replicaID>
% \end{equation*}
% \begin{equation*}
%     rejection = <\texttt{REJECT}, clientID, reqID, replicaID>
% \end{equation*}
% where $h$ is the hash value, and $result$ is the execution result (If the replica is the leader), 
% Then client considers the request as \emph{successful} after it receives the leader reply and $f+\lceil f/2 \rceil$ follower replies, AND the hash values in these $1+f+\lceil f/2 \rceil$ replicas are the same. Only when the request is successful, can Nezha reveal the execution result to the upper application. We explain why we need $1+f+\lcei f/2 \rceil$ replies (rather than $1+f$) in \S~\ref{sec:superquorum}.

% When the request is not successful, the client is experiencing either timeout case (\S~\ref{sec:timeout}) or conflict case (\S~\ref{sec:conflict}). For timeout case, client simply resends the request, but with some different time information (more details at \S~\ref{sec:timeout}). 
% For conflict case, client sends a $resolve$ request to the leader, and leader will reply to the client. After receiving the reply to its $resolve$ request, the client also considers the request as successful (more details at \S~\ref{sec:conflict}). 


\subsection{Fast Path}
\label{sec:normal}
\subsubsection{Replicated Submission}
\label{sec:replicated-submission}
When the client submits its request, it broadcasts the request to every replica. In the request, it includes its submission timestamp $s$, and a latency bound $d$. The request is expected to reach all replicas by $t_a = s+d$. The format of the client request can be described as 
\begin{equation*}
    req = <clientID, reqID, s, d, command>
\end{equation*}

The four fields, i.e. $clientID$, $reqID$, $s$ and $d$, are required for every request. $<clientID, reqID>$ can uniquely identify one request. $<s, d>$ can be used by the replicas to decide whether they should accept or reject the request. If the request is accepted by the replica, it will be converted into a log entry, with $t_a = s+d$ as the ordering rank, and eventually added to the log set of the replica.

\subsubsection{Selective Acceptance}
In order to eliminate ordering ambiguity among the received requests, the replicas add the requests to its log set strictly following the ranking order of their $ta$. To realize that, the replica keeps a hold-and-release (HR) buffer, which holds and releases the requests based on their $ta$. 

When the request $req$ arrives at the replica, the replica first compares its local clock time $t_l$ with $t_a$. The replica rejects the request if it finds $t_a < t_l$, and sends a rejection reply immediately to the client. 


The replica chooses to accept $req$ if $t_a \geq t_l$. Then $req$ will be held by the HR buffer until $t_a$. Then $req$ is released and appended as a log entry to the replica's log set. If the replica is the leader, it also executes the request. Meanwhile, the replica sends an acceptance reply to the client. Inside the acceptance reply, each replica includes a hash value, which encodes current log set (denoted as $logSet$) of the replica with an incremental hash  function~\cite{increment-hash}, i.e. 
\begin{equation}
\texttt{Hash}(logSet) = 
\bigoplus_{log_i \in logSet} h(log_i)
\end{equation}
where $h(*)$ is a standard hash function (e.g. SHA1) and  $\oplus$ is the XOR operation. Since the hash value is calculated based on all the requests, it represents the current state of the replica. 

The incremental hash enjoys two advantages: 
First, it provides an easy way to check set equality, which is sufficient to ensure the replica consistency in \sysname because the ordering rank has already been included in every request.

Second, the hash value is computed in an incremental way. Adding or deleting requests only requires incremental computation of XOR and $h(*)$. Such a property is useful while \sysname resolves the inconsistency (described in \S~\ref{sec:sync-process}) and causes trivial overheads.

\subsubsection{Quorum Check}
The client considers the request as committed when it receives the acceptance replies from the fast quorum. The fast quorum is composed of 1 leader reply and $f+\lceil f/2 \rceil$ follower replies, which have the same hash value. Besides, from the leader's acceptance reply, the client obtains the execution result of the request. 

By contrast, it becomes impossible for the client to form a fast quorum under one of the three situations.
\begin{enumerate}
    \item The client receives the leader's rejection reply;
    \item The client receives the leader's acceptance reply, as well as $>\lfloor f/2 \rfloor$ follower replies, which are either rejection, or acceptance with a different hash value; 
    \item The client does not receive the leader's reply. Denote the number of received replies as $r$. Among the $r$ replies, denote the number of the most frequent hash value as $m$, then $m+(2f+1 -r)<f+\lceil f/2 \rceil+1$~\footnote{In other words, even all the other replies are received later with the same hash value as the most frequent one, it is still insufficient to form a fast quorum.}
\end{enumerate}

Under such situations, the client considers the request as conflicted and stops waiting for other replies. Instead, the client issues a sync request to the client and tries to commit its previous request through the slow path (described in \S~\ref{slow-path}).

\subsubsection{Timeout}
There are situations when the client cannot decide whether the request is committed or conflicted. Such situations can trigger the timeout of the client, and client will retry the replicated submission of the same request, but with a different $s$. The resubmitted request is treated as a fresh request and replicas reply with a new hash value if they accept the requests. However, the leader maintains at-most-once semantics during the execution. When noticing it has previously executed the request with the same $<clientID, reqID>$, the leader reply the previous execution result instead of executing it for a second time.

Since \sysname allows at most $f$ replica to crash at the same time, at the worst case, there is less than a fast quorum of healthy replicas, which makes it impossible to commit requests through the fast path, and leads to infinite retry. 

To ensure progress under the worst case, \sysname maintains a bound for the retry times. After retrying the replicated submission for a certain times, the client will abandon the fast path and try to commit its previous request through the slow path (described in \S~\ref{slow-path}).

\subsection{Slow Path}
\label{slow-path}
\subsubsection{Issue Sync Request}
When the client notices the request is conflicted, or has retried for a bounded times but fails to commit the request, the client chooses to commit the request through the slow path. To do that, the client issues a sync request to the leader, which includes the body of the previous uncommitted request (i.e. $clientID$, $reqID$, and $command$ ), without time information (i.e. $s$ and $d$). The format of the sync request can be described as 
\begin{equation*}
    sync = <\texttt{SYNC}, clientID, reqID,command>
\end{equation*}

Once the leader receives the sync request, it first checks the existence of its logs with $<clientID, reqID>$. If the request does not exist on the leader's log, then leader chooses the current time as the $ta$ for this request, and appends the request as a new log entry to its logs, then the leader starts the sync process among replicas. Otherwise, the request already exists on the leader, then the leader directly starts the sync process without appending. 

\subsubsection{Sync Process}
\label{sec:sync-process}
The leader conducts the sync process with the followers periodically, or after receiving the sync request from clients. The workflow of the sync process is similar to Multi-Paxos/Raft: The leader contacts a slow quorum of replicas ($f+1$ replicas including the leader itself), to ensure the consistency among them. 

Since the ordering rank has already been included in each log, the two replicas are considered as consistent if and only if the set equality is achieved regarding their logs. 

During the sync process, the leader chooses the latest log entry (i.e. with the largest $ta$) in its log set as the sync point. It uses its own log set as the reference to modify the log set of followers, adding/deleting logs to/from their log sets. Along with the addition/deletion of logs, the incremental hash value is also updated to keep representing the current state of the replica. Since XOR is self-associative, the incremental hash can be incrementally modified by simply XOR the hash ($h(*)$) of the added/deleted logs, which only costs subtle overheads~\footnote{According to our measurement, while using the standard openssl library to compute SHA1 hash for the request with 16-byte input (i.e. the size of $<ta, clientID, reqID>$), the time cost is about  0.15$\mu s$. Besides, the XOR computation with two 20-byte value (the size of the SHA1 hash value) only costs 0.0087$\mu s$  }. 

After the leader receives the replies from $f$ followers, confirming that they have become consistent with the leader up to the sync point. The leader ensures its log entries up to the sync point will survive the crash. If there are pending sync requests from the clients and the $<clientID, reqID>$ indicates a log entry within the synced scope, then the leader replies to the client with a \texttt{SYNCED} confirmation. After receiving that, the client considers its request as committed through the slow path.

\section{Recovery}
\label{sec:recovery}




$req$ is not immediately appended to the log, because other requests with smaller ordering rank may come between $[t_l, ta]$. 



When it comes to $t_a$, the replica converts $req$ to a log entry and appends it to its logs, denoted as $logSet$. $logSet$ is a sorted set, and each entry in $logSet$ has the format as follows. 
\begin{equation*}
    \forall e_i \in logSet,  e_i = <t_i, clientID_i, reqNo_i, content_i, h_i, result_i>
\end{equation*}
$t_i$ is the time when $e_i$ is added to $logSet$ (it is $t_a$ mentioned above). $<clientID_i, reqNo_i, content_i>$ are copied from the request. $h_i$ is a hash value, which is calculated from the first entry of $logSet$ to $e_i$, i.e. $$h_i=\texttt{Hash}(logSet.begin(),\cdots, logSet.find(e_i))$$
$result_i$ is the execution result of the request content $content_i$. Only leader executes the request, and the followers just append the request (i.e. $result_i=$NULL) to their $logSet$ (as an optimization, followers can also execute requests during sync process, described in \S~\ref{sec:sync}).

$logSet$ sorts its entries based on the first 2 fields of each entry $e_i$, i.e. $<t_i, client_i>$. The comparator is defined as follows.
\begin{equation*}
\begin{split}
    & \forall e_i, e_j \in logSet, \\
    & e_i=<t_i, clientID_i, reqNo_i, content_i, h_i, result_i>, \\
    & e_j = <t_j, clientID_j, reqNo_j, content_j, h_j, result_j> \\
\end{split}
\end{equation*}
we say $e_i < e_j$ iff (1) $t_i < t_j$, or (2) $t_i=t_j$ and $clientID_i < clientID_j$. 

Hence, there are two 2-tuples that can be used as searching key to uniquely identify an entry in $logSet$, i.e. $<t_i, clientID_i>$ or $<clientID_i, reqNo_i>$, but only $<t_i, clientID_i>$ decides the order of the entry in $logSet$. 

Even when $t_a < t_l$, there is still some possibility to add $req$ to $logSet$, so long as the latest entry in $logSet$ is smaller than $req$ based on the comparator, i.e. 
Denote $e_i=logSet.last()$, when $t_a<t_l$, $req$ can still be added into $logSet$, so long as (1) $e_i.t_i< t_a$ or (2) $e_i.t_i=t_a$ and $e_i.clientID < req.clientID$. Under such conditions, $req$ will become an entry that is appended to the \textbf{end} of $logSet$, so it will not affect the  order of existing entries. 


Note the hash value $h_i$ for the entry $e_i$ is calculated based on all the entries in $logSet$, up to $e_i$. It involves much repeated calculation since each hash computation starts from scratch. 
To accelerate the hash computation, we adopt incremental hash functions~\cite{increment-hash}, which enjoys incrementality and parallelizability. We describe the details of computing incremental hash function in \S~\ref{sec:inhash}. 

After adding $req$ into $logSet$ (leader also needs to execute $req$ to generate $result$) and computing the hash value $h$, the replica replies to the client, and the format of the reply is as follows.
\begin{equation*}
    reply = <clientID, reqID, h, result, replicaID>
\end{equation*}

In the normal case, $req$ can arrive at the replicas before $t_a=s+d$. If (1) the latency bound is true and (2) the clocks of clients and replicas are well synchronized, then replicas will reply with \emph{acceptance} with a hash value. The client considers $req$ as successful only when it receives the leader reply and $f+\lceil f/2 \rceil$ follower acceptance reply, AND the hash values in their replies are the same. Otherwise, the client encounters \emph{timeout} (described in \S~\ref{sec:timeout}) or \emph{conflict} (described in \S~\ref{sec:conflict}) .



% Otherwise, $t_a < t_l$, and it means $req$ comes too late. The replica then sends $rejection$ to the client. Meanwhile, the replica starts a \emph{sync process} (described in \S~\ref{sec:sync}).  


\section{Timeout Case}
\label{sec:timeout}
After the client submits a request, it will wait for the reply from the replicas for a certain time period (e.g. 10ms). 

However, it is possible that the request is dropped during the transmission to some replica, and it is also possible that the reply is dropped during the transmission to the client. 


If the client fails to receive 1 leader reply and $f+\lceil f/2 \rceil$ replies within the time period, then the client encounters \emph{timeout}. To solve such a situation, the client simply resubmits the request, but with a different submission time $s$ and (possibly) a different latency bound $d$.  

Besides, the replica maintains \emph{at-most-once} semantic, by checking whether $<clientID, reqNo>$ exists in $logSet$. If the replica find the incoming request has already been executed (leader) or appended (follower), it will simply resend the previous reply and will not add it to $logSet$ any more. 

It provides liveness as long as messages that are repeatedly resent are eventually delivered before the recipients time out. This requirement is the same as in Paxos.


\section{Conflict Case}
\label{sec:conflict}
Replicas do not always reply $acceptance$ to clients. When the replica receives the request $req$ from the client, and find its $t_a<t_l$ and $req>logSet.last()$, then such a request can not be added to $logSet$ for fear of breaking consistency and linearizability. Therefore, replicas will send $rejection$. Meanwhile, if the replica is a follower, it will contact the leader to ask whether $req$ can be added into $logSet$. If the replica is the leader, it will immediately start the sync process (described in \S~\ref{sec:sync}).


The client encounters \emph{conflict} under one of the following situations.
\begin{enumerate}
    \item The client receives the leader's \emph{rejection} reply.
    \item The client receives the leader's \emph{acceptance} reply, but also receives more than $\lfloor f/2 \rfloor$ followers' replies, which are \emph{rejection}, or \emph{acceptance} with a different hash value from that hash value in leader reply.
\end{enumerate}

If either situation occurs, then the client knows it cannot form a quorum with 1 leader and $f+\lceil f/2 \rceil$ followers, with \emph{acceptance} and the same hash value. We call such situations $conflict$ situations. To resolve $conflict$, the client must send \texttt{Resolve} request to the leader replica. 

The format of the \texttt{Resolve} request is as follows.
\begin{equation*}
    resolveReq = <\texttt{RESOLVE}, clientID, reqNo,content>
\end{equation*}

Note that $resolveReq$ does not need to involve time information such as $<s,d>$. The leader will accept it and process it so long as it is not dropped in flight. 
% $<clientID, reqNo>$ is sufficient to identify $req$, and $<s, t>$ no longer makes sense during the sync process, therefore, the sync signal only includes the 3 fields (i.e. $clientID, reqNo, content$) from $req$, and excludes $s$ and $t$.

After receiving $resolveReq$, the leader stops processing incoming client requests (i.e. it can keep receiving the requests and add them into its pending queue). The leader needs to handle $resolveReq$ before it can continue to process client requests. The processing workflow can b summarized as Algorithm~\ref{algo:resolve-handle}.

% % Algorithms
\begin{algorithm}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Handle Resolve Request}
\label{algo:resolve-handle}
\SetAlgoLined
\SetKwInOut{r}{}
 \Input{$resolveReq$ - the resolve request sent from some client}
  $id$=<$resolveReq.clientID$, $resolveReq.reqNo$>\\
  $entry$=$logSet$.find($id$) \\
  \uIf{entry$\neq\emptyset$}{
    \tcp{This entry exists in $logSet$}
    \uIf{entry>syncPoint}{
    \tcp{This entry has not been synced by leader with its followers}
        Start sync process (described in \S~\ref{sec:sync}) \\
    }
    $reply=$<\texttt{SYNCED}, $id.clientID$, $id.reqNo$, $entry.h$, $entry.result$, $replicaIdx$> \\
    Ack $reply$ to client \\
  }
  \uElse{
  $t=$\texttt{GetCurrentTime}()\\
  $entry=$<$t, resolveReq.clientID,resolveReq.reqNo,$\\
  \Indp$resolveReq.content,$ NULL, NULL>\\
  \Indm\dosemic\tcp{Add entry to logSet, and execute it after sync process}
  $logSet$.insert($entry$)\\
   Start sync process (described in \S~\ref{sec:sync}) \\
   \tcp{Execute entry, update result and hash value}
   \texttt{Execute}($entry$)\\
   $reply=$<\texttt{SYNCED}, $id.clientID$, $id.reqNo$, $entry.h$, $entry.result$, $replicaIdx$> \\
    Ack $reply$ to client \\
}
  
\end{algorithm}
As shown in Algorithm~\ref{algo:resolve-handle},The leader first checks whether $<resolve.clientID, resolve.reqNo>$ exists its $logSet$ (remember that $<clientID, reqNo>$ uniquely identifies one request).

\begin{enumerate}
    \item If the leader can find the log entry $entry$ with $<resolve.clientID, resolve.reqNo>$ (line 3), 
    \begin{enumerate}
        \item the leader then checks whether this log entry has already been synchronized by the leader and its followers. If $entry$ has not been synced among the leader and its followers(line 4), then the leader immediately start the sync process (described in \S~\ref{sec:sync}).
        
        \item If the leader ensures that this log has already been synchronized, it can safely reply to the client with \texttt{SYNCED} (line 6-7). After receiving \texttt{SYNCED} reply corresponding to its request, the client considers this request as successful and can continue to submit its following requests.

    \end{enumerate}
    
    \item Otherwise, the leader's $logSet$ does not contain $<resolve.clientID, resolve.reqNo>$. Then the leader uses its current time $t$ and the $clientID$, $reqNo$ and $content$ in $resolveReq$, to form a new log entry $entry$. The hash value and execution result are set NULL for now (line 9-10), and append this element to the end of $logSet$ (line 12). Instead of executing it immediately, the leader starts the sync process (described in \S~\ref{sec:sync}). After finishing the sync process, the leader then executes the entry and update the corresponding result and hash value in $logSet$ (line 14), afterwards it sends the \texttt{SYNCED} reply to the client (line 15-16). 
\end{enumerate}
 






% If so (i.e. it has replied \emph{acceptance} to the client before), it immediately starts the sync process (described in \S~\ref{sec:sync}).

% \paragraph{} \label{para:other} Otherwise (i.e. it has replied \emph{rejection} to the client before), it first makes a 2-tuple with its current time $t_l$ and $resolve.req$, and inserts $<t_l, resolve.req>$ to $logSet$. In this way, the leader ensures that $resolve.req$ does not affect the execution result of previous logs (i.e. $req$ does not cause rollback to the leader). After the leader inserts $req$ to its log, it does not execute it immediately, then it starts the sync process (described in \S~\ref{sec:sync}).

\section{Sync Process}
\label{sec:sync}
Leader periodically runs sync process with its followers. A bit different from the client request submission, the sync process only needs 1 leader and $f$ followers to participate, i.e. its quorum size is $f+1$. 

The periodic sync process has two purposes.
\begin{enumerate}
    \item By doing sync process, followers can discover their inconsistency from the leader, and resolve the divergence at an early time. 
    \item The sync process enables the follower to safely execute the requests. In that way, when the leader fails and some follower becomes the new leader, the new leader does not need to execute all the logged entries from scratch, thus accelerating the recovery. 
\end{enumerate}

Initially, each replica maintains a variable, i.e. $syncPoint$. $syncPoint$ is intialized as NULL, which means the replica has not synchronized its $logSet$. 

To start the sync process, the leader issues a sync request $syncReq$ to all the other replicas. The format of the \texttt{SYNC} request is as follows.
\begin{equation*}
    syncReq = \{syncRequestID, logIndices \}
\end{equation*}
where $logIndices=[<t_1, clientID_1, reqNo_1>, <t_2, clientID_2, reqNo_2>, \cdots]$

$syncRequestID$ is used to identify the message. The leader increments $syncRequestID$ for every new round of sync process. The follower executes the sync process, strictly following the consecutive order of $syncRequestID$s. 

$logIndices$ encodes the indices of entries in $logSet$, from $syncPoint$ to its latest entry in $logSet$. Since $logSet$ is sorted by $<t_i, clientID_i>$, $logIndices$ is also sorted by $<t_i, clientID_i>$, and we can use either $<t_i, clientID_i>$ or $<clientID_i, reqNo_i>$ to identify a specific entry.


While the follower is handing $syncReq$,
it starts from its $syncPoint$ ($syncPoint$=NULL means starting from the beginning of $logSet$), and compare the indices of its entries with the indices in $syncReq$. The follower tries to make its $logSet$ consistent with the leader's $logSet$. The workflow can be described as Algorithm~\ref{algo:set-diff} and Algorithm~\ref{algo:set-diff-cont} .

% % Algorithms
\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Handle Sync Request}
\label{algo:set-diff}
\SetAlgoLined
\SetKwInOut{r}{}
 \Input{$syncReq$ - the sync request from the leader,$syncReq=$<$syncRequestID$,$logIndices$> \newline $logSet$ - the follower's log set \newlien $lastSyncRequestID$- $syncRequestID$ of last $syncReq$ that has been executed by the follower}
 
 \uIf{$syncRequestID \leq lastSyncRequestID$}{
    \tcp{This syncReq is stale}
    $syncReply = <syncRequestID, \texttt{SYNCED}>$ \\
    Send syncReply to the leader
    return\\
  }\uElseIf{$syncRequestID > lastSyncRequestID+1$}{
    \tcp{There are some syncReq missing, fetch them from the leader}
    $mss$ =\texttt{FetchSyncReqs}($lastSyncRequestID$+1, $syncRequestID$-1) \\ 
    \For{$sReq \in mss$}{
        Run Algorithm~\ref{algo:set-diff} with $sReq$\\
    }
  }
  
  \tcp{Before the sync process, the follower knows log entries up to syncPoint has been synced in previous sync processes, so the follower starts from the next entry after syncPoint}
  \uIf{syncPoint=NULL}{
    $startEntry = logSet$.begin()
  }\uElse{
  $startEntry=logSet$.find($syncPoint$)+1 \\}
  
  $startIndex$=<$startEntry.t$,$startEntry.clientID$, $startEntry.reqNo$> \\ 
  $redundantEntries = \{\}$\\
  \While{startIndex \leq logIndices.last()}{
    \uIf{logIndices.contains(startIndex)=False}{
    \tcp{Leader does not contain this entry}
        $redundantEntries += \{startEntry\}$
    }
    \tcp{Advance the iterator}
    startEntry++ \\
    $startIndex$=<$startEntry.t$,$startEntry.clientID$, $startEntry.reqNo$> \\ 
  }
  \tcp{Remove all redundant entries from follower's logSet}
  \For{entry \in redundantEntries}{
    logSet.erase(entry)}
\end{algorithm}


\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Handle Sync Request (cont.)}
\label{algo:set-diff-cont}
\SetAlgoLined
  \tcp{missingEntries contains the indices of entries that exist on the leader but do not exist on this follower}
  $missingEntries = \{\}$\\
  \For{$index \in logIndices$}{
    \tcp{index is a 3-tuple, but <clientID, reqNo> is enough to identify an entry}
    $id=<index.clientID, index.reqNo>$ \\
    $entry=logSet.find(id)$ \\ 
    \uIf{$entry == \emptyset$}{
        $missingEntries += \{ id \}$
    }\uElse{
        \uIf{$entry.t \neq index.t$}{
            $entry.t = index.t$
        }
    }
  }
  \uIf{$missingEntries \neq \emptyset$}{
    \tcp{Fetch the missing entries from the leader}
    mss = \texttt{FetchEntry}(missingEntries) \\
    \For{$entry \in mss$}{logSet.insert(entry)}
  }
  
  \tcp{Since follower's logSet may add/delete some elements, the following hash values since syncPoint should be updated correspondingly}
  \texttt{UpdateHash}(syncPoint+1, logSet.end())\\
   \tcp{After the execution of the algorithm, the leader's and follower's logSet should be consistent up to syncPoint}
   syncPoint = logSet.find(logIdices.last())\\
  
  \tcp{At the end of the sync process, follower acks a reply to the syncRequest of the leader}
  syncReply = <syncRequstID, \texttt{SYNCED}> \\
  Send syncReply to leader 
\end{algorithm}

After the execution of Algorithm~\ref{algo:set-diff} and Algorithm~\ref{algo:set-diff-cont}, followers update their $syncPoint$ (line 17 in Algorithm~\ref{algo:set-diff-cont}) and ensures that it has the same logs as the leader up to $syncPoint$, so it sends back a reply to the leader (refer to line 18-19 in Algorithm~\ref{algo:set-diff-cont}), notifying the leader that it has become consistent with the leader up to $syncPoint$. 

After the leader receives $f$ followers' replies to its $syncReq$,  the leader also updates its $syncPoint$ (similar to line 19 in Algorithm~\ref{algo:set-diff-cont}), and it knows that there are $f+1$ replicas which have consistent logs up to $syncPoint$. Therefore, it ensures that the $syncPoint$ will persist even after $f$ failures. 


\section{Optimization of Sync Process}
\label{sec:sync-optimization}

\subsection{Checkpoints}
In essence, Line 15-20 in Algorithm~\ref{algo:set-diff}
 and line 2-10 in Algorithm~\ref{algo:set-diff-cont} are doing diff operation between follower's $logSet$ and $logIndices$, and the range is from $syncPoint+1$ to $logIndices.last()$. However, considering that conflict is a rare event, and most of the follower's entries are consistent with leader's entries. We can select a few checkpoints from $logIndices$. 
 
 A simple example is to choose the index in the middle (denoted as $mid=<t_m, clientID_m, reqNo_m>$) of $logIndices$, and we include its hash value (denoted as $h_m$) in $syncReq$. During the sync process, we first search for $<clientID_m, reqNo_m>$ in the follower's $logSet$. If we can find the entry and the hash value of the entry equals $h_m$, then we consider the follower's log entries are consistent with the leader's log entries up to $mid$. Then we can immediately start the following diff oepration from $mid+1$, instead of $syncPoint$. In this way, the traveral workload is reduced by half. 
 

\subsection{Parallel Hash Update}
\label{sec:parallel}
In line 16 of Algorithm~\ref{algo:set-diff-cont}, when there are addition/deletion in the $logSet$ (i.e. $redundantEntries\neq \emptyset$ or $missingEntries \neq \emptyset$), we need to update the hash values from the last syncPoint to the latest log entry. If the update is executed iteratively, it can be time consuming and linear to the length from the last syncPoint to the latest log entry. However, since we are using incremental hash functions, the hash update can be parallelized, and the time complexity is only proportional to the length of the change scope of $logSet$. We described more details in \S~\ref{sec:inhash}.

\section{Recovery}
\label{sec:recovery}
\subsection{Follower Fail}
The case of follower crash is easy to handle. When the follower crashes and relaunches, before it can process new requests, it needs to completely copy the $logSet$ of the leader. Then, it can continue to append new requests and reply to the clients.

\subsection{Leader Fail}
When the leader fails, all the replicas stop processing new requests. The followers first elect a new leader via standard Viewstamped Replication protocol~\cite{viewstamp}. Then, the new leader first gathers the $logSet$ of the other $f$ replicas. Together with its own $logSet$, the new leader will recover the state based on the $f+1$ $logSet$s.

First, it initializes an empty $logSet$, and then it finds the replica which has the largest $syncPoint$, then it replicates the $logSet$ of that replica, up to $syncPoint$. 

Starting from $syncPoint$, the leader checks every entry, if $entry > syncPoint$ and $entry$ exists in at least $\lceil f/2 \rceil +1$ of the $f+1$ replicas, then leader adds the entry into its $logSet$ and also execute the entry.

After the new leader recovers $logSet$, it asks all the followers to use its $logSet$ to replcace their own (i.e. the leader forces the followers to keep consistent with its logs via sync process). Completing this step, the system is fully recovered and continues to work. 

The the new leader's operation can be described as Algorithm~\ref{algo:recovery}.

\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Recovery}
\label{algo:recovery}
\SetAlgoLined
\SetKwInOut{r}{}
 \Input{$logSets$- The $f+1$ replicas' logSets, e.g. $logSets[1]$ is the $logSet$ of the 1st replica. \newline $syncPoints$- The $f+1$ replicas' yncPoints, e.g. $syncPoints[1]$ is the $syncPoint$ of the 1st replica  }
 \tcp{Initialize a new logSet}
 $nLogSet=\{\}$
 $i = \argmax_x syncPoints[x]$ \\
 $largestSyncPoint=syncPoints[i]$ \\
 \For{$entry \in logSets[i]$}{
    \uIf{$entry \leq largestSyncPoint$ }{
        $nLogSet.insert(entry)$\\
    }
 }
 \tcp{it records the log entry beyond largestSyncPoint, as well as the number of replicas containing the entry}
 $logMap=\{\}$ \\
 \For{$logSet \in logSets$}{
    \For{$entry \in logSet$}{
        \uIf{$entry > largestSyncPoint$}{
            $logMap[entry]++$\\
        }
    }
 }
 \For{$<entry, freq> \in logMap$}{
    \uIf{$freq > \lceil f/2 \rceil$}{
        $nLogSet.insert(entry)$ 
    }
 }
\tcp{The leader uses nLogSet to replicace its old logSet}
$logSet=nLogSet$ \\
\tcp{Force the followers to keep consistent with the recovered logs via sync process}
Start sync process \\
\tcp{After finishing the sync processs (i.e. receiving $f$ follower's reply), then the leader can continue to process new requests}
\end{algorithm}


\section{Proof of Correctness}
\label{sec:proof}
We follow the proof method in CURP paper(refer to Appendix A in ~\cite{nsdi19-curp}).
We want to prove that the recovery protocol of Nezha guarantees the following correctness properties.

\begin{enumerate}
    \item \textbf{Durability:} if a client considers a request as successful, the request survives replica crashes.
    \item \textbf{Consistency:} if a client considers a request as successful, the execution result remains consistent after replica crash recoveries.
    \item \textbf{Linearizability:} a request appears to be executed exactly once between start and completion. The definition of linearizability can be reworded as following: if the execution of a request is observed by the issuing client or other clients, no contrary observation can occur afterwards (i.e. it should not appear to revert or be reordered). 
\end{enumerate}

\subsection{Proof of Durability}
If the client considers $req$ as successful, then $req$ has been replicated to the leader and at least $f+\lceil f/2 \rceil$ followers. Besides, we also know the $f+\lceil f/2 \rceil$ replies with the same hash value as the leader, indicating these followers' $logSet$s are consistent with the leader's $logSet$ up to $req$. Therefore, $req$ (and also all entries before $req$) will not be erased during the sync process. When the leader crashes, 
\begin{enumerate}
    \item if $req<largestSyncPoint$ (refer to \S~\ref{sec:recovery}), then it will be directly copied to the new leader's new $logSet$ (line 8-13 in Algorithm~\ref{algo:recovery}). 
    \item  Otherwise, among the $f+1$ replicas selected by the new leader, $req$ exist in at least $\lceil f/2 \rceil+1$ of them for sure, due to quorum intersection. Therefore,$req$ will be added to the new $logSet$ of the leader.
\end{enumerate}
 
 Therefore, any successful request will always survives replica crashes.

\subsection{Proof of Consistency}
Followers' crash and recovery does not affect consistency, since the follower does not execute the request (or log entry). Then we only need to consider leader crash and recovery.

Taking an arbitrary successful request $req$. If $req$ has been synced before leader crash, then $req$ and all the previous entries will be unchanged and directly copied to the new leader (line 3-6 in Algorithm~\ref{algo:recovery}). Therefore, the execution result of $req$ remains unchanged. 

Otherwise, $req$ has not been synced (line 7-17 in Algorithm~\ref{algo:recovery}).

Based on the proof of durability, we know that every successful requests can survive. If $req$ is successful, then leader and at least $f+ \lceil f/2 \rceil$ followers have the same hash values up to $req$. Without considering hash conflict, we know the leader and $f+ \lceil f/2 \rceil$ followers have the same log, up to $req$, and they can all survive the crash. 

Besides, the leader executes the entries based on the order of their time ($entry.t$). Therefore, for any successful requests (entries), their execution order will remain the same after crash and recovery (If $req_1$ is executed ahead of $req_2$ before crash, then after recovery, $req_1$ is still executed ahead of $req_2$).  

Then we only need to exclude one risky case: is it possible for another \textbf{uncommitted} request $req'$, which is executed ahead of $req$ in the old leader, but lost after the recovery? 

\textbf{Corollary:} \texttt{If there exists an uncommitted request $req'$, $req'$ is appended to replica's $logSet$ before $req$, then $req'$ can only exist in at most $\lceil f/2 \rceil$ replicas.} 

We can prove this by contradiction. 

Suppose $req'$ exists in more than $\lceil f/2 \rceil$ replicas but it is not committed (less than $1+f+\lceil f/2 \rceil$ replicas contain $req'$). Since $req'$'s position appears before $req$, i.e. The computation of the hash value for $req$ is based on all the previous requests, including $req'$. Therefore, the hash values replied by the replicas with $req'$ differs from the hash value replied by replicas without $req$. Since there are more than $\lceil f/2 \rceil$  but less than $1+f+\lceil f/2 \rceil$ replicas containing $req'$, Among the $1+f+\lceil f/2 \rceil$ replies for $req$, some replicas will contain $req'$ whereas others not. Therefore, they cannot reply with the same hash value, and $req$ cannot be successful. Contradiction!

Therefore, it is impossible for such requests $req'$ to exist in more than $\lceil f/2 \rceil$ replicas. Therefore, such requests $req'$ cannot appear in the recovered $logSet$ (refer to line 15 in Algorithm~\ref{algo:recovery}). Therefore, there exists, and only exists successful requests in the recovered $logSet$, so consistency is guaranteed. 

\subsection{Proof of Linearizability}
The leader executes the requests (entries) stictly based on the order of the time value $entry.t$ (as well as $entry.clientID$ if $entry.t$ encounters a tie). 

Besides, Nezha will not reveal leader's execution result to clients until the client gets 1 leader reply and $f+\lceil f/2 \rceil$ replies, and with the same hash. In other words, when the client notices the execution result of the request, then this request is already successful. 

For any two entries on the leader replica, $entry_1$ and $entry_2$, if the execution result of $entry_1$ is observed before $entry_2$ (i.e. $entry_1$ is executed before $entry_2$), then the position of $entry_1$ is ahead of $entry_2$ (i.e. either $entry_1.t<entry_2.t$ or $entry_1.t=entry_2.t \ \&\&\  entry_1.clientID < entry_2.clientID$). Meanwhile, if the execution results of the $entries$ can be both observed by some client, then that means the 2 entries both have been successful. Based on the durability and consistency property, after the replica fails and recovers, $entry_1$ and $entry_2$ can survive and the execution results remain consistent. In the recovered system, the two entries will still be executed based on $<entry.t, entry.clientID>$. Therefore, the $entry_1$'s execution will still be observed ahead of $entry_2$.

\section{Why $1+f+\lceil f/2 \rceil$ replies?}
\label{sec:superquorum}
Why is a superquorum of responses needed rather than a simple majority as in Paxos? The reasoning is the same as in Fast Paxos: A simple majority ($f+1$) in Fast Paxos can only guarantee the durability of committed requests, but cannot eliminate the ambiguity between committed and uncommitted requests (i.e. During recovery, one cannot tell which survived requests are committed before crash).  

Consider there are 2 clients $C1$ and $C2$. All replicas have consistent (and clean) system state initially. $C1$ submits its request $<C1, 1>$ to all replicas, and it is only received by $f$ follower replicas. $C2$ submits $<C2,1>$ to all replicas, and it is only received by the other $f$ follower replicas, and the leader replica. 

If the quorum size is $f+1$ instead of $1+f+\lceil f/2 \rceil$, then $<C2,1>$ should be considered as committed as the first log entry in the state machine. 

Then the leader crashes. Among the remaining $2f$ replicas, half of them have $<C1, 1>$ as their first log entry, and the other half has $<C2, 1>$ as their log entry. Without extra knowledge, one cannot decide which request should become the first log entry in the recovered state machine.


\section{Incremental Hash Calculation}
\label{sec:inhash}

Without considering security attack, the easiest incremental hash for the $logSet$ can be implemented with XOR. Other set-collision resistant hash designs (e.g. ~\cite{set-hash}) are also available and can be adopted by Nezha if security attack (e.g. birthday attack) needs to be considered.

For any log entry, we have $<t, clientID, reqNo>$, which can identify the log entry among all the logs from replicas. $<clientID, reqNo>$ can already uniquely identify a log entry on one replica, but it is still possible that different replicas may have log entries with the same $<clientID, reqNo>$, but with different $t$ (refer to the last paragraph in \S~
\ref{sec:conflict}). Therefore, to uniquely represent one log entry among all log entries from all replicas, we use the 3-tuple $<t, clientID, reqNo>$.

In our implementation, $t$ is a 64-bit integer, $clientID$ and $reqNo$ are both 32-bit integers. Concatenating them together, we get a 128-bit string to uniquely identify one log entry. 

We calculate the hash by simply XORing all the log entries. Then we can get a 128-bit string. Considering two $logSet$, denoted as $S_1$ and $S_2$. The probability that $S_1 \neq S_2$ but $\texttt{Hash}(S_1=\texttt{Hash}(S_2)$ is $\frac{1}{2^{127}}$, which is negligible.

The good thing for the incremental hash is that, it is incremental and can be easily paralleled. Coming back to \S~\ref{sec:parallel}, during the sync process,suppose the synced range is from $entry_{start}$ to $entry_{end}$. Then we only need to \textbf{iteratively} update the hash values for the entries between $[entry_{start}, entry_{end}]$. For the entries beyond $entry_{end}$, the hash value can be updated in parallel: We first XOR all the entries in $redundantEntries$ and $missingEntries$, denoted the result as $\Delta h$. For any entries after $entry_{end}$, we use their previous hash value to XOR $\Delta h$ and then get the new hash value for the entry. The reason for that is because XOR is invertible by itself. Therefore, adding a new entry into $logSet$ or deleting an existing entry from $logSet$ lead to the same operation, i.e. XOR the 128-bit string of the entry. 






\iffalse
The idea of incremental hash is proposed in~\cite{increment-hash1}. The definition of incrementality is defined as:

Given a map $f$ and inputs $x$ and $x'$ where $x'$ is a small modification of $x$. Then $f$ is said to be incremental if one can update $f(x)$ in time proportional to the amount of modification between $x$ and $x'$ rather than having to recompute $f(x')$ from scratch. 


Since there are many types of incremental hash function, we adopt the typical one, MSet-XOR-Hash~\cite{set-hash}, and has been proved to be set-collision resistant~\footnote{set-collision resistant means it is computationally infeasible to find a set $S$ and a multiset $M$ such that the cardinalities of $S$ and $M$ are of polynomial size in $m$, $S \neq M$, but $\mathcal{H}(S)=\mathcal{H}(M)$. Note that we do not assume hash attack existing in our system, so the set-collision resistance is a good thing, but it is not necessary.}.

In our scenario, the MSet-XOR-Hash is executed as follows.

For any log entry, we have $<t, clientID, reqNo>$, which can identify the log entry among all the logs from replicas. $<clientID, reqNo>$ can already uniquely identify a log entry on one replica, but it is still possible that different replicas may have log entries with the same $<clientID, reqNo>$, but with different $t$ (refer to the last paragraph in \S~
\ref{sec:conflict}). Therefore, to uniquely represent one log entry among all log entries from all replicas, we use the 3-tuple $<t, clientID, reqNo>$.

In our implementation, $t$ is a 64-bit integer, $clientID$ and $reqNo$ are both 32-bit integers. Concatenating them together, we get a 128-bit string to uniquely identify one log entry. Then the $logSet$ is converted to an \textbf{unordered} set $M$ (the order information has been encoded in the log entries, and we do not worry about order in the set). Then the MSet-XOR-Hash is calculated as follows.

\begin{equation*}
    \mathcal{H}_K(M)=[ H_K(0,r) \oplus  \underset{b\in M}{\bigoplus} H_K(1,b); |M|\ mod\ 2^m ; r ]|_{r\xleftarrow{} M}
\end{equation*}
$m$ is the bit-length of the element in $M$. In our case $m=128$. $r$ is randomly choose from $M$. $H_K$ is a hash function randomly chose from a pseudorandom family of hash functions~\cite{pfh}. 

$\mathcal{H}_K(M)$ is composed of 3 parts, i.e. $\mathcal{H}_K(M)$=
The length of the output hash will be around $3m=384$ bits. 

It is obvious that $\mathcal{H}_K(M)$ is commutative. 
if $x\not \in M$, and I want to add it to $M$, based on the description of the paper, the new hash will become
\begin{equation*}
    \mathcal{H}_K(M \cup \{x\} )=[ H_K(0,r') \oplus  (\underset{b\in M}{\bigoplus} H_K(1,b) \oplus H_k(1,x)) ); (|M|+1)\ mod\  2^m ; r' ]|_{r'\xleftarrow{} B}
\end{equation*}
Such a new hash can be incrementally calculated from $\mathcal{H}_K(M)$.


Then we use the ideal hash function, SHA-1, to hash the 192-bit string to a hash value (which is 160 bits). For all the log entries (blocks), denoted as $x_1, x_2, \cdots, x_n$, the final hash value is calculated as 
\begin{equation*}
    AdHash_{M}^{k}(x_1, x_2, \cdots, x_n)= \sum_{i=1}^{n} h(<i>.x_i) \mod M
\end{equation*}
where $h$ is SHA-1 function, $<i>.x_i$ is the 192-bit string, $M$ is a random $k$-bit integer.

Based on the modular operation, we know the final hashed value is $M-1$ at most. To reduce collision probability, we prefer to make $M$ larger, say $M=2^{256}-1$, so the hashed value will be 256-bit length, and the collision probability is $2^{-256}$, which is negligible. 

Coming back to the scenario of Nezha. For any log entry $x_n$, the incremental hash function should represent the log sequence from the beginnign of $logSet$ to $x_n$, denoted as $logSeq=[x_1, x_2, \cdots, x_n]$. We calculate the hash value with AdHASH. 

Now suppose after the sync process, some entries are modified



\begin{equation*}
    \mathcal{H}_K(M)=[ H_K(0,r) \oplus  \underset{b\in M}{\bigoplus} H_K(1,b); |M|\mod2^m ; r ]|_{r\xleftarrow{} B}
\end{equation*}

\clearpage


Now I am considering deleting elements from $M$. If $x \in M$, I am wondering whether the following hash is fine:
\begin{equation*}
    \mathcal{H}_K(M - \{x\} )=[ H_K(0,r') \oplus  (\underset{b\in M}{\bigoplus} H_K(1,b) \oplus H_k(1,x)) ); (|M|-1)\ mod\  2^m ; r' ]|_{r'\xleftarrow{} B}
\end{equation*}
XOR is invertible, so I think addition and deletion should be the same operation for the first part. For the second part, when adding an element, the cardinality should +1. When deleting an element, the cardinality should -1. Therefore, I think MSet-XOR-Hash also supports deleting elements and remain set-collision resistance. Is that right?

\fi
%This section is under construction...
\newpage




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Replicated Submission}
\label{sec:replicated-submission}
When the client submits its request, it broadcasts the request to every replica. The format of a complete request can be described as a 5-tuple.
\begin{equation*}
    req = <clientID, reqID, command, s, d>
\end{equation*}

$clientID$ and $reqID$ represent the identifiers of the client and its request, and they combine to uniquely identify one request. $command$ represents the content of the request. 

Besides the three fields, the request also includes the submission timestamp $s$, and a latency bound $d$. $<s, d>$ is used by the replicas to decide whether they should accept the request. When receiving the request, the replica calculates the ordering rank as $rank = s + d$. 

If the request is accepted by the replica, it will be converted into a log entry, with $rank = s+d$ as the ordering rank, and eventually added to the log set of the replica.

\subsubsection{Selective Acceptance}
In order to eliminate ordering ambiguity among the received requests, the replicas add the requests to its log set strictly following their order ranks, which is jointly decided by $<ta, clientID, reqID>$.~\footnote{The ordering of requests is mainly decided by comparing $ta$. Rarely, when two requests have the same $ta$, the tie is broken by their $clientID$s. When they both have the same $ta$ and $clientID$, the tie is broken by $reqID$.} To realize that, the replica keeps a hold-and-release (HR) buffer, which holds the requests when they arrive early, and releases them based on their $ta$. 

When the request $req$ arrives at the replica, the replica first compares its local clock time $t_l$ with $t_a$. The replica rejects the request if it finds $t_a < t_l$, and sends a rejection reply immediately to the client. 


The replica chooses to accept $req$ if $t_a \geq t_l$. Then $req$ will be held by the HR buffer until $t_a$. Then $req$ is released and appended as a log entry to the replica's log set (denoted as $logSet$). If the replica is the leader, it also executes the request. Meanwhile, the replica sends an acceptance reply to the client. Inside the acceptance reply, each replica includes a hash value, which encodes current log set of the replica with an incremental hash  function~\cite{increment-hash}, i.e. 
\begin{equation}
\texttt{Hash}(logSet) = 
\bigoplus_{log_i \in logSet} h(log_i)
\end{equation}
where $h(*)$ is a standard hash function (e.g. SHA1) and  $\oplus$ is the XOR operation. Since the hash value is calculated based on all the requests (log entries), it represents the current state of the replica. 

The incremental hash enjoys two advantages: 


First, it provides an easy way to check set equality, which is sufficient to ensure the replica consistency in \sysname because the ordering rank has already been included in every request.

Second, the hash value is computed in an incremental way. Adding or deleting requests only requires incremental computation of XOR and $h(*)$. Such a property is useful while \sysname resolves the inconsistency (described in \S~\ref{sec:sync-process}) and causes trivial overheads.

\subsubsection{Index Synchronization}


\subsubsection{Quorum Check}
The client considers the request as committed when it receives the acceptance replies from the fast quorum. The fast quorum is composed of 1 leader reply and $f+\lceil f/2 \rceil$ follower replies, which have the same hash value. Besides, from the leader's acceptance reply, the client obtains the execution result of the request. 

By contrast, it becomes impossible for the client to form a fast quorum under one of the three situations.
\begin{enumerate}
    \item The client receives the leader's rejection reply;
    \item The client receives the leader's acceptance reply, as well as $>\lfloor f/2 \rfloor$ follower replies, which are either rejection, or acceptance with a different hash value; 
    \item The client does not receive the leader's reply. Denote the number of received replies as $r$. Among the $r$ replies, denote the number of the most frequent hash value as $m$, then $m+(2f+1 -r)<f+\lceil f/2 \rceil+1$~\footnote{In other words, even all the other replies are received later with the same hash value as the most frequent one, it is still insufficient to form a fast quorum.}
\end{enumerate}

Under such situations, the client considers the request as conflicted and stops waiting for other replies. Instead, the client issues a sync request to the client and tries to commit its previous request through the slow path (described in \S~\ref{slow-path}).

\subsubsection{Timeout}
There are situations when the client cannot decide whether the request is committed or conflicted. Such situations trigger the timeout of the client, and client will retry the replicated submission of the same request, but with a different $s$. The resubmitted request is treated as a fresh request and replicas reply with a new hash value if they accept the requests. However, the leader maintains at-most-once semantics during the execution. When noticing it has previously executed the request with the same $<clientID, reqID>$, the leader reply the previous execution result instead of executing it for a second time.

Since \sysname allows at most $f$ replica to crash at the same time, at the worst case, there is less than a fast quorum of healthy replicas, which makes it impossible to commit requests through the fast path, and leads to infinite retry. 

To ensure progress under the worst case, \sysname maintains a bound for the retry times. After retrying the replicated submission for a certain times, the client will abandon the fast path and try to commit its previous request through the slow path (described in \S~\ref{slow-path}).

\subsection{Slow Path}
\label{slow-path}
\subsubsection{Issue Sync Request}
When the client notices the request is conflicted, or has retried for bounded times but fails to commit the request, the client chooses to commit the request through the slow path. To do that, the client issues a sync request to the leader, which includes the body of the previous uncommitted request (i.e. $clientID$, $reqID$, and $command$ ), without time information (i.e. $s$ and $d$). The format of the sync request can be described as 
\begin{equation*}
    sync = <\texttt{SYNC}, clientID, reqID,command>
\end{equation*}

Once the leader receives the sync request, it first checks the existence of its logs with $<clientID, reqID>$. If the request does not exist on the leader's log, then the leader chooses the current clock time as the $ta$ for this request, and appends the request as a new log entry to its $logSet$, then the leader starts the sync process among replicas. Otherwise, the request already exists on the leader but has not been synced, then the leader directly starts the sync process without appending. 

\subsubsection{Sync Process}
\label{sec:sync-process}
The leader conducts the sync process with the followers periodically, or after receiving the sync request from clients. The workflow of the sync process is similar to Multi-Paxos/Raft: The leader contacts a slow quorum of replicas ($f+1$ replicas including the leader itself), to ensure the consistency among them. 

Since the ordering rank has already been included in each log entry, the two replicas are considered as consistent if and only if the set equality is achieved regarding their logs. 

During the sync process, the leader chooses the latest log entry (i.e. with the largest $ta$) in its $logSet$ as the sync point (denoted as $syncPoint$). It uses its own $logSet$ as the reference to modify the $logSet$s of followers, adding/deleting log entries to/from them. Along with the log addition/deletion, the incremental hash value is also updated to keep representing the current state of the follower replica. Since XOR is self-associative, the incremental hash can be incrementally modified by simply XOR the hash ($h(*)$) of the added/deleted logs, which only costs subtle overheads~\footnote{According to our measurement, while using the standard openssl library to compute SHA1 hash for the request with 16-byte input (i.e. the size of $<ta, clientID, reqID>$), the time cost is about  0.15$\mu s$. Besides, the XOR computation with two 20-byte value (the size of the SHA1 hash value) only costs 0.0087$\mu s$  }. 

After the leader receives the replies from $f$ followers, confirming that they have become consistent with the leader up to $syncPoint$. The leader ensures its log entries up to $syncPoint$ will survive the crash. If there are pending sync requests from the clients and the $<clientID, reqID>$ indicates a log entry within the synced scope, then the leader replies to the client with a \texttt{SYNCED} confirmation. After receiving that, the client considers its request as committed through the slow path.


==> old/a-refinement.tex <==
\section{Course Deployments and Refinements}
\label{sec:refinement}

To understand the challenges of operating \sysname, we deployed it in two courses using students as participants. We discuss learnings from these deployments and how we refined \sysname based on them.

\Para{Deployment Setup.} For our first deployment, we held a 3-hour trading competition between 13 trading groups of high school students as part of a summer course. Over this competition, students placed roughly 1000 orders and 1000 trades across 10 symbols. For each symbol we initiated trading bots to place trades to induce specific price-time patterns on which students could engineer algorithms. For our second, larger, deployment, we deployed \sysname in a financial technologies and algorithms course attended by undergraduate, masters, and PhD students. Over 8 trading days, 32 groups of students placed 4.2 million orders and 330 thousand trades on \sysname.

\Para{Learnings from Deployments.} Our first deployment led to changes in our APIs to make \sysname more user-friendly. It also led us to the observation that we could support more symbols in \sysname by sharding the matching engine over symbols. In our second deployment, we observed that with a fixed delay parameter, the unfairness ratios varied daily due to changing network conditions. This led us to develop a control scheme to tune delay parameters automatically based on sensed network conditions. We also observed that straggler and faulty gateways can inflate latency, leading us to a scheme to replicate orders through multiple gateways for lower latency. 

% Outline
% Shtem deployment and experience -> api and scale of deployment. Scale and numbers.
% Orders -
% Undergraduate course -> tradeoff between fairness and throughput in the exchange. Some figures/statistics from the deployment
% From these deployments, we developed techniques in CloudEx that offer better throughput and fairness guarantees which we explored in Section \ref{sec:optimizations} and evaluated in Section 
% \ref{sec:evaluation}.
% \todo{summarize}
%We deployed \sysname in two courses to better understand its shortcomings and to create approaches to address them.

%respectively. 
% In the appendix, we report fairness, throughput and delay metrics from the latter half of the deployment with Figures \ref{cs349f-tps}-\ref{cs349f-outbound-fairness}.

\Para{Sharding.} We shard the matching engine based on symbols, with each shard dequeuing orders from its own order priority queue and managing the limit order books of a subset of symbols. Based on its symbol, an order is routed to the corresponding shard.

\Para{Dynamic Delay Parameters (DDP).} Empirically, in our deployments, we observed that there is no simple relationship between the unfairness ratios and the delay parameters (Figs.~\ref{fig-perf-noart} and \ref{fig-perf-art} further illustrate this). Hence, we cannot easily derive and directly control the unfairness ratio by setting the delay parameter to a static value. Further, time-varying latencies in the cloud necessitate that these parameters should be updated {\em continuously} to achieve a target unfairness ratio. To directly control the unfairness ratio, \sysname continuously and independently tunes each delay parameter. For each parameter, DDP uses a sliding window of order/market data samples to calculate the unfairness ratios in real time. If the current unfairness ratio is above the target unfairness ratio, DDP increases the delay parameter by a small fixed amount (\SI{5}{\micro\second}), else DDP decreases it by the same amount.
% and adjust the delay parameters accordingly.
% Hence, a static configuration of delay parameters yields unpredictable unfairness ratios
%While running \sysname, we noticed that it is difficult but essential to properly configure the delay parameters. 

%\ag{competition deployment is not mentioned until later, remove this next sentence?} This effect can be seen in Figure \ref{cs349f-owd} where the latency between gateways and the matching engine of CloudEx vary each day of the trading competition we hosted. 

% Even if we can figure out the best configuration for today's cluster and network conditions, we cannot guarantee that the configuration is still proper for tomorrow.


%~\footnote{Better tuning algorithms may be possible, and we leave these for future work}. 
% achieve finer-grained control and 

%Periodically, \sysname monitors the inbound/outbound unfairness ratios and compares them with the predefined target, thus increasing/decreasing the sequencing/releasing delay parameters accordingly.

% We optimize $d_f$ and $d_s$ with Algorithm \ref{delayparamalgo}. 


% Algorithms
% \begin{algorithm}
% \SetAlgoLined
% \SetKwInOut{r}{}
%  \textbf{Input}: \\ $r$ - target unfairness percent \\ $u_0$ - initial delay parameter \\ $W$ - window size \\ $S(e)$ - step size given an error \\ $f(W, u)$ - fairness given window and delay parameter \\
%  \hrulefill \\
%  $u \xleftarrow{} u_0$ \\
%  \While{true}{
%   $e \xleftarrow{} f(W, u) - r$ \;
%   $u \xleftarrow{} u + S(e)$ \;
%  }
%  \caption{Dynamic Delay Tuning}
%  \label{delayparamalgo}
% \end{algorithm}

\Para{Replicated Order Submission (ROS).}
VMs are not homogeneous and stragglers are common in the cloud~\cite{hotos-straggler}. When market participants submit orders to a slow gateway, they suffer from a long delay before receiving an order confirmation. Even worse, if a gateway crashes, the corresponding participants will not be able to submit any orders until that gateway restarts. To address such stragglers and achieve fault tolerance, we use message replication by letting market participants submit replicas of the same order through \textit{multiple} gateways instead of one gateway. The matching engine processes the earliest-arriving replica and drops the others.
% Similarly, at the outbound, the confirmation will be sent to multiple gateways and forwarded to the trader. For every order submission, the trader will only take the earliest confirmation and ignore the others. 


==> old/abstract.tex <==
%Resume here.
% \todo{.}
% \todo{adapt to cloudex only.}
% Public cloud infrastructure offers scaling and security benefits attractive to financial exchanges. As the number of investors is experiencing a booming increase, there is an emerging demand for democratizing access. However, their uneven and varying network delays can cause information in an exchange to be processed or disseminated unfairly. 

% In several modern application areas such as autonomous vehicles, electronic trading systems and massive multi-player games, the state of the system is sensed at some nodes in a network and is used to take real-time control action at other nodes. In order to cater to these applications, the network is required to provide time-sensitive functionalities such as: jitter-free or deterministic message delivery, synchronized multicast, and event scheduling based on global timestamps.  This paper provides an approach for designing networks which can support such {\em time-sensitive applications}.  Two key primitives of the approach are: (i) a highly accurate and scalable (in the number of nodes and the distance between them) clock synchronization method, and (ii) {\em time perimeters}: a subset of nodes, including the sensor and control nodes, whose clocks are tightly synchronized.  We present a detailed case study of using time perimeters to build  \sysname, a stock exchange in the cloud. \sysname contrasts with current stock exchanges which use highly bespoke networks to provide fairness guarantees to market participants. We also discuss how time perimeters provide simpler and more scalable solutions to several classical distributed systems problems.

Financial exchanges have begun a move from custom-engineered and on-premise datacenters to the public cloud, accelerated by a rush of new investors, the rise of remote work, cost savings from the cloud, and the desire for more resilient infrastructure. While the promise of the cloud is enticing, the cloud's varying network latencies can lead to market unfairness: orders can be processed out of sequence, and market data can be disseminated to market participants at incorrect times due to varying latencies between participants and the exchange. We present CloudEx, a fair-access cloud exchange, which leverages high-precision software clock synchronization to compensate for noisy network conditions in the public cloud. We also discuss refinements to the CloudEx design that were informed by lessons learned from deploying CloudEx in two academic courses and conclude by outlining future research directions.
% We detail and evaluate two techniques developed to achieve this compensation -- dynamic delay threshold (DDT) and replicated order submission (ROS).

==> old/background-old.tex <==
\section{Background and Related Works}
\label{sec:background}
\subsection{Typical Consensus Protocols}
% In this section, we begin by reviewing the typical consensus protocols and illuminate the intuition behind \sysname by comparison. We do not intend to enumerate every consensus protocol given the explosive emergence in the past decades. Specifically, we will briefly compare the design of four main protocols closely related to \sysname, namely, Multi-Paxos~\cite{paxos}/Raft~\cite{atc14-raft}, Fast Paxos~\cite{fastpaxos}, Speculative Paxos~\cite{nsdi15-specpaxos}, NOPaxos~\cite{osdi16-nopaxos}. Then, based on the comparison, we will explain the design rationale of \sysname. The basic properties of these protocols can be summarized as Table~\ref{tab:cmp}.

In this section, we begin by reviewing the typical consensus protocols. We do not intend to enumerate every consensus protocol given the explosive emergence in the past decades. Specifically, we will briefly compare the design of four main protocols closely related to \sysname, namely, Multi-Paxos~\cite{paxos}/Raft~\cite{atc14-raft}, Fast Paxos~\cite{fastpaxos}, Speculative Paxos~\cite{nsdi15-specpaxos}, NOPaxos~\cite{osdi16-nopaxos}. The basic properties of these protocols and \sysname can be summarized as Table~\ref{tab:cmp}.


\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
\begin{table*}[t]
\begin{threeparttable}
  \centering
\caption{Basic Properties of Typical Consensus Protocols}
    % \centering
\begin{tabular}{x{1.6cm}x{2.5cm}x{2.5cm}cx{2cm}c}
\hline 
\ & {\small \makecell{Latency~\tnote{1}\\( Message Delays)}} & {\small \makecell{Bottleneck Load on \\ Leader~\tnote{2}\ (Messages)}} & {\small Quorum Size} & {\small \makecell{Inconsistency\\Penalty}} & {\small \makecell{Deployment\\Requirement}} \\
\hline
{\small\makecell{Multi-Paxos\\/Raft}} & 4 & $2(2f+1)$ & $f+1$ & Low & No special requirement \\
\hline 
{\small NOPaxos}  & \makecell{2 or 3~\tnote{3}~(fast path) \\  4 or 5 (slow path)}  & 2 & \makecell{$f+1$ for both\\ fast and slow paths} & Low & \makecell{SDN control,\\  priority scheduling, \\ programmable switch~\tnote{4}, etc. }\\
\hline 
{\small Fast Paxos} & \makecell{3 (fast path)\\ 5 (slow path) }  & $2f+2$ & \makecell{$f+\lceil\frac{f}{3}\rceil+1$ (fast path) \\ $f+1$ (slow path) } & Medium & No special requirement \\
\hline 
{\small \makecell{Speculative\\Paxos}}
 & \makecell{2 (fast path) \\ 6 (slow path)} & 2 & \makecell{$f+\lceil\frac{f}{2}\rceil+1$ (fast path) \\ $f+1$ (slow path)} & High & \makecell{SDN control,\\priority scheduling, etc.} \\ 
\hline 
{\small Nezha}  & \makecell{2 (fast path) \\ 3 (slow path)} & 2+($2f+1$) & \makecell{$f+\lceil\frac{f}{2}\rceil+1$ (fast path) \\ $f+1$ (slow path)} & Low & Clock synchronization\\
\hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item[1] Latency indicate how many message delays required for a client to know the committed result its request. Here we refer to the latency in the fast path for the protocols except Multi-Paxos/Raft.
      \item[2] Load on Leader indicate how many messages the leader processes per client request. 
      \item[3] When using hardware sequencer, the message flow client$\xrightarrow{}$sequencer$\xrightarrow{}$replica is considered as one message delay, so the overall latency is 2 message delays. However, with a software sequencer, both client$\xrightarrow{}$sequencer and sequencer$\xrightarrow{}$replica are considered as one message delay, so the overall latency is 3 message delays.
      \item[4] Programmable switch is required only when NOPaxos uses hardware sequencer, and it is unnecessary when NOPaxos uses software sequencer.
    \end{tablenotes}
\label{tab:cmp}
\end{threeparttable}
\end{table*}



Generally speaking, in order to commit a request, the workflow of the consensus protocol can be decomposed into at least three main tasks.
\begin{enumerate}
    \item Ordering. The consensus protocol needs to serialize all the requests and decide a definitive execution order~\footnote{Here we do not consider the optimization of commutativity. Some protocols, including EPaxos~\cite{sosp13-epaxos,nsdi21-epaxos} and CURP~\cite{nsdi19-curp} takes advantage of commutativity, and only requires eventual consistency instead of execution order consistency. }. Specifically, conservative protocols such as Multi-Paxos/Raft and NOPaxos uses \emph{definitive ordering}, which means the order is decided globally and maintains correct so long as the system does not crash. By contrast, other more aggressive protocols, such as Fast Paxos and Speculative Paxos use \emph{approximate ordering}, which means the ordering is temporarily decided by each replica, which is believed to be probably correct, but may also be reverted later (because it is inconsistent with the majority). 
    
    \item Replication. The consensus protocol needs to replicate the request to all replicas, so that each replica can apply the request to its state machine. 
    \item Quorum check. The consensus protocol needs to ensure that a quorum of replicas have consistent states after applying the request to their state machine, so that the state machine can be recovered after crash.
    % \item Execution. For most requests~\footnote{We use the term \emph{most}, because there are exceptional cases, such as blind write requests, that do not need the execution results after their commits.}, the consensus protocol needs to execute them before replying to the client, so that the client can know the execution result of its request from the reply and decide their following actions.
\end{enumerate}


Among the four main tasks, ordering is the key task deciding the consistency, but \emph{definitive ordering} needs to be globally consistent and requires a centralized serialization point. However, a centralized serialization point can easily become the throughput bottleneck and also extend the overall latency. By comparison, \emph{approximate ordering} is cheaper and can be conducted by each replica without coordinating with the others, but the ordering may cause inconsistency and requires further confirmation in quorum check. Once the inconsistency really happens, it costs extra penalty in the slow path to resolve it. The key difference of these protocols lies in the choice between \emph{definitive ordering} and \emph{approximate ordering}, as well as the corresponding schedule of the four tasks, as described in \S~\ref{sec-paxos-background}$\sim$\S~\ref{sec-speculative-paxos-background}.

In the following subsections, we aim to compare the protocols in a unified way, so we illustrate each protocol with 5 replicas, denoted as R1$\sim$R5, and 2 clients, denoted as C1 and C2. Except Multi-Paxos/Raft, the other protocols have both fast path and slow path. We distinguish the quorum of the two paths as fast quorum and slow quorum. Besides, for simplicity, we ommit messages less relevant to the workflow and keeps the minimal set of messages (e.g. to satisfy the quorum) in the figure. 

\subsection{Multi-Paxos/Raft}
\label{sec-paxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/Paxos-Normal.pdf}
    \caption{Multi-Paxos/Raft workflow}
    \label{Paxos-Normal}
\end{figure}
In Multi-Paxos/Raft, the workflow (shown in Figure~\ref{Paxos-Normal}) can be summarized as\\
\centerline{definitive ordering$\xrightarrow{}$replication$\xrightarrow{}$quorum check$\xrightarrow{}$execution}
The message flow follows\\ 
\centerline{client $\xrightarrow{}$ leader $\xrightarrow{}$ follower $\xrightarrow{}$ leader $\xrightarrow{}$ client}

The leader takes all the responsibility and makes itself a potential performance bottleneck, and it also costs more message delays (4 message delays) for the client knows the committed result. However, because of the centralized control from the leader, Multi-Paxos/Raft suffers from much less inconsistency penalty compared with the other protocols described below. Each replica follows the \emph{definitive ordering} to append and execute the requests. There is no concept of fast path and slow path in the design of Multi-Paxos/Raft.  
%So long as the leader is alive, the ordering decided by the leader is always correct and cannot be reverted. 


\subsection{NOPaxos}
\label{sec-nopaxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/NoPaxos-Fast.pdf}
    \caption{NOPaxos workflow (fast path)}
    \label{NOPaxos-Fast}
\end{figure}
In NOPaxos, the workflow of the fast path (shown in Figure~\ref{NOPaxos-Fast}) can be summarized as\\
\centerline{definitive ordering$\xrightarrow{}$replication$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
The message flow follows \\
\centerline{client $\xrightarrow{}$ sequencer  $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client}
Unlike Multi-Paxos/Raft, NOPaxos offloads the ordering responsibility to an independent sequencer, which is implemented by either hardware (e.g. programmable switch) or software (e.g. a standalone server). Besides, it also offloads the responsibility of replication and quorum check to the clients. To keep correctness, NOPaxos enforces the constraints during quorum check: the client considers the request as committed after it receives the reply from a fast/slow quorum (3 replicas), and the quorum must include the leader. 

The design of NOPaxos much relieves the leader bottleneck, but brings more risk of inconsistency. Though each replica also uses the \emph{definitive ordering} like Multi-Paxos/Raft, the request reordering/drop from sequencer to the replicas can make replica states become inconsistent. Fortunately, the sequencer tags each request with a sequential number, which enables the replica to detect the inconsistency early when they receive requests with nonconsecutive sequential numbers. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/NoPaxos-Slow.pdf}
    \caption{NOPaxos workflow (slow path)}
    \label{NOPaxos-Slow}
\end{figure}
In Figure~\ref{NOPaxos-Slow}, we show a case when the leader (R3) experiences the reordering of C1's request and C2's request. To ensure consistency, the leader needs to take an extra round-trip time (2 message delays) to resolve the inconsistency (which is called gap agreement in NOPaxos design~\cite{osdi16-nopaxos}). The gap agreement routine erases C1's request from the follower replicas and ensure that at least a slow quorum (3 replicas including leader) have consistent states. After resolving the inconsistency, the leader can move on to execute the request and reply to the client. In the case of Figure~\ref{NOPaxos-Slow}, C2's request is eventually committed, whereas C1's request is uncommitted, because it misses the reply from the leader.

\subsection{Fast Paxos}
\label{sec-fast-paxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/FastPaxos-Fast.pdf}
    \caption{Fast Paxos workflow (fast path)}
    \label{Fast-Paxos-Fast}
\end{figure}
In Fast Paxos, the workflow of the fast path (shown in Figure~\ref{Fast-Paxos-Fast}) can be summarized as\\
\centerline{replication$\xrightarrow{}$approx ordering$\xrightarrow{}$quorum check$\xrightarrow{}$execution}
The message flow follows \\
\centerline{client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ leader $\xrightarrow{}$ client}


Similar to NOPaxos, Fast Paxos also relies on clients to do the replication (i.e. the client broadcasts its request to every replica), but each replica uses \emph{approximate ordering} decided by itself to to append the request to its log list (according to the receiving order of requests). However, the \emph{approximate ordering} decided by each replica may be inconsistent, so they need to contact the leader to confirm the ordering consistency. Normally, each replica maintains the consistent ordering of the requests. After the leader ensures the consistency of a fast quorum (4 replicas including the leader itself), it executes the request and replies the result to the client. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/FastPaxos-Slow.pdf}
    \caption{Fast Paxos workflow (slow path)}
    \label{Fast-Paxos-Slow}
\end{figure}
The design of Fast Paxos is more aggressive than NOPaxos, since it does replication even before ordering. On the other hand, the inconsistency can only be detected later after the followers have appended the request and contacted the leader. In Figure~\ref{Fast-Paxos-Slow}, we show a case when 2 replicas (R4 and R5) have inconsistent states from the others, due to the reordering of C1's and C2's requests. After appending the requests, followers contact the leader (R3) for consistency confirmation, then R3 detects the inconsistency. Similar to NOPaxos, the leader needs to take an extra RTT to resolve the inconsistency and ensure consistency among at least a slow quorum (3 replicas including itself), before executing the request and replying to the client. 

\subsection{Speculative Paxos}
\label{sec-speculative-paxos-background}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/SpecPaxos-Fast.pdf}
    \caption{Speculative Paxos workflow (fast path)}
    \label{SpecPaxos-Fast}
\end{figure}
In Speculative Paxos, the  workflow of the fast path (shown in Figure~\ref{SpecPaxos-Fast}) can be summarized as\\
\centerline{replication$\xrightarrow{}$approx ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
The message flow follows \\
\centerline{client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client}
Speculative Paxos also relies on clients to do the replication. Similar to Fast Paxos, each replica in Speculative Paxos also uses \emph{approximate ordering} decided by each replica. But unlike Fast Paxos, Speculative Paxos takes more aggressive (and risky) action and makes each replica immediately execute the request and reply to the client. In the reply, the replica includes the execution result of the request, as well as a hash value indicating the system state of the replica. In the fast path, the client considers the request as committed after receiving a fast quorum (4 replicas) of replies with the same hash value.

The design of Speculative Paxos can achieve the optimal latency in the fast path, but it suffers from very costly penalty in the slow path. Unlike Fast Paxos, the fast path of NOPaxos runs in a leaderless way essentially: all the replicas have executed request even if the execution order proves to be inconsistent later. When inconsistency occurs, it takes much longer time for the leader to detect that, either by the notification from the client (as shown in Figure~\ref{SpecPaxos-Slow}), or by the leader's periodical synchronization. Even after the inconsistency has already been detected, it still costs much to resolve the inconsistency. 
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{figures/SpecPaxos-Slow.pdf}
    \caption{Speculative Paxos workflow (slow path)}
    \label{SpecPaxos-Slow}
\end{figure}
In Figure~\ref{SpecPaxos-Slow}, we showcase how Speculative Paxos resolves the inconsistency. R4 and R5 have inconsistent states from the other replicas because they have executed C2's request before executing C1's request. Such inconsistency is first noticed by C1 while doing the quorum check and finding it impossible to form a fast quorum (4 replicas) of replies with the same hash, so C1 sends broadcast a reconciliation request to every replica, notifying them of the inconsistency. After receiving the reconciliation request, the leader coordinates a slow quorum of replicas (3 replicas including itself) to decide a definitive execution order of the requests. Then the leader broadcasts the new order to all replicas. The problematic replicas, either executing requests in an inconsistent order (e.g. R4 and R5), or missing the execution of some requests (e.g. R1, R2 and R3), need to rollback and/or re-execute the requests in the correct order. The rollback mechanism requires the support from application, which can be very costly and even impossible in practical cases~\footnote{The rollback requires the application have checkpointing mechanism to record the system state periodically~\cite{vldb14-fast-recovery}. Since checkpointing can be costly, it is not conducted for every execution of requests. Suppose the application has executed 1 million requests and it records checkpoints for every 1000 requests. When the Speculative Consensus Protocol encounters conflict, it needs to rollback 1000 requests and re-execute them in the definitive and consistent order. Even worse, if the application is not equipped with checkpoint mechanism, the rollback essentially means re-executing all the requests from scratch, which is unbearable in practice.}.

% \subsection{Summary of Comparison and Motivation of \sysname}


% Reviewing these typical consensus protocols, we can notice they are aggressive to different degrees. According to their aggressive degrees, The four typical consensus protocols can be sorted as\\ 
% \centerline{\small Multi-Paxos/Raft < NOPaxos < Fast Paxos < Speculative Paxos}


% % Among the four main tasks, ordering is the key task deciding the consistency, but \emph{definitive ordering} needs to be globally consistent and requires a centralized serialization point (e.g. the leader in Multi-Paxos/Raft and the sequencer in NOPaxos). However, a centralized serialization point can easily become the throughput bottleneck and also extend the overall latency.~\footnote{Though the number of message delay is considered as unchanged for NOPaxos with a hardware sequencer. The length for the single message delay is also increased since all requests must be routed to the root switch and detour through a sequencer~\cite{nsdi19-curp}.} 

% Multi-Paxos/Raft is the most conservative protocol, which uses \emph{definitive ordering} throughout the whole process, and each replica appends/executes requests following the definitive order. However, such a conservative design makes it suffer from the longest latency and the most serious throughput bottleneck. By contrast, NOPaxos takes a more aggressive approach than Multi-Paxos/Raft. It decouples the ordering from the leader, and is willing to pay the potential cost when replicas miss some requests from sequencer before appending the following requests. The more aggressive protocol, Fast Paxos, postpones the ordering task later after replication, and is willing to pay the cost after replicas have appended requests in the wrong order due to \emph{approximate ordering}. The most aggressive protocol, Speculative Paxos, postpones the ordering task even later after replication and execution, and is willing pay the cost after replicas have appended and executed in the wrong order due to \emph{approximate ordering}


% Overall, the more aggressive approach tends to bring more performance benefit with regard to latency and throughput, when request reordering/drop does not occur. In turn, it also incurs higher performance penalty while resolving the inconsistency due to request reordering/drop. Besides, some promising protocols, such as NOPaxos and Speculative Paxos, imposes very stringent requirements to achieve optimal latency/throughput, which makes it hard to deploy in common scenarios, such as public cloud. 

% The comparison of these existing protocols motivates our design of \sysname. The design rationale of \sysname is to \emph{be aggressive in the fast path but pay trivial penalty cost in the slow path}. \sysname achieves this by further decomposing the ordering agreement...

% \sysname learns from the design principles of the three previous protocols, but sidesteps their drawbacks/overheads. 
% \begin{enumerate}
%     \item Similar to NOPaxos, \sysname also decouples the ordering responsibility from the leader. However, \sysname uses synchronized clocks to implement cheaper \emph{approximate ordering}. Instead of going through the centralized sequencer, \sysname pre-assigns the ordering rank for each request at the client side, without adding throughput bottleneck or extra message delay. 
    
%     \item 
%     Similar to Speculative Paxos, \sysname also follows the workflow of replication$\xrightarrow{}$approx ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check. However, \sysname only allows the leader to execute the request in the fast path, and the followers only maintains the requests for durability. Since there is only single execution order, the order is correct by definition and no rollback is needed even when inconsistency occurs.
    
%     \item Similar to Fast Paxos and Speculative Paxos, the leader is responsible to resolve inconsistency when fast quorum cannot be formed. However, \sysname's consistency only cares about \emph{set equality} of requests on different replicas, because the ordering rank has been tagged in each request, and the ordering will be consistent so long as replicas have an equal set of requests.
    
%     % \sysname checks the consistency with relaxed standards. For Fast Paxos, the consistency between two replicas indicate they have the same requests and the requests are appended in the same order. For \sysname, the ordering of requests is decided by clock time, which is tagged into each request during submission. Therefore, \sysname only needs to check \emph{set equality} of replicas' requests, without considering their appending order. 
% \end{enumerate}

% To realize the target, \sysname adopts a similar workflow as Speculative Paxos, i.e 
% \centerline{replication$\xrightarrow{}$ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
% However, unlike Speculative Paxos, which essentially works in a leaderless way in the fast path, \sysname uses a strong form of leadership for both the fast path and the slow path. The leader is the only executor of requests, so its executor ordering is correct by definition.  


% it is also the centralized bottleneck constraining the throughput and the overall latency. Multi-Paxos/Raft lets the leader decides the ordering, so the leader will never experience ordering inconsistency. On the other hand, it also suffers from the worst throughput and latency overheads. NOPaxos, Fast Paxos and Speculative Paxos try to ??

% the aggressive protocol tries to postpone the ordering task in order to yield better latency and throughput


%Generally speaking, the consensus protocol needs to guarantee both consistent ordering and durability. 

% Multi-Paxos and Raft are both single-leader protocol and share very similar workflow, shown in Figure~\ref{Paxos-Normal}. For simplicity, the less relevant part of the workflow (e.g. the follower replicas also learn from the leader and execute the request) are omitted in the figure, and we also makes similar simplification for Figure~\ref{NOPaxos-Fast}$\sim$Figure~\ref{SpecPaxos-Slow}.
% The message flow is 

% client $\xrightarrow{}$ leader $\xrightarrow{}$ follower $\xrightarrow{}$ leader $\xrightarrow{}$ client\\
% and so it requires 4 message delays for the client to know its request has been committed. 

% Multi-Paxos/Raft is the most conservative protocol among the four in comparison. Leader takes two-fold responsibility of ordering and durability. The leader needs to decide the ordering after receiving the client's requests. Before replying to the client, the leader also needs to ensure the request has been replicated to a quorum (3 replicas including the leader itself) of replicas.

% In Multi-Paxos/Raft, the order of requests has been early decided by the leader. So long as the leader is alive, the inconsistency (due to request reordering/drop) never leads to divergent states among replicas, so Multi-Paxos/Raft does not have the concept of fast path and slow path. 



% NOPaxos is also a single-leader protocol, which is more aggressive than Multi-Paxos/Raft. NOPaxos offloads the ordering responsibility to the sequencer, either implemented by hardware (e.g. programmable switch) or software (e.g. an independent server). Besides, it relies on the clients to check the (fast) quorum and ensure the durability. Normally, there is no request reordering/drop, and the clients' requests go through the fast path, shown in Figure~\ref{NOPaxos-Fast}, i.e.  



% All clients' requests will first go to the sequencer for globally ordering, and then be multicast to every replica. The client consider the request as committed if it receives the reply from a fast quorum (1 leader replica and 2 follower replicas).

% Although the fast path saves 1 or 2 message delays~\footnote{With a software sequencer, the fast path of NOPaxos requires 3 message delays for client to know the request is committed. With a programmable switch as the hardware sequencer, the message flow client $\xrightarrow{}$ sequencer  $\xrightarrow{}$ leader/follower is considered as one message delay, so the fast path requires 2 message delays for client to know the request is committed.} compared with Multi-Paxos/Raft, the inconsistency can occur while the request message goes from the sequencer to the leader/followers. In that case, NOPaxos has to commit the request via the slow path shown in Figure~\ref{NOPaxos-Slow}.



% In Figure~\ref{NOPaxos-Slow}, C1's request (green dash line) and C2's request (blue dash line) become reordered while transmitting to the leader, which causes inconsistent state between the leader and other followers. Fortunately, each request is tagged with a consecutive sequential number by the sequencer, so the leader can detect the inconsecutiveness of the sequential number once it receives C2's request. Before replying to C2, the leader first resolves the inconsistency by contacting followers to erase C1's request. After receiving feedback from the majority (3 replicas including the leader itself), the leader executes the request and reply the committed result to the client (C2).  




% Fast Paxos is more aggressive than NOPaxos and it does not involve a sequencer to order the requests, instead, the clients directly broadcast their requests to every replica, and then follower replicas contact the leader to confirm their consistency. Normally, the clients' requests go through the fast path shown in Figure~\ref{Fast-Paxos-Fast}, i.e.

% client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ leader $\xrightarrow{}$ client\\
% If there is no request reordering/drop from the client to leader/followers, every replica should have consistent state. Then after leader ensures a fast quorum of replicas (4 replicas including the leader itself) have consistent states, it executes the request and replies the committed result to the client.

% The fast path of Fast Paxos requires 3 message delays for the client to know its request has been committed. However, when request reordering/drop occurs, replicas may have inconsistent states and cannot form a fast quorum, the request will go through the slow path as shown in Figure~\ref{Fast-Paxos-Slow}. In this case, it replies on the leader to resolve the inconsistency. 




% In Figure~\ref{Fast-Paxos-Slow}, R4 and R5 have inconsistent states from the other 3 replicas, because they have received and appended C2's request before C1's request. Therefore, a fast quorum (4) cannot be formed and the leader needs to decide a definitive order of requests and broadcast to all the replicas, after it receives the reply from a slow quorum (3 replicas including itself), it can safely exeucte the request and reply to the client. 



% Speculative Paxos the most aggressive protocols among the four. Although Speculative Paxos also maintains a single leader, the leader does not play a special role in its fast path. Essentially, Speculative Paxos works in a \emph{leaderless} way in the fast path, and every replica executes the incoming requests. Normally, the clients' requests go through the fast path shown in Figure~\ref{SpecPaxos-Fast}, i.e.

% client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client\\
% The client broadcasts the request to all replicas, and each replica immediately executes the request and reply the result to the client, together with a hash value representing the system state of the replica. Then client needs to check the quorum, as well as the system state of the replicas. If the client notices the request has been executed by a fast quorum (4 replicas), and each replica in the quorum has consistent state, then it considers the request as committed. Such a design can achieve the optimal latency and throughput in the fast path, but leads to very costly reconciliation in the slow path, as shown in Figure~\ref{SpecPaxos-Slow}. 



% In Figure~\ref{SpecPaxos-Slow}, R4 and R5 have inconsistent states from the other 3 replicas, because they have appended and executed C2's request before C1's request. Therefore, C1 cannot form a fast quorum (4) with consistent states. In this case, C1 broadcast a reconciliation request to all replicas to resolve the inconsistency. After receiving the reconciliation request, the leader needs to coordinate the followers and decide a definitive order of the requests. Since replicas have executed the request following their receiving order, they need to rollback the execution and execute requests following the new order designated by the leader. Such rollback mechanism requires the support from application, which can be very costly and even impossible in practical cases~\footnote{The rollback requires the application have checkpointing mechanism to record the system state periodically~\cite{vldb14-fast-recovery}. Since checkpoint mechanism can be costly, it is not conducted for every execution of requests. Suppose the application has executed 1 million requests and it records checkpoints for every 1000 requests. When the Speculative Consensus Protocol encounters conflict, it needs to rollback 1000 requests and re-execute them in the definitive and consistent order. Even worse, if the application is not equipped with checkpoint mechanism, the rollback essentially means re-executing all the requests from scratch, which is unbearable in practice.}.

==> old/background_snippets.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t]
% \begin{threeparttable}
%   \centering
% \caption{Basic Properties of Typical Consensus Protocols}
%     % \centering
% \begin{tabular}{x{1.6cm}x{2.5cm}x{2.5cm}cx{2cm}c}
% \hline 
% \ & {\small \makecell{Latency~\tnote{1}\\( Message Delays)}} & {\small \makecell{Bottleneck Load on \\ Leader~\tnote{2}\ (Messages)}} & {\small Quorum Size} & {\small \makecell{Inconsistency\\Penalty}} & {\small \makecell{Deployment\\Requirement}} \\
% \hline
% {\small\makecell{Multi-Paxos\\/Raft}} & 4 & $2(2f+1)$ & $f+1$ & Low & No special requirement \\
% \hline 
% {\small NOPaxos}  & \makecell{2 or 3~\tnote{3}~(fast path) \\  4 or 5 (slow path)}  & 2 & \makecell{$f+1$ for both\\ fast and slow paths} & Low & \makecell{SDN control,\\  priority scheduling, \\ programmable switch~\tnote{4}, etc. }\\
% \hline 
% {\small Fast Paxos} & \makecell{3 (fast path)\\ 5 (slow path) }  & $2f+2$ & \makecell{$f+\lceil\frac{f}{2}\rceil+1$ (fast path)~\tnote{5} \\ $f+1$ (slow path) } & Medium & No special requirement \\
% \hline 
% {\small \makecell{Speculative\\Paxos}}
%  & \makecell{2 (fast path) \\ 6 (slow path)} & 2 & \makecell{$f+\lceil\frac{f}{2}\rceil+1$ (fast path) \\ $f+1$ (slow path)} & High & \makecell{SDN control,\\priority scheduling, etc.} \\ 
% \hline 
% {\small Nezha}  & \makecell{2 (fast path) \\ 3 (slow path)} & $2f+2$~\tnote{6} & \makecell{$f+\lceil\frac{f}{2}\rceil+1$ (fast path) \\ $f+1$ (slow path)} & Low & Clock synchronization\\
% \hline
% \end{tabular}
%     \begin{tablenotes}
%       \small
%       \item[1] Latency indicate how many message delays required for a client to know the committed result its request. Here we refer to the latency in the fast path for the protocols except Multi-Paxos/Raft.
%       \item[2] Load on Leader indicate how many messages the leader processes per client request. 
%       \item[3] When using hardware sequencer, the message flow client$\xrightarrow{}$sequencer$\xrightarrow{}$replica is considered as one message delay, so the overall latency is 2 message delays. However, with a software sequencer, both client$\xrightarrow{}$sequencer and sequencer$\xrightarrow{}$replica are considered as one message delay, so the overall latency is 3 message delays.
%       \item[4] Programmable switch is required only when NOPaxos uses hardware sequencer, and it is unnecessary when NOPaxos uses software sequencer.
%       \item[5] The quorum of Fast Paxos in the fast path is usually defined as $2f$ out of $3f+1$ replicas~\cite{fastpaxos}. However, when it works with $2f+1$ replicas, the quorum becomes the same as Speculative Paxos and \sysname. 
%       \item[6] 2 of the messages are the request and the reply message respectively, whereas the other $2f$ messages are index messages, which are much smaller in size (details in \S~\ref{index-sync}).
%     \end{tablenotes}
% \label{tab:cmp}
% \end{threeparttable}
% \end{table*}



% \begin{table*}[t]
% \begin{threeparttable}
%   \centering
% \caption{Basic Properties of Typical Consensus Protocols}
%     % \centering
% \begin{tabular}{|x{2.3cm}|x{2.3cm}|x{3cm}|x{2.3cm}|x{2.5cm}|x{2.3cm}|}
% \hline 

% \  & {\small \makecell{Multi-Paxos/Raft}} & {\small \makecell{NOPaxos}} & {\small Fast Paxos} & {\small \makecell{Speculative Paxos}} & {\small \makecell{\sysname}} 
% \\ \hline
% % Row-1
% {\small \makecell{Message Delays}} & {\small \makecell{4}} &
% {\small \makecell{F~\tnote{\color{green} 1} : 2 or 3~\tnote{\color{green} 2}\quad\   S: 4 or 5}} &
% {\small \makecell{F: 3\quad S: 5}} &
% {\small \makecell{F: 2 \quad S: 6}} &
% {\small \makecell{F: 2 \quad S: 3}} 
% \\ \hline

% % Row-2
% {\small \makecell{Load on Leader~\tnote{\color{green} 3}}} & {\small \makecell{ $2(2f+1)$ }} &
% {\small \makecell{ 2 }} &
% {\small \makecell{ $2f+2$  }} &
% {\small \makecell{ 2 }} &
% {\small \makecell{ $2f+2$~\tnote{\color{green} 4} }} 
% \\ \hline

% % Row-3
% {\small \makecell{Quorum Size}} &
% {\small \makecell{ $f+1$ }} &
% {\small \makecell{ F: $f+1$ \\ S: $f+1$ }} &
% {\small \makecell{ F: $f+\lceil f/2 \rceil+1$~\tnote{\color{green} 5} \\ S: $f+1$  }} &
% {\small \makecell{ F: $f+\lceil f/2 \rceil+1$ \\ S: $f+1$  }} &
% {\small \makecell{ F: $f+\lceil f/2 \rceil+1$ \\ S: $f+1$  }} 
% \\ \hline

% % Row-4
% {\small \makecell{Quorum Check \\Point }} &
% {\small \makecell{ Leader }} &
% {\small \makecell{ F: Client \\ S: Leader }} &
% {\small \makecell{ F: Leader \\ S: Leader }} &
% {\small \makecell{ F: Client \\ S: Leader }} &
% {\small \makecell{ F: Client \\ S: Client }} 
% \\ \hline


% % Row-5
% {\small \makecell{Inconsistency \\ Penality }} &
% {\small \makecell{ Low }} &
% {\small \makecell{ Medium }} &
% {\small \makecell{ Medium }} &
% {\small \makecell{ High }} &
% {\small \makecell{ Low }} 
% \\ \hline

% % Row-5
% {\small \makecell{Deployment \\ Requirement }} &
% {\small \makecell{No special \\ requirement }} &
% {\small \makecell{ Priority scheduling, \\ programmable switch\tnote{\color{green}6},\\ SDN control, etc.}} &
% {\small \makecell{ No special \\ requirement }} &
% {\small \makecell{ Priority scheduling, \\ SDN control,etc. }} &
% {\small \makecell{ Clock\\ synchronization }} 
% \\ \hline

% \end{tabular}
%     \begin{tablenotes}
%       \small
%     %   \item[1] Latency indicate how many message delays required for a client to know the committed result of its request. 
%       \item[1] F--- fast path; S--- slow path.
%       \item[2] When NOPaxos is equipped with the hardware sequencer, the message flow client$\xrightarrow{}$sequencer$\xrightarrow{}$replica is considered as one message delay, so the overall latency is 2 message delays. However, with a software sequencer, both client$\xrightarrow{}$sequencer and sequencer$\xrightarrow{}$replica are considered as one message delay, so the overall latency is 3 message delays. The same is true for the slow path.
%       \item[3] Load on Leader indicates how many messages the leader processes per client request. 
%       \item[4] 2 of the messages are the request and the reply. The other $2f$ messages are \emph{sync} messages with much smaller size (details in \S~\ref{index-sync}).
%       \item[5] The quorum of Fast Paxos in the fast path is usually defined as $2f$ out of $3f+1$ replicas~\cite{fastpaxos}. However, when it works with $2f+1$ replicas with the tolerance of $f$ replica failures, the quorum becomes the same as Speculative Paxos and \sysname. 
%       \item[6] Programmable switch serves as the hardware sequencer, and it is unnecessary when NOPaxos uses software sequencer.
%     \end{tablenotes}
% \label{tab:cmp}
% \end{threeparttable}
% \vspace{-0.6cm}
% \end{table*}






% \subsection{Key Insights and Motivation}
% \label{sec-motivation}
% \sysname aims to be both high-performance and easily deployable. To meet both targets in \sysname design, we first take an in-depth analysis of the workflows of typical consensus protocols.  

% Generally speaking, in order to commit a request, the consensus protocol needs to perform three main tasks.
% \begin{itemize}[wide, labelwidth=!,nosep]
%     \item \textbf{Ordering agreement.} The protocol needs to serialize all the requests and decide a definitive execution order. Each replica follows the commonly agreed order to execute the requests so that they can reach the same state. 
%     % To be more specific, ordering agreement imposes two-fold requirements on the protocol: each replica contains the same requests (i.e. set equality) and each replica serialize its requests in the same order (i.e. no order ambiguity).
    
%     \item \textbf{Replication.} The protocol needs to replicate the request to all replicas, so that replicas can either execute it, or simply store the request in logs for failure recovery. 
%     \item \textbf{Quorum check.} The protocol needs to ensure a sufficient number (i.e. a quorum) of replicas have accepted the request before confirming its commit, so that there is enough information for recovery after replicas' crash.
%     % \item Execution. For most requests~\footnote{We use the term \emph{most}, because there are exceptional cases, such as blind write requests, that do not need the execution results after their commits.}, the consensus protocol needs to execute them before replying to the client, so that the client can know the execution result of its request from the reply and decide their following actions.
% \end{itemize}

% Among the three tasks, ordering agreement is essential for consistency and linearizability (defined in~\S~\ref{sec-correctness}). Though expensive, an early ordering agreement can avoid heavy penalty when inconsistency really happens. The typical protocols make different trade-offs between the cost of early ordering agreement and the potential penalty of resolving inconsistency. 

% \begin{itemize}[wide, labelwidth=!,nosep]
% \item \textbf{Early ordering agreement with expensive overheads.} Multi-Paxos/Raft and NOPaxos choose to prioritize ordering agreement over replication and quorum check. They rely on a centralized serialization point (i.e. the leader replica or a standalone sequencer) to decide the order for requests before replicating them to every replica. Such a design adds more latency overheads and the serialization point can also become a throughput bottleneck. 

% \item \textbf{Late ordering agreement with potential heavy penalty.} Fast Paxos and Speculative Paxos defer the ordering agreement after replication and quorum check. The client can directly broadcast the requests to every replica and each replica decides the order of the requests based on their arrival time. Such a design can save latency/throughput overheads if the order of requests is typically the same across a majority of replicas. Otherwise, the inter-replica inconsistency will be detected during the quorum check, and the protocols have to take costly effort (i.e. extra RTT(s) and quorum check) to reach ordering agreement among the replicas. 
% \end{itemize}

%     % The protocols such as Multi-Paxos/Raft and NOPaxos are more conservative, and they decide a definitive ordering for all the requests with a centralized serialization point~\footnote{Multi-Paxos/Raft rely on the leader replica as the serialization point whereas NOPaxos replies on the sequencer as the serialization point.}. By contrast, the other protocols such as Fast Paxos and Speculative Paxos are more aggressive, and each replica uses a temporary ordering decided by itself. The ordering may be reverted later, because it is not agreed by the majority. 
    
% % \begin{enumerate}[wide, labelwidth=!,nosep,label=(\arabic*)]
% % \item Multi-Paxos/Raft and NOPaxos are more conservative. They choose to prioritize ordering agreement over replication, and the workflow can be summarized as 

% % \emph{Ordering Agreement}$\xrightarrow{}$\emph{Replication}$\xrightarrow{}$\emph{Quorum Check}

% % Every request needs to first go through a centralized serialization point to get a definitive ordering rank, which cannot be reverted later (so long as the leader does not change). Multi-Paxos/Raft rely on the leader replica as the serialization point to reach the agreement, which constrains throughput/latency performance. NOPaxos relies on a standalone sequencer as the serialization point, which relieves the throughput bottleneck, but also incurs longer or extra message delay. Besides, such a design can seriously degrade NOPaxos performance in the open-loop test, which will be further explained in \S~\ref{sec-latency-throughput}.
% % % ~\footnote{The software sequencer costs 1 extra message delay for NOPaxos. The hardware sequencer requires every request message detour the root switch, thus prolonging the message delay. Besides, the hardware sequencer also imposes stringent requirements, making it unable to deploy in public cloud.}
% % \item Fast Paxos and Speculative Paxos are more aggressive. They choose to prioritize replication over ordering agreement, and the workflow can be summarized as

% % \emph{Replication}$\xrightarrow{}$\emph{Quorum Check}$\xrightarrow{}$\emph{Ordering Agreement}

% % Instead of going through a centralized serialization point at the beginning, each request is broadcast to all replicas first, and each replica decides the order of the request by itself. Then, Fast Paxos relies on the leader replica for quorum check whereas Speculative Paxos relies on the client for quorum check. During the quorum check phase, if a majority (quorum) of replicas agree with the order of the request, then this request is committed. Otherwise, it has to take extra (and costly) effort to reach ordering agreement among the replicas.  

% % % Each request is broadcast to all 
% % % Therefore, they allow each replica to adopt a temporary ordering decided by itself. The ordering may be reverted later if not agreed by the majority. Such approaches can save some latency and/or throughput overheads in the fast path. But when inconsistency really happens and the temporary order proves to be wrong, it costs significant overheads to resolve the inconsistency. 
% % \end{enumerate}

% From the study of the four typical protocols, we notice that, \emph{neither an early ordering agreement nor a late ordering agreement is desirable}. To avoid such a dilemma of decision-making, we seek the third way in \sysname design, i.e. we decompose the ordering agreement into two finer-grained tasks, prioritizing one task early and deferring the other to a later time. More specifically, the ordering agreement imposes two-fold requirements on the consensus protocol.

% \begin{itemize}[wide, labelwidth=!,nosep]
%     \item \textbf{No ordering ambiguity.} Ordering ambiguity means some replicas order request $a$ ahead of $b$ whereas the other replicas order them in a reverse way. Ordering ambiguity should not exist if the replicas have consistent states.
    
%     \item \textbf{Set equality.} Set equality means the replicas have exactly the same requests (i.e. the sets of requests are equal).
% \end{itemize}

% It is challenging to satisfy both requirements without a centralized serialization point. However, we will show in \sysname that, by using clock synchronization, the ordering ambiguity can be eliminated during the replication process at a low cost, and we can fix the \emph{potential} set inequality later with lightweight leader$\xrightarrow{}$follower communication.




% \begin{enumerate}[wide, labelwidth=!,nosep,label=(\arabic*)]
% \item Neither an early ordering agreement nor a late ordering agreement is desirable. Prioritizing the ordering agreement over replication is expensive (e.g. Multi-Paxos/Raft and NOPaxos), whereas deferring ordering agreement after replication is risky and even more costly once inconsistency really happens (e.g. Fast Paxos and Speculative Paxos). This motivates us to seek the third way in \sysname design, i.e. we decompose the ordering agreement into two finer-grained tasks, prioritizing one task early and deferring the other to a later time. More details are explained in \S~\ref{protocol-overview}$\sim$\S~\ref{sec-slow-quorum-check}.

% \item Quorum check also constrains the performance, especially the throughput. It is a wise choice for Speculative Paxos and NOPaxos to offload quorum check from replicas to clients. However, their offloading only works in the fast path and the slow path suffers from serious performance degradation because they still rely on the leader for quorum check. This motivate us to make a more thorough offloading of quorum check in \sysname design, i.e. we let the clients take the full responsibility of quorum check for both the fast path and slow path. 

% \item Fast Paxos and Speculative Paxos start to fix the inconsistency only after the violation of ordering agreement is detected during the quorum check. The fixing action is not timely and costs the slow path 1 or 2 more RTTs than the fast path. This motivate us to take actions early to fix the \emph{potential} inconsistency in \sysname design, i.e. we let the replicas launch the routine to fix the \emph{potential} inconsistency even before it is detected in quorum check. The fixing routine does not benefit if the inconsistency does not happen among replicas. By contrast, if the inconsistency really happens, the early start of the fixing routine can save latency overheads for the slow path, making it not much worse than the fast path.

% % which constrains the throughput and/or latency performance. Deferring ordering agreement after replication can benefit the performance when inconsistency does not occur, but it costs more overheads to resolve the inconsistency after it is detected during the quorum check phase. 

% \end{enumerate}



% \vspace{-0.4cm}
% \subsection{Decomposing Ordering Agreement}
% \label{sec-decompose}
% \vspace{-0.1cm}
% \sysname also prioritizes replication over ordering agreement. But unlike Fast Paxos/Speculative Paxos, \sysname can avoid the heavy penalty to resolve the (possible) inconsistency. The key idea of \sysname is to decompose the expensive ordering agreement into two finer-grained tasks: 


% \begin{itemize}[wide, labelwidth=!,nosep]
%     \item \textbf{Eliminate ordering ambiguity.} If one replica orders request $a$ ahead of request $b$, no other replicas can order them in a reverse way.   
%     \item \textbf{Maintain set equality.} All the replicas have exactly the same requests (i.e. the sets of requests are equal).
% \end{itemize}

% Without the centralized serialization point, it is quite challenging to achieve ordering agreement. However, we will show in \sysname, by using clock synchronization, it is fairly easy to \emph{eliminate ordering ambiguity early}, and we can defer to \emph{fix the (potential) set equality later} (with low cost) during the sync process among replicas. 

% To be more specific, \sysname synchronizes the clocks between clients and replicas. It allows the clients to decide an ordering rank (i.e. the sum of its submission time and a latency bound) for the request. With reference to the rank and the appended entries in its \emph{log}, the replica decides whether the request can be accepted without ordering ambiguity (\S\ref{selective-acceptance}). Ideally, each replica is expected to accept the same requests, thus they are committed via the fast path with 2 message delays (1 RTT). However, when replicas take different actions (acceptance/rejection) towards some requests, set inequality will occur among replicas and \sysname relies on the lightweight index synchronization process (\S~\ref{index-sync}) to fix set inequality, thus the requests are committed via the slow path with 3 message delays (1.5 RTTs). 

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=8cm]{figures/Nezha-Arch-Fast-Path.pdf}
%     \caption{Workflow of \sysname (fast path) }
%     \label{fig-workflow-fast}
% \end{figure}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=8cm]{figures/Nezha-Arch-Slow-Path.pdf}
%     \caption{Workflow of \sysname (slow path) }
%     \label{fig-workflow-slow}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% but \emph{definitive ordering} needs to be globally consistent and requires a centralized serialization point. However, a centralized serialization point can easily become the throughput bottleneck and also extend the overall latency. By comparison, \emph{approximate ordering} is cheaper and can be conducted by each replica without coordinating with the others, but the ordering may cause inconsistency and requires further confirmation in quorum check. Once the inconsistency really happens, it costs extra penalty in the slow path to resolve it. The key difference of these protocols lies in the choice between \emph{definitive ordering} and \emph{approximate ordering}, as well as the corresponding schedule of the four tasks, as described in \S~\ref{sec-paxos-background}$\sim$\S~\ref{sec-speculative-paxos-background}.


% \subsection{Summary of Comparison and Motivation of \sysname}


% Reviewing these typical consensus protocols, we can notice they are aggressive to different degrees. According to their aggressive degrees, The four typical consensus protocols can be sorted as\\ 
% \centerline{\small Multi-Paxos/Raft < NOPaxos < Fast Paxos < Speculative Paxos}


% % Among the four main tasks, ordering is the key task deciding the consistency, but \emph{definitive ordering} needs to be globally consistent and requires a centralized serialization point (e.g. the leader in Multi-Paxos/Raft and the sequencer in NOPaxos). However, a centralized serialization point can easily become the throughput bottleneck and also extend the overall latency.~\footnote{Though the number of message delay is considered as unchanged for NOPaxos with a hardware sequencer. The length for the single message delay is also increased since all requests must be routed to the root switch and detour through a sequencer~\cite{nsdi19-curp}.} 

% Multi-Paxos/Raft is the most conservative protocol, which uses \emph{definitive ordering} throughout the whole process, and each replica appends/executes requests following the definitive order. However, such a conservative design makes it suffer from the longest latency and the most serious throughput bottleneck. By contrast, NOPaxos takes a more aggressive approach than Multi-Paxos/Raft. It decouples the ordering from the leader, and is willing to pay the potential cost when replicas miss some requests from sequencer before appending the following requests. The more aggressive protocol, Fast Paxos, postpones the ordering task later after replication, and is willing to pay the cost after replicas have appended requests in the wrong order due to \emph{approximate ordering}. The most aggressive protocol, Speculative Paxos, postpones the ordering task even later after replication and execution, and is willing pay the cost after replicas have appended and executed in the wrong order due to \emph{approximate ordering}


% Overall, the more aggressive approach tends to bring more performance benefit with regard to latency and throughput, when request reordering/drop does not occur. In turn, it also incurs higher performance penalty while resolving the inconsistency due to request reordering/drop. Besides, some promising protocols, such as NOPaxos and Speculative Paxos, imposes very stringent requirements to achieve optimal latency/throughput, which makes it hard to deploy in common scenarios, such as public cloud. 

% The comparison of these existing protocols motivates our design of \sysname. The design rationale of \sysname is to \emph{be aggressive in the fast path but pay trivial penalty cost in the slow path}. \sysname achieves this by further decomposing the ordering agreement...

% \sysname learns from the design principles of the three previous protocols, but sidesteps their drawbacks/overheads. 
% \begin{enumerate}
%     \item Similar to NOPaxos, \sysname also decouples the ordering responsibility from the leader. However, \sysname uses synchronized clocks to implement cheaper \emph{approximate ordering}. Instead of going through the centralized sequencer, \sysname pre-assigns the ordering rank for each request at the client side, without adding throughput bottleneck or extra message delay. 
    
%     \item 
%     Similar to Speculative Paxos, \sysname also follows the workflow of replication$\xrightarrow{}$approx ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check. However, \sysname only allows the leader to execute the request in the fast path, and the followers only maintains the requests for durability. Since there is only single execution order, the order is correct by definition and no rollback is needed even when inconsistency occurs.
    
%     \item Similar to Fast Paxos and Speculative Paxos, the leader is responsible to resolve inconsistency when fast quorum cannot be formed. However, \sysname's consistency only cares about \emph{set equality} of requests on different replicas, because the ordering rank has been tagged in each request, and the ordering will be consistent so long as replicas have an equal set of requests.
    
%     % \sysname checks the consistency with relaxed standards. For Fast Paxos, the consistency between two replicas indicate they have the same requests and the requests are appended in the same order. For \sysname, the ordering of requests is decided by clock time, which is tagged into each request during submission. Therefore, \sysname only needs to check \emph{set equality} of replicas' requests, without considering their appending order. 
% \end{enumerate}

% To realize the target, \sysname adopts a similar workflow as Speculative Paxos, i.e 
% \centerline{replication$\xrightarrow{}$ordering$\xrightarrow{}$execution$\xrightarrow{}$quorum check}
% However, unlike Speculative Paxos, which essentially works in a leaderless way in the fast path, \sysname uses a strong form of leadership for both the fast path and the slow path. The leader is the only executor of requests, so its executor ordering is correct by definition.  


% it is also the centralized bottleneck constraining the throughput and the overall latency. Multi-Paxos/Raft lets the leader decides the ordering, so the leader will never experience ordering inconsistency. On the other hand, it also suffers from the worst throughput and latency overheads. NOPaxos, Fast Paxos and Speculative Paxos try to ??

% the aggressive protocol tries to postpone the ordering task in order to yield better latency and throughput


%Generally speaking, the consensus protocol needs to guarantee both consistent ordering and durability. 

% Multi-Paxos and Raft are both single-leader protocol and share very similar workflow, shown in Figure~\ref{Paxos-Normal}. For simplicity, the less relevant part of the workflow (e.g. the follower replicas also learn from the leader and execute the request) are omitted in the figure, and we also makes similar simplification for Figure~\ref{NOPaxos-Fast}$\sim$Figure~\ref{SpecPaxos-Slow}.
% The message flow is 

% client $\xrightarrow{}$ leader $\xrightarrow{}$ follower $\xrightarrow{}$ leader $\xrightarrow{}$ client\\
% and so it requires 4 message delays for the client to know its request has been committed. 

% Multi-Paxos/Raft is the most conservative protocol among the four in comparison. Leader takes two-fold responsibility of ordering and durability. The leader needs to decide the ordering after receiving the client's requests. Before replying to the client, the leader also needs to ensure the request has been replicated to a quorum (3 replicas including the leader itself) of replicas.

% In Multi-Paxos/Raft, the order of requests has been early decided by the leader. So long as the leader is alive, the inconsistency (due to request reordering/drop) never leads to divergent states among replicas, so Multi-Paxos/Raft does not have the concept of fast path and slow path. 



% NOPaxos is also a single-leader protocol, which is more aggressive than Multi-Paxos/Raft. NOPaxos offloads the ordering responsibility to the sequencer, either implemented by hardware (e.g. programmable switch) or software (e.g. an independent server). Besides, it relies on the clients to check the (fast) quorum and ensure the durability. Normally, there is no request reordering/drop, and the clients' requests go through the fast path, shown in Figure~\ref{NOPaxos-Fast}, i.e.  



% All clients' requests will first go to the sequencer for globally ordering, and then be multicast to every replica. The client consider the request as committed if it receives the reply from a fast quorum (1 leader replica and 2 follower replicas).

% Although the fast path saves 1 or 2 message delays~\footnote{With a software sequencer, the fast path of NOPaxos requires 3 message delays for client to know the request is committed. With a programmable switch as the hardware sequencer, the message flow client $\xrightarrow{}$ sequencer  $\xrightarrow{}$ leader/follower is considered as one message delay, so the fast path requires 2 message delays for client to know the request is committed.} compared with Multi-Paxos/Raft, the inconsistency can occur while the request message goes from the sequencer to the leader/followers. In that case, NOPaxos has to commit the request via the slow path shown in Figure~\ref{NOPaxos-Slow}.



% In Figure~\ref{NOPaxos-Slow}, C1's request (green dash line) and C2's request (blue dash line) become reordered while transmitting to the leader, which causes inconsistent state between the leader and other followers. Fortunately, each request is tagged with a consecutive sequential number by the sequencer, so the leader can detect the inconsecutiveness of the sequential number once it receives C2's request. Before replying to C2, the leader first resolves the inconsistency by contacting followers to erase C1's request. After receiving feedback from the majority (3 replicas including the leader itself), the leader executes the request and reply the committed result to the client (C2).  




% Fast Paxos is more aggressive than NOPaxos and it does not involve a sequencer to order the requests, instead, the clients directly broadcast their requests to every replica, and then follower replicas contact the leader to confirm their consistency. Normally, the clients' requests go through the fast path shown in Figure~\ref{Fast-Paxos-Fast}, i.e.

% client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ leader $\xrightarrow{}$ client\\
% If there is no request reordering/drop from the client to leader/followers, every replica should have consistent state. Then after leader ensures a fast quorum of replicas (4 replicas including the leader itself) have consistent states, it executes the request and replies the committed result to the client.

% The fast path of Fast Paxos requires 3 message delays for the client to know its request has been committed. However, when request reordering/drop occurs, replicas may have inconsistent states and cannot form a fast quorum, the request will go through the slow path as shown in Figure~\ref{Fast-Paxos-Slow}. In this case, it replies on the leader to resolve the inconsistency. 




% In Figure~\ref{Fast-Paxos-Slow}, R4 and R5 have inconsistent states from the other 3 replicas, because they have received and appended C2's request before C1's request. Therefore, a fast quorum (4) cannot be formed and the leader needs to decide a definitive order of requests and broadcast to all the replicas, after it receives the reply from a slow quorum (3 replicas including itself), it can safely exeucte the request and reply to the client. 



% Speculative Paxos the most aggressive protocols among the four. Although Speculative Paxos also maintains a single leader, the leader does not play a special role in its fast path. Essentially, Speculative Paxos works in a \emph{leaderless} way in the fast path, and every replica executes the incoming requests. Normally, the clients' requests go through the fast path shown in Figure~\ref{SpecPaxos-Fast}, i.e.

% client $\xrightarrow{}$ leader/follower $\xrightarrow{}$ client\\
% The client broadcasts the request to all replicas, and each replica immediately executes the request and reply the result to the client, together with a hash value representing the system state of the replica. Then client needs to check the quorum, as well as the system state of the replicas. If the client notices the request has been executed by a fast quorum (4 replicas), and each replica in the quorum has consistent state, then it considers the request as committed. Such a design can achieve the optimal latency and throughput in the fast path, but leads to very costly reconciliation in the slow path, as shown in Figure~\ref{SpecPaxos-Slow}. 



% In Figure~\ref{SpecPaxos-Slow}, R4 and R5 have inconsistent states from the other 3 replicas, because they have appended and executed C2's request before C1's request. Therefore, C1 cannot form a fast quorum (4) with consistent states. In this case, C1 broadcast a reconciliation request to all replicas to resolve the inconsistency. After receiving the reconciliation request, the leader needs to coordinate the followers and decide a definitive order of the requests. Since replicas have executed the request following their receiving order, they need to rollback the execution and execute requests following the new order designated by the leader. Such rollback mechanism requires the support from application, which can be very costly and even impossible in practical cases~\footnote{The rollback requires the application have checkpointing mechanism to record the system state periodically~\cite{vldb14-fast-recovery}. Since checkpoint mechanism can be costly, it is not conducted for every execution of requests. Suppose the application has executed 1 million requests and it records checkpoints for every 1000 requests. When the Speculative Consensus Protocol encounters conflict, it needs to rollback 1000 requests and re-execute them in the definitive and consistent order. Even worse, if the application is not equipped with checkpoint mechanism, the rollback essentially means re-executing all the requests from scratch, which is unbearable in practice.}.

% \todo{Categorize: Generally Deployable but low performance; high performance but need specific assistance}
% In this section, we begin by reviewing the typical consensus protocols and illuminate the intuition behind \sysname by comparison. We do not intend to enumerate every consensus protocol given the explosive emergence in the past decades. Specifically, we will briefly compare the design of four main protocols closely related to \sysname, namely, Multi-Paxos~\cite{paxos}/Raft~\cite{atc14-raft}, Fast Paxos~\cite{fastpaxos}, Speculative Paxos~\cite{nsdi15-specpaxos}, NOPaxos~\cite{osdi16-nopaxos}. Then, based on the comparison, we will explain the design rationale of \sysname. The basic properties of these protocols can be summarized as Table~\ref{tab:cmp}.
% We do not intend to enumerate every consensus protocol given the explosive emergence in the past decades.

==> old/design-bk.tex <==
\section{Design}
\label{sec:design}


\subsection{Time-based Virtual Sequencer}
{\color{red}Refer to Section 4.2 in NOPaxos paper for comparison }

\blue{Unlike NOPaxos, Nezha does not involve a real sequencer entity in the system. Instead, it uses clock time to implement similar sequencer function in \emph{a distributed way}}.

The sequencer plays a simple but critical role: assigning \rst{a sequence number} a \blue{time-based} consistent order to each message destined for a particular OUM group, and writing \rst{that sequence number} \blue{the time information} into the packet header. This establishes a total order over packets and is the key element that elevates our design from a best-effort ordering property to an ordering guarantee. Even if packets are dropped (e.g., due to congestion or link failures) or reordered (e.g., due to multipath effects) in the network, receivers can use \rst{the sequence numbers} \blue{the attached time information} to ensure that they process packets in order and deliver drop notifications for missing packets.

\rst{Sequencers maintain one counter per OUM group. For every packet destined for that group, they increment the counter and write it into a designated field in the packet header. The counter must be incremented by 1 on each packet (as opposed to a timestamp, which monotonically increases but may have gaps)}. \blue{The virtual sequencer always maintains the synchronized clock time from Huygens, and it partitions the continuous time period into discrete blocks according to a consistent length. Each client is only allowed to submit one request in each time block. The request submitted will be tagged with the start time and end time of the time block.} \rst{This counter lets libOUM return DROP-NOTIFICATIONs when it notices gaps in the sequence numbers of incoming messages.} \blue{The end time indicates the expected deadline for this request to arrive at the replicas.} \rst{Sequencers also maintain and write into each packet the OUM session number that is used to handle sequencer failures; we describe its use in \S4.3.} \blue{Unlike NOPaxos, Nezha does not need to handle sequencer failure since the sequencer is not a real entity. Besides, Nezha's correctness is not related to clock synchronization either. During its runtime, Nezha only requires the clock synchronization to increase monotonically (Huygens will periodically correct the clocks by adding a positive/negative offset). Such a requirement is easy to satisfy. Nezha keeps recording the value of last call to get clock timestamp. During every function call to get clock timestamp, Nezha will compare it with the timestamp recorded in the last function call. If the current value is smaller than previous one, the function call will not return the value to the application. Instead, it  will abandon the value and repeatedly fetch the clock timestamp, until the returned value satisfies the  monotonicity across consecutive function calls.As what will be shown in \S\ref{sec:fault}, even when Huygens fails in some rare cases, Nezha only suffers from liveness issue and the correctness is still guaranteed. } 


Our sequencer design is general; \rst{we discuss three possible implementations here.} \rst{The most efficient one targets upcoming programmable network switches, using the switch itself as the sequencer, incurring no latency cost (\S4.2.1)} \blue{The virtual sequencer relies on clock timestamps, which can be acquired by each node locally, without requesting from a centralized controller, incurring no latency cost}. \src{As this hardware is not yet available, NOPaxos adopts a prototype that uses a network processor to implement a middlebox-like sequencer (\S4.2.2).} Comparing with the hardware-based sequencer in NOPaxos, Nezha can be directly deployed in public cloud. \rst{Finally, we discuss using an end-host as a sequencer (\S4.2.3).} Comparing with the end-host sequencer in NOPaxos, Nezha's virtual sequencer does not suffer from centralized bottlenneck. 

\subsection{Sequencer Scalability}
Since all OUM packets for a particular group go through the sequencer, a valid concern is whether the sequencer will become the performance bottleneck. \rst{Switches and network processors are designed to process packets at line rate and thus will not become the bottleneck for a single OUM group (group receivers are already limited by the link bandwidth)}. \blue{Programmable switches and network processors have not been available in public cloud.} \rst{Previous work [28] has demonstrated that an end-host sequencer using RDMA can process close to 100 million requests per second, many more than any single OUM group can process.} \blue{RDMA relies on special RNIC, which has not been used in public cloud due to security and isolation issues}  \rst{We note that different OUM groups need not share a sequencer, and therefore deployment of multiple OUM groups can scale horizontally.} \blue{However, different OUM groups can only guarantee the linearizability inside its own group. Therefore, the horizontal scale of multiple OUM groups does not make sense.}


\subsection{Fault Tolerance}
\label{sec:fault}
Designating a sequencer and placing it on the common path for all messages to a particular group introduces an obvious challenge: \rst{what if it fails or becomes unreachable?} \blue{what if the clock synchronization fails?} \rst{If link failures or failures of other switches render the sequencer unreachable, local rerouting mechanisms may be able to identify an alternate path [43]. However, if the sequencer itself fails, or local rerouting is not possible, replacing the sequencer becomes necessary.}

In our design, \st{the network controller monitors the sequencer’s availability. If it fails or no longer has a path to all OUM group members, the controller selects a different switch.} \blue{each node (i.e. replica or client) monitors return values of its function call to get clock timestamp. It guarantees that only monotonic clock timestamps are visible to the system.} \rst{It reconfigures the network to use this new sequencer by updating routes in other switches. During the reconfiguration period, multicast messages may not be delivered.}\blue{When clocks are not synchronized, replicas' clocks may go ahead of clients' clock, which can cause the replicas to refuse the incoming requests tagged with a smaller timestamp (or more accurately, a smaller TOUM-ID, as defined later). On the other hand, clients' clock may go ahead of replicas' clock, which can cause the replicas to hold the requests for unnecessarily longer time before replying to clients. Such clock deviation degrades liveness of Nezha, but still guarantees correctness.} \rst{However, failures of root switches happen infrequently [21], and rerouting can be completed within a few milliseconds [43], } \blue{However, Huygens failures happen infrequently thanks to its probing mesh. Its fault tolerance is based on etcd, and the recovery can be completed within XX[ask Yilong for a number],}so this should not significantly affect system availability \blue{and liveness}.

We must also ensure that the ordering guarantee of \rst{multicast} messages is robust to \rst{sequencer failures}\blue{clock-sync failures}. This requires the \rst{continuous}, ordered assignment of \rst{sequence numbers}\blue{TOUM-IDs} even when the \rst{network controller fails over to a new sequencer}\blue{clocks fail to be synchronized}.


To address this, we introduce \rst{a unique, monotonically increasing session number, incremented each time sequencer failover occurs}\blue{a unique, comparable indetifier for each request, denoted as TOUM-ID. TOUM-ID can be represented by a tuple <\emph{block-start-time}, \emph{block-end-time}, \emph{client-id}>. The comparison is executed first on \emph{block-end-time}, and the one with smaller \emph{block-end-time} goes ahead (i.e. it will be first processed by the replica). For two request with equal \emph{block-end-time}, the one with smaller \emph{block-start-time} goes ahead. Since each client is only allowed to submit one request in each block, the TOUM-IDs maintain increasing monotonicity locally on each client. At the replica side, TOUM-IDs are still compared in the same way. More than that, when two TOUM-IDs have the same \emph{block-start-time} and \emph{block-end-time}, but from two different clients, each replica follows a deterministic and consistent order~\footnote{There can be different options to compare two \emph{client-ids}. For example, we can compare them in an ascending order or descending order. In order to add more randomness and fairness to the processing orders in the same time block (i.e. to avoid one client's request always being processed ahead of the other's request when they are in the same block), we can install a consistent hash function on each replica, which maps \emph{block-start-time} or \emph{block-end-time} to an order sequence of all \emph{client-ids}. While processing the requests in the same block, we follow the order sequence to break the tie and decide their processing order. } of \emph{client-id}s to process them.  
} \rst{When the controller detects a sequencer failure, it updates the forwarding rules and contacts the new sequencer to set its local session number to the appropriate value.}\blue{Replicas only processes the requests with monotonically increasing TOUM-IDs. If a request comes to the replica after the replica has finished processing another request with a larger identifier, then the stale request will just be ignored.} As a result, the total order of messages follows \rst{the lexicographical order} \blue{a consistent order} of the \rst{<\emph{session-number, sequence-number}>} \blue{<\emph{block-start-time, block-end-time, client-id}>}⟩ tuple, and \rst{clients}\blue{replicas} can still discard packets received out of order.


\st{Once libOUM receives a message with a session number higher than the receiver is listening for, it realizes that a new sequencer is active and stops delivering messages from the old session. However, libOUM does not know if it missed any packets from the old sequencer. As a result, it cannot deliver DROP-NOTIFICATIONs during a session change. Instead, it delivers a SESSION-TERMINATED notification, exposing this uncertainty to the application. NOPaxos, for example, resolves this by executing a view change (§5.2.3) so that replicas agree on exactly which requests were received in the old session.}

\rst{The network controller must ensure that session numbers for any given group monotonically increase, even across controller failures.} \blue{Nezha must ensure that the processed TOUM-IDs for any replicas monotonically increase, even across Huygens failures}. \rst{Many design options are available, for example using timestamps as session numbers, or recording session numbers in stable or replicated storage. Our implementation uses a Paxos-replicated controller group, since SDN controller replication is already com- mon in practice [26, 31] }. Our option is just to block the clock function call if the return value will break the monotonicity. \rst{We note that our replication protocol, NOPaxos (\S 5), is completely decoupled from controller replication, and the controller updates only on sequencer failures, not for every NOPaxos request}. We note that our replication protocol, Nezha (\S \ref{sec-protocol}) is completely decoupled from Huygens fault tolerance. Huygens failure only (possibly) leads to slow progress of Nezha for a period, but will not affect the correctness of Nezha.

\section{Protocol Design}
\label{sec-protocol}
\st{NOPaxos, or Network-Ordered Paxos, is a new replication protocol which leverages the Ordered Unreliable Multicast sessions provided by the network layer.}
Nezha is a new replication protocol which leverages the \emph{almost-correct} consistency provided by software-based clock synchronization.

\subsection{Model}
\rst{NOPaxos}\blue{Nezha} replicas communicate over an asynchronous network that provides OUM sessions (via libOUM). \rst{NOPaxos}\blue{Nezha} requires the network to provide ordered but unreliable delivery of \rst{multicast}\blue{unicast} messages \rst{within a session}\blue{across the entire runtime}. In the normal case, these messages are delivered \rst{sequentially}\blue{on time} and are not dropped \blue{ or ignored by replicas}; however, it remains robust to dropped packets (presented as DROP-NOTIFICATION through libOUM). \rst{NOPaxos}\blue{Nezha} is also robust to \rst{SESSION-TERMINATED notifications}\blue{clock deviation} that occur if \rst{the sequencer}\blue{Huygens} fails. These \rst{network anomalies}\blue{clock-sync failures} do not affect \rst{NOPaxos}\blue{Nezha}’s safety guarantees, and we discuss how they affect \rst{NOPaxos}\blue{Nezha}’s performance\blue{liveness} in \S-.


\rst{NOPaxos}\blue{Nezha} assumes a crash failure model. It uses 2$f$ + 1 replicas, where $f$ replicas are allowed to fail. However, in the presence of more than $f$ failures, the system still guarantees safety. Furthermore, \rst{NOPaxos}\blue{Nezha} guarantees safety even in an asynchronous network with no bound on message latency (provided the OUM guarantees continue to hold).

\rst{NOPaxos}\blue{Nezha} provides linearizability of client requests. It provides at-most-once semantics using the standard mechanism of maintaining a table of the most recent request from each client [42].

\subsection{Protocol}
\textbf{Overview.} \rst{NOPaxos}\blue{Nezha} is built on top of the guarantees of the OUM network primitive. During a single \rst{OUM session} time block, REQUESTs broadcast \blue{by multiple unicast sending from clients} to the replicas are totally ordered but can be dropped \blue{or ignored by the replica}. As a result, the replicas have to agree only on which REQUESTs to execute and which to permanently ignore, a simpler task than agreeing on the order of requests. Conceptually, this is equivalent to running multiple rounds of binary consensus. However, NOPaxos must explicitly run this consensus only when DROP-NOTIFICATIONs are \rst{received}\blue{triggered by timeout}. \st{To switch OUM sessions (in the case of sequencer failure), the replicas must agree on the contents of their shared log before they start listening to the new session.}


To these ends, \rst{NOPaxos}\blue{Nezha} uses a view-based approach: each view has a single \rst{OUM session-num}\blue{view-num} and a single replica acting as leader. The leader executes requests and
drives the agreement to skip a dropped request. That is, it decides which of the sequencer’s REQUESTs to ignore and treat as NO-OPs. The view ID is \st{a tuple <leader-num,session-num>} \blue{exactly \emph{leader-num}}. Here, leader-num is incremented each time a new leader is needed; the current leader of any view is leader-num (mod n); \st{and session-num is the latest session ID from libOUM.} View IDs in \rst{NOPaxos}\blue{Nezha} are \rst{partially}\blue{completely} ordered. However,the IDs of all views that successfully
start will be comparable.

In the normal case, the replicas receive a REQUEST
from libOUM. The replicas then reply to the client, the leader replying with the result of the REQUEST, so the client’s REQUEST is processed in only a single round-trip. \rst{NOPaxos}\blue{Nezha} uses a single round-trip in the normal case because, like many speculative protocols, the client checks the durability of requests. However, unlike most speculative protocols, \rst{NOPaxos}\blue{Nezha} clients have a guarantee regarding ordering of operations; they need only check that the operation was received.

When replicas receive a DROP-NOTIFICATION from libOUM\blue{\  triggered by timeout}, they first try to recover the missing REQUEST from each other. Failing that, the leader initiates a round of agreement to commit a NO-OP into the corresponding slot in the log. Finally, \rst{NOPaxos}\blue{Nezha} uses a view change protocol to handle leader failures \st{and OUM session termination} while maintaining consistency.


\textbf{Outline.} \rst{NOPaxos}\blue{Nezha} consists of four subprotocols:

\begin{itemize}
    \item \emph{Normal Operations} (\S5.2.1): \rst{NOPaxos}\blue{Nezha} processes client REQUESTs in a single round-trip in the normal case.
    \item \emph{Gap Agreement} (\S5.2.2):\rst{NOPaxos}\blue{Nezha} ensures correctness in the face of DROP-NOTIFICATIONs by having the replicas reach agreement on which \rst{sequence numbers}\blue{TOUM-IDs} should be permanently dropped.
    \item \emph{View Change} (\S5.2.3):\rst{NOPaxos}\blue{Nezha} ensures correctness in the face of leader failures \rst{or OUM session termination} using a variation of a standard view change protocol.
    
    \item \emph{Synchronization} (\S5.2.4): Periodically, the leader synchronizes the logs of all replicas.
\end{itemize}

\blue{The following is Figure 4 in NOPaxos paper}

\noindent\textbf{Replica:}

\begin{itemize}
    \item \emph{replica-num}---replica number
    \item \emph{status}---one of \texttt{Normal} or \texttt{ViewChange}
    \item \emph{view-id}=⟨\rst{\emph{leader-num}},\emph{session-num}⟩---the view number ,a tuple of the current leader number \rst{and OUM session number}, \rst{partially} ordered, initially ⟨\rst{0,} 0⟩
    \item \rst{\emph{session-msg-num}---the number of messages (REQUESTs or DROP-NOTIFICATIONs) received in this OUM session} \blue{<\emph{client-id}, \emph{msg-num}>--- the number of messages (REQUESTs or DROP-NOTIFICATIONs) processed for this client}
    \item log---client REQUESTs and NO-OPs in \rst{sequential order}\blue{consistent order of TOUM-IDs described in \S\ref{sec:fault} }
    \item sync-point---the latest synchronization point
\end{itemize}


Figure 4 illustrates the state maintained at each \rst{NOPaxos}\blue{Nezha} replica. Replicas tag all messages sent to each other with their current view-id, and while in the Normal Operations, Gap Agreement, and Synchronization subprotocols, replicas ignore all messages from different views. Only in the View Change protocol do replicas with different view-ids communicate.

\subsubsection{Normal Operation}
In the normal case when replicas receive REQUESTs in- stead of DROP-NOTIFICATIONs, client requests are committed and executed in a single phase. Clients broadcast \blue{via multiple unicast operations in public cloud} ⟨REQUEST, op, request-id, \blue{TOUM-ID}⟩ to all replicas through libOUM, where op is the operation they want to execute, and request-id is a unique id \blue{on each client} used to match requests and their responses.


When each replica receives the client’s REQUEST, it \rst{increments session-msg-num}\blue{increments the \emph{msg-num} in <\emph{client-id}, \emph{msg-num}> for the client} and appends op to the log. If the replica is the leader of the current view, it executes the op (or looks up the previous result if it is a duplicate of a completed request). Each replica then replies to the client with ⟨REPLY, view-id, log-slot-num, request-id, result⟩, where log-slot-num is the index of op in the log. If the replica is the leader, it includes the result of the operation; NULL otherwise.

The client waits for REPLYs to the REQUEST with matching view-ids and log-slot-nums from $f$ + 1 replicas, where one of those replicas is the leader of the view. This indicates that the request will remain persistent even across view changes. If the client does not receive the required REPLYs within a timeout, it retries the request.

\subsubsection{Gap Agreement}
\rst{NOPaxos}\blue{Nezha} replicas always process operations in order \blue{TOUM-IDs}. When a replica receives a DROP-NOTIFICATION from libOUM\blue{, which is triggered by timeout,} (and increments \rst{its session-msg-num}\blue{the corresponding \emph{msg-num} of the client}), it must either recover the contents of the missing request or prevent it from succeeding before moving on to subsequent requests. Non-leader replicas do this by contacting the leader for a copy of the request. If the leader itself receives a DROP-NOTIFICATION, it coordinates to commit a NO-OP operation in place of that request:

\begin{enumerate}
    \item If the leader receives a DROP-NOTIFICATION\blue{, which is triggered by timeout}, it inserts a NO-OP into its log and sends a ⟨GAP-COMMIT, log-slot⟩ to the other replicas, where log-slot is the slot into which the NO-OP was inserted.
    \item When a non-leader replica receives the GAP-COMMIT and has filled all log slots up to the one specified by the leader, it inserts a NO-OP into its log at the specified lo- cation3 (possibly overwriting a REQUEST) and replies to the leader with a ⟨GAP-COMMIT-REP, log-slot⟩.
    \item  The leader waits for $f$ GAP-COMMIT-REPs (retrying if necessary).
\end{enumerate}



Clients need not be notified explicitly when a NO-OP has been committed in place of one of their requests. They simply retry their request after failing to receive a quorum of responses. Note that the retried operation will be considered a new request and will have a new slot in the replicas’ logs. Replicas identify duplicate client requests by checking if they have processed another request with the same client-id and request-id, as is commonly done in other protocols.


This protocol ensures correctness because clients do not consider an operation completed until they receive a response from the leader, so the leader can propose a NO-OP regardless of whether the other replicas received the REQUEST. However, before proceeding to the next sequence number, the leader must ensure that a majority of replicas have learned of its decision to commit a NO-OP. When combined with the view change protocol, this ensures that the decision persists even if the leader fails.

As an optimization, the leader can first try to contact the other replicas to obtain a copy of the REQUEST and initiate the gap commit protocol only if no replicas respond before a timeout. While not necessary for correctness, this reduces the number of NO-OPs.

\subsubsection{View Change}
During each view, a \rst{NOPaxos}\blue{Nezha} group has a particular leader \rst{and OUM session number}. \rst{NOPaxos}\blue{Nezha} must perform view changes to ensure progress in \rst{two cases}\blue{one case}: (1) when the leader is suspected of having failed (e.g, by failing to respond to pings), \rst{or (2) when a replica detects the end of an OUM session}. To successfully replace the leader \rst{or move to a new OUM session}, \rst{NOPaxos}\blue{Nezha} runs a view change protocol. This protocol ensures that all successful operations from the old view are carried over into the new view and that all replicas start the new view in a consistent state.


\rst{NOPaxos}\blue{Nezha}’s view change protocol resembles that used in Viewstamped Replication [42]. The principal difference is that \rst{NOPaxos views serve two purposes, and so NOPaxos view IDs are therefore a tuple of <leader-num, session-num> rather than a simple integer.} \rst{A view change can increment either one.} \rst{However, NOPaxos ensures that each replica's leader-num and session-num never go backwards.}\blue{Nezha's view change protocol is exactly the same as that used in Viewstamped Replication.} This maintains a total order over all views that successfully start. \blue{Compared with NOPaxos, Nezha does not need to consider sequencer failure, and its view change follows exactly the standard protocol in Viewstamped Replication, and is much simpler than that in NOPaxos. }

\begin{enumerate}
    \item   A replica initiates a view change when: (1) it suspects that the leader in its current view has failed; \rst{(2) it receives a SESSION-TERMINATED notification from libOUM;} or (3) it receives a VIEW-CHANGE or VIEW-CHANGE-REQ message from another replica with a higher leader-num \rst{or session-num}. In all cases, the replica appropriately increments the leader-num \rst{and/or session-num} in its view-id and sets its status to ViewChange. \rst{If the replica incremented its sessionnum, it resets its session-msg-num to 0}.
    
    It then sends ⟨VIEW-CHANGE-REQ, view-id⟩ to the other replicas and ⟨VIEW-CHANGE, view-id, v′, \rst{session-msg-num,} log⟩ to the leader of the new view, where v′ is the view ID of the last view in which its status was Normal. While in ViewChange status, the replica ignores all replica-to-replica messages (except START-VIEW, VIEW-CHANGE, and VIEW-CHANGE-REQ).
    
    If the replica ever times out waiting for the view change to complete, it simply rebroadcasts the VIEW-CHANGE and VIEW-CHANGE-REQ messages.
    
    \item When the leader for the new view receives $f$ + 1 VIEW-CHANGE messages (including one from itself) with matching view-ids, it performs the following steps:
    \begin{itemize}
        \item The leader merges the logs from the most recent (largest) view in which the replicas had status \texttt{Normal}. For each slot in the log, the merged result is a NO-OP if any log has a NO-OP. Otherwise, the result is a REQUEST if at least one has a REQUEST. It then updates its log to the merged one.
        \item The leader sets its view-id to the one from the VIEW-CHANGE messages \rst{and its session-msg-num to the highest out of all the messages used to form the merged log}. %???
        
        \item  It then sends ⟨START-VIEW, view-id, \rst{session-msg-num,} log⟩ to all replicas (including itself).

    \end{itemize}
    
    \item When a replica receives a START-VIEW message with a view-id greater than or equal to its current view-id, it first updates its view-id, log, \rst{and session-msg-num} to the new values. \rst{It then calls listen(session-num,
session-msg-num) in libOUM}. The replica sends RE-
PLYs to clients for all new REQUESTs added to its log (executing them if the replica is the new leader). Finally, the replica sets its status to \texttt{Normal} and begins receiving messages from libOUM again.

\end{enumerate}

\subsubsection{Synchronization}
During any view, only the leader executes operations and provides results. Thus, all successful client REQUESTs are committed on a stable log at the leader, which contains only persistent client REQUESTs. In contrast, non-leader replicas might have speculative operations throughout their logs. If the leader crashes, the view change protocol ensures that the new leader first recreates the stable log of successful operations. However, it must then execute all operations before it can process new ones. While this protocol is correct, it is clearly inefficient.


Therefore, as an optimization, \rst{NOPaxos}\blue{Nezha} periodically executes a synchronization protocol in the background. This protocol ensures that all other replicas learn which operations have successfully completed and which the leader has replaced with NO-OPs. That is, synchronization ensures that all replicas’ logs are stable up to their sync-point and that they can safely execute all REQUESTs up to this point in the background.

For brevity, we omit the details of this protocol. See [39] for the full specification.

\subsection{Recovery and Reconfiguration}
While the \rst{NOPaxos}\blue{Nezha} protocol as presented above assumes a crash failure model and a fixed replica group, it can also facilitate recovery and reconfiguration using adaptations of standard mechanisms (e.g. Viewstamped Replication [42]). While the recovery mechanism is a direct equivalent of the Viewstamped Replication protocol, the reconfiguration protocol \rst{additionally requires a membership change in the OUM group. The OUM membership is changed by contacting the controller and having it install new forwarding rules for the new members, as well as a new session-num in the sequencer (terminating the old session)}\blue{ is exactly the same as that used in Viewstamped Replication}. The protocol then ensures all members of the new configuration start in a consistent state.

\subsection{Inherited Benefit from NOPaxos}
\rst{NOPaxos}\blue{Nezha} achieves the theoretical minimum latency and maximum throughput: it can execute operations in one round-trip from the client to the replicas and does not require replicas to coordinate on each request. By relying on the \rst{network}\blue{local but synchronized clock time} to stamp requests with sequence numbers, it requires replies only from a simple majority of replicas and uses a cheaper and rollback-free mechanism to correctly account for network anomalies.

The \rst{OUM}\blue{TOUM} session guarantees mean that the replicas already agree on the ordering of all operations. As a consequence, clients need not wait for a super quorum of replicas to reply, as in Fast Paxos and Speculative Paxos (and as is required by any protocol that provides fewer message delays than Paxos in an asynchronous, unordered network [37]). In \rst{NOPaxos}\blue{Nezha}, a simple majority of replicas suffices to guarantee the durability of a REQUEST in the replicas’ shared log.


Additionally, the \rst{OUM}\blue{TOUM} guarantees enable \rst{NOPaxos}\blue{Nezha} to avoid expensive mechanisms needed to detect when replicas are not in the same state, such as using hashing to detect conflicting logs from replicas. To keep the replicas’ logs consistent, the leader need only coordinate with the other replicas when it receives DROP-NOTIFICATIONs. Committing a NO-OP takes but a single round-trip and requires no expensive reconciliation protocol.

\rst{NOPaxos}\blue{Nezha} also avoids rollback, which is usually necessary in speculative protocols. It does so not by coordinating on every operation, as in non-speculative protocols, but by having only the leader execute operations. Non-leader replicas do not execute requests during normal operations (except, as an optimization, when the synchronization protocol indicates it is safe to do so), so they need not rollback. The leader executes operations speculatively, without coordinating with the other replicas, but clients do not accept a leader’s response unless it is supported by matching responses from $f$ other replicas. The only rare case when a replica will execute an operation that is not eventually committed is if a functioning leader is incorrectly replaced through a view change, losing some operations it executed. Because this case is rare, it is reasonable to handle it by having the ousted leader transfer application state from another replica, rather than application-level rollback.

Finally, unlike many replication protocols, \rst{NOPaxos}\blue{Nezha} replicas send and receive a constant number of messages for each REQUEST in the normal case, irrespective of the total number of replicas. This means that \rst{NOPaxos}\blue{Nezha} can be deployed with an increasing number of replicas without the typical performance degradation, allowing for greater fault-tolerance. \S6.3 demonstrates that \rst{NOPaxos}\blue{Nezha} achieves the same throughput regardless of the number of replicas.


\subsection{Benefit of Nezha over NOPaxos}
\label{sec:nezha-advantage}
{\color{blue}
As described in previous sections, TOUM relies on a virtual sequencer, which enables Nezha to be free from special hardware requirement. Therefore, Nezha enjoys much better scalability than NOPaxos and can be directly deployed in public cloud. Besides, since Nezha does not need to worry about the failure of sequencer, it simplifies both the recovery protocol and reconfiguration protocol. Unlike NOPaxos, which needs to adapt the viewstemp replication protocol to handle more attributes, Nezha just follows the standard viewstamp replication protocol for recovery and reconfiguration.

Nezha uses timeout to detect gap and start gap agreement, whereas NOPaxos relies on sequential numbers for the same purpose. Comparing the two mechanism, the timeout-based approach can detect the gap and trigger gap agreement in a more reasonable way, whereas the sequential number-based approach can easily go to conservative/aggressive cases.

\begin{enumerate}
    \item NOPaxos can be too conservative in gap agreement. NOPaxos can only detect gaps when the sequential numbers are not consecutive. Therefore, it cannot detect the gap when the replicas is suffering from consecutive request drops. For example, when Request-1 arrives at the replicas but Request-2$\sim$Request-100 are all lost, NOPaxos cannot detect the gap until Request-101 arrives at the replicas. From then on, it needs to recover the missing 99 requests or starts gap agreement for these 99 requests at one time. Obviously, such a \textbt{burst recovery} procedure will seriously affect the performance of NOPaxos. By contrast, Nezha uses timeout to detect the gaps. So long as the timeout is properly set (by leveraging Huygens, we can obtain good knowledge of the one-way delay between replicas and clients, thus enabling us to set a proper timeout span), Nezha can trigger the gap agreement procedure in time, and avoid the burst problem in NOPaxos.
    \item NOPaxos can also be too aggressive in gap agreement. Since data center usually uses multipath for data transfer. Therefore, it is possible that requests can be reordered even when they are sequentially multicast by the same switch. However, NOPaxos will \textbf{strictly} regard it as a gap so long as the incoming requests do not have consecutive sequential numbers. For example, after the switch multicast Request-1 and Request-2 to the replicas, it is still likely that Request-2 can arrive at the replicas earlier. Under such circumstances, NOPaxos will start the \textbt{unnecessary} gap agreement immediately, even if Request-1 will arrive soon. By contrast, Nezha triggers he gap agreement based the timeout. Targetting at such cases, Nezha will not trigger gap agreement even when Request-2 comes earlier than Request-1.Instead, Nezha will wait for the requests based on the timeout span, and then process the requests in the same block according to the order described in \S\ref{sec:fault}.
\end{enumerate}
}

\subsection{Correctness}
\rst{NOPaxos}\blue{Nezha} guarantees linearizability: that operations submitted by multiple concurrent clients appear to be executed by a single, correct machine. In a sense, correctness in \rst{NOPaxos}\blue{Nezha} is a much simpler property than in other systems, such as Paxos and Viewstamped Replication [33, 48], because the replicas need not agree on the order of the REQUESTs they execute. Since the REQUEST order is already provided by the guarantees of \rst{OUM}\blue{TOUM} sessions, the replicas must only agree on which REQUESTs to execute and which REQUESTs to drop. \blue{Besides, the correctness is also simpler than that in NOPaxos, because Nezha does not need to consider the failure of sequencers and the clock synchronization failure only affects liveness rather than correctness} 
Below, we sketch the proof of correctness for the \rst{NOPaxos}\blue{Nezha} protocol. For a full, detailed proof, see [39]. Additionally, see [39] for a TLA+ specification of the \rst{NOPaxos}\blue{Nezha} protocol.


\textbf{Definitions.} We say that a REQUEST or NO-OP is committed in a log slot if it is processed by $f$ + 1 replicas with matching view-ids, including the leader of that view. We say that a REQUEST is successful if it is committed and the client receives the $f$+1 suitable REPLYs. We say a log is stable in view v if it will be a prefix of the log of every replica in views higher than v.


\textbf{Sketch of Proof.} During a view, a leader’s log grows monotonically (i.e., entries are only appended and never overwritten). Also, leaders execute only the first of duplicate REQUESTs. Therefore, to prove linearizability it is sufficient to show that: (1) every successful operation was appended to a stable log at the leader and that the resulting log is also stable, and \rst{(2) replicas always start a view listening to the correct session-msg-num in an OUM session (i.e., the message corresponding to the number of REQUESTs or NO-OPs committed in that OUM session).}


First, note that any REQUEST or NO-OP that is committed in a log slot will stay in that log slot for all future views: it takes $f$ + 1 replicas to commit a view and $f$ + 1 replicas to complete a view change, so, by quorum intersection, at least one replica initiating the view change will have received the REQUEST or NO-OP. Also, because it takes the leader to commit a REQUEST or NO-OP and its log grows monotonically, only a single REQUEST or NO-OP is ever committed in the same slot during a view. Therefore, any log consisting of only committed REQUESTs and NO-OPs is stable.


Next, every view that starts (i.e., $f$ + 1 replicas receive the START-VIEW and enter Normal status) trivially starts with a log containing only committed REQUESTs and NO-OPs. Replicas send REPLYs to a REQUEST only after all log slots before the REQUEST’s slot have been filled with REQUESTs or NO-OPs; further, a replica inserts a NO-OP only if the leader already inserted that NO-OP. Therefore, if a REQUEST is committed, all previous REQUESTs and NO-OPs in the leader’s log were already committed.

This means that any REQUEST that is successful in a view must have been appended to a stable log at the leader, and the resulting log must also be stable, showing (1). \rst{To see that (2) is true, notice that the last entry in the combined log formed during a view change and the session-msg-num are taken from the same replica(s) and therefore must be consistent.}


\rst{NOPaxos}\blue{Nezha} also guarantees liveness given a sufficient amount of time during which the following properties hold: \blue{clocks are synchronized among nodes and the error bound is less than one message delay;} the network over which the replicas communicate is fair-lossy; there is some bound on the relative processing speeds of replicas; there is a quorum of replicas that stays up; there is a replica that stays up that no replica suspects of having failed; all replicas correctly suspect crashed nodes of having failed; no replica receives a DROP-NOTIFICATION \rst{or SESSION-TERMINATED} from libOUM; and clients’ REQUESTs eventually get delivered through libOUM.


\section{Dynamic Rate Control}
TO DO...


\section{Lazy Write}
TO DO..

==> old/design-old.tex <==
\section{Protocol Design}
\vspace{-0.3cm}
\label{sec:design}
% \sysname is a new consensus protocol that allows the client to complete linear updates in 1 RTT (2 message delays) in fast path and 1.5 RTT (3 message delays) in slow path. To ensure the durability, the client broadcasts the request to every replica. Different from previous protocols (e.g. Multi-Paxos/Raft, Fast Paxos, Speculative Paxos, NOPaxos, etc), the client itself decides the ordering rank of the request by tagging synchronized clock time in the request. Each replica \textbf{selectively} accepts the requests and appends them to its \emph{log} according to the ordering rank. Since the ordering rank of requests has been pre-assigned during submission, the ordering ambiguity is eliminated and \sysname only needs to consider set equality among replicas. To maintain set equality, the leader replica keeps broadcasting its log indices to the follower replicas, and follower replicas add/delete log items from their log set, so as to maintain set equality with the leader. 
% \subsection{Separating Uniform Ordering from Set Equality}
\subsection{Roamap of Design}

\textbf{Fast path/slow path division:} Multi-Paxos/Raft takes 4 message delays to commit one request. To reduce that, a commonly shared design principle in the following variants (i.e. Fast Paxos~\cite{fastpaxos}, Generalized Paxos~\cite{lamport2005generalized}, EPaxos~\cite{sosp13-epaxos}, Speculative Paxos~\cite{nsdi15-specpaxos}, NOPaxos~\cite{osdi16-nopaxos}) is to involve two different paths--fast path and slow path--to commit requests. While the fast path can usually commit requests more efficiently, it may not always succeed and needs to fall back to the slow path once it fails. \sysname shares the same principle in its protocol design, employing the fast path to opportunistically commit requests for high efficiency, and relying on the slow path as a remedy when the fast path fails.

\textbf{Primitive/protocol decoupling:}
The underlying assumption behind the fast path/slow path division is that the fast path succeeds in common cases. However, the assumption can be over-optimistic in practice. For instance, Fast Path, when deployed in highly-engineered network~\cite{nsdi15-specpaxos, osdi16-nopaxos}, can yield desirable latency/throughput performance. By contrast, when it is deployed in public cloud environment, the performance degrades drastically, as observed in~\cite{conext20-domino} and our evaluation (\S~\ref{sec:evaluation}). Therefore, to make the assumption more realistic, the recent works, such as Speculative Paxos~\cite{nsdi15-specpaxos} and NOPaxos~\cite{osdi16-nopaxos}, decouple the whole consensus responsibility into two separate components, i.e. a primitive and a replication protocol. While the primitive cannot guarantee consensus by itself, it creates favorable conditions for the following replication protocol to commit via the fast path more easily. For example, the MOM primitive~\cite{nsdi15-specpaxos} used by Speculative Paxos creates the network environment to make most requests arrive at all replicas in the same order. the OUM primitive~\cite{osdi16-nopaxos} used by NOPaxos ensures ordered delivery of requests without reliability guarantee. Both primitives are essential for the protocol to achieve high performance. Inspired by their decoupling design, we also build a primitive, which is called Deadline-Ordered Multicast (\primname), for \sysname to achieve high-performance consensus in general environment.

\subsection{Deadline-Ordered Multicast}

The consistency among replicas imposes two-fold responsibility on the consensus protocol, i.e. uniform ordering and set equality. Considering any two replicas $R_1$ and $R_2$, we say their states are consistent if the following requirements are both satisfied. 
\begin{itemize}[wide, labelwidth=!,nosep]
    \item \textbf{Uniform ordering.} If $R_1$ processes request $a$ before request $b$, then $R_2$ cannot process request $b$ before request $a$, and vice versa.
    
    \item \textbf{Set equality.} If $R_1$ contains request $a$, then $R_2$ also contains request $a$, and vice versa~\footnote{In NOPaxos paper~\cite{osdi16-nopaxos}, the authors describe a similar requirement called reliable delivery. Whereas their definition describes the requirement from the network perspective, we choose a more straightforward way to describe the requirement from the replica perspective. }.
\end{itemize}

Between the two requirements, uniform ordering is more challenging: generally-deployable protocols, such as Multi-Paxos/Raft, make it a heavy burden for the leader replica to achieve this. Network-demanding protocols, such as Speculative Paxos and NOPaxos, rely on their special-purpose primitives (MOM and OUM) to ease the task for the replication protocol. 

Unlike MOM and OUM, which go to great length to build the highly-engineered network, our \primname primitive takes general deployment as the first priority and eschews the demanding network assistance. The main idea for \primname to create favorable environment for consensus is to \emph{rectify the arrival order of requests with the predicted deadlines}. Nowadays clock synchronization has become generally available, and the message delays of packets can be mostly bounded with a good quality-of-service (QoS) guarantee~\cite{socc12-chronos,hotos15-tail-latency, nsdi15-c3,silo}. Based on these facts, \primname can let the clients decide an expected deadline for its submitted requests, and the replicas can buffer the incoming requests until their deadlines. Since most requests come before their deadlines, these requests will be presented in uniform ordering (of deadlines) when \primname releases them to the replication protocol. The replication protocol only needs to handle those outliers which arrive beyond their deadlines. Our protocol takes a lightweight approach (\S\ref{sec-fix-set-inequality}) to that: All replicas, except one leader replica, simply ignore those outliers and append the requests to their logs in uniform ordering (i.e. the ascending order of the deadlines). The leader modifies the deadlines for those outliers to make them eligible to be appended according to the order of deadlines, and then the leader broadcasts its log indices as the reference, so that the other replicas can add/delete entries to/from their \emph{logs} to maintain set equality. 


The \emph{buffering-and-ordering} design enables \primname to rectify requests' order after they have been reordered in the network. Such a capability proves to be a distinct advantage for \primname over MOM/OUM in general-purpose network environment (e.g. public cloud). When network is not highly-engineered, and packet reordering becomes a frequent pattern, MOM/OUM can easily trigger the slow path of their replication protocols. By contrast, most packet reordering in the network can be rectified by \primname at the replica edge, if the clocks are well synchronized and the deadlines are properly decided. We include a more formal analysis and comparison among the three primitives in Appendix~\ref{appendix-formulation}.

% modify the deadlines for them to enable them appended to the replica logs without breaking the uniform ordering property. 

% In general-purpose network environment (e.g. public cloud), packet reordering can easily occur due to multi-path routing, network congestion, etc. Such circumstances make MOM/OUM far less effective to boost the performance of the corresponding replication protocols.    


% %practical case and uncommon case
% % Fast/Slow Path --> Fast Path [Done]
% % Primitive -> Replication Protocol --> NOPaxos/SpecPaxos [Done]
% % Our pritmive from MOM/OUM [Done]
% % disguinish ORM from OUM [Done]
% Ablation study 
%commutativity 
% client offloading vs non-offloading



% \textbf{State of the art}. 
% Typical protocols, including Multi-Paxos/Raft and NOPaxos,  employ a centralized serialization point to establish the uniform ordering. More specifically, Multi-Paxos/Raft depend on the leader to decide the order for requests (i.e. \textbf{late binding} of order) whereas NOPaxos inserts a sequencer between clients and replicas to decide the order of requests (i.e. \textbf{early binding} of order). The \textbf{late binding} design places heavy workloads on the leader replica, causing it to become a potential bottleneck for throughput. The \textbf{early binding} design, on the other hand, optimistically assume the    

% There are two lines of works conducted trying to satisfy both requirements in different ways. 


% The first line of work  employs a centralized serialization point to decide uniform ordering for replicas. Multi-Paxos/Raft elect one replica as the leader to decide the ordering of requests, causing the leader replica to become a throughput bottleneck. NOPaxos deploys a sequencer between clients and replicas to free the leader replica from the serialization bottleneck. However, the ordering of client requests are early decided at the sequencer. Whenever the request order at replicas differs from the order decided by the sequencer, the NOPaxos protocol triggers reconciliation (which is called gap agreement in~\cite{osdi16-nopaxos}) even if replica states are consistent.  

% It is challenging to satisfy both requirements without a centralized serialization point. 

% However, we will show in \sysname that, by using clock synchronization, the ordering ambiguity can be eliminated during the replication process at a low cost, and we can fix the \emph{potential} set inequality later with lightweight leader$\xrightarrow{}$follower communication.


% To achieve this, we develop a generally deployable primitive called ORM.

% \subsection{Deadline-Ordered Multicast(ORM)}

\subsection{\primname Design and Implementation}
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=8cm]{figures/DOM.pdf}
    \caption{\primname design. On the client side, \primname broadcasts the  messages. On the replica side, the message is destined to either \circleincap{1}\emph{early-buffer} or \circleincap{2}\emph{late-buffer}, and the messages in the \emph{early-buffer} is released to replicas in uniform ordering.}
    \label{dom-design}
\end{figure}

Figure~\ref{dom-design} illustrates the major components of \primname. \primname is built atop clock synchronization. It inserts a shim layer on both edges of clients and replicas and provide three main interfaces shown in Figure~\ref{dom-interface}. 


\begin{figure}[!h]
\vspace{-0.5cm}
    \centering
    \begin{tcolorbox}[colback=white!10,%gray background %colframe=black,% black frame colour
                      width=8cm,% Use 8cm total width,
                      arc=1mm, auto outer arc,
                      boxrule=0.5pt,
                     ]
    \begin{itemize}[leftmargin=*]
        \item \texttt{DOMSend}---The client calls it to broadcast its message to replicas with sending time ($s$) and latency bound ($l$) tagged.
        \item \texttt{DOMReceive}--- The replica calls it to receive the message from the client, and place the message to either the \emph{early-buffer} or the \emph{late-buffer}.  
        
        \item \texttt{DOMProbe}--- Both the client and replica call it so that the replica can measure the client-replica OWD and piggybacks it to the client.
        
    \end{itemize}
    \end{tcolorbox}
    \caption{\primname Interfaces}
    \label{dom-interface}
    \vspace{-0.4cm}
\end{figure}

On the client side, \primname provides \texttt{DOMSend} for the client to broadcast its messages to the replicas. In each broadcast message, \primname also tags the sending time ($s$) and the latency bound ($l$) for this message, with $s$ and $l$ summing up to be the deadline $D=s+l$ for this message to arrive at replicas.

On the replica side, \primname provides \texttt{DOMReceive} for the replicas to receive the messages from the client, and place the message to two different destinations, namely, \emph{early-buffer} and \emph{late-buffer}. The \emph{early-buffer} is implemented as a priority queue, with the deadline of the message as the sorting rank, whereas the \emph{late-buffer} is implemented as a hash map, indexed by the combination of the client identifier and the request identifier (i.e. $<\emph{client-id},\emph{request-id}>$). 

\primname keeps checking the local clock time to release the messages from the \emph{early-buffer}, i.e. when the local clock time has passed the message deadline, this message is released by \primname and handled to the replication protocol to achieve consensus among replicas. However, not all messages can be destined to the \emph{early-buffer}, because \primname aims to ensure uniform ordering for the messages released from the \emph{early-buffer}. For those messages whose deadline is smaller than the last released message from the \emph{early-buffer}, they will be destined to the \emph{late-buffer} instead.

Meanwhile, \primname provides \texttt{DOMProbe} interfaces to keep measuring the one-way delay (OWD) between the two edges. Once the replicas receive the message from the clients, it can calculate the OWD by using the receiving time minus the sending time ($s$). The OWD stats will be piggybacked to the clients to facilitate the clients to decide more reasonable latency bound (and correspondingly a more reasonable deadline) for the following messages. More details about the latency bound estimation are described in \S\ref{mov-avg-bound}.

When equipped with \primname, every replica can see the messages (requests) in uniform ordering (of the deadline). However, set equality is not guaranteed among replicas: The message may be placed into the \emph{early-buffer}s on some replicas and finally visible to these replicas, whereas it fails to satisfy the condition to enter the \emph{early-buffer} on the other replicas (possibly due to clock skew, latency variance, etc) and is left in their \emph{late-buffer}s. Nevertheless, such an uniform ordering guarantee has already eased the burden for the replication protocol. 



\section{\sysname Protocol}
We design \sysname, a new replication protocol which leverages \primname to achieve high-performance consensus in general-purpose network environment, such as public cloud.
\subsection{Model and Assumptions}
\vspace{-0.2cm}
\sysname assumes a fail-stop model and does not handle Byzantine failure. As in typical consensus protocols, it uses $2f+1$ replicas, including 1 leader and $2f$ followers. Compared with the classic Multi-Paxos/Raft protocol, \sysname guarantees the correctness and liveness under the same assumptions. However, the performance of \sysname relies on the power of \primname, which is closely related to the inter-VM clock synchronization and the variance of one-way delay between clients and replicas. In \sysname, requests can be committed via either the fast path in 1 RTT or the slow path in 1.5 RTTs. We will explain more details in \S\ref{protocol-overview}. 

%Requests via the fast path can be committed in 1 RTT with no throughput bottleneck. Alternatively, requests via the slow path can be committed in 1.5 RTTs.  

% The requests can be committed via the fast path (shown in Figure~\ref{fig-workflow-fast}) or the slow path (shown in Figure~\ref{fig-workflow-slow}). 


% \subsection{Design Principles}
% To yield a high performance for \sysname without special network assistance, we hope the fast path can achieve optimal latency (1 RTT) with no throughput bottleneck, and most requests can be committed via the fast path. In the meantime, we also hope the slow path is not much slower than the fast path. Motivated by the key insights in \S\ref{sec-motivation}, we develop three main principles in the design of \sysname.

% \textbf{Principle 1: Decomposing ordering agreement}. From the analysis in \S\ref{sec-motivation} we know that, it is undesirable either prioritizing ordering agreement over replication or deferring the ordering agreement after replication and quorum check. To avoid such a dilemma of decision-making, we choose to first decompose the ordering agreement task. More specifically, the ordering agreement imposes two-fold requirements on the protocol.

% \begin{enumerate}[wide, labelwidth=!,nosep,label=(\arabic*)]
%     \item \textbf{No ordering ambiguity.} Ordering ambiguity means some replicas order request $a$ ahead of $b$ whereas the other replicas order them in a reverse way. Ordering ambiguity should not exist if the replicas have consistent states.
    
%     \item \textbf{Set equality.} Set equality means the replicas have exactly the same requests (i.e. the sets of requests are equal).
% \end{enumerate}

% % \textbf{Principle 1: Eliminating ordering ambiguity during replication}.

% It is challenging to satisfy both requirements without a centralized serialization point. However, we will show in \sysname that, by using clock synchronization, the ordering ambiguity can be eliminated during the replication process at a low cost, and we can fix the \emph{potential} set inequality later by letting the leader broadcast small-sized \emph{sync} messages to followers


% \textbf{Principle 2: Completely offloading quorum check to clients.} For both the fast path and the slow path in \sysname, we let the clients do the quorum check and decide whether the request has been committed. Such a design benefits in two aspects. First, it relieves the bottleneck of the leader replica. Second, it reduces the commit/execution latency and clients can know the commit/execution result even earlier than the replicas.

% \textbf{Principle 3: Early fixing set inequality.}
% Since ordering ambiguity has been eliminated during the replication process, the only source of inconsistency comes from set inequality, i.e. some replicas contain a specific request whereas the others do not. Unlike Fast Paxos and Speculative Paxos, which start fixing inconsistency only after it is really detected during the quorum check, we will show \sysname can launch the routine to fix set inequality much earlier (i.e. in parallel with the leader's execution of the request). When the client detects the set inequality during the quorum check, the fixing routine of \sysname is already in progress.

% % \todo{Fast Path and Slow Path }
% % \todo{2 pseudo-code}

% % \vspace{-0.4cm}
% % \subsection{Decomposing Ordering Agreement}
% % \label{sec-decompose}
% % \vspace{-0.1cm}
% % \sysname also prioritizes replication over ordering agreement. But unlike Fast Paxos/Speculative Paxos, \sysname can avoid the heavy penalty to resolve the (possible) inconsistency. The key idea of \sysname is to decompose the expensive ordering agreement into two finer-grained tasks: 


% % \begin{itemize}[wide, labelwidth=!,nosep]
% %     \item \textbf{Eliminate ordering ambiguity.} If one replica orders request $a$ ahead of request $b$, no other replicas can order them in a reverse way.   
% %     \item \textbf{Maintain set equality.} All the replicas have exactly the same requests (i.e. the sets of requests are equal).
% % \end{itemize}

% % Without the centralized serialization point, it is quite challenging to achieve ordering agreement. However, we will show in \sysname, by using clock synchronization, it is fairly easy to \emph{eliminate ordering ambiguity early}, and we can defer to \emph{fix the (potential) set equality later} (with low cost) during the sync process among replicas. 

% % To be more specific, \sysname synchronizes the clocks between clients and replicas. It allows the clients to decide an ordering rank (i.e. the sum of its submission time and a latency bound) for the request. With reference to the rank and the appended entries in its \emph{log}, the replica decides whether the request can be accepted without ordering ambiguity (\S\ref{selective-acceptance}). Ideally, each replica is expected to accept the same requests, thus they are committed via the fast path with 2 message delays (1 RTT). However, when replicas take different actions (acceptance/rejection) towards some requests, set inequality will occur among replicas and \sysname relies on the lightweight index synchronization process (\S\ref{index-sync}) to fix set inequality, thus the requests are committed via the slow path with 3 message delays (1.5 RTTs). 


% % Besides, \sysname makes two assumption of the system. 

% % \begin{itemize}[wide, labelwidth=!,nosep]
% %     \item \textbf{Measurable and predictable latency}. Nezha assumes that the latency between clients and replicas is measurable and predictable. Such an assumption has been proved to be realistic in today's cloud environment~\cite{socc12-chronos,silo,nsdi13-bobtail,nsdi15-c3}. Based on the assumption, the client can decide a proper latency bound so that the request is more likely to be committed in the fast path. 
    
% %     \item \textbf{Mostly-synchronized clocks}. \sysname assumes that the clocks on VMs are synchronized \emph{in most time} with a small error bound. Such an assumption has become true with the recent emergence of high-precision clock-sync solutions~\cite{huygens,osdi20-sundial,tsn_ptp}. In our case, we rely on Huygens~\cite{huygens} to provide  \emph{mostly} synchronized clock time, which improves the likelihood for replicas to take consistent actions (acceptance/rejection) towards the incoming requests. Meanwhile, the synced clocks also benefit clients' decisions on the latency bound because it provides more accurate measurement of client-replica latency (details in \S\ref{selective-acceptance}). 
% % \end{itemize}

% % In addition, \sysname also requires the clock time of each server to increase monotonously. Since Huygens periodically corrects the clock of each server with an offset, in rare cases, the negative offset may break the monotonicity between two adjacent calls of the clock API, and that will affect the correctness of \sysname. However, this property is easy to guarantee: We record the return value every time when the replica/client calls the clock API. If the returned value is smaller than that of the last API call, we simply abandon the value and retry the clock API until it returns a larger time than the last returned value. In this way, non-monotonicity is masked. \sysname (as well as the upper applications) can only see monotonic clock time.

% % Although \sysname makes assumptions about latency bound and clock synchronization, it only relies on these assumptions for performance rather than correctness. Besides, as explained in \S\ref{protocol-overview}$\sim$\S\ref{quorum-check}, although the fast path of \sysname requires a larger quorum (i.e. $f+\lceil f/2 \rceil + 1$) and cannot work with only $f+1$ replicas, the slow path serves as a remedy and enables \sysname to maintain the same liveness level (i.e. $f+1$ replicas) as Multi-Paxos/Raft.

% \vspace{-0.4cm}
\subsection{Protocol Overview}
\label{protocol-overview}

\begin{figure}[!h]
\vspace{-0.5cm}
    \centering
    \begin{tcolorbox}[colback=white!10,%gray background %colframe=black,% black frame colour
                      width=8cm,% Use 8cm total width,
                      arc=1mm, auto outer arc,
                      boxrule=0.5pt,
                     ]
    \begin{itemize}[leftmargin=*]
        \item \emph{replica-id}--- replica identifier ($0,1,\cdots, 2f$)
        \item \emph{status}--- one of \textsc{normal}, \textsc{viewchange}, or \textsc{recovering}
        \item \emph{crash-vector}--- a vector of $2f+1$ counters initialized as 0s, which is used to guarantee correctness during replica rejoin and view change process %(details in \S\ref{sec:recovery} and Appendix~\ref{recovery-algo})
        \item \emph{view-id}--- the view identifier, initialized as 0 and increased after every view change
        \item \emph{early-buffer}--- the priority queue provided by \primname, which sorts and releases the requests according to their deadlines. %(details in \S\ref{selective-acceptance})
        \item \emph{late-buffer}-- the hash map provided by \primname, and the requests are indexed by 2-tuple $<\emph{client-id}, \emph{request-id}>$ of the request.
        \item \emph{log}--- a list of client requests, appended according to their \emph{ranks}' order.  
        \item \emph{sync-point}--- the latest synchronization point, to which the replica state (\emph{log}) is consistent with the leader. 
    \end{itemize}
    \end{tcolorbox}
    \caption{Local state of \sysname replicas}
    \label{fig:replica-state}
    \vspace{-0.4cm}
\end{figure}

Figure~\ref{fig:replica-state} illustrates the state maintained at each \sysname replica. Replicas leverage a view-based approach~\cite{viewstamp}: Each replica is assigned with a unique \emph{replica-id}, ranging from 0 to $2f$. Each view is indicated by a \emph{view-id}, and the \emph{view-id} is incremented each time a new leader is needed. In each view, only a single replica acts as the leader, whose \emph{replica-id} equals $\emph{view-id} \% (2f+1)$. Replicas tag all messages with their current \emph{view-id} while communicating with other replicas. During the normal process (i.e. when \emph{status} is \textsc{normal}), replicas ignore all messages tagged with different \emph{view-id}s. Only during the view change process (i.e. when \emph{status} is \textsc{viewchange}), replicas with different \emph{view-id}s communicate with each other and eventually recover to the normal process. Besides, since the diskless recovery in~\cite{viewstamp} has proved to be incorrect~\cite{disc17-dcr,disc17-dcr-techreport}, we also tag \emph{crash-vector}s to the messages during the view change or replica recovery (i.e. when \emph{status} is \textsc{recovering}) to fix the critical flaw and ensure correctness (details in \S\ref{sec:recovery}).


The workflow of \sysname consists of the fast path and the slow path, illustrated in
Figure~\ref{fig-workflow-fast} and Figure~\ref{fig-workflow-slow} respectively. 

%\sysname handles every requests based on its key attribute, $rank$. The $rank$ of the request is calculated by summing up its submission time ($s$) and a latency bound ($d$). $s$ is tagged by the client as its local clock time during submission. $d$ is decided by the client based on the estimation of client-replica latency. Specifically, the replica uses a sliding window to estimate the one-way delays (OWD) from each client to itself and piggybacks the estimated value when replying to the client. The client collects the estimated OWDs from each replica and uses the maximum as the latency bound (More details in \S\ref{mov-avg-bound}). With reference to the \emph{ranks}, \sysname can determine a definitive order among requests.
%~\footnote{If two requests have the same \emph{rank}, the tie is broken by comparing their \emph{client-id}s. Further, if they have the same \emph{rank} and \emph{client-id}, the tie is broken by comparing their \emph{request-id}s   }. 

% Each replica adopts an \emph{append-only} way to add requests into its \emph{log}, but the leader can instruct the followers to add/delete their \emph{log} entries. Thanks to DOM, the appended requests on each replica satisfy the uniform ordering requirement, despite of the network which can reorder the requests frequently. 

% After the request is appended to the replica, a reply message is sent back to the client, which we call \emph{fast-reply}. 

%Since requests may arrive at replicas in different order, blindly appending can easily lead to ordering ambiguity among replicas. To avoid that, the replica only appends the request if its \emph{rank} is larger than that of the last appended one in the \emph{log}. In this way, ordering ambiguity is eliminated since the \emph{log} entries on each replica follows an ascending order of their \emph{ranks}.


% The drawback of such appending is also obvious. If a request with a very large \emph{rank} is appended early, then many following requests, which have smaller \emph{rank}s, can no longer be appended. To avoid this and append requests more reasonably, \sysname designs an \emph{early-buffer} and a \emph{late-buffer} on each replica. 

% Instead of immediately appending the request once it arrives, the replica places the request into one of the two buffers:

% If the \emph{rank} of the request is larger than the that of the last appended one, this request is put into \emph{early-buffer}. It will be released and appended when the replica's clock time has passed its \emph{rank} ($s+d$). This gives chances for other requests with smaller ranks to be appended, so long as they arrive within their predefined latency bound (i.e. before $s+d$). 

% Otherwise, this request is put into \emph{late-buffer}. As a follower, \emph{late-buffer} just serves as a cache. In case the request is needed later, the follower can directly fetch it from \emph{late-buffer} instead of asking from the others. As the leader, it needs to ensure progress even when all replicas put this request into \emph{late-buffer}. To achieve that, the leader replaces the \emph{rank} of the request with its current local clock time. Then the \emph{rank} is larger than the last appended entry for sure and becomes eligible to go into the \emph{early-buffer}.

% flip left part of fig 2
% H/R buffer -> early request buffer 
%recycle buffer->late request buffer
% put figure 2 and figure 3 side by side
% add a note in figure 2, including the leader 
% refer to cache coherence 

% put secion no on Figure 4
\clearpage
\begin{figure}[!t]
    \centering
    \includegraphics[width=8cm]{figures/Nezha-Arch-Fast-Path.pdf}
    \caption{Fast path of \sysname}
    \label{fig-workflow-fast}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=8cm]{figures/Nezha-Arch-Slow-Path.pdf}
    \caption{Slow path of \sysname}
    \label{fig-workflow-slow}
\end{figure}

The workflow of \sysname consists of the fast path and the slow path, illustrated in
Figure~\ref{fig-workflow-fast} and Figure~\ref{fig-workflow-slow} respectively. Both paths start from the replication process, i.e. the client broadcasts the request to every replica (\circled{1} in Figure~\ref{fig-workflow-fast} and Figure~\ref{fig-workflow-slow}). Once the request arrives at the replica, it can be directed to one of the two destinations, namely \emph{hold/release (H/R) buffer} and \emph{recycle-pool}. If appending the request to the replica's \emph{log} does not cause potential ordering ambiguity, then replica directs it to the \emph{H/R buffer} and the request has an opportunity~\footnote{We say ``an opportunity" because the request may also be committed in the slow path or abandoned, e.g. After the client broadcasts the request to all replicas, the request only arrives at the leader but is lost while transmitting to followers. In this case, the request is unable to commit in the fast path. Another case is that the request only arrives at some followers but is lost while transmitting to the leader and other followers. Since the leader is unaware of the request, it cannot be committed in either path and will finally be abandoned by its replica.} to be committed in the fast path. Otherwise, the replica directs it to the \emph{recycle-pool} and the request only has an opportunity to be committed in the slow path. 


Figure~\ref{nezha-flow-chart} summarizes four major steps in \sysname design. The fast path consists of two of them which costs 1 RTT, whereas the slow path consists of three of them which costs 1.5 RTTs.
In the following sub-sections (\S\ref{selective-acceptance}$\sim$\S\ref{sec-slow-quorum-check}), we will describe the four steps in more details. 
\begin{figure}[!h]
    \centering
    \includegraphics[width=8cm]{figures/Nezha-flow-chart.pdf}
    \caption{Workflow of \sysname protocol}
    \label{nezha-flow-chart}
\end{figure}


% The replicas decide the destination for the request with reference to its arrival time and the relevant information tagged by the client. We explain how replicas make such decisions in \S\ref{selective-acceptance}.

% \textbf{Fast path.} Ideally, every replica directs the request to its \emph{H/R buffer} (\circled{2}). The replica releases the request based on its local clock time and appends the request to its \emph{log} (\circled{3}). Only the leader replica executes the request by applying the request to its state machine (\circled{4}). After the appending/execution, all replicas reply to the client (\circled{5}) and we name this type of reply as \emph{fast-reply}. The \emph{fast-reply} includes the information of the replica's current state. The client collects \emph{fast-replies} and conducts the quorum check. If the client receives the \emph{fast-replies} for this request from $1+f+\lceil f/2\rceil$ replicas (including the leader), and these \emph{fast-replies} indicate consistent replica states, then the client considers the request as committed in the fast path and obtains the execution result from the leader's \emph{fast-reply}. From Figure~\ref{fig-workflow-fast} we know the fast path only costs 1 RTT (\circled{1} and \circled{5}) to commit the request.

% \textbf{Slow path.}  However, the replica may also direct the request to its \emph{recycle-pool} instead of \emph{H/R buffer}, for fear that directing the request to \emph{H/R buffer} and later appending to the \emph{log} can cause ordering ambiguity among replicas. As shown in Figure~\ref{fig-workflow-slow}, after directing the request to the \emph{recycle-pool} (\circled{2}), the leader replica can pick the request back and modify the request to make it eligible for entering \emph{H/R buffer} (\circled{3}). After that, the request on the leader replica follows the same workflow as in the fast path: The leader releases the request and appends it to the \emph{log} (\circled{4}), then the leader applies the request to the state machine (\circled{5}) and gives a \emph{fast-reply} to the client (\circled{6}). In parallel with \circled{5}, the leader also broadcasts a \emph{sync} message to the followers (\circled{7}), notifying them of the current entries in its \emph{log}. After receiving the \emph{sync} message from the leader, the followers modify their logs (\circled{8}) to keep consistent (i.e. maintain set equality) with the leader. Such modification may include deleting entries from the log, picking entries back from the recycle-pool (\circled{9}) and fetching the missing entries from other replicas (if not found in the \emph{recycle-pool}). After ensuring the consistency with the leader, the followers reply to the client (\circled{10}), and we name this type of reply as \emph{slow-reply}. The \emph{slow-reply} indicates the follower's state is consistent with the leader's state.  The client considers the request as committed after it receives 1 \emph{fast-reply} from the leader and $f$ \emph{slow-replies} from the followers. Since the follower can only send the \emph{slow-reply} after it receives the \emph{sync} message from the leader, it costs 1 additional message delay (0.5 RTT) for the client to receive the \emph{slow-replies}. Therefore, the slow path costs 1.5 RTTs to commit the request. 


% \textbf{Summary.} The complete workflow of \sysname protocol can be summarized as Figure~\ref{nezha-flow-chart}. In the following sub-sections (\S\ref{selective-acceptance}$\sim$\S\ref{sec-slow-quorum-check}), we will describe the workflow in more details. 
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=8cm]{figures/Nezha-flow-chart.pdf}
%     \caption{Workflow of \sysname protocol}
%     \label{nezha-flow-chart}
% \end{figure}

% The workflow of \sysname can be divided into fast path and slow path. The fast path allows the request to be committed in 1 RTT (i.e. 2 message delays). When inconsistency (i.e. set inequality) occurs between the leader and followers, the request is committed through the slow path, which costs 1.5 RTTs (i.e. 3 message delays). Among the $2f+1$ replicas, only the leader executes the request and replies with the execution result. The other $2f$ followers only append the request to their \emph{log}s without execution. For both the fast path and slow path, the client takes the full responsibility to check the quorum and decide whether the request has been committed. %, and whether the execution result has been persisted (i.e. the execution result remains consistent  after crash and recovery).

% In general, \sysname protocol consists of three main components:
% \begin{itemize}[wide, labelwidth=!,nosep]
%     \item \textbf{Selective acceptance} (\S\ref{selective-acceptance}): Replicas selectively accept the client request if appending the request does not introduce ordering ambiguity. Otherwise, the follower ignores the request whereas the leader modifies the ordering rank for the request to make it eligible for acceptance.
%     \item \textbf{Index synchronization} (\S\ref{index-sync}): The leader runs a polling thread, which keeps broadcasting the indices of requests appended to its \emph{log}. Followers modify their own \emph{log}s according to the index information, adding/deleting requests to/from their \emph{log}s for set equality.   
%     \item \textbf{Quorum check} (\S\ref{quorum-check}). Clients take the full responsibility of quorum check. They collect the replies from replicas and notify the upper application when the request has been committed/executed.
% \end{itemize}





% Client requests can be directed to two different destinations once received by the replica. If the request is accepted by the replica, it will be put into the replica's \emph{hold/release (H/R) buffer}, and finally appended to its \emph{log}. Otherwise, the request is put into the \emph{recycle-pool}, in case the request needs to be recovered during the index synchronization process (\S\ref{index-sync}). The index synchronization process allows the follower to advance its \emph{sync-point}, which divides the follower's \emph{log} into two parts (refer to Figure~\ref{sync-demo}). The left part is consistent with the leader's \emph{log}, whereas the right part only eliminates ordering ambiguity but without guaranteeing set equality.

\vspace{-0.4cm}
\subsection{Eliminating Order Ambiguity in Replication}
\vspace{-0.1cm}
\label{selective-acceptance}
Both the fast path and the slow path start with the client replicating (broadcasting) its request to every replica. The format of a complete request message can be described as a 5-tuple.
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.2cm}
    request = <\emph{client-id}, \emph{request-id}, command, s, l>
\end{equation*}

\emph{client-id} and \emph{request-id} represent the identifiers of the client and its request, and they combine to uniquely identify the request on one replica. $command$ represents the content of the request, which will be executed by the leader. Besides, $s$ and $l$ are also tagged in the message by DOM.

Besides, the client also tags the submission time $s$ and the latency bound $d$. The latency bound $d$ is an estimation of the one-way delay (OWD) between the client and the replicas, indicating that the request is expected to arrive at replicas before $s+d$. When receiving the request, the replica calculates the ordering rank as $rank=s+d$. Any two different requests can be compared according to their $rank$ value. In rare cases, when two different requests have the same $rank$ value, the tie is broken by comparing their $\emph{client-id}$s.~\footnote{Even more rarely, when two requests have the same $rank$ and \emph{client-id} (e.g. The client submits one request first with a smaller $s$ and a larger $d$, but later submits another request with a larger $s$ and a smaller $d$, thus these two requests have the same $rank=s+d$ and they are from the same client), the tie is broken by comparing their \emph{request-id}s}

The $rank$ of the request serves two proposes. First, it decides whether the replica can accept the request. Second, replicas append the accepted requests to \emph{log}s following the order of their $rank$s, thus establishing a definitive order without ambiguity. During the recovery, the survived requests are still sorted (and executed) by their \emph{ranks}.

The replica only accepts requests which do not introduce risks of ordering ambiguity. To be more specific, if the request has a $rank$ larger than the last entry appended to the \emph{log}, it is accepted by the replica. After the request is accepted, it is not appended to the \emph{log} immediately. Instead, the replica puts the request into its \emph{H/R buffer} (\circled{2} in Figure~\ref{fig-workflow-fast}). The replica releases the request when its clock time passes $s+d$, and appends it to the \emph{log} as a log entry (\circled{3} in Figure~\ref{fig-workflow-fast}). The replica chooses to hold the request until $s+d$ because the other requests with smaller $rank$s may arrive before $s+d$. If the request with $rank=s+d$ is appended too early, the other requests cannot be accepted and appended any more. 

The replica cannot accept the request which arrives at the replica with a smaller $rank$ than the last appended entry, because appending it after entries with larger $rank$s would lead to ordering ambiguity (i.e. The other replicas may append the two requests in the reverse order). Besides, inserting the request into the \emph{log} according to $rank$ order is also infeasible due to the potential violation of consistency and linearizability.~\footnote{For example, we assume two requests \emph{req-1} and \emph{req-2} with $rank=1$ and $rank=2$ respectively. \emph{req-2} has already been committed (and executed by the leader) before \emph{req-1} is submitted. If \emph{req-1} is inserted by the majority and the leader crashes afterwards. \emph{req-1} can be recovered and executed ahead of \emph{req-2} by the new leader, thus reverting the execution order (linearizability violation) and causing different execution result (consistency violation). } Under such situations, replicas put the request into its \emph{recycle-pool} (\circled{2} in Figure~\ref{fig-workflow-slow}), in case the request is needed later. Specially, if the replica is the leader, it aims to ensure progress (liveness) in such cases, so it picks back the request from the \emph{recycle-pool} (\circled{3} in Figure~\ref{fig-workflow-slow}). It replaces the $rank$ of the request with its current clock time (i.e. larger than the \emph{rank} of last appended entry), so that the request becomes eligible for acceptance without ordering ambiguity. The request is eventually appended to the \emph{log} (\circled{4} in Figure~\ref{fig-workflow-slow}) and applied to the state machine (\circled{5} in Figure~\ref{fig-workflow-slow}). 

From the replication process we know that, all the accepted requests will be appended to the \emph{log} according to an ascending order of their \emph{rank}s. For any two replicas, so long as they accept the same requests, they will order them in the same way without ordering ambiguity.


\subsection{Quorum Check of Fast Path}
\label{sec-fast-quorum-check}
As shown in Figure~\ref{fig-workflow-fast}, after appending the request to its \emph{log} (\circled{3}), followers immediately send a reply to the client without executing the request (\circled{5}), whereas the leader first executes the request (\circled{4}) and sends a reply including the execution result. We name this type of reply as \emph{fast-reply}. The format of the \emph{fast-reply} message can be described as a 5-tuple.
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.1cm}
   \begin{aligned}
        \emph{fast-reply} = <\emph{view-id}, \emph{request-id},\emph{replica-id},  result, hash>
\end{aligned} 
\end{equation*}

Inside the reply, the replica tags its current \emph{view-id}, \emph{replica-id}, and  the \emph{request-id} of the corresponding request. If the replica is the leader, it also includes the execution result of the request, otherwise, the \emph{result} field is \emph{null}. 

Moreover, the replica includes an additional field, \emph{hash}, to facilitate the client to check the consistency of replica states. The \emph{hash} field encodes all the previously appended entries with an incremental hash function~\cite{increment-hash}, i.e.  
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.2cm}
hash_n = \bigoplus_{1\leq i \leq n} h(request_i)
\end{equation*}
where $h(*)$ is a standard hash function (e.g. SHA1) and  $\oplus$ is the exclusive-or (XOR) operation. To calculate $h(request_i)$,  we concat the values of $rank$ (i.e. $s+d$), \emph{client-id}, \emph{request-id}, and the other optional information as a string, and then transform it into a hash value. The final hash value $hash_n$ is obtained by XORing all the $n$ hash values generated from each request. Without considering hash collision~\footnote{ We use SHA1 in \sysname to generate 160-bit hash with the collision rate of $1/2^{160}$, which is negligible in practice. Other stronger hash functions are compatible for even lower collision rate.}, $hash_n$ represents the state of the replica when it replies to the client. 
%By comparing the \emph{hash} field of the \emph{fast-reply} messages from different replicas, the client knows whether they are consistent. 

The incremental hash enjoys two advantages. First, it provides an easy way for clients to check set equality among replicas. Since the ordering ambiguity has been eliminated during the replication, set equality is sufficient to ensure the state consistency among replicas. Second, the hash is computed incrementally. Adding/deleting requests only requires incremental computation of XOR and $h(*)$, this property is useful because it enables followers to rapidly fix set inequality and correct the hash value with subtle cost, instead of computing the hash from scratch. 


The client waits for reply messages related to its request with matching \emph{view-id}s and \emph{request-id}s. It considers the request as committed when it receives the \emph{fast-reply} from the leader and  $f+\lceil f/2 \rceil$ followers, with the same \emph{hash}. The client also obtains the execution result of the request from the leader's \emph{fast-reply}.


The reason why the fast path requires a super quorum ($f+\lceil f/2 \rceil+1$) rather than a simple majority ($f+1$) is the same as in Fast Paxos and Speculative Paxos: Without leader-follower communication, a simple majority cannot provide sufficient information for the new leader to distinguish committed requests from uncommitted requests after crash. Consider what would happen if we had used a simple majority ($f+1$) in the fast path. Suppose there are two requests \emph{req-1} and \emph{req-2}, and \emph{req-1} has a larger  \emph{rank}. \emph{req-1} is accepted by the leader and $f$ followers. They send \emph{fast-replies} to the client, and then the client considers the request as committed and delivers the execution result from the leader's \emph{fast-reply} to the upper application. Meanwhile, \emph{req-2} is accepted by the other $f$ followers. After that, the leader fails, leaving $f$ followers possessing \emph{req-1} and the other $f$ followers possessing \emph{req-2}. Under such a situation, the new leader cannot tell which one is the committed request. Even worse, if the new leader involves \emph{req-2} into the recovered \emph{log}, it will be appended and executed ahead of \emph{req-1} due to the smaller \emph{rank}. Therefore, it causes inconsistent execution result for \emph{req-1}, compared with the result before the leader crash. 


\subsection{Early Fixing Set Inequality}
\label{sec-fix-set-inequality}
Set equality requires the replicas to accept the same requests. However, replicas can fail to satisfy the requirement because of multiple reasons. For example, the broadcast request arrives at some replicas before $s+d$ but arrives at the others after $s+d$. In this case, some replicas accept the request whereas the others reject it. Besides, even if the request arrives late on every replica, the leader will modify its \emph{rank} and finally accept it, whereas all the followers reject it. Although no ordering ambiguity exists among replicas, the set inequality still causes inconsistency across replicas. 

Although the inconsistency can be finally detected during the quorum check of the fast path (i.e. the client will notice the inconsistency of the hash values included in \emph{fast-replies}), it is quite late for \sysname to start fixing the inconsistency (set inequality) from that moment. 

Since \sysname only allows appending requests rather than inserting them, the position of the request in the \emph{log} will not change once it has been appended. As shown in Figure~\ref{fig-workflow-slow}, after the leader replica appends entry 6 to its \emph{log} (\circled{4}), the positions of all the log entries (requests) from 1 to 6 become immutable. By this time, the leader can already notify the followers of its current state, instead of waiting until set inequality really happens. Therefore, in parallel with the leader's execution (\circled{5}), the leader runs a polling thread, which keeps broadcasting the \emph{sync} messages to all followers and urging them to fix the \emph{potential} set inequality. The format of the \emph{sync} message can be described as a 5-tuple. 
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.2cm}
    sync = <\emph{view-id}, \emph{client-id}, \emph{request-id}, \emph{rank}, \emph{log-id}>
\end{equation*}

The \emph{sync} message serves two purposes. First, it works as the heartbeat of the leader. Once failing to receive the leader's heartbeat for a threshold of time, followers initiate a view change to elect a new leader (\S\ref{sec-leader-change}).  
Second, it can timely correct the set inequality, making the followers' \emph{log}s consistent with the leader's \emph{log}. 

The \emph{sync} message has much smaller size than the \emph{request}, because it does not include the body (i.e.the \emph{command} field) of the request. Among the five fields, \emph{client-id} and \emph{request-id} combine to identify the request on one replica. \emph{rank} is the ordering rank of the request, which is calculated based on the request's submission time and latency bound, or replaced by the leader with its clock time. \emph{log-id} is the position of the request in the leader's \emph{log}. Under high workload, multiple \emph{sync} messages can be batched into one message for space/communication efficiency, because they share the same \emph{view-id}, and \emph{log-id}s are consecutive and can represented with only two integers (i.e. $[begin, end]$).

After the followers receive the \emph{sync} message, they add/delete entries to/from their \emph{log}s to maintain set equality with the leader's \emph{log}. While adding entries, the follower first searches the missing entry from its \emph{recycle-pool}, with $<\emph{client-id}, \emph{request-id}>$ as the index. In most cases, the follower can find the request locally, and it uses the \emph{rank} value in the \emph{sync} message as the ordering rank for this request~\footnote{For those requests accepted by the leader, the $rank$ value equals $s+d$; for those rejected by the leader, the $rank$ is replaced by the leader's clock time, which is different from $s+d$ originally tagged by the client.}. When the follower fails to find the request in its \emph{recycle-pool} (probably due to packet drop), it asks the other replicas for the missing request. 

After processing the \emph{sync} message, the follower updates its \emph{sync-point}, indicating its \emph{log} is consistent with the leader up to this point. Specially, the leader itself can directly advance its \emph{sync-point} after appending the request to its \emph{log}. 

Adding/deleting log entries will change the \emph{hash} field to be included in \emph{fast-replies}. However, the incremental nature of the hash computation enables a fast update of the hash value with subtle cost.~\footnote{We use the SHA1 API in openssl library, and one SHA1 hash computation costs 0.15$\mu s$. Besides, one XOR computation between two 160-bit SHA1 strings costs 0.0087$\mu s$, so the cost of the incremental computation is negligible. }. As shown later in \S\ref{sec-fix-set-inequality} As shown in Figure~\ref{sync-demo},  followers maintain two hash values during runtime, i.e. $h_{left}$ and $h_{right}$, to encode the synced requests and unsynced requests respectively. The follower's unsynced part may include inconsistent requests causing set inequality.~\footnote{ "Inconsistent requests" refer to the requests that only exist in the leader's \emph{log}, or only exist in the follower's \emph{log}.} 
While sending the \emph{fast-reply} to the clients, followers simply XOR $h_{left}$ and $h_{right}$ to get the hash value to include in the \emph{fast-reply}. The final hash value will be inconsistent with the leader's reply if some \emph{inconsistent requests} exist in the unsynced part. However, as more and more fresh \emph{sync} messages are received from the leader replica, the followers can rapidly update $h_{left}$ and $h_{right}$ and moves \emph{sync-point} from left to right, thus eliminating the inconsistent requests and generating consistent hashes for the requests appended later.


\begin{figure}
    \centering
    \includegraphics[width=6cm]{figures/sync-demo.pdf}
    \caption{Illustration of \emph{sync-status}}
    \label{sync-demo}
    \vspace{-0.6cm}
\end{figure}

\subsection{Quorum Check of Slow Path}
\label{sec-slow-quorum-check}

For every synced request, the follower also sends a reply to the client (\circled{10} in Figure~\ref{fig-workflow-slow}). We name this type of reply as \emph{slow-reply}. The format of the \emph{slow-reply} can be described as a 3-tuple. 
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.2cm}
        \emph{slow-reply} = <\emph{view-id}, \emph{request-id},\emph{replica-id}>
\end{equation*}

Different from the \emph{fast-reply}, which can be sent immediately after appending the request, the \emph{slow-reply} can only be sent by followers after it ensures that all the previous requests have been synced with the leader up to this one. Inside the \emph{slow-reply} message, the three fields have the same meaning as in the \emph{fast-reply}. \emph{slow-reply} does not include \emph{hash}, because it is consistent with the leader for sure. \emph{slow-reply} does not include \emph{result} because it is only sent by followers, which do not execute requests. 


The client waits for reply messages related to its request with matching \emph{view-id}s and \emph{request-id}s. It considers the request as committed when it receives the \emph{fast-reply} from the leader and the \emph{slow-replies} from  $f$ followers. The client also obtains the execution result of the request from the leader's \emph{fast-reply}. 


Unlike the quorum check of the fast path (\S\ref{sec-fast-quorum-check}), the slow path does not require a super quorum ($1+f+\lceil f/2 \rceil$). Before sending the \emph{slow-replies} to the clients, the followers have updated their \emph{sync-point}s and ensures all the requests (log entries) are consistent with the leader up to the \emph{sync-point}s. A simple majority ($f+1$) is sufficient for the \emph{sync-point} to survive the crash. All requests before \emph{sync-point} are committed requests, and they are directly copied to the new leader’s \emph{log} during the recovery (\S\ref{sec:recovery}).


Specially, the \emph{slow-reply} can also serve as a \emph{fast-reply}. The request is also considered as committed when the client receives a mix set of \emph{fast-replies} and \emph{slow-replies}, including the \emph{fast-reply} from the leader, and the reply messages from the other $f+\lceil f/2 \rceil$ replicas, which are either \emph{fast-replies} with the same \emph{hash}, or \emph{slow-replies}.

On the other hand, the \emph{fast-reply} cannot serve as a \emph{slow-reply} to form the simple quorum ($f+1$) in the slow path, because \emph{slow-reply} indicates it has been synced with the leader up to the current request, and \sysname can guarantee its \emph{sync-point} survive failure. However, while the follower is sending the \emph{fast-reply}, there is no guarantee that its \emph{sync-point} has been updated in time. In other words, a simple quorum ($f+1$) of \emph{fast-replies} cannot ensure the survival of a \emph{sync-point} whose \emph{rank} is greater or equal to the \emph{rank} of the current request, so \sysname cannot guarantee the request can be recovered.

Since \sysname offloads the quorum check of both paths (fast/slow path) to clients, its leader suffers from much less bottleneck, compared with other protocols such as Fast Paxos, Speculative Paxos and NOPaxos, which still rely on the leader for the quorum check of the slow path. The thorough offloading also saves latency overheads for \sysname, because the client can know whether the request is committed even earlier than the replicas in both paths.

% \emph{sync-status} indicates whether the request has been synced with the leader. For leader replica, \emph{sync-status} is always TRUE in each reply message. For follower replicas, its \emph{sync-point} will be advanced during the index synchronization process (\S\ref{index-sync}). The \emph{sync-status} is set TRUE only if the request has been covered by the \emph{sync-point} (refer to Figure~\ref{sync-demo}). 




% \vspace{-0.4cm}
% \subsection{Index Synchronization}
% \vspace{-0.2cm}
% \label{index-sync}
% The selective acceptance avoids ordering ambiguity but may cause set inequality, if replicas take different actions (acceptance/rejection) towards the same request due to clock skewness, latency variance, etc. Therefore, \sysname conducts index synchronization process in the background to maintain set equality among replicas. 

% The leader runs a polling thread, which keeps broadcasting the \emph{sync} messages to all replicas. The format of a complete \emph{sync} message can be described as a 5-tuple. 
% \vspace{-0.2cm}
% \begin{equation*}
% \vspace{-0.2cm}
%     sync = <\emph{view-id}, \emph{client-id}, \emph{request-id}, \emph{rank}, \emph{log-id}>
% \end{equation*}

% The \emph{sync} message serves two purposes. First, it works as the heartbeat of the leader. Once failing to receive the leader's heartbeat for a threshold of time, followers enter the view change process~\cite{viewstamp} and elect a new leader (\S\ref{sec:recovery}).  
% Second, it can timely correct the set inequality, making the followers' \emph{log}s consistent with the leader's \emph{log}. 

% The \emph{sync} message has much smaller size than the \emph{request}, because it does not include the body (i.e.the \emph{command} field) of the request. Among the five fields, \emph{client-id} and \emph{request-id} combine to identify the request. \emph{rank} is the ordering rank of the request, which is calculated based on the request's submission time and latency bound, or replaced by the leader with its clock time. \emph{log-id} is the position of the request in the leader's \emph{log}. Under high workload, multiple \emph{sync} messages can be batched into one message for space/communication efficiency, because they share the same \emph{view-id}, and \emph{log-id}s are consecutive and can represented with only two integers (i.e. $[begin, end]$).

% After the followers receive the \emph{sync} message, they add/delete entries to/from their \emph{log}s to maintain set equality with the leader's \emph{log}. While adding entries, the follower first searches the missing entry from its \emph{recycle-pool}, with $<\emph{client-id}, \emph{request-id}>$ as the index. In most cases, the follower can find the request locally, and it uses the \emph{rank} value in the \emph{sync} message as the ordering rank for this request~\footnote{For those requests accepted by the leader, the $rank$ value equals $s+d$; for those rejected by the leader, the $rank$ is replaced by the leader's clock time, which is different from $s+d$ originally tagged by the client.}. When the follower fails to find the request in its \emph{recycle-pool} (probably due to packet drop), it asks the other replicas for the missing request. 

% After finishing the sync, the follower updates its \emph{sync-point}, indicating its \emph{log} is consistent with the leader up to this point. Specially, the leader itself can directly advance its \emph{sync-point} after appending the request to its \emph{log}. 

%  for every synced request, the follower also sends a \emph{slow-reply} to the corresponding client (\circled{10}). The format of the reply message can be described as a 3-tuple. 
% \vspace{-0.2cm}
% \begin{equation*}
% \vspace{-0.2cm}
%         \emph{slow-reply} = <\emph{view-id}, \emph{request-id},\emph{replica-id}>
% \end{equation*}



% \vspace{-0.4cm}
% \subsection{Quorum Check}
% \vspace{-0.2cm}
% \label{quorum-check}
% The client waits for reply messages related to its request with matching \emph{view-id}s and \emph{request-id}s. It considers the request as committed under one of the two conditions.
% \begin{itemize}[wide, labelwidth=!,nosep]
%     \item \textbf{Fast path:} The client receives the \emph{fast-reply} from the leader and the replies from $f+\lceil f/2 \rceil$ followers, which are either \emph{fast-replies} with the same hash values as the leader's reply, or \emph{slow-replies} (because the \emph{slow-reply} also indicates the follower is consistent with the leader up to the current request).
%     \item \textbf{Slow path:} The client receives the \emph{fast-reply} from the leader and the \emph{slow-replies} from $f$ followers.
% \end{itemize}

% The reason why the fast path requires a super quorum ($f+\lceil f/2 \rceil+1$) rather than a simple majority ($f+1$) is the same as in Fast Paxos and Speculative Paxos: Without leader-follower communication, a simple majority cannot provide sufficient information for the new leader to distinguish committed requests from uncommitted requests after crash. Consider what would happen if we had used a simple majority ($f+1$) in the fast path. Suppose there are two requests \emph{req-1} and \emph{req-2}, and \emph{req-1} has a larger  \emph{rank}. \emph{req-1} is accepted by the leader and $f$ followers. They send \emph{fast-replies} to the client, and then the client considers the request as committed and delivers the execution result from the leader's \emph{fast-reply} to the upper application. Meanwhile, \emph{req-2} is accepted by the other $f$ followers. After that, the leader fails, leaving $f$ followers possessing \emph{req-1} and the other $f$ followers possessing \emph{req-2}. Under such a situation, the new leader cannot tell which one is the committed request. Even worse, if the new leader involves \emph{req-2} into the recovered \emph{log}, it will be appended and executed ahead of \emph{req-1} due to the smaller \emph{rank}. Therefore, it causes inconsistent execution result for \emph{req-1}, compared with the result before the leader crash. 

% By contrast, the slow path does not require a super quorum. Before sending the \emph{slow-reply} messages to the clients, the follower replicas have updated their \emph{sync-point}s based on the index information from the leader. A simple majority is sufficient for the \emph{sync-point} to survive the crash and all requests before \emph{sync-point} are committed requests, and they are directly copied to the new leader’s \emph{log} during the recovery (details in \S\ref{sec:recovery}).

\subsection{Timeout and Retry}
\label{sec-timeout}
In addition, the client maintains a timeout threshold while waiting for \emph{fast-replies}/\emph{slow-replies}. If timeout is triggered and the client has not received enough reply messages, it retries the request with a different submission time and (possibly) a different latency bound. Meanwhile, as in traditional distributed systems, replicas maintain \emph{at-most-once} semantics. When receiving a request with duplicate \emph{<client-id, request-id>}, which have already been appended/executed, 
the replica simply resends the previous reply to the client instead of appending/executing the request for twice.


\subsection{Client-Side Knowledge}
\todo{include a subsection to discuss how client is resistant to failure: because client takes more responsibility in \sysname than in Raft, do we need auxiliary node to store quorum information for clients?}

%\vspace{-0.5cm}
\section{Recovery}
\label{sec:recovery}
\vspace{-0.2cm}
% Raft~\cite{atc14-raft} leverages stable storage and every replica needs to persist its information before sending RPCs. Therefore, the crashed replica can easily recover its state from the stable storage. However, such a protocol is unattractive since it adds significant delays (0.5ms$\sim$20ms per write) to normal processing. By contrast, viewstamped replication and Paxos have developed diskless versions~\cite{viewstamp,podc07_diskless_paxos} respectively, which does not rely on stable storage for recovery. 

%However, such protocols are later proved to be incorrect~\cite{disc17-dcr,disc17-dcr-techreport, tdsn21-recovery} due to \emph{stray messages}~\footnote{\emph{Stray messages} refer to messages that are sent out but not delivered before replica crash. The diskless recovery protocols of Paxos~\cite{podc07_diskless_paxos} and Viewstamped Replication~\cite{viewstamp} can forget \emph{stray messages} and lead to incorrect outcomes (refer to B.1 and B.2 in ~\cite{disc17-dcr-techreport}. ) }. 

When a replica crashes, it can be relaunched but needs to recover its state before it can resume the request processing. Raft~\cite{atc14-raft} leverages stable storage and every replica persists its information before sending remote procedure calls (RPCs). Once it crashes, the replica can recover its state from the stable storage for recovery. Such a protocol is unattractive since it adds significant delays (0.5ms$\sim$20ms per write) to normal processing. By contrast, Speculative Paxos and NOPaxos inherit the diskless recovery protocol from Viewstamped Replication~\cite{viewstamp}, which preserves the efficiency of normal processing but proves to be incorrect~\cite{disc17-dcr,disc17-dcr-techreport,tdsn21-recovery} due to \emph{stray messages}~\footnote{\emph{Stray messages} refer to messages that are sent out but not delivered before replica crash. Viewstamped Replication, Speculative NOPaoxs and NOPaxos cannot handle \emph{stray messages} properly and can lead to incorrect outcomes.}. We include an error trace of NOPaxos recovery to illustrate this in Appendix~\ref{error-trace-nopaxos}.



\sysname also adopts diskless recovery for the sake of efficiency in the normal process, but different from Speculative Paxos and NOPaxos, \sysname avoids the effect of \emph{stray messages} by means of \emph{crash vector}~\cite{disc17-dcr, disc17-dcr-techreport}. \emph{crash-vector} is a vector containing $2f+1$ integer counters corresponding to the $2f+1$ replicas. Each replica maintains such a vector, with all counters initialized as 0s. \emph{crash-vector}s can be aggregated by taking the max operation element-wisely. During the view change process, replicas communicate with each other with their \emph{crash-vector}s tagged in the messages. Receivers can make their \emph{crash-vector}s more up-to-date by aggregating it with the \emph{crash-vector} from the sender. 

The key idea of \emph{crash-vector} is that, it enables the replicas to recognize potential \emph{stray messages} by comparing the \emph{crash-vector} tagged in the message with its local one.
During the recovery, the \textsc{recovering} replica first recovers its \emph{crash-vector} by collecting and aggregating the \emph{crash-vector}s from a majority of \textsc{normal} replicas. Then, the replica increments its own counter (i.e. replica $i$ increments the $ith$ counter in the vector) and tags the new \emph{crash-vector} to the messages sent afterwards. Once the update of \emph{crash-vector} is exposed to the other replicas, they can recognize the \emph{stray messages} sent by the replica before crash (i.e. those messages have a smaller value at the $ith$ counter), and avoid processing those messages. In this way, the recovery will not be affected by \emph{stray messages} (refer to~\cite{disc17-dcr-techreport} for detailed description of \emph{crash-vector}). 


% While replicas communicate with each other, the sender tags its \emph{crash-vector} to the message and the receiver can

% Since each counter is self-incremented, replicas can recognize the potential \emph{stray message} by comparing its local \emph{crash-vector} and the one included in the message (refer to).


Generally speaking, the recovery of \sysname consists of two main components, i.e. replica rejoin and leader change. We include the algorithms for each in Appendix~\ref{recovery-algo} and more details can also be found in the TLA+ specification ( Appendix~{\color{green} G}). In the following subsections, we sketch the major steps for each component.

    
    % Before a relaunched replica rejoins the system, it is required to contact the other \textsc{normal} replicas to update its crash vector, and notify the majority of replicas of its crash vector, so that the majority can avoid the misleading effect from the \emph{stray messages} sent by this replica.  
% \textbf{Leader change.} When the followers suspect the leader has failed (e.g. the follower has not heard the heartbeat from the leader for a threshold of time), they will initiates a view change and elect a new leader.  



\subsection{Replica Rejoin}

After a replica crashes and is relaunched, it can rejoin the system as a follower. The replica sets its \emph{status} as \textsc{recovering}, and the rejoin consists of two main steps.


\begin{enumerate}[wide, labelwidth=!,nosep,label=\textbf{Step \arabic*:}]
\item \textbf{Update \emph{crash-vector}}.
 The \textsc{recovering} replica inquires the majority of \textsc{normal} replicas of their \emph{crash-vector}s, and aggregates them. It increments its own counter in the aggregated \emph{crash-vector}, and then notifies the other replicas by broadcasting \textsc{recovery-req} messages. Once the other replicas receive the \textsc{recovery-req} message, they can update their local \emph{crash-vector} by aggregating it with the one included in the \textsc{recovery-req} message. After that, they can recognize and avoid processing the \emph{stray messages} from the recovering replica.
 
\item \textbf{Recover state} The \textsc{normal} replicas send \textsc{recovery-rep} messages in response to the \textsc{recovery-req} messages from the \textsc{recovering} replica. Replicas include their current \emph{view-id}s in the \textsc{recovery-rep} message. The \textsc{recovering} replica picks the  highest \emph{view-id} among the $f+1$ \textsc{recovery-rep} messages and calculates the \emph{replica-id} of the leader ($\emph{highest-view}\% (2f+1)$). Then it contacts the leader to recover its state, including \emph{crash-vector}, \emph{view-id}, \emph{log} and \emph{sync-point}. After the state is recovered, the replica switches its \emph{status} from \textsc{recovering} to \textsc{normal}, and works as a \textsc{normal} follower. 
\end{enumerate}

Specially, the \textsc{recovering} replica(s) do not participate into the view change process (\S\ref{sec-leader-change}). When the majority of replicas are conducting the view change (possibly due to leader failure), the \textsc{recovering} replica(s) just wait until the majority completes the view change and elects the new leader. The algorithm is described as Algorithm~\ref{algo-replica-rejoin} in Appendix~\ref{recovery-algo}.
 

% Then it contacts the majority ($f+1$) of replicas to collect their \emph{crash-vector}s. \emph{crash-vector} is a vector containing $2f+1$ integer counters corresponding to the $2f+1$ replica. \emph{crash-vector}s can be aggregated by taking \texttt{max} operations in a element-wise way (refer to XX). 



\subsection{Leader Change}
\label{sec-leader-change}
% When the follower crashes, \sysname simply relaunches it. But before processing new requests, the follower needs to completely copy the \emph{log} from the leader.


% When the leader crashes, the followers enter the view change process to recover the system state. During the process, replicas do not process new client requests. Instead, they perform the following steps to elect a new leader and resume request processing.

If the follower(s) fail to hear from the leader for a threshold of time, the followers will suspect the leader has failed and stop processing client requests. Then, a view change process will be initiated to elect a new leader. The view change process consists of three main steps.

\begin{enumerate}[wide, labelwidth=!,nosep,label=\textbf{Step \arabic*:}]
\item \textbf{Broadcast view change request.} The follower switches its \emph{status} from \textsc{normal} to \textsc{viewchange}. Then it increments its \emph{view-id} and broadcasts \textsc{view-change-req} messages to all replicas, notifying them of the view change. After receiving the \textsc{view-change-req} message, \textsc{normal} replicas also participate into the view change process by switching to \textsc{viewchange} \emph{status} and incrementing their \emph{view-id}s. 

\item \textbf{Rebuild leader's $\textbf{log}$.} During the view change process, replicas can calculate the \emph{replica-id} of the leader in the new view (i.e. $\emph{view-id} \% (2f+1)$), and they 
send \textsc{view-change} messages to the new leader, including their \emph{log}s and \emph{sync-point}s.
The leader can build its state after collecting \textsc{view-change} messages from $f+1$ replicas with matching \emph{view-id}s. It aggregates \emph{log}s to ensure all the previously committed \emph{log} entries survive. To attain this, the aggregation involves two key sub-steps. 
\begin{enumerate}[wide, labelwidth=!,nosep,label={(\arabic*)}]
    \item It chooses the largest \emph{sync-point} from \emph{the most recent view} in which the replicas have \textsc{normal} \emph{status}. Then the leader directly copies all the \emph{log} entries up to the \emph{sync-point} from the corresponding replica. 
    \item For those \emph{log} entries after the \emph{sync-point},~\footnote{The \emph{rank} of the \emph{log} entry is larger than that of the \emph{sync-point}.} the replica checks whether this entry exists on $\lceil f/2 \rceil +1$ out of the $f+1$ replicas. If so, the entry will also be added to the leader's \emph{log}. All the entries added to the leader's \emph{log} are sorted by their \emph{rank}s.
\end{enumerate}



\item \textbf{Start new view.} After the leader rebuilds its \emph{log}, it executes the \emph{log} entries following their \emph{rank} order and switches its \emph{status} back to \textsc{normal}. Meanwhile, the leader broadcasts \textsc{start-view} messages to followers, including its \emph{log}. Once receiving the \textsc{start-view} messages, followers replace their \emph{log}s with the leader's \emph{log}, and update their \emph{sync-point}s. Then, followers also switch \emph{status}es back to \textsc{normal}. Finally, all replicas enter the new view and the system is fully recovered.

\end{enumerate}

During the view change process, messages (\textsc{view-change-req}, \textsc{view-change} and \textsc{start-view}) will be repeatedly transmitted in case of packet drop. Besides, the senders include their \emph{crash-vector}s in the messages, so that the receivers can recognize \emph{stray messages} by comparing the sender's \emph{crash-vector} with their local one.

Note that the view change protocol chooses the leader in a round-robin way ($\emph{view-id} \% (2f+1)$). Specially, a view change process may not succeed because the new leader also fails (as mentioned in~\cite{viewstamp}). In this case (i.e. after followers have spent a threshold of time without completing the view change), followers will continue to increment their \emph{view-id}s to initiate a further view change, with yet another leader. The algorithm is described as Algorithm~\ref{algo-leader-change} in Appendix~\ref{recovery-algo}


\vspace{-0.4cm}
\subsection{Correctness}
\label{sec-correctness}
\vspace{-0.2cm}
% With the normal behavior described in \S\ref{selective-acceptance}$\sim$\S\ref{quorum-check},
We can prove that the recovery procedure in \S\ref{sec:recovery} guarantees the following correctness properties. We include the correctness proof in Appendix~\ref{append-correctness}. We also include a TLA+ specification of \sysname protocol in Appendix~{\color{green} G}.

\begin{itemize}[wide, labelwidth=!,nosep]
    \item \textbf{Durability:} if a client considers a request as committed, the request survives replica crashes.
    \item \textbf{Consistency:} if a client considers a request as committed, the execution result remains consistent after the replica's crash and recovery.
    \item \textbf{Linearizability:} A request appears to be executed exactly once between start and completion.
\end{itemize}

    
    % The recovered log entries will be executed in the same order, thus providing consistent execution result for $req$.
    
% Taking an arbitrary committed request $req$. If $req$ has been synced before leader crash, then $req$ and all the previous entries will be unchanged and directly copied to the new leader. Therefore, the execution result of $req$ remains unchanged. 

% Otherwise, $req$ has not been synced before leader crash. Based on the proof of durability, we know that every committed requests can survive. Besides, the leader executes the requests (log entries) based on their ordering ranks. Therefore, the execution order of committed requests will remain the same after crash and recovery (If $req_1$ is executed ahead of $req_2$ before crash, then after recovery, $req_1$ is still executed ahead of $req_2$).  

% Then we only need to exclude one risky case: is it possible for an \textbf{uncommitted} request $req'$, which is executed ahead of $req$ on the old leader, but lost after the recovery? 

% \textbf{Corollary:} \texttt{If there exists an uncommitted request $req'$, $req'$ is appended to replica's $logSet$ before $req$, then $req'$ can only exist in at most $\lceil f/2 \rceil$ replicas.} 

% We can prove this by contradiction. 

% Suppose $req'$ exists in more than $\lceil f/2 \rceil$ replicas but it is not committed (less than $1+f+\lceil f/2 \rceil$ replicas contain $req'$). Since $req'$'s position appears before $req$, i.e. The computation of the hash value for $req$ is based on all the previous requests, including $req'$. Therefore, the hash values replied by the replicas with $req'$ differs from the hash value replied by replicas without $req$. Since there are more than $\lceil f/2 \rceil$  but less than $1+f+\lceil f/2 \rceil$ replicas containing $req'$, Among the $1+f+\lceil f/2 \rceil$ replies for $req$, some replicas will contain $req'$ whereas others not. Therefore, they cannot reply with the same hash value, and $req$ cannot be successful. Contradiction!

% Therefore, it is impossible for such a request $req'$ to exist on more than $\lceil f/2 \rceil$ replicas. Therefore, $req'$ cannot appear in the recovered $logSet$. Therefore, only committed requests survive before $req$, so the consistency is guaranteed. 


% The existence of ordering ranks insider each request eliminates the ordering ambiguity during execution. For any two committed requests, denoted $req_1$ and $req_2$. If $req_1$ is executed before $req_2$, then it means $req_1$ has a smaller ordering rank than $req_2$. Based on the durability property, the two committed requests can both survive crash. Since the ordering rank is an affiliated attributes of the request, the ordering ranks of the two requests also survives the crash. Therefore, the new leader also follows the same execution order to execute the two requests and no contrary observation can occur after recovery. 










==> old/formulation-old-1124-2.tex <==
\clearpage
\onecolumn
\section{Formulation}
\subsection{Notation}
\begin{itemize}
    % \item Clients: $C_1, C_2,\dots$
    \item Replicas: $R_1, R_2,\dots$  (Leader is $R_L$)
    \item Messages: $M_1, M_2, \dots$
    % \item $t(M_i, C_j)$:  the departure time of $M_i$ from $C_j$ 
    \item $t(M_i, R_k)$:  the arrival time of  $M_i$ at $R_k$
    \item $e(M_i,R_k)$: the execution/appending time of $M_i$ at $R_k$
    \item $S(M_i)$: the sequential number of $M_i$ given by Sequencer.(OUM Oracle Information). 
    %$S(M_i)$ is visible to replicas, but becomes immutable once it is visible.
    \item $D(M_i)$: the \textbf{planned} execution time of $M_i$ at all replicas. (ORM Oracle Information). %$D(M_i)$ is visible to all replicas, and it is mutable.
    
    % \item $OWD(R_i, R_j)$: The one-way delay from $R_i$ to $R_j$.
    \item  $A(M_i)$: the arrival time of $M_i$ at the oracle (OUM Oracle and ORM Oracle Information). %$A(M_i)$ is invisible to replicas.
    
\end{itemize}

In OUM, $S(M_i)$ has casual relation to $A(M_i)$, i.e. the value of $S(M_i)$ is decided only after $A(M_i)$ is decided. 

In ORM, the value of $D(M_i)$ can be decided without $A(M_i)$ but $D(M_i)$ can be rectified after $A(M_i)$ is decided. 

\subsection{Definition}
\begin{itemize}
    % \item Reordering: $M_1$ and $M2$ are reordered towards $R_x$ iff $t(M_{1}, C_i)<t(M_{2},C_j)$ and $t(M_1,R_x)>t(M_2,R_x)$ ($i$ and $j$ can be the same or different)
    \item Packet drop: $M_i$ is lost to $R_x$ if $t(M_i, R_x)=\infty$
    \item Order ambiguity: $R_1$ and $R_2$ are \emph{order-ambiguous} (denoted as $OA(R_1,R_2,M_1,M_2)$) regarding $M_1$ and $M_2$ if:
    \begin{itemize}
        \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
        \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
    \end{itemize}
    
    
    \item Set inequality: $R_1$ and $R_2$ are \emph{set-inequal} regarding $M_1$ (denoted as $SI(R_1,R_2, M_1)$) if
    \begin{itemize}
        \item $e(M_1, R_1)=\infty$ and $e(M_1, R_2)< \infty$
        \item Or $e(M_1, R_1)< \infty$ and $e(M_1, R_2)= \infty$
    \end{itemize}
    
    \item Consistency: $R_1$ and $R_2$ are consistent if
    \begin{equation*}
        \forall M_i,M_j: 
  \neg OA(R_1,R_2,M_i,M_j) \And \neg SI(R_1,R_2,M_i) \And  \neg SI(R_1,R_2,M_j)
    \end{equation*}
    
\end{itemize}
    
    
%     % For $e(M_1, R_1),e(M_1, R_2), e(M_2, R_1), e(M_2, R_2) < \infty$
%     \begin{itemize}
%         \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
%         \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
%     \end{itemize}
%     Inconsistency = order ambiguity or set inequality.

% By taking packet drop as a special case of packet reordering, inconsistency=order ambiguity.

%     \item $S(M_1)$ and $S(M_2)$ become visible to replicas only after $A(M_1)$ and $A(M_2)$ are known to OUM Oracle. $S(M_1)$ and $S(M_2)$ are immutable once visible to replicas.
%     \item $D(M_1)$ and $D(M_2)$ are already visible even when $A(M_1)$ and $A(M_2)$ have not been known to BORM Oracle. $D(M_1)$ and $D(M_2)$ are mutable by Oracle even after they are visible to replicas.
% \end{itemize}



\section{Primitive Actions}

\subsection{MOM}
% $$e(M_1, R_1)=t(M_1,R_1)$$
% $$e(M_2, R_1)=t(M_2,R_1)$$
% $$e(M_1, R_2)=t(M_1,R_2)$$
% $$e(M_2, R_2)=t(M_2,R_2)$$
\begin{equation*}
    \forall M_i \forall R_x:\qquad e(M_i, R_x) = t(M_i, R_x)
\end{equation*}
$e(*,*)$ is completely determined by $t(*,*)$, and \textbf{MOM} just takes best effort to make $e(*,*)$ satisfy the consistency condition. 

% takes no remedies to inconsistency (just best effort). 
%If it happens, the majority order eventually wins. Others roll back.

% MOM does not modify $e(*,*)$ but OUM and BOM can modify $e(*,*)$ based on their Oracle information.


MOM has no Oracle to provide information for replicas to fix inconsistency, whereas OUM/ORM has Oracle to provide information for replicas to fix inconsistency.

\textbf{OUM's Oracle information can cause false positives whereas ORM's Oracle information can cause false negatives.}
\begin{itemize}
    \item OUM's Oracle information can cause false positives:  in fact there is no inconsistency, but Oracle information still indicates there is inconsistency.
    \item ORM's Oracle information can cause false negative: Replicas believe $D(*)$ is correct and follow the guidance of $D(*)$, but later Oracle modifies $D(*)$ and claims the original $D(*)$ incorrect, i.e. the \emph{used-to-be-correct} consistency finally proves to be inconsistency.) 
\end{itemize}







% MOM has no Oracle to provide information for replicas, so replicas have no idea on fixing inconsistency;
% OUM Oracle provides information for replicas to completely 
% % \textbf{OUM and BORM}: decides a definite order based on their Oracle information.

\subsection{OUM}


Without loss of generality, assume $A(M_1)<A(M_2)$, \textbf{After $A(M_1)$ and $A(M_2)$ are known to Oracle},  
the OUM Oracle gives $S(M_1)<S(M_2)$.

For simplification, only consider $S(M_2)=S(M_1)+1$. It can be generalized to non-consecutive cases $(M_2)=S(M_1)+k$ (with more complexity).



\begin{itemize}
    \item Case 1: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then 
    \begin{equation*}
    \begin{split}
        &e(M_1,R_1)=t(M_1,R_1)\qquad\texttt{Normal}\\
        &e(M_2,R_1)=t(M_2,R_1)\qquad\texttt{Normal}\\
        &e(M_1,R_2)=t(M_1,R_2)\qquad\texttt{Normal}\\
        &e(M_2,R_2)=t(M_2,R_2)\qquad\texttt{Normal}
    \end{split}
    \end{equation*}
    
    \item Case 2: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then
    \begin{equation*}
    \begin{split}
    &e(M_1,R_1)=t(M_1,R_1)\qquad\texttt{Normal}\\
    &e(M_2,R_1)=t(M_2,R_1)\qquad\texttt{Normal}\\
    &e(M_1,R_2)= 
    \begin{cases}
      %\min\{t(M_2,R_2)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or from $R_2$ itself} \\
      \infty, & \text{otherwise (no replicas have $M_1$) }
    \end{cases}\\
    &\texttt{$R_2$ can only execute $M_1$ after obtaining $M_1$, either from others or itself.}\\
    &\texttt{$\Phi$ is the time cost to fetch $M_1$ from others, i.e.} \\
    &\texttt{After $\Phi$, $R_2$ gets either $M_1$ or NOOP}\\
    &e(M_2,R_2)=
    \begin{cases}
      % e(M_1,R_2)+\Delta, & \text{If $e(M_1,R_2)<\infty$, i.e. $M_1$ is recovered and executed}\\      
      t(M_2,R_2)+\Phi, & \text{Otherwise, $R_2$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
    \end{cases}\\
    \end{split}
    \end{equation*}
    \item Case 3: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)= 
    \begin{cases}
      % \min\{t(M_2,R_1)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_1$ itself} \\
      \infty, & \text{otherwise (no replicas have $M_1$) }
    \end{cases}\\
    &e(M_2,R_1)=
    \begin{cases}
      % e(M_1,R_1)+\Delta, & \text{if } e(M_1,R_1)<\infty, \text{i.e. $M_1$ is recovered} \\      
      t(M_2,R_1)+\Phi, & \text{Otherwise, and $R_1$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
    \end{cases}\\
    &e(M_1,R_2)=t(M_1,R_2)\qquad\texttt{Normal}\\
    &e(M_2,R_2)=t(M_2,R_2)\qquad\texttt{Normal}
    \end{split}
\end{equation*}
    
\item Case 4: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)= 
    \begin{cases}
      % \min\{t(M_2,R_1)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_1$ itself } \\
      \infty, & \text{otherwise (no replicas have $M_1$) }
    \end{cases}\\
    &e(M_2,R_1)=
    \begin{cases}
      % e(M_1,R_1)+\Delta, & \text{if } e(M_1,R_1)<\infty, \text{i.e. $M_1$ is recovered} \\      
      t(M_2,R_2)+\Phi, & \text{Otherwise, $R_1$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
    \end{cases}\\
    &e(M_1,R_2)= 
    \begin{cases}
      % \min\{t(M_2,R_2)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_2$ itself } \\
      \infty, & \text{otherwise (no replicas have $M_1$) }
    \end{cases}\\
    &e(M_2,R_2)=
    \begin{cases}
      % e(M_1,R_2)+\Delta, & \text{if } e(M_1,R_2)<\infty, \text{i.e. $M_1$ is recovered} \\      
      t(M_2,R_2)+\Phi, & \text{Otherwise, $R_2$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
    \end{cases}
    \end{split}
\end{equation*}
\end{itemize}



% Note: Case 2 and Case 3 have already considered Jialin's optimization (i.e. first try to recover the gap by asking the others, instead of immediately starting gap agreement). 

\subsection{ORM}
Without loss of generality, assume $D(M_1)<D(M_2)$ (i.e. Oracle plans to execute $M_1$ before $M_2$). Later $A(M_1)$ and $A(M_2)$ are known to Oracle. 
\begin{itemize}
    \item If $A(M_1)<D(M_2)$, no change to $D(M_1)$ and $D(M_2)$
    \item Otherwise, $D(M_1)=A(M_1)$
\end{itemize}

\begin{equation*}
\forall M_i \forall R_x:\qquad
    e(M_i, R_x)=\max\{D(M_i), \min\{t(M_i,R_x), D(M_i)+\lambda \} \}
\end{equation*}


To execute $M_i$, the max indicates two necessary conditions 
\begin{itemize}
    \item The time reaches the deadline $D(M_i)$
    \item $M_i$ is obtained by $R_x$, which costs $\min\{t(M_i,R_x), A(M_i)+\lambda \}$, the min indicates two alternative options (satisfying one is fine):
    \begin{itemize}
        \item $M_i$ is received by $R_x$ (at $t(M_i, R_x)$)
        \item $M_i$ has been appended by Oracle, and it takes $\lambda$ time cost for $R_x$ to get it.
    \end{itemize}
\end{itemize}



% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_1)\\=&\max\{
%         D(M_1), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_1), 
%         \\&\qquad\qquad A(M_1)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}

% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{
%         D(M_2), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad A(M_2)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}


% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_1)+\Delta,
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad OWD(R_1, R_2)+t(M_2,R_2)+OWD(R_2,R_1), \\ 
%         &\qquad\qquad OWD(R_1, Oracle)+A(M_2)+OWD(Oracle,R_1)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_2)\\=&\max\{ D(M_1),
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_2),
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_1,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_1)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_2)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_2)+\Delta,
%         \\&\qquad \min\{
%         \\&\qquad\qquad t(M_2,R_2), 
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_2,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_2)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}




\subsection{Oracle State}
Both OUM Oracle and ORM Oracle have their own states. After failure, the new OUM Oracle and ORM Oracle need to recover their states before serving the system.

\begin{enumerate}
    \item The new OUM Oracle needs to remember the largest $S(M_i)$ that has been output by the old Oracle. The new OUM oracle can only start with a value larger than that.
    \item The new ORM Oracle needs to remember the largest $D(M_i)$ that has been output by the old Oracle.The new ORM oracle can only start with a value larger than that. 
\end{enumerate}

Mapped to the implementation, 
\begin{enumerate}
    \item NOPaxos relies on the SDN controller to provide an incremented session number for every new OUM Oracle, $S(M_i)=(sessNum, msgNum)$. We say $S(M_i)<S(M_j)$ iff ($S(M_i),sessNum<S(M_j).sessNum$) or ($S(M_i).sessNum=S(M_j).sessNum\And S(M_i).msgNum<S(M_j).msgNum$) 
    
    \textbf{But how to guarantee the SDN controller always output an monotonous session number (Considering the SDN can also fail, how should SDN remember the session number it has output before crash)? The paper does not say that.} 
    
    Possible methods: Maybe SDN controller writes the session number to stable storage every time before using it; Maybe SDN controller commits its session number to another Paxos/Raft system before using it.
    
    {\color{red} In one word, NOPaxos is not self-sufficient.}
    
    \item {\color{red} Nezha is a self-sufficient system.}
    Nezha puts the leader as the ORM Oracle. Whenever the old leader (Oracle) fails and the new leader (Oracle) is established, it recovers the logs (state) first. The leader (Oracle) gets the largest $D(M_i)$ by checking the last log entry in the recovered logs. And the new leader (Oracle) will start with a larger $D$ value than $D(M_i)$.
\end{enumerate}








==> old/formulation-old-1124-3.tex <==
\clearpage
\onecolumn
\section{Formulation}
\subsection{Notation}
\begin{itemize}
    % \item Clients: $C_1, C_2,\dots$
    \item Replicas: $R_1, R_2,\dots$  (Leader is $R_L$)
    \item Messages: $M_1, M_2, \dots$
    % \item $t(M_i, C_j)$:  the departure time of $M_i$ from $C_j$ 
    \item $t(M_i, R_k)$:  the arrival time of  $M_i$ at $R_k$
    \item $e(M_i,R_k)$: the execution/appending time of $M_i$ at $R_k$
    \item $S(M_i)$: the sequential number of $M_i$ given by Sequencer.(OUM Oracle Information). 
    %$S(M_i)$ is visible to replicas, but becomes immutable once it is visible.
    \item $D(M_i)$: the \textbf{planned} execution time of $M_i$ at all replicas. (ORM Oracle Information).ORM Oracle broadcasts $M_i$ to all replicas after $D(M_i)$ in case some replicas are missing that. %$D(M_i)$ is visible to all replicas, and it is mutable.
    
    % \item $OWD(R_i, R_j)$: The one-way delay from $R_i$ to $R_j$.
    \item  $A(M_i)$: the arrival time of $M_i$ at the oracle (OUM Oracle and ORM Oracle Information). %$A(M_i)$ is invisible to replicas.
    
\end{itemize}

In OUM, $S(M_i)$ has casual relation to $A(M_i)$, i.e. the value of $S(M_i)$ is decided only after $A(M_i)$ is decided. Every time OUM Oracle releases a $S(*)$, it must be larger than all previous $S(*)$ values (monotonous requirement).

In ORM, the value of $D(M_i)$ can be decided without $A(M_i)$ but $D(M_i)$ can be rectified after $A(M_i)$ is decided. Every time ORM Oracle releases a $D(*)$, it must be larger than all previous $D(*)$ values (monotonous requirement).

\subsection{Definition}
\begin{itemize}
    % \item Reordering: $M_1$ and $M2$ are reordered towards $R_x$ iff $t(M_{1}, C_i)<t(M_{2},C_j)$ and $t(M_1,R_x)>t(M_2,R_x)$ ($i$ and $j$ can be the same or different)
    \item Packet drop: $M_i$ is lost to $R_x$ if $t(M_i, R_x)=\infty$
    \item Order ambiguity: $R_1$ and $R_2$ are \emph{order-ambiguous} (denoted as $OA(R_1,R_2,M_1,M_2)$) regarding $M_1$ and $M_2$ if:
    \begin{itemize}
        \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
        \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
    \end{itemize}
    
    
    \item Set inequality: $R_1$ and $R_2$ are \emph{set-inequal} regarding $M_1$ (denoted as $SI(R_1,R_2, M_1)$) if
    \begin{itemize}
        \item $e(M_1, R_1)=\infty$ and $e(M_1, R_2)< \infty$
        \item Or $e(M_1, R_1)< \infty$ and $e(M_1, R_2)= \infty$
    \end{itemize}
    
    \item Consistency: $R_1$ and $R_2$ are consistent if
    \begin{equation*}
        \forall M_i,M_j: 
  \neg OA(R_1,R_2,M_i,M_j) \And \neg SI(R_1,R_2,M_i) \And  \neg SI(R_1,R_2,M_j)
    \end{equation*}
    
\end{itemize}
    
    
%     % For $e(M_1, R_1),e(M_1, R_2), e(M_2, R_1), e(M_2, R_2) < \infty$
%     \begin{itemize}
%         \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
%         \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
%     \end{itemize}
%     Inconsistency = order ambiguity or set inequality.

% By taking packet drop as a special case of packet reordering, inconsistency=order ambiguity.

%     \item $S(M_1)$ and $S(M_2)$ become visible to replicas only after $A(M_1)$ and $A(M_2)$ are known to OUM Oracle. $S(M_1)$ and $S(M_2)$ are immutable once visible to replicas.
%     \item $D(M_1)$ and $D(M_2)$ are already visible even when $A(M_1)$ and $A(M_2)$ have not been known to BORM Oracle. $D(M_1)$ and $D(M_2)$ are mutable by Oracle even after they are visible to replicas.
% \end{itemize}



\section{Primitive Actions}

\subsection{MOM}
% $$e(M_1, R_1)=t(M_1,R_1)$$
% $$e(M_2, R_1)=t(M_2,R_1)$$
% $$e(M_1, R_2)=t(M_1,R_2)$$
% $$e(M_2, R_2)=t(M_2,R_2)$$
\begin{equation*}
    \forall M_i \forall R_x:\qquad e(M_i, R_x) = t(M_i, R_x)
\end{equation*}
$e(*,*)$ is completely determined by $t(*,*)$.
%and \textbf{MOM} just takes best effort to make $e(*,*)$ satisfy the consistency condition. 

% takes no remedies to inconsistency (just best effort). 
%If it happens, the majority order eventually wins. Others roll back.

% MOM does not modify $e(*,*)$ but OUM and BOM can modify $e(*,*)$ based on their Oracle information.


%MOM has no Oracle to provide information for replicas to fix inconsistency, whereas OUM/ORM has Oracle to provide information for replicas to fix inconsistency.

% \textbf{OUM's Oracle information can cause false positives whereas ORM's Oracle information can cause false negatives.}
% \begin{itemize}
%     \item OUM's Oracle information can cause false positives:  in fact there is no inconsistency, but Oracle information still indicates there is inconsistency.
%     \item ORM's Oracle information can cause false negative: Replicas believe $D(*)$ is correct and follow the guidance of $D(*)$, but later Oracle modifies $D(*)$ and claims the original $D(*)$ incorrect, i.e. the \emph{used-to-be-correct} consistency finally proves to be inconsistency.) 
% \end{itemize}







% MOM has no Oracle to provide information for replicas, so replicas have no idea on fixing inconsistency;
% OUM Oracle provides information for replicas to completely 
% % \textbf{OUM and BORM}: decides a definite order based on their Oracle information.

\subsection{OUM}


Without loss of generality, assume $A(M_1)<A(M_2)$, \textbf{After $A(M_1)$ and $A(M_2)$ are known to Oracle},  
the OUM Oracle gives $S(M_1)<S(M_2)$.

For simplification, only consider $S(M_2)=S(M_1)+1$. It can be generalized to non-consecutive cases $S(M_2)=S(M_1)+k$ (with more complexity).


\begin{equation*}
    \begin{split}
    &\forall R_x:\\
    &e(M_1,R_x)=
    \begin{cases}
      t(M_1,R_x), & \text{if  $t(M_1,R_x)<t(M_2,R_x)$} \qquad \texttt{Normal}\\
      t(M_2,R_x)+\Phi, & \text{else if $t(M_1,R_x)>t(M_2,R_x)$, but fetch $M_1$ successfully from the others}\\
      \infty, & \text{Otherwise} \qquad \texttt{NOOP}
    \end{cases}\\
    & e(M_2,R_x)=
    \begin{cases}
      t(M_2,R_x), & \text{if  $t(M_1,R_x)<t(M_2,R_x)$}  \qquad \texttt{Normal} \\
      t(M_2,R_x)+\Phi, & \text{Otherwise (After  $M_1$ is fetched or knowing it is NOOP, $R_x$ can execute $M_2$ after $M_1$)\footnotemark} 
    \end{cases}\\
    \end{split}
\end{equation*}
\footnotetext{We assume the execution does not cause time, so If $M_1$ is recovered and executed at $t(M_2,R_x)+\Phi$, then $M_2$ is executed immediately after that, which is also executed at $t(M_2,R_x)+\Phi$. }


Mapped to NOPaxos implementation, 
\begin{itemize}
    \item $\Phi$ is 1 RTT: As for the leader, it sends gap agreement requests and collect $f$ replies. As for the follower, it sends gap request, and receives either the request or NOOP from the leader. 
    \item  Logs are sorted by $S(*)$, so Oracle should release $S(*)$ in a monotonously-increasing way. Otherwise, small $S(*)$ could be appended after larger $S(*)$. When failure happens, the recovered logs have different order. In NOPaxos, $S(*)$ is generated by the sequencer. The monotonous property is preserved when the sequencer does not fail. It requires extra fault tolerant mechanism (i.e. stable storage or another Raft/Paxos system) to preserve monotonous property when the sequencer fails and relaunches.
\end{itemize}
 

% \begin{itemize}
%     \item Case 1: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then 
%     \begin{equation*}
%     \begin{split}
%         &e(M_1,R_1)=t(M_1,R_1)\qquad\texttt{Normal}\\
%         &e(M_2,R_1)=t(M_2,R_1)\qquad\texttt{Normal}\\
%         &e(M_1,R_2)=t(M_1,R_2)\qquad\texttt{Normal}\\
%         &e(M_2,R_2)=t(M_2,R_2)\qquad\texttt{Normal}
%     \end{split}
%     \end{equation*}
    
%     \item Case 2: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then
%     \begin{equation*}
%     \begin{split}
%     &e(M_1,R_1)=t(M_1,R_1)\qquad\texttt{Normal}\\
%     &e(M_2,R_1)=t(M_2,R_1)\qquad\texttt{Normal}\\
%     &e(M_1,R_2)= \infty \qquad \texttt{NOOP} \\
%     % \begin{cases}
%     %   %\min\{t(M_2,R_2)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or from $R_2$ itself} \\
%     %   \infty, & \text{otherwise (no replicas have $M_1$) }
%     % \end{cases}\\
%     % &\texttt{$R_2$ can only execute $M_1$ after obtaining $M_1$, either from others or itself.}\\
%     % &\texttt{$\Phi$ is the time cost to fetch $M_1$ from others, i.e.} \\
%     % &\texttt{After $\Phi$, $R_2$ gets either $M_1$ or NOOP}\\
%     &e(M_2,R_2)=t(M_2,R_2)+\Phi 
%     \qquad\texttt{After $t(M_2,R_2)+\phi$, $R_2$ knows that $M_1$ is NOOP}
%     % \begin{cases}
%     %   % e(M_1,R_2)+\Delta, & \text{If $e(M_1,R_2)<\infty$, i.e. $M_1$ is recovered and executed}\\      
%     %   t(M_2,R_2)+\Phi, & \text{Otherwise, $R_2$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
%     % \end{cases}\\
%     \end{split}
%     \end{equation*}
%     \item Case 3: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then
% \begin{equation*}
%     \begin{split}
%     &e(M_1,R_1)= 
%     \begin{cases}
%       % \min\{t(M_2,R_1)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_1$ itself} \\
%       \infty, & \text{otherwise (no replicas have $M_1$) }
%     \end{cases}\\
%     &e(M_2,R_1)=
%     \begin{cases}
%       % e(M_1,R_1)+\Delta, & \text{if } e(M_1,R_1)<\infty, \text{i.e. $M_1$ is recovered} \\      
%       t(M_2,R_1)+\Phi, & \text{Otherwise, and $R_1$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
%     \end{cases}\\
%     &e(M_1,R_2)=t(M_1,R_2)\qquad\texttt{Normal}\\
%     &e(M_2,R_2)=t(M_2,R_2)\qquad\texttt{Normal}
%     \end{split}
% \end{equation*}
    
% \item Case 4: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then
% \begin{equation*}
%     \begin{split}
%     &e(M_1,R_1)= 
%     \begin{cases}
%       % \min\{t(M_2,R_1)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_1$ itself } \\
%       \infty, & \text{otherwise (no replicas have $M_1$) }
%     \end{cases}\\
%     &e(M_2,R_1)=
%     \begin{cases}
%       % e(M_1,R_1)+\Delta, & \text{if } e(M_1,R_1)<\infty, \text{i.e. $M_1$ is recovered} \\      
%       t(M_2,R_2)+\Phi, & \text{Otherwise, $R_1$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
%     \end{cases}\\
%     &e(M_1,R_2)= 
%     \begin{cases}
%       % \min\{t(M_2,R_2)+\Phi, t(M_1,R_2)\}, & \text{if $M_1$ can be obtained, either from others or $R_2$ itself } \\
%       \infty, & \text{otherwise (no replicas have $M_1$) }
%     \end{cases}\\
%     &e(M_2,R_2)=
%     \begin{cases}
%       % e(M_1,R_2)+\Delta, & \text{if } e(M_1,R_2)<\infty, \text{i.e. $M_1$ is recovered} \\      
%       t(M_2,R_2)+\Phi, & \text{Otherwise, $R_2$ knows $M_1$ cannot be recovered at $t(M_2,R_2)+\Phi$, and continues to execute $M_2$}
%     \end{cases}
%     \end{split}
% \end{equation*}
% \end{itemize}



% Note: Case 2 and Case 3 have already considered Jialin's optimization (i.e. first try to recover the gap by asking the others, instead of immediately starting gap agreement). 

\subsection{ORM}
Without loss of generality, assume $D(M_1)<D(M_2)$ (i.e. Oracle plans to execute $M_1$ before $M_2$). Later $A(M_1)$ and $A(M_2)$ are known to Oracle. 
\begin{itemize}
    \item If $A(M_1)<D(M_2)$, no change to $D(M_1)$ and $D(M_2)$
    \item Otherwise, $D(M_1)=A(M_1)$
\end{itemize}

\begin{equation*}
\forall M_i \forall R_x:\qquad
    e(M_i, R_x)=\max\{D(M_i), \min\{t(M_i,R_x), D(M_i)+\lambda \} \}
\end{equation*}


To execute $M_i$, the 2 items in max indicates two necessary conditions 
\begin{itemize}
    \item The time reaches the deadline $D(M_i)$
    \item $M_i$ is obtained by $R_x$, which costs $\min\{t(M_i,R_x), D(M_i)+\lambda \}$, the 2 items in min indicates two alternative options (satisfying one is fine):
    \begin{itemize}
        \item $M_i$ is received by $R_x$ (at $t(M_i, R_x)$)
        \item $M_i$ has been appended by Oracle, and it takes $\lambda$ time cost for $R_x$ to get $M_i$ from the Oracle after that.
    \end{itemize}
\end{itemize}

Mapped to \sysname implementation, 
\begin{itemize}
    \item $\lambda$ is 0.5 RTT (i.e. the leader replica broadcasts the index information, and the followers get the request from its Late Buffer).

    \item  Logs are sorted by $D(*)$, so Oracle should release $D(*)$ in a monotonously-increasing way. Otherwise, small $D(*)$ could be appended after larger $D(*)$. When failure happens, the recovered logs have different order. In Nezha, $D(*)$ is generated by the the leader replica's clock. The monotonous property is preserved when the leader does not fail. After the leader fails and the new leader is elected, the new leader recovers the log first and find the largest $D(*)$ value among log entries, then it can start from a larger value to preserve monotonous property.
\end{itemize}


\subsection{Comparison between MOM, OUM and ORM}
MOM does not have Oracle, so replica's execution order may prove to be inconsistent, and needs rollback to solve that. 

OUM and ORM rely on the strong leadership of Oracle to solve inconsistency. Both Oracles release ordering information ($S(*)$ and $D(*)$ respectively). 

\begin{itemize}
    \item $S(*)$ is immutable (early binding), leading to false positives (i.e. there is no inconsistency among replicas, but $S(*)$ still indicate inconsistency and triggers replicas to resolve that).
    \item $D(*)$ is mutable, leading to false negatives (i.e. the replicas believe they have appended the messages in the correct way following $D(*)$, but later $D(*)$ is modified by Oracle. Thus those messages, which were assumed to have been ordered consistently with Oracle, were finally discovered to be ordered inconsistently with Oracle.)
\end{itemize}



% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_1)\\=&\max\{
%         D(M_1), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_1), 
%         \\&\qquad\qquad A(M_1)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}

% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{
%         D(M_2), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad A(M_2)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}


% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_1)+\Delta,
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad OWD(R_1, R_2)+t(M_2,R_2)+OWD(R_2,R_1), \\ 
%         &\qquad\qquad OWD(R_1, Oracle)+A(M_2)+OWD(Oracle,R_1)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_2)\\=&\max\{ D(M_1),
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_2),
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_1,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_1)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_2)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_2)+\Delta,
%         \\&\qquad \min\{
%         \\&\qquad\qquad t(M_2,R_2), 
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_2,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_2)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}




% \subsection{Oracle State}
% Both OUM Oracle and ORM Oracle have their own states. After failure, the new OUM Oracle and ORM Oracle need to recover their states before serving the system.

% \begin{enumerate}
%     \item The new OUM Oracle needs to remember the largest $S(M_i)$ that has been output by the old Oracle. The new OUM oracle can only start with a value larger than that.
%     \item The new ORM Oracle needs to remember the largest $D(M_i)$ that has been output by the old Oracle.The new ORM oracle can only start with a value larger than that. 
% \end{enumerate}

% Mapped to the implementation, 
% \begin{enumerate}
%     \item NOPaxos relies on the SDN controller to provide an incremented session number for every new OUM Oracle, $S(M_i)=(sessNum, msgNum)$. We say $S(M_i)<S(M_j)$ iff ($S(M_i),sessNum<S(M_j).sessNum$) or ($S(M_i).sessNum=S(M_j).sessNum\And S(M_i).msgNum<S(M_j).msgNum$) 
    
%     \textbf{But how to guarantee the SDN controller always output an monotonous session number (Considering the SDN can also fail, how should SDN remember the session number it has output before crash)? The paper does not say that.} 
    
%     Possible methods: Maybe SDN controller writes the session number to stable storage every time before using it; Maybe SDN controller commits its session number to another Paxos/Raft system before using it.
    
%     {\color{red} In one word, NOPaxos is not self-sufficient.}
    
%     \item {\color{red} Nezha is a self-sufficient system.}
%     Nezha puts the leader as the ORM Oracle. Whenever the old leader (Oracle) fails and the new leader (Oracle) is established, it recovers the logs (state) first. The leader (Oracle) gets the largest $D(M_i)$ by checking the last log entry in the recovered logs. And the new leader (Oracle) will start with a larger $D$ value than $D(M_i)$.
% \end{enumerate}








==> old/formulation-old-1124-4.tex <==
\clearpage
\onecolumn
\section{Formulation}
\subsection{Notation}
\begin{itemize}
    % \item Clients: $C_1, C_2,\dots$
    \item Replicas: $R_1, R_2,\dots$  (Leader is $R_L$)
    \item Messages: $M_1, M_2, \dots$
    % \item $t(M_i, C_j)$:  the departure time of $M_i$ from $C_j$ 
    \item $t(M_i, R_k)$:  the arrival time of  $M_i$ at $R_k$
    \item $e(M_i,R_k)$: the execution/appending time of $M_i$ at $R_k$
    \item $S(M_i)$: the sequential number of $M_i$ given by Sequencer.(OUM Oracle Information). 
    %$S(M_i)$ is visible to replicas, but becomes immutable once it is visible.
    \item $D(M_i)$: the \textbf{planned} execution time of $M_i$ at all replicas. (ORM Oracle Information).ORM Oracle broadcasts $M_i$ to all replicas after $D(M_i)$ in case some replicas are missing that. %$D(M_i)$ is visible to all replicas, and it is mutable.
    
    % \item $OWD(R_i, R_j)$: The one-way delay from $R_i$ to $R_j$.
    \item  $A(M_i)$: the arrival time of $M_i$ at the oracle (OUM Oracle and ORM Oracle Information). %$A(M_i)$ is invisible to replicas.
    
\end{itemize}

In OUM, $S(M_i)$ has casual relation to $A(M_i)$, i.e. the value of $S(M_i)$ is decided only after $A(M_i)$ is decided. Every time OUM Oracle releases a $S(*)$, it must be larger than all previous $S(*)$ values (monotonous requirement).

In ORM, the value of $D(M_i)$ can be decided without $A(M_i)$ but $D(M_i)$ can be rectified after $A(M_i)$ is decided. Every time ORM Oracle releases a $D(*)$, it must be larger than all previous $D(*)$ values (monotonous requirement).

\subsection{Definition}
\begin{itemize}
    % \item Reordering: $M_1$ and $M2$ are reordered towards $R_x$ iff $t(M_{1}, C_i)<t(M_{2},C_j)$ and $t(M_1,R_x)>t(M_2,R_x)$ ($i$ and $j$ can be the same or different)
    \item Packet drop: $M_i$ is lost to $R_x$ if $t(M_i, R_x)=\infty$
    \item Uniform ordering: $R_1$ and $R_2$ are \emph{order-ambiguous} (denoted as $OA(R_1,R_2,M_1,M_2)$) regarding $M_1$ and $M_2$ if:
    \begin{itemize}
        \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
        \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
    \end{itemize}
    
    
    \item Set inequality: $R_1$ and $R_2$ are \emph{set-inequal} regarding $M_1$ (denoted as $SI(R_1,R_2, M_1)$) if
    \begin{itemize}
        \item $e(M_1, R_1)=\infty$ and $e(M_1, R_2)< \infty$
        \item Or $e(M_1, R_1)< \infty$ and $e(M_1, R_2)= \infty$
    \end{itemize}
    
    \item Consistency: $R_1$ and $R_2$ are consistent if
    \begin{equation*}
        \forall M_i,M_j: 
  \neg OA(R_1,R_2,M_i,M_j) \And \neg SI(R_1,R_2,M_i) \And  \neg SI(R_1,R_2,M_j)
    \end{equation*}
    
\end{itemize}
    
    
%     % For $e(M_1, R_1),e(M_1, R_2), e(M_2, R_1), e(M_2, R_2) < \infty$
%     \begin{itemize}
%         \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
%         \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
%     \end{itemize}
%     Inconsistency = order ambiguity or set inequality.

% By taking packet drop as a special case of packet reordering, inconsistency=order ambiguity.

%     \item $S(M_1)$ and $S(M_2)$ become visible to replicas only after $A(M_1)$ and $A(M_2)$ are known to OUM Oracle. $S(M_1)$ and $S(M_2)$ are immutable once visible to replicas.
%     \item $D(M_1)$ and $D(M_2)$ are already visible even when $A(M_1)$ and $A(M_2)$ have not been known to BORM Oracle. $D(M_1)$ and $D(M_2)$ are mutable by Oracle even after they are visible to replicas.
% \end{itemize}



\section{Primitive Actions}

\subsection{MOM}
% $$e(M_1, R_1)=t(M_1,R_1)$$
% $$e(M_2, R_1)=t(M_2,R_1)$$
% $$e(M_1, R_2)=t(M_1,R_2)$$
% $$e(M_2, R_2)=t(M_2,R_2)$$
\begin{equation*}
\begin{split}
    &e(M_1, R_1) = t(M_1,R_1) \\
    &e(M_2, R_1) = t(M_2,R_1)  
\end{split}
\end{equation*}
$e(*,*)$ is completely determined by $t(*,*)$.
%and \textbf{MOM} just takes best effort to make $e(*,*)$ satisfy the consistency condition. 

% takes no remedies to inconsistency (just best effort). 
%If it happens, the majority order eventually wins. Others roll back.

% MOM does not modify $e(*,*)$ but OUM and BOM can modify $e(*,*)$ based on their Oracle information.


%MOM has no Oracle to provide information for replicas to fix inconsistency, whereas OUM/ORM has Oracle to provide information for replicas to fix inconsistency.

% \textbf{OUM's Oracle information can cause false positives whereas ORM's Oracle information can cause false negatives.}
% \begin{itemize}
%     \item OUM's Oracle information can cause false positives:  in fact there is no inconsistency, but Oracle information still indicates there is inconsistency.
%     \item ORM's Oracle information can cause false negative: Replicas believe $D(*)$ is correct and follow the guidance of $D(*)$, but later Oracle modifies $D(*)$ and claims the original $D(*)$ incorrect, i.e. the \emph{used-to-be-correct} consistency finally proves to be inconsistency.) 
% \end{itemize}







% MOM has no Oracle to provide information for replicas, so replicas have no idea on fixing inconsistency;
% OUM Oracle provides information for replicas to completely 
% % \textbf{OUM and BORM}: decides a definite order based on their Oracle information.

\subsection{OUM}


Without loss of generality, assume $A(M_1)<A(M_2)$, \textbf{After $A(M_1)$ and $A(M_2)$ are known to Oracle},  
the OUM Oracle gives $S(M_1)<S(M_2)$.

For simplification, only consider $S(M_2)=S(M_1)+1$. It can be generalized to non-consecutive cases $S(M_2)=S(M_1)+k$ (with more complexity).


If $t(M_1,R_1)<t(M_2,R_1)$ (Normal)
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)=t(M_1,R_1)\\
    &e(M_2,R_1)=t(M_2,R_1)
    \end{split}
\end{equation*}

Otherwise $t(M_1,R_1)>t(M_2,R_1)$
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)=
    \begin{cases}
      t(M_2,R_1)+\Phi, & \text{If $M_1$ is recovered successfully}\\
      \infty, & \text{Otherwise, $M_1$ commonly agreed to be NOOP}
    \end{cases}\\
    &e(M_2,R_1)=t(M_2,R_1)+\Phi~\footnotemark
    \end{split}
\end{equation*}

\footnotetext{We assume the execution does not cause time, so If $M_1$ is recovered and executed at $t(M_2,R_x)+\Phi$, then $M_2$ is executed immediately after that, which is also executed at $t(M_2,R_x)+\Phi$. }



Mapped to NOPaxos implementation, 
\begin{itemize}
    \item $\Phi$ is 1 RTT: As for the leader, it sends gap agreement requests and collect $f$ replies. As for the follower, it sends gap request, and receives either the request or NOOP from the leader. 
    \item  Logs are sorted by $S(*)$, so Oracle should release $S(*)$ in a monotonously-increasing way. Otherwise, small $S(*)$ could be appended after larger $S(*)$. When failure happens, the recovered logs have different order. In NOPaxos, $S(*)$ is generated by the sequencer. The monotonous property is preserved when the sequencer does not fail. It requires extra fault tolerant mechanism (i.e. stable storage or another Raft/Paxos system) to preserve monotonous property when the sequencer fails and relaunches.
\end{itemize}
 

\subsection{ORM}
Without loss of generality, assume $D(M_1)<D(M_2)$ (i.e. Oracle plans to execute $M_1$ before $M_2$). Later $A(M_1)$ and $A(M_2)$ are known to Oracle. 
\begin{itemize}
    \item If $A(M_1)<D(M_2)$, no change to $D(M_1)$ and $D(M_2)$
    \item Otherwise, $D(M_1)=A(M_1)$
\end{itemize}


If $t(M_1,R_1)<t(M_2,R_1)$
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)=\max\{D(M_1), t(M_1,R_1)\}\\
    &e(M_2,R_1)=\max\{D(M_2), t(M_2,R_1)\}
    \end{split}
\end{equation*}

Otherwise, $t(M_1,R_1)>t(M_2,R_1)$
\begin{equation*}
    \begin{split}
    &e(M_1,R_1)=
    \begin{cases}
      \max\{D(M_1), t(M_1,R_1)\} & \text{If $\max\{D(M_1), t(M_1,R_1)\}<D(M_2)$}\\
      D(M_1)+\lambda & \text{Otherwise, }
    \end{cases}\\
    &e(M_2,R_1)=\max\{D(M_2),t(M_2,R_1)\}
    \end{split}
\end{equation*}


% \begin{equation*}
% \forall M_i \forall R_x:\qquad
%     e(M_i, R_x)=\max\{D(M_i), \min\{t(M_i,R_x), D(M_i)+\lambda \} \}
% \end{equation*}


To execute $M_i$, the 2 items in max indicates two necessary conditions 
\begin{itemize}
    \item The time reaches the deadline $D(M_i)$
    \item $M_i$ is obtained by $R_x$, which costs $\min\{t(M_i,R_x), D(M_i)+\lambda \}$, the 2 items in min indicates two alternative options (satisfying one is fine):
    \begin{itemize}
        \item $M_i$ is received by $R_x$ (at $t(M_i, R_x)$)
        \item $M_i$ has been appended by Oracle, and it takes $\lambda$ time cost for $R_x$ to get $M_i$ from the Oracle after that.
    \end{itemize}
\end{itemize}

Mapped to \sysname implementation, 
\begin{itemize}
    \item $\lambda$ is 0.5 RTT (i.e. the leader replica broadcasts the index information, and the followers get the request from its Late Buffer).

    \item  Logs are sorted by $D(*)$, so Oracle should release $D(*)$ in a monotonously-increasing way. Otherwise, small $D(*)$ could be appended after larger $D(*)$. When failure happens, the recovered logs have different order. In Nezha, $D(*)$ is generated by the the leader replica's clock. The monotonous property is preserved when the leader does not fail. After the leader fails and the new leader is elected, the new leader recovers the log first and find the largest $D(*)$ value among log entries, then it can start from a larger value to preserve monotonous property.
\end{itemize}


\subsection{Comparison between MOM, OUM and ORM}
MOM does not have Oracle, so replica's execution order may prove to be inconsistent, and needs rollback to solve that. 

OUM and ORM rely on the strong leadership of Oracle to solve inconsistency. Both Oracles release ordering information ($S(*)$ and $D(*)$ respectively). 

\begin{itemize}
    \item $S(*)$ is immutable (early binding), leading to false positives (i.e. there is no inconsistency among replicas, but $S(*)$ still indicate inconsistency and triggers replicas to resolve that).
    \item $D(*)$ is mutable, leading to false negatives (i.e. the replicas believe they have appended the messages in the correct way following $D(*)$, but later $D(*)$ is modified by Oracle. Thus those messages, which were assumed to have been ordered consistently with Oracle, were finally discovered to be ordered inconsistently with Oracle.)
\end{itemize}



% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_1)\\=&\max\{
%         D(M_1), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_1), 
%         \\&\qquad\qquad A(M_1)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}

% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{
%         D(M_2), 
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad A(M_2)+\lambda
%         \\&\qquad  \}
%         \\& \}
%     \end{split}
% \end{equation*}


% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_1)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_1)+\Delta,
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_2,R_1), 
%         \\&\qquad\qquad OWD(R_1, R_2)+t(M_2,R_2)+OWD(R_2,R_1), \\ 
%         &\qquad\qquad OWD(R_1, Oracle)+A(M_2)+OWD(Oracle,R_1)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_1,R_2)\\=&\max\{ D(M_1),
%         \\&\qquad\min\{
%         \\&\qquad\qquad t(M_1,R_2),
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_1,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_1)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}
% \begin{equation*}
%     \begin{split}
%         &e(M_2,R_2)\\=&\max\{ D(M_2), 
%         \\&\qquad e(M_1,R_2)+\Delta,
%         \\&\qquad \min\{
%         \\&\qquad\qquad t(M_2,R_2), 
%         \\&\qquad\qquad OWD(R_2, R_1)+t(M_2,R_1)+OWD(R_1,R_2), 
%         \\&\qquad\qquad OWD(R_2, Oracle)+A(M_2)+OWD(Oracle,R_2)
%         \\&\qquad \} 
%         \\& \}
%     \end{split}
% \end{equation*}




% \subsection{Oracle State}
% Both OUM Oracle and ORM Oracle have their own states. After failure, the new OUM Oracle and ORM Oracle need to recover their states before serving the system.

% \begin{enumerate}
%     \item The new OUM Oracle needs to remember the largest $S(M_i)$ that has been output by the old Oracle. The new OUM oracle can only start with a value larger than that.
%     \item The new ORM Oracle needs to remember the largest $D(M_i)$ that has been output by the old Oracle.The new ORM oracle can only start with a value larger than that. 
% \end{enumerate}

% Mapped to the implementation, 
% \begin{enumerate}
%     \item NOPaxos relies on the SDN controller to provide an incremented session number for every new OUM Oracle, $S(M_i)=(sessNum, msgNum)$. We say $S(M_i)<S(M_j)$ iff ($S(M_i),sessNum<S(M_j).sessNum$) or ($S(M_i).sessNum=S(M_j).sessNum\And S(M_i).msgNum<S(M_j).msgNum$) 
    
%     \textbf{But how to guarantee the SDN controller always output an monotonous session number (Considering the SDN can also fail, how should SDN remember the session number it has output before crash)? The paper does not say that.} 
    
%     Possible methods: Maybe SDN controller writes the session number to stable storage every time before using it; Maybe SDN controller commits its session number to another Paxos/Raft system before using it.
    
%     {\color{red} In one word, NOPaxos is not self-sufficient.}
    
%     \item {\color{red} Nezha is a self-sufficient system.}
%     Nezha puts the leader as the ORM Oracle. Whenever the old leader (Oracle) fails and the new leader (Oracle) is established, it recovers the logs (state) first. The leader (Oracle) gets the largest $D(M_i)$ by checking the last log entry in the recovered logs. And the new leader (Oracle) will start with a larger $D$ value than $D(M_i)$.
% \end{enumerate}








==> old/formulation-old.tex <==
\clearpage
\section{Formulation}
\subsection{Notation}
\begin{itemize}
    \item Clients: $C_1, C_2,\dots$
    \item Replicas: $R_1, R_2,\dots$  (Leader is $R_L$)
    \item Sequencer: $S$
    \item Messages: $M_1, M_2, \dots$
    \item $t(M_i, C_j)$:  the departure time of $M_i$ from $C_j$ 
    \item $t(M_i, R_k)$:  the arrival time of  $M_i$ at $R_k$
    \item $e(M_i,R_k)$: the execution time of $M_i$ at $R_k$
    \item $t(M_i, S)$: the arrival/departure time of $M_i$ at/from Sequencer $S$.(OUM-specific information).
    \item $d(M_i)$: the \textbf{expected} arrival time of $M_i$ at all replicas. (BORM-specific information).
    
\end{itemize}

\subsection{Definition}
\begin{itemize}
    \item Reordering: $M_1$ and $M2$ are reordered towards $R_x$ iff $t(M_{1}, C_i)<t(M_{2},C_j)$ and $t(M_1,R_x)>t(M_2,R_x)$ ($i$ and $j$ can be the same or different)
    \item Packet drop: $M_1$ is lost to $R_x$ iff $t(M_1, R_x)=\infty$
    \item Inconsistent: $R_1$ and $R_2$ are inconsistent iff $t(M_1, R_1)> t(M_2, R_1)$ and $t(M_1, R_2)< t(M_2, R_2)$. (iff $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$.)
\end{itemize}

\section{Primitive Actions}

When $R_1$ and $R_2$ are inconsistent:

\textbf{MOM}: No action. Finally, the majority's order wins.

\textbf{OUM and BORM}: The leader's order always wins, but how does the leader decide the final order?

\textbf{OUM:} 
\begin{itemize}
    \item Case 1: $t(M_1,S)<t(M_2,S)$ and $t(M_1,R_L)<t(M_2,R_L)$, then OK.
    \item Case 2: $t(M_1,S)>t(M_2,S)$ and $t(M_1,R_L)>t(M_2,R_L)$, then OK.
    \item Case 3: $t(M_1,S)<t(M_2,S)$ and $t(M_1,R_L)>t(M_2,R_L)$, then $t(M_1,R_L)=\infty$.
    \item Case 4: $t(M_1,S)>t(M_2,S)$ and $t(M_1,R_L)<t(M_2,R_L)$, then $t(M_2,R_L)=\infty$.
\end{itemize}

Case 3 and Case 4 are gap agreement. If we consider Jialin's optimization (first try to fetch from the other replicas), then it becomes
\begin{itemize}
    \item Case 3: $t(M_1,S)<t(M_2,S)$ and $t(M_1,R_L)>t(M_2,R_L)$, then $t(M_1,R_L)=T$ and $t(M_2,R_L)=T+\Delta$. ($T$ is the time that the fetched $M_1$ arrives at $R_L$)
    \item Case 4: $t(M_1,S)>t(M_2,S)$ and $t(M_1,R_L)<t(M_2,R_L)$, then $t(M_2,R_L)=T$ and $t(M_1,R_L)=T+\Delta$.
\end{itemize}




\textbf{BORM:} 
\begin{itemize}
    \item Case 1: $d(M_1)<d(M_2)$  and $t(M_1, R_L) < t(M_2, R_L)$, then $t(M_1,R_L)=\max\{ t(M_1,R_L), d(M_1)\}$ and $t(M_2,R_L)=\max\{ t(M_2,R_L), d(M_2)\}$.
    

    \item Case 2: $d(M_1)<d(M_2)$  and $t(M_1, R_L) > t(M_2, R_L)$, then
    \begin{itemize}
        \item 2.1: $t(M_1,R_L)<d(M_1)$, then $t(M_1, R_L)=d(M_1)$ and $t(M_2,R_L)=d(M_2)$
        \item 2.2: $d(M_1)<t(M_1,R_L)<d(M_2)$, then
        \begin{itemize}
            \item 2.2.1: $t(M_2,R_L)<d(M_2)$, then $t(M_1,R_L)$ does not change, $t(M_2,R_L)=d(M_2)$
            \item 2.2.2: $t(M_2,R_L)>d(M_2)$, then $t(M_2,R_L)$ does not change and $t(M_1,R_L)$ does not change.
        \end{itemize}
        \item 2.3: $t(M_1, R_L)>d(M_2)$, then
        \begin{itemize}
            \item 2.3.1: $t(M_2, R_L)<d(M_2)$, then $t(M_2,R_L)=d(M_2)$ and $t(M_1,R_L)=d(M_2)+\Delta$
            \item 2.3.2: $t(M_2, R_L)>d(M_2)$, then $t(M_2, R_L)$ does not change and $t(M_1,R_L)$ does not change
        \end{itemize}
        \item Case 3: Flip $M_1$ and $M_2$ in Case 1.
        \item Case 4: Flip $M_1$ and $M_2$ in Case 2.
    \end{itemize}
\end{itemize}










==> old/formulation-old1124.tex <==
\clearpage
\section{Formulation}
\subsection{Notation}
\begin{itemize}
    \item Clients: $C_1, C_2,\dots$
    \item Replicas: $R_1, R_2,\dots$  (Leader is $R_L$)
    \item Messages: $M_1, M_2, \dots$
    \item $t(M_i, C_j)$:  the departure time of $M_i$ from $C_j$ 
    \item $t(M_i, R_k)$:  the arrival time of  $M_i$ at $R_k$
    \item $e(M_i,R_k)$: the execution/appending time of $M_i$ at $R_k$
    \item $S(M_i)$: the sequential number of $M_i$ given by Sequencer.(OUM Oracle Information). $S(M_i)$ is visible to replicas, but becomes immutable once it is visible.
    \item $D(M_i)$: the \textbf{planned} execution time of $M_i$ at all replicas. (BORM Oracle Information). $D(M_i)$ is visible to all replicas, and it is mutable.
    
    \item $OWD(R_i, R_j)$: The one-way delay from $R_i$ to $R_j$.
    \item  $A(M_i)$: the arrival time of $M_i$ at the oracle (OUM Oracle and BORM Oracle Information). $A(M_i)$ is invisible to replicas.
    
\end{itemize}


\subsection{Definition}
\begin{itemize}
    \item Reordering: $M_1$ and $M2$ are reordered towards $R_x$ iff $t(M_{1}, C_i)<t(M_{2},C_j)$ and $t(M_1,R_x)>t(M_2,R_x)$ ($i$ and $j$ can be the same or different)
    \item Packet drop: $M_1$ is lost to $R_x$ iff $t(M_1, R_x)=\infty$
    \item Inconsistency: $R_1$ and $R_2$ are inconsistent iff 
    
    % For $e(M_1, R_1),e(M_1, R_2), e(M_2, R_1), e(M_2, R_2) < \infty$
    \begin{itemize}
        \item $e(M_1, R_1)> e(M_2, R_1)$ and $e(M_1, R_2)< e(M_2, R_2)$
        \item Or $e(M_1, R_1)< e(M_2, R_1)$ and $e(M_1, R_2)> e(M_2, R_2)$
    \end{itemize}
    Inconsistency = order ambiguity or set inequality.

By taking packet drop as a special case of packet reordering, inconsistency=order ambiguity.

    \item $S(M_1)$ and $S(M_2)$ become visible to replicas only after $A(M_1)$ and $A(M_2)$ are known to OUM Oracle. $S(M_1)$ and $S(M_2)$ are immutable once visible to replicas.
    \item $D(M_1)$ and $D(M_2)$ are already visible even when $A(M_1)$ and $A(M_2)$ have not been known to BORM Oracle. $D(M_1)$ and $D(M_2)$ are mutable by Oracle even after they are visible to replicas.
\end{itemize}



\section{Primitive Actions}

\subsection{MOM Remedies to Inconsistency}
$$e(M_1, R_1)=t(M_1,R_1)$$
$$e(M_2, R_1)=t(M_2,R_1)$$
$$e(M_1, R_2)=t(M_1,R_2)$$
$$e(M_2, R_2)=t(M_2,R_2)$$

\textbf{MOM} takes no remedies to inconsistency (just best effort). 
%If it happens, the majority order eventually wins. Others roll back.


\textbf{OUM and BORM}: decides a definite order based on their Oracle information.

\subsection{OUM Remedies to Inconsistency}


Without loss of generality, assume $A(M_1)$ and $A(M_2)$ are known to Oracle as $A(M_1)<A(M_2)$, \textbf{After $A(M_1)$ and $A(M_2)$ are known to Oracle},  
the OUM Oracle gives $S(M_1)<S(M_2)$.

For simplification, only consider $S(M_2)=S(M_1)+1$. It can be generalized to non-consecutive cases $(M_2)=S(M_1)+k$ (with more complexity).

\begin{itemize}
    \item Case 1: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then $$e(M_1,R_1)=t(M_1,R_1)$$
    $$e(M_2,R_1)=t(M_2,R_1)$$
    $$e(M_1,R_2)=t(M_1,R_2)$$
    $$e(M_2,R_2)=t(M_2,R_2)$$
    
    \item Case 2: $t(M_1,R_1)<t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then
    $$e(M_1,R_1)=t(M_1,R_1)$$
    $$e(M_2,R_1)=t(M_2,R_1)$$
\begin{equation*}
    \begin{split}
       e(M_1,R_2)=\min\{& OWD(R_2,R_1)+t(M_1,R_1)+OWD(R_1,R_2),\\ & t(M_1,R_2)\}
    \end{split}
\end{equation*}
    $$e(M_2,R_2)=e(M_1,R_2)+\Delta$$
    
    \item Case 3: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)<t(M_2, R_2)$, then
\begin{equation*}
    \begin{split}
       e(M_1,R_1)=\min\{& OWD(R_1,R_2)+t(M_1,R_2)+OWD(R_2,R_1),\\ & t(M_1,R_1)\}
    \end{split}
\end{equation*}
    $$e(M_2,R_1)=e(M_1,R_1)+\Delta$$
    $$e(M_1,R_2)=t(M_1, R_2)$$
    $$e(M_2,R_2)=t(M_2,R_2)$$
    
\item Case 4: $t(M_1,R_1)>t(M_2, R_1)$ and $t(M_1,R_2)>t(M_2, R_2)$, then

% (Case 4.1) If $t(M_2,R_1)+OWD(R_1,R_2)<t(M_1,R_2)$, then 
%     $$e(M_1,R_1)=\infty$$
%     $$e(M_2,R_1)=t(M_2,R_1)+OWD(R_1,R_2)+OWD(R_2,R_1)$$

% (Case 4.2) If $t(M_2,R_1)+OWD(R_1,R_2)>t(M_1,R_2)$, then
%     $$e(M_1,R_1)=t(M_2,R_1)+OWD(R_1,R_2)+OWD(R_2,R_1)$$
%     $$e(M_2,R_1)=\max\{t(M_2,R_1), e(M_1,R_1)+\Delta\}$$

    $$e(M_1,R_1)=\infty$$
    $$e(M_2,R_1)=t(M_2,R_1)+OWD(R_1,R_2)+OWD(R_2,R_1)$$
    $$e(M_1,R_2)=\infty$$
    $$e(M_2,R_2)=t(M_2,R_2)+OWD(R_2,R_1)+OWD(R_1,R_2)$$
\end{itemize}



Note: Case 2 and Case 3 have already considered Jialin's optimization (i.e. first try to recover the gap by asking the others, instead of immediately starting gap agreement). 

\subsection{BORM Remedies to Inconsistency}
$D(M_1)$ and $D(M_2)$ are already decided by Oracle and broadcast to replicas, even when $A(M_1)$ and $A(M_2)$ are still unknown. Without loss of generality, assume $D(M_1)<D(M_2)$ (i.e. Oracle plans to execute $M_1$ before $M_2$). Later $A(M_1)$ and $A(M_2)$ are known to Oracle.

Case 1: $A(M_1)<A(M_2)$, 
\begin{equation*}
    \begin{split}
        &e(M_1,R_1)\\=&\max\{
        D(M_1),
        \\&\qquad\min\{
        \\&\qquad\qquad t(M_1,R_1), 
        \\&\qquad\qquad  OWD(R_1, R_2)+t(M_1,R_2)+OWD(R_2,R_1), \\ 
        &\qquad\qquad OWD(R_1, Oracle)+A(M_1)+OWD(Oracle,R_1)
        \\&\qquad  \}
        \\& \}
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        &e(M_2,R_1)\\=&\max\{ D(M_2), 
        \\&\qquad e(M_1,R_1)+\Delta,
        \\&\qquad\min\{
        \\&\qquad\qquad t(M_2,R_1), 
        \\&\qquad\qquad OWD(R_1, R_2)+t(M_2,R_2)+OWD(R_2,R_1), \\ 
        &\qquad\qquad OWD(R_1, Oracle)+A(M_2)+OWD(Oracle,R_1)
        \\&\qquad \} 
        \\& \}
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        &e(M_1,R_2)\\=&\max\{ D(M_1),
        \\&\qquad\min\{
        \\&\qquad\qquad t(M_1,R_2),
        \\&\qquad\qquad OWD(R_2, R_1)+t(M_1,R_1)+OWD(R_1,R_2), 
        \\&\qquad\qquad OWD(R_2, Oracle)+A(M_1)+OWD(Oracle,R_2)
        \\&\qquad \} 
        \\& \}
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        &e(M_2,R_2)\\=&\max\{ D(M_2), 
        \\&\qquad e(M_1,R_2)+\Delta,
        \\&\qquad \min\{
        \\&\qquad\qquad t(M_2,R_2), 
        \\&\qquad\qquad OWD(R_2, R_1)+t(M_2,R_1)+OWD(R_1,R_2), 
        \\&\qquad\qquad OWD(R_2, Oracle)+A(M_2)+OWD(Oracle,R_2)
        \\&\qquad \} 
        \\& \}
    \end{split}
\end{equation*}


Case 2: $A(M_1)>A(M_2)$, we further divide into two cases (Based on comparison between $A(M_1)$ and $D(M_2)$).
\begin{itemize}
    \item Case 2.1: $A(M_1)<D(M_2)$. Oracle does not modify $D(M_1)$ and $D(M_2)$ (because $M_1$ can still be executed before $M_2$, Oracle does not need to change its original plan), the formulas of $e(M_1,R_1)$, $e(M_2,R_2)$, $e(M_1,R_2)$, $e(M_2,R_2)$ are the same as Case 1. 
    \item Case 2.2: $A(M_1)>D(M_2)$ ({\color{red}Combined with $A(M_1)>A(M_2)$, we have $D(M_1)<\max\{D(M_2),A(M_2)\}<A(M_1)$}). The original plan to execute $M_1$ before $M_2$ has to be modified. Oracle modifies $D(M_1)=A(M_1)$. Then, the formulas of $e(M_1,R_1)$, $e(M_2,R_2)$, $e(M_1,R_2)$, $e(M_2,R_2)$ are the same as Case 1. 
\end{itemize}


\subsection{Oracle State}
Both OUM Oracle and BORM Oracle have their own states. After failure, the new OUM Oracle and BORM Oracle need to recover their states before serving the system.

\begin{enumerate}
    \item The new OUM Oracle needs to remember the largest $S(M_i)$ that has been output by the old Oracle. The new OUM oracle can only start with a value larger than that.
    \item The new BORM Oracle needs to remember the largest $D(M_i)$ that has been output by the old Oracle.The new OUM oracle can only start with a value larger than that. 
\end{enumerate}

Mapped to the implementation, 
\begin{enumerate}
    \item NOPaxos relies on the SDN controller to provide an incremented session number for every new OUM Oracle, $S(M_i)=(sessNum, msgNum)$. We say $S(M_i)<S(M_j)$ iff ($S(M_i),sessNum<S(M_j).sessNum$) or ($S(M_i).sessNum=S(M_j).sessNum\And S(M_i).msgNum<S(M_j).msgNum$) 
    
    \textbf{But how to guarantee the SDN controller always output an monotonous session number (Considering the SDN can also fail, how should SDN remember the session number it has output before crash)? The paper does not say that.} 
    
    Possible methods: Maybe SDN controller writes the session number to stable storage every time before using it; Maybe SDN controller commits its session number to another Paxos/Raft system before using it.
    
    {\color{red} In one word, NOPaxos is not self-sufficient.}
    
    \item {\color{red} Nezha is a self-sufficient system.}
    Nezha puts the leader as the BORM Oracle. Whenever the old leader (Oracle) fails and the new leader (Oracle) is established, it recovers the logs (state) first. The leader (Oracle) gets the largest $D(M_i)$ by checking the last log entry in the recovered logs. And the new leader (Oracle) will start with a larger $D$ value than $D(M_i)$.
\end{enumerate}








==> old/intro-old.tex <==
\section{Introduction}
\label{sec:introduction}
Consensus protocols have been a long-lasting topic for decades. As two most widely used consensus protocols, Raft~\cite{raft} and Multi-Paxos~\cite{paxos} require 2 RTTs (round-trip time) for every submitted request, and their throughput capacity is bottlenecked by the single leader. 

Targeting at the performance (both latency and throughput) drawbacks of Raft/Multi-Paxos, extensive efforts have been made to improve the efficiency of consensus protocols. However, none of them can satisfy all the major dimensions, as shown in Table~\ref{tab-related-work}. 


As one of the most attractive variants, NOPaxos~\cite{nopaxos} achieves the optimal latency (i.e. 1 RTT) and throughput (i.e. 1 RPC/Request), without suffering from larger quorum size or costly rollback. However, NOPaxos relies on a high-performance sequencer to guarantee its OUM (ordered unreliable multicast) primitive, which is usually implemented by special hardware. Such a stringent requirement makes NOPaxos hardly deployable in common public cloud~\cite{some-critic-paper, erpc}, where network is considered as a blackbox and users have little capability to control it. Although NOPaxos also supports a software endhost as the sequencer (refer to Section 4.2.3 in NOPaxos paper), such an implementation leads to serious performance discount. An endhost-based sequencer adds one message delay for each submits request. It does not eliminate the throughput bottleneck essentially, instead, it only migrates the bottleneck from the replica to the sequencer itself.


Our goal is to build a consensus protocol which can inherit the performance benefit of NOPaxos, but achieve good scalability in public cloud. We design Nezha, which leverages highly-synchronized clocks to achieve optimal latency and throughput in theory. 


The design of Nezha is based on two aspects.
\begin{enumerate}
    \item Today's data center has become more predictable~\cite{specpaxos, other-citations-in-specpaxos}. Therefore, a good estimation of latency between replicas and clients can serve as useful information to build consensus protocols. 
    \item Highly synchronized and scalable clocks have been available in public cloud~\cite{huygens}. Therefore, clients and replicas can work according to their local clocks to achieve \emph{approximate} consensus,  without \emph{explicit} communication.  
\end{enumerate}


In order for Nezha to yield a good performance (liveness), we need two conditions.
\begin{enumerate}
    \item \textbf{Mostly-Bounded-Latency}. The latency between clients and replicas are bounded \textit{for most time}. 
    \item \textbf{Mostly-Synchronized-Time}. The clock time for clients and replicas is synchronized \textit{for most times}. 
\end{enumerate}

We are requiring neither \emph{completely-bounded-latency} nor \emph{perfectly-synchronized-time}. Bounded latency and synchronized time are not necessary for the correctness of Nezha. However, better latency bound and clock synchronization leads to better performance of Nezha.


Clock synchronization has been rapidly developed in recent years, a couple of new solutions has come out~\cite{spanner, huygens,  sundial(osdi20)}. (The latest Precision Time Protocol improves clock synchronization to achieve su-bmicrosecond accuracy~\cite{osdi20-mu}.) While choosing the clock-sync solutions, we place scalability as the first priority. Spanner and Sundial, though provides tight error bounds, require special hardware and cannot be deployed in public cloud. By contrast, Huygens is a pure software solution and meets our requirement of scalability. However, since Huygens is built on the probabilistic model (i.e. SVM), its error bound is not 100\% certain~\cite{sundial}, although it achieves very small 99\% discrepancies.

%Good sentences: A consensus protocol ensures that all replicas agree on what request is stored in each slot of the log. Replicas then apply the requests in the log (i.e., execute the corresponding operations), in log order [OSDI20-Mu]. 

The key idea behind Nezha is, we compromise (very little) liveness, in order to leverage both the clock-sync benefit and scalability benefit from Huygens, and not to violate the correctness of consensus protocol. In Nezha, replicas and clients are synchronized by Huygens and the one-way delay can be well measured and estimated between them. Based on the one-way delay statistics, replicas partition the time into consecutive blocks, and expect the clients' request to arrive in each time block. Once the request fails to come on time, replicas will start gap-agreement procedure to fill NO-OP in the corresponding log slot. We will explain more details in the design section.

In general, Nezha incorporates three main strategies to obtain advantages over existing works.
\begin{enumerate}
    \item \textbf{TDMA-Style OUM (TOUM)}. Nezha implements a TDMA-Style OUM to achieve theorectically optimal latency/throughput as NOPaxos. Unlike NOPaxos' OUM, which uses sequential number for consistency guarantee, the TOUM leverages timeout mechanism for gap detection and gap agreement. Compared with the hardware-based OUM of NOPaxos, TOUM enjoys much better scalability and can be deployed in public cloud. Compared with the software-based OUM of NOPaxos, TOUM only needs a virtual sequencer, thus Nezha does not suffer from the additional message delay and sequencer bottlneck as NOPaxos. Moreover, as what will be shown in  \S\ref{sec:nezha-advantage}, TOUM enables Nezha to handle the gap in a more reasonable way, whereas NOPaxos may start the gap agreement too conservatively or too aggressively. 
     
    \item \textbf{Dynamic Rate Control}. Nezha fully utilizes the measurement ability of clock synchronization, and it can monitor the variance of one-way delay between replicas and nodes. Based on the measurement result, Nezha dynamically adjusts the sending rate of clients and the time block lengths of replicas, so as to adapt to the time-varying cloud environment and heterogeneity of clients.
    
    \item \textbf{Lazy Write}. Nezha also considers the optimization to skewed workload. Since read requests dominate the workload in many practical cases, Nezha develops lazy-write policy, which compromises write performance for better read throughput. 
\end{enumerate}

==> old/intro_snippets.tex <==
%Our evaluation reveals that existing protocols (e.g. Fast Paxos~\cite{fastpaxos} and NOPaxos~\cite{osdi16-nopaxos}) suffer from a serious performance degradation in the open-loop test, whereas \sysname not only outperforms these baselines, but also remains robust performance in both test scenarios.  

%The basic intuition behind \sysname is to use clock synchronization to build \emph{approximate consensus} and then take a small extra effort to refine the approximate consensus to the intact consensus. As explained in \S\ref{sec-dom}, the replica consistency can be decomposed into two finer-grained tasks: (a) \emph{uniform ordering}---i.e., requests occur in the same order in different replicas, and (b) \emph{set equality}---i.e., the replicas have the same sets of requests. Instead of completely relying on the replication protocol, we first build a primitive--which we call Deadline-Ordered Primitive, or DOM--to complete the first task, and then we design our replication protocol--\sysname--to complete the second task and finally reach consensus.

%DOM relies on synchronized clocks to achieve uniform ordering, and then \sysname protocol uses the lightweight leader$\xrightarrow{}$follower communication to maintain set equality among replicas. Since we design \sysname as a leader-based protocol, we try to mitigate the workload of the leader by completely offloading the quorum check to the clients, which is a task usually performed by the leader in Multi-Paxos/Raft and Fast Paxos, as well as in the slow path of Speculative Paxos and NOPaxos. Offloading quorum check to the clients not only relieves the leader, it also reduces the number of message delays incurred in committing requests.  

%consensus protocols tend not to depend on clocks, because clocks do not keep perfect time and can drift with respect to one another~\cite{podc84-byzantine-clock-sync}. Therefore, it is necessary to keep the correctness of consensus protocol independent of clock synchronization, and only ``depend on synchronization for performance but not for correctness''~\cite{podc91-clock-sync-remark} %Although a variety of high-precision clock synchronization techniques (e.g. PTP~\cite{tsn_ptp}, Spanner~\cite{spanner}, DTP~\cite{sigcomm16-dtp}, Huygens~\cite{huygens},  Sundial~\cite{osdi20-sundial}) have emerged in recent years, it is still too risky to rely on clock synchronization for the correctness of consensus protocols. On one hand, software-based clock-sync solutions, such as Huygens~\cite{huygens}, can be easily deployed in public cloud. However, Huygens uses a probabilistic model and cannot guarantee a certain error bound. Using such clock time to generate consistent ordering among replicas can lead to incorrect outcomes. On the other hand, hardware-based clock-sync solutions, such as PTP~\cite{tsn_ptp} and Sundial~\cite{osdi20-sundial}, can provide a certain error bound, but they are difficult to deploy and not supported by the public cloud yet. Even regardless of the deployment requirements, hardware-based clock-sync solutions can neither provide correctness guarantee for consensus protocols, because the solutions may also fail while the consensus protocol is stilling working without awareness of that.

%We fully recognize the risks and avoid using clock synchronization for the correctness of \sysname. Instead, we choose to ``depend on synchronization for performance but not for correctness''~\cite{podc91-clock-sync-remark}.

% Meanwhile, clients take full responsibility for ensuring there is a quorum, a task performed by the leader in Multi-Paxos and Paxos. Offloading quorum checking to the clients not only relieves the leader, it also reduces the number of message delays incurred in committing requests.  

    %\item We present \sysname, a scalable consensus protocol working in public cloud without special hardware/network support.
    % \item We decouple commit and execution in \sysname, and conduct optimization strategies respectively to further reduce commit latency and execution latency. 
    % \item Evaluations show that in a wide range of settings \sysname outperforms four baselines (i.e. Multi-Paxos~\cite{paxos}, Fast Paxos~\cite{fastpaxos}, NOPaxos~\cite{osdi16-nopaxos} and Raft~\cite{atc14-raft}).
    % \item We find that speculative protocols such as FastPaxos and NOPaxos which yield high performance in highly-engineered network environments suffer from distinct degradation in the public cloud, especially when they are benchmarked with open-loop clients; by contrast, \sysname achieves high performance in both closed- and open-loop tests. 
    % \item Finally, we compare the fault tolerance provided by \sysname with that provided by the three baseline schemes (Multi-Paxos, Fast Paxos and NOPaxos) in the context of two applications: Redis~\cite{redis} and CloudEx~\cite{hotos21-cloudex}. Evaluations show that \sysname delivers the highest performance for the applications.
    
    % \item We show that \sysname enjoys much stronger resistance to bursts. By contrast, although some speculative protocols (e.g. Fast Paxos and NOPaxos), which, such as Fast Paxos and NOPaxos, are expected to achieve desirable performance in their fast paths, we reveal in the public cloud environment, these solutions suffer from serious degradation (especially with open-loop clients) because the conflicts make them go through their slow paths very frequently.
    
% Evaluations show that in a wide range of settings \sysname outperforms four baselines (i.e. Multi-Paxos~\cite{paxos}, Fast Paxos~\cite{fastpaxos}, NOPaxos~\cite{osdi16-nopaxos} and Raft~\cite{atc14-raft}).
%     \item We find that speculative protocols such as FastPaxos and NOPaxos which yield high performance in highly-engineered network environments suffer from distinct degradation in the public cloud, especially when they are benchmarked with open-loop clients; by contrast, \sysname achieves high performance in both closed- and open-loop tests. 
%     \item Finally, we compare the fault tolerance provided by \sysname with that provided by the three baseline schemes (Multi-Paxos, Fast Paxos and NOPaxos) in the context of two applications: Redis~\cite{redis} and CloudEx~\cite{hotos21-cloudex}. Evaluations show that \sysname delivers the highest performance for the applications.
    
% The rest of the paper is organized as follows. \S\ref{sec:background} introduces the background and summarizes the key idea behind \sysname. %to achieve high performance with clock synchronization. 
% \S\ref{sec:design} presents the details of the \sysname protocol. %including the three main components (\S\ref{selective-acceptance}$\sim$\S\ref{quorum-check}), the recovery procedure (\S\ref{sec:recovery}), and the correctness proof (\S\ref{sec:proof}).
% \S\ref{sec:refinement} designs optimization strategies to further reduce the commit/execution latency. \S\ref{sec:evaluation} conducts comparative evaluation of \sysname and relevant baselines. \S\ref{sec:app} considers the fault tolerance of \sysname in the context of two applications: Redis and CloudEx. \S\ref{sec:related-work} includes the related work and \S\ref{sec:conclusion} concludes the paper.   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old/key_idea.tex <==

\section{Decomposing Ordering Agreement}
\label{sec:key-idea}

While committing requests from concurrent clients, the consensus protocol is required to undertake two key responsibilities.
\begin{itemize}
    \item \textbf{Ordering agreement.} The consensus protocol needs to establish a definitive order for all requests, so that every replica can process the requests following the consistent order.
    \item \textbf{Replication.} The consensus protocol needs to replicate the requests to at least a majority of replicas, so that the requests can be recovered after failure.  
\end{itemize}

Ordering agreement is essential for consistency and lineaizability whereas replication is necessary for durability. 

Reaching ordering agreement is expensive, but an early ordering agreement can avoid heavy penalty when inconsistency really happens later. The typical consensus protocols makes different trade-off between the cost of ordering agreement and the potential penalty of resolving inconsistency. 

(1) Multi-Paxos/Raft and NOPaxos choose to prioritize ordering agreement over replication. The ordering agreement indicates the \emph{definitive ordering} agreed by all replicas, which cannot be reverted later. Multi-Paxos/Raft relies on the leader replica as the centralized serialization point to reach the agreement, which suffers from the worst throughput/latency performance. NOPaxos relies on a standalone sequencer as the serialization point, which relieves the throughput bottleneck, but also incurs longer or extra message delay~\footnote{The software sequencer costs 1 extra message delay for NOPaxos. The hardware sequencer does not add extra message delays but requires every request message detour the root switch, thus prolonging the message delay. }. Besides, it also imposes stringent networking requirement, making it hard to deploy in public cloud. 

(2) Fast Paxos and Speculative Paxos choose to prioritize replication over ordering agreement. Therefore, they allow each replica to adopt \emph{approximate ordering}, which is \textbf{probably} commonly agreed by replicas, but may also be reverted later. Such approaches can save some latency and/or throughput overheads in the fast path. But when inconsistency really happens and the \emph{approximate ordering} proves to be wrong, it takes longer time for the leader to detect it and costs more overheads to resolve it. 


\sysname shares the same principle with the latter category, i.e. \sysname also prioritizes replication over ordering agreement. But more importantly, \sysname also avoids heavy penalty to resolve the (possible) inconsistency. The key idea of \sysname is to decompose the expensive ordering agreement into two finer-grained tasks: 

%\emph{eliminating ordering ambiguity} earlier during replication and \emph{fixing set equality} later during synchronization. 

\begin{enumerate}
    \item \textbf{Eliminate ordering ambiguity.} If one replica orders request $a$ ahead of request $b$, no other replicas can order them in a reverse way.   
    \item \textbf{Maintain set equality.} All the replicas should have exactly the same requests (i.e. the sets of requests are equal).
\end{enumerate}
Without introducing the centralized serialization point or inter-replica communication, it is quite challenging to achieve ordering agreement among replicas. However, we will show in \sysname, {\color{red} [key sentence:] by using clock synchronization, it is fairly easy to \textbf{eliminate ordering ambiguity early} during the replication process, and we can defer to \textbf{confirm the set equality later} (with subtle cost) during the sync process among replicas.} 

==> old/old_dom.tex <==

%~\footnote{According to our measurement in Google Cloud, the reordering rate can reach more than 30\% with the throughput of 80K reqs/second.\todo{30\% is not accurate, it is the fraction of gap triggered in NOPaxos, not the fraction of packet reordering. To be updated with the number of micro-test} }
%and provides relevant interfaces shown in Figure~\ref{dom-interface}. 


% \begin{figure}[!h]
% \vspace{-0.5cm}
%     \centering
%     \begin{tcolorbox}[colback=white!10,%gray background %colframe=black,% black frame colour
%                       width=8cm,% Use 8cm total width,
%                       arc=1mm, auto outer arc,
%                       boxrule=0.5pt,
%                      ]
%     \begin{itemize}[leftmargin=*]
%         \item \texttt{DOMSend}---The client calls it to broadcast its request to replicas with sending time ($s$) and latency bound ($l$) tagged.
%         \item \texttt{DOMReceive}--- The replica calls it to receive the request from the client, and to place the message to either the \emph{early-buffer} or the \emph{late-buffer}.  
        
%         \item \texttt{DOMProbe}--- Both the client and replica call it so that the replica can measure the client-replica \emph{one-way delays} and piggyback it to the client (details in \S\ref{mov-avg-bound}).
        
%     \end{itemize}
%     \end{tcolorbox}
%     \caption{\primname Interfaces}
%     \label{dom-interface}
%     \vspace{-0.4cm}
% \end{figure}


% On the client side, \primname provides \texttt{DOMSend} for the client to broadcast its messages to the replicas. In each broadcast message, \primname also tags the sending time ($s$) and the latency bound ($l$) for this message, with $s$ and $l$ summing up to be the deadline $D=s+l$ for this message to arrive at replicas.

% On the replica side, \primname provides \texttt{DOMReceive} for the replicas to receive the messages from the client, and place the message to one of the two destinations, namely, \emph{early-buffer} and \emph{late-buffer}. The \emph{early-buffer} is implemented as a priority queue, with the deadline of the message as the sorting rank, whereas the \emph{late-buffer} is implemented as a map, indexed by the combination of the client identifier and the request identifier (i.e. <\emph{client-id},\emph{request-id}>). 


%\primname keeps checking the replicas' local clock time to release the request messages from their \emph{early-buffer}s, i.e. when the local clock time has passed the request deadline, this request is released by \primname and passed to the protocol to achieve consensus among replicas. However, not all requests can be destined to the \emph{early-buffer}, because \primname aims to ensure uniform ordering for the requests released from the \emph{early-buffer}. .

%Meanwhile, \primname provides \texttt{DOMProbe} to keep measuring the \emph{one-way delay} (OWD) between the two edges. Once the replicas receive the message from the clients, it can calculate the OWD by using the receiving time minus the sending time ($s$). The OWD stats will be piggybacked to the clients to facilitate the clients to decide more reasonable latency bounds (and correspondingly more reasonable deadlines) for the following messages. More details about the latency bound estimation are described in \S\ref{mov-avg-bound}.

% When equipped with \primname, every replica can see the released requests in uniform ordering (of the deadlines). However, set equality is not guaranteed among replicas: The request may be placed into the \emph{early-buffer}s on some replicas and finally appended to replica logs, whereas it may fail to satisfy the entrance condition of the \emph{early-buffer} on the other replicas (possibly due to clock skew, latency variance, etc) and be left in their \emph{late-buffer}s. Nevertheless, such a uniform ordering guarantee has already eased the burden for the replication protocol. \S\ref{sec-protocol} will describe the protocol to reach set equality, thus leading to the consistency among replicas. 

%Anirudh: This monotonicity discussion can be moved to the appendix because it doesn't affect correctness.
%We preserve the \emph{locally monotonically increasing property} for every clock used in \primname~\footnote{Huygens periodically corrects the clocks with an offset and a negative offset causes the clock to violate the monotonically increasing property. To preserve the locally monotonically increasing property for each clock, DOM records the return value every time the clock API is called. When the clock value is smaller than the last returned one, DOM simply disposes it and retry the clock API, until it returns a larger value.}. So long as the requests arrive before their deadlines, replicas can see a uniform release order (i.e. the ascending order of their deadlines) of these requests, even if they are reordered in the network. 

==> other-refine.tex <==
\subsection{Optimization of Commit Latency}
\label{optim-commit}
\todo{Rephrase a bit }
\todo{3 figures of 4.1. give a table of default values, default change to Read-100, default change to Key 1}



% \vspace{-0.2cm}
% \begin{figure*}[!h]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%     \includegraphics[width=5.8cm]{figures/exp/optim1-20pt.pdf}
%     \vspace{-0.5cm}
%     \caption{Comparison of FCR and CL\ \ \ \ }
%     \label{eval-optim-commit}
%     \end{minipage}\hfill
%     \begin{minipage}{0.32\textwidth}
%     \includegraphics[width=5.8cm]{figures/exp/optim2-1-20pt.pdf}
%     \vspace{-0.5cm}
%     \caption{Comparison of FER and EL (different read ratios) }
%     \label{eval-optim-exec-1}
%     \end{minipage}\hfill
%     \begin{minipage}{0.32\textwidth}
%     \includegraphics[width=5.8cm]{figures/exp/optim2-2-20pt.pdf}
%     \vspace{-0.5cm}
%     \caption{Comparison of FER and EL (different skew factors) }
%     \label{eval-optim-exec-2}
%     \end{minipage}
%     \vspace{-0.6cm}
% \end{figure*}
The overall commit latency (CL) of \sysname is closely related to the ratio of requests committed in the fast path (i.e. fast commit ratio). However, as the throughput grows, we notice the fast commit ratio (FCR) drops seriously. With a fixed latency bound of 80$\mu s$, the FCR of vanilla \sysname drops from 68.2\% to 16.4\% as the throughput increases from $\sim$20 K requests/second to $\sim$96 K requests/second. 
%Under high throughput, replicas need to process more requests, making set inequality occur more frequently (i.e. some replicas accept a specific request whereas the others reject it). Once set inequality occurs due to the inconsistent replica actions towards a specific request, all the subsequent requests cannot obtain a super quorum of \emph{fast-reply} messages with consistent \emph{hashes}. Therefore, they cannot be committed in the fast path, until the set inequality is fixed via the index synchronization process. Meantime, the set inequality may recur due to the inconsistent replica actions towards another request.    

The reason for the drop of FCR is because the hash consistency of \emph{fast-reply} is \emph{too sensitive} to the acceptance/rejection of \emph{every} request. Two replicas fail to reply with consistent hashes so long as they take different actions towards any one request. 
Increasing the latency bound can improve the likelihood for a super quorum to accept the same request, thus increasing FCR. However, it also makes requests held by the \emph{H/R buffer}s for longer time, thus undermining the benefit of the fast path. 

%A commit acknowledgement guarantees that the request is durable and will be eventually executed by the leader. Such acknowledgements are useful for requests which do not care about the execution results. 

In order to improve FCR without adding extra latency, we decouple commit from execution in \sysname. \sysname requires consistent \emph{hash}es to ensure the consistent replica states among a super quorum, so that the consistency property is preserved during recovery. However, such a stringent requirement becomes unnecessary when requests do not return execution results or the results are not important. For instance, typical logging systems or storage systems execute write requests but have no execution results~\cite{conext20-domino,hpdc14-rs-paxos,fast20-coded-raft}. Some transaction systems~\cite{vldb14-available-transaction,middleware15-swiftcloud} allow reading stale data, so the fresh execution result is not urgently needed and can be fetched later. 

To enable fast commit for requests which do not care about the execution result, we also add the request's \emph{deadline} in the \emph{fast-reply}, indicating the request is appended to the replica's \emph{log} with the \emph{deadline} as the ordering rank. The client considers a request as committed when it receives a super quorum (including the leader) of \emph{fast-replies} in the same view, which include consistent \emph{deadline}s. Compared with the original requirement of consistent \emph{hash}es, the consistency of \emph{deadline}s is much easier to attain, since it only requires the super quorum to append this request with the same rank, regardless of their inconsistent actions towards the other requests.


The requirement of consistent \emph{deadline}s is necessary. Towards a specific request, different replicas may reply to the client with inconsistent \emph{deadline}s because of two reasons. First, the leader may modify the \emph{deadline} of the request with its current clock time whereas some followers may directly accept the unmodified request (\S\ref{sec-fix-set-inequality}). Second, the client retries the request with different submission time (\S\ref{sec-timeout}) when timeout is triggered, causing some replicas to accept the previous request but the others to accept the retried one. A super quorum of \emph{fast-replies} with inconsistent ranks introduce ordering ambiguity and do not guarantee durability during recovery.
%~\footnote{Consider the leader and $f$ followers accept the request with an ordering rank, and the other $f$ followers accept the retried request, which has the same $<\emph{client-id}, \emph{request-id}>$ but with a different ordering rank. Without the requirement of consistent ordering rank, the client will consider the request as committed. However, the requests with different ordering ranks are not treated as the same entry in Step 6 of the recovery procedure (\S\ref{sec:recovery}), and the request may not be recovered to the \emph{new-log}.}.

% \textbf{Strategy evaluation.} To evaluate the effectiveness of the strategy, we run \sysname with 3 replicas and 10 open-loop clients. Each client uses a Poisson process to schedule requests. We fix the latency bound as 80 $\mu s$ and vary the throughput (load) by increasing the rate of the Poisson process. Then, we compare FCR and the mean of CL between vanilla \sysname and the optimized version.


% As shown in Figure~\ref{eval-optim-commit}, the gap between vanilla \sysname and the optimized version increases as the throughput grows. The FCR of vanilla \sysname drops significantly, because the hash consistency is sensitive to replicas' behavior towards \emph{every} previous requests. Correspondingly, since most requests can only be committed through the slow path, the CL also increases.
% By contrast, the optimized version only checks \emph{rank} consistency, so it enjoys a much higher FCR and lower CL than vanilla Nezha. 





% we conduct an optimization strategy by taking the request type (i.e. read or write) into consideration. 

% As for the read request, its execution result is not affected by the other read requests. Therefore, while sending the \emph{fast-reply} for the read requests, the hash value only needs to encode all the previously appended write requests in the replica's \emph{log}. In this way, even the replicas take different actions (acceptance or rejection) towards the other read requests with smaller ranks, the inconsistency does not reflect from the \emph{fast-reply} message, thus improving the probability for the read request to commit in the fast path. 

% As for the write request, it modifies the replica state but has no execution result. The only concern to commit a write request is to ensure its ordering rank is consistent among replicas~\footnote{The ordering rank may be inconsistent among replicas due to two reasons. First, the leader may modify the ordering rank of the request with its current clock time (refer to \S\ref{selective-acceptance}). Second, the client retries the request with different submission time (refer to \S\ref{quorum-check}) when timeout is triggered. Therefore, it is possible for some replicas receiving the previous request whereas the others receive the retried ones. }, so that it does not introduce ordering ambiguity and damage the correctness after recovery~\footnote{Consider the leader and $f$ followers accept the request with an ordering rank, and the other $f$ followers accept the retried request, which has the same $<\emph{client-id}, \emph{request-id}>$ but with a different ordering rank. Without the requirement of consistent ordering rank, the client will consider the request as committed. However, the requests with different ordering ranks are not treated as the same entry in Step 3 of the recovery procedure (\S\ref{sec:recovery}), and the request may not be recovered to the \emph{new-log}.}. Therefore, as an optimization, we add one additional field $rank$ in the \emph{fast-reply} message, which indicates the ordering rank of the request when it is accepted by the replica. While handling the \emph{fast-reply} messages for the write request, the client checks the consistency of the $rank$ fields instead of the $hash$ fields. Compared with the \emph{hash} field, it is much easier to form a super quorum (including the leader) of \emph{fast-reply} messages with consistent \emph{rank} value, because it only requires the replicas accept this request without caring about the acceptance of the other requests before this request.

%The write request is considered as committed if it receives the corresponding \emph{fast-reply} messages from  $f+\lceil f/2 \rceil + 1$ replicas (including the leader) with consistent $rank$ values. 

==> refinement.tex <==
\vspace{-0.5cm}
\section{Optimization}
\label{sec:refinement}
\vspace{-0.2cm}



\subsection{Optimization of Execution Latency}
\label{optim-execution}
The strategy of CL optimization only benefits those requests which have no execution results, or the results are not important. It is not globally sufficient, because there are also many practical scenarios where clients depend on the execution result returned by previous requests. For example, the write requests to Zookeeper~\cite{zookeeper} and Redis~\cite{redis} also have execution results. Using stale results in some banking systems may cause business errors. In such user cases, the execution latency (EL) becomes the key factor affecting the performance.

% The read/write optimization introduced in \S\ref{read-write-optim} improves the fast commit ratio for both read and write requests. However, compared with the read requests, the write requests can commit through the fast path more easily.

To further optimize EL, \sysname considers two facts to refine hash computation, so that the hash consistency can be easily reached and the request can be committed in the fast path. First, read requests do not modify replica states. Therefore, the \emph{hash} field in the \emph{fast-reply} do not need to encode the previous read requests. Second, most requests are commutative in practical scenarios~\cite{nsdi19-curp}. For example, the execution result of the request ``{read} $x$'' is not affected by the other request ``$y \xleftarrow{} 5$''. Therefore, the $hash$ field in the \emph{fast-reply} only needs to encode all of the non-commutative requests previously appended to the \emph{log}. Based on the two facts, \sysname is able to prune the hash computation and reduce its sensitivity to replica's inconsistent actions. 

\sysname maintains a table of per-key hashes for the write requests. For every newly appended write request, the replica will XOR its hash to update the corresponding entry in the table according to its key. While sending the \emph{fast-reply} for a specific request, the replica only includes the hash of the same key. For compound requests which is non-commutative with multiple keys (e.g. ``move 10 from $x$ to $y$ and return $x$ and $y$''), the replica fetches the hashes of all the relevant keys (e.g. $x$ and $y$), and includes the XORed hash value (e.g. $hash_x \oplus hash_y$) in the \emph{fast-reply}.

Compared with the original \emph{hash}, the refined \emph{hash} can reach consistency more easily. It only requires the super quorum to accept the same set of previous write requests which are not commutative to the target request, and it is not sensitive to replicas' inconsistent actions towards the previous read requests or commutative write requests.

We evaluate the two refinement strategies ( \S~\ref{optim-commit} and \S~\ref{optim-execution}) under a wide range of workloads and proves their effectiveness. 

% \textbf{Strategy evaluation. }To evaluate the effectiveness of the strategy, we also run vanilla \sysname and the optimized version in the same setting. This time we fix the Poisson rate to maintain a nearly constant throughput ($\sim$96K requests/second), and use two different series of workloads. For the first series, we make all the requests operate on one single key, and vary the read ratio from 0\% to 100\%. For the second series, we maintain 1 million keys and fix the read ratio as 0\% (i.e. complete write workloads). We use a Zipfian distribution to generate workloads with different skew factors varying from 0 to 0.99.
% %~\footnote{A skew factor of 0.99 represent highly skewed workload, whereas a skew factor of 0 represent an evenly distributed workload.}. 
% Then we compare the fast execution ratio~\footnote{The ratio of requests which can obtain execution result in fast path.} (FER) and the mean of EL between vanilla \sysname and the optimized version.

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=8cm]{figures/exp/optim2-1.pdf}
%     \caption{Comparison of fast execution ratio (FER) and execution latency (EL) under the first series of workloads }
%     \label{eval-optim-exec-1}
% \end{figure}



% The comparison under the first series of workloads is shown in Figure~\ref{eval-optim-exec-1}. Regarding both FER and EL, the gap between vanilla \sysname and the optimized version increases as the read ratio grows. This is because the hash consistency of the optimized version is only sensitive to the previous write requests, whereas vanilla \sysname is sensitive to all previous requests. Therefore, a high read ratio is more favorable to the optimized version. Such a property is especially desirable in read-intensive workloads, which are very common in practice~\cite{sigmetric12-workload-analysis, socc14-read-lease, fast14-eval-storage, osdi20-pegasus, osdi20-twitter-analysis}.

% % \begin{figure}[!htbp]
% %     \centering
% %     \includegraphics[width=8cm]{figures/exp/optim2-2.pdf}
% %     \caption{Comparison of execution latency (mean value) under the second series of workloads }
% %     \label{eval-optim-exec-2}
% % \end{figure}
% The comparison under the second series of workloads is shown in Figure~\ref{eval-optim-exec-2}. The optimized version enjoys higher FER and EL for every skew factor. Since the key space is large (1 million keys), even for the most skewed workload (i.e. skew factor = 0.99), the hottest key only occupies 12.9\%, so the probability is very low for two adjacent requests to be non-commutative~\footnote{The probability is about $12.9\%\times12.9\%\approx 1.66\%$}. In most cases, even if replicas take inconsistent actions towards previous non-commutative requests, there is sufficient interval to sync them and correct the hash, so that the replicas can still reply with the consistent hash for the current request.

% The gap between vanilla \sysname and the optimized version increases as the skew factor declines. A smaller skew factor indicates the requests are more evenly distributed across the keys, thus improving the ratio of commutative requests. Therefore, the optimized version yields more chance to attain hash consistency among a super quorum of replicas and obtain the valid execution result in the fast path.



\subsection{Dynamic Latency Bound}
\label{mov-avg-bound}
\vspace{-0.1cm}
The latency bound is the key parameter that introduces a trade-off between FCR/FER and the overall latency. A large latency bound can increase FCR/FER, but also leads to longer waiting time in the \emph{early-buffer}s, and vice versa. Since the workload can be various, and inter-VM latency is also time-varying in cloud~\cite{nsdi13-bobtail,nsdi15-c3}, a dynamic latency bound is more desirable than a fixed empirical value.

% Thanks to the high-precision clock synchronization, \sysname is able to measure the one-way delay (OWD) between clients and replicas more accurately. Since the client tags the sending time in the request, the replicas can calculate OWD of the request by simply subtracting its submission time from its arrival time.

We previously intend to use the moving average to estimate the client-replica OWD. Later we found that, under high workload, the moving average values can be much elevated by a few super large outlier samples. To make the OWD estimation more robust, we turn to use the moving median value as the estimation. Replicas maintains a sliding window for each client, which records the OWDs of the client requests. Periodically, replicas calculate the median value in the window for each client and piggyback it in the \emph{fast-reply/slow-reply}. The client uses the estimated OWDs to decide the latency bound for the subsequent requests, i.e.
\vspace{-0.2cm}
\begin{equation*}
\vspace{-0.1cm}
    d_1 = \underset{0 \leq i \leq 2f}{\max}\{owd_i\}
\end{equation*}

where $owd_i$ is the estimated OWD between the client and the replica whose \emph{replica-id} is $i$.

In case that clock synchronization fails, which leads to very large or negative $d_1$, we also add a default value $d_0$ to decide the latency bound, i.e. when the output $d_1$ is invalid due to clock synchronization failure, \sysname falls back to use the fixed value $d_0$ as the latency bound.
\begin{equation*}
    l = \begin{cases}
      d_1 & \text{if $0<d_1<d_0$}\\
      d_0 & \text{otherwise}
    \end{cases} 
\end{equation*}

We believe that more elaborate tuning algorithms exist. For example, other percentiles instead of the median value may provide a better estimation of OWD; when OWDs have very large variance across replicas, a thrifty design is to set $d_1$ as the max OWD among a super majority of replicas rather than the max among all replicas. We leave the exploration of such designs in our future work.


==> scratch/TODO <==
0. Why synchronize gateways (as opposed to market participants)?
1. orders vs. in order. ambiguous terms. 


0a. Add FIFO Case and also delete 0-delay case. Make it a bar chart with whiskers. 4 Values: {NO RESEQ, 250, 500, 700}

Market data unfairness bar chart - Ahmad's new metric.

4c - also make it a bar chart.

0b. Inherent Unfairness - explain that this is w/ delay 0.

Discuss intrinsic unfairness in all cases


later on (non infra work)
  - matching engine batch auctions, multiple markets

----------------------

Need to be consistent:

8. Let's use paragraphs instead of subsubsections.
9. space between 0 and ms in 0ms (7.2 here: https://www.nist.gov/pml/special-publication-811/nist-guide-si-chapter-7-rules-and-style-conventions-expressing-values)

10. Footnotes shouldn't break pronunciation.
11. textbf vs. \Para{}. Let's use \Para{}

==> scratch/background.tex <==
\section{Background}

% Auctions, Order Types, Matching Engine Simulators

Electronic exchanges facilitate the rapid buying and selling of financial instruments such as shares, bonds, and futures. At the infrastructure level, these stock exchanges consist of three kinds of entities. First, matching engines are responsible for matching buyers and sellers and executing trades. Second, market participants are responsible for placing orders for various financial instruments, whose unique identifier is denoted as a symbol. Third, gateways are responsible for authenticating and routing orders from market participants to the matching engines.

This stock exchange infrastructure needs to ensure low latency from the matching engine to the different participants because participants are increasingly algorithms issuing orders at significantly shorter timescales than humans. The infrastructure also needs to ensure low latency variability between the matching engine and different participants. This is to ensure that the infrastructure is fair to market participants, not giving any one participant a speed advantage over others. We define an exchange's notions of fairness precisely below.

In the inbound direction, i.e., from the market participant to the matching engine, an order is unfairly processed at the matching engine if it processed by the matching engine earlier than an order with an earlier arrival time at the gateway. In other words, orders must be processed at the matching engine in order of their arrival timestamps even if one order overtakes another in the path from the gateway to the matching engine. In the outbound direction, i.e., from the matching engine to the market participants, unfairness arises if market data (e.g., the new price of a symbol), which is multicasted from the matching engine to the gateways, arrives at one gateway earlier than another.

Exchanges achieve low unfairness in both inbound and outbound directions by carefully measuring and equalizing cable lengths between the gateways and the matching engines. In this paper, we propose a different approach based on scalable software time synchronization where the matching engines and gateways are all synchronized to the same time reference.  This approach has the benefit of being deployable on commodity hardware in the public cloud without requiring bespoke engineering.

Once the gateways and matching engine have been synchronized, for the outbound direction, we can declare a certain global release time at which market data must be simultaneously released to all market participants. For the inbound direction, we can enforce a minimum delay requirement relative to the gateway arrival timestamp to ``wait out'' the variability in network paths between the gateways and matching engine.
% Define in-bound and out-bound fairness.
% Define low latency requirements.

==> scratch/cloudex.tex <==
%% TODO: Maybe some motivation and design goals of the cloudex.
%% Rapid price discovery: fairness and liquidity.
% \newcommand{\sysname}[0]{\texttt{CloudEx}\xspace}
\section{Design}
\label{sec:cloudex}

\sysname is a a fair-access stock exchange designed to run on commodity hardware and networks available in the public cloud---in contrast to today's stock exchanges which are engineered with bespoke hardware and networks. In this section, we  describe the system architecture of \sysname and evaluate the level of fairness that it provides when run on jitter-prone public cloud infrastructure.

\subsection{System Architecture}
The full exchange ecosystem consists of traders, gateways, a central exchange server, and cloud storage. Figure \ref{fig-arch} summarizes this architecture. Each gateway clock is precisely synchronized to the reference clock of the central exchange server.
%, defining the system's time perimeter.
%\as{Can we show in the diagram that: (1) all gateways are connected to the cloud server by bidirectional arrows and (2) the time perimeter encapsulates, rather than runs through the gateways? This might go better with the current thinking of time perimeters as an area, rather than as a one-dimensional concept. We could even shade the time perimeter box.}

\begin{figure}[h]	
	\centering
	\includegraphics[width=8cm]{fig/sys_v3.pdf}
	\caption{System Architecture of \sysname}
	\label{fig-arch}
	\vspace{-0.15in}
\end{figure}

\Para{Traders.} Each trader owns a VM that is connected to one of the exchange gateways. The traders are provided an API that allows them to (1) submit orders and receive order and trade confirmations, (2) subscribe to real-time market data streams, and (3) query for historical market data from a long-term cloud storage module (for brevity, we've omitted the this module from Figure \ref{fig-arch}). Placing an order involves constructing an order message and forwarding it to the assigned gateway. An order message consists of the symbol to be traded (e.g., a stock or futures contract), the action (buy or sell), the number of shares, the order type (limit order~\cite{SECgovLimitOrder:online} or market order~\cite{SECgovMarketOrder:online}), and the limit price for limit orders. 
% Limit orders execute at a variable future time when the symbol reaches the fixed limit price, while market orders execute immediately but with the market price.

\begin{figure}[h]
	\centering
	\includegraphics[width=8cm]{fig/life_v3.pdf}
	\caption{Lifecycle of an Order in \sysname}	
	\label{fig-order-lifecycle}
	\vspace{-0.15in}
\end{figure}

\Para{Gateways.} The gateways sit between the traders and the central exchange server, routing orders to the central exchange server and sending market data to the traders. Each gateway hosts two modules: an order handler and a hold/release (H/R) buffer. The order handler validates and assigns a timestamp to orders received from the traders before forwarding these orders to the central exchange server. The order handler is also responsible for routing order confirmations received from the central exchange server back down to the traders (Figure \ref{fig-order-lifecycle}). Meanwhile, real-time market data received from the central exchange server is dispensed to each market participant via the H/R buffers. Each H/R buffer {\em holds} a given atomic piece of data until the prescribed {\em release} time for that piece of data. Precise clock synchronization and identical release times guarantee that market data is simultaneously dispensed to all market participants.

%\label{sec:ces} 
\Para{Central Exchange Server.} The central exchange server hosts two modules: the sequencer and the matching engine. The sequencer receives inbound orders from the gateways and enqueues each received order into a priority queue based on the order's gateway-assigned timestamp. 

\begin{figure}[!t]
\centering
% \vspace{-0.15in}
    \begin{subfigure}[t]{0.3\textwidth}
	\includegraphics[width=\textwidth]{fig/lob.pdf}
	\vspace{-0.9in}
	\end{subfigure}
	\caption{Visualization of a Limit Order Book}
\vspace{-0.15in}
\label{fig-lob}
\end{figure}

% ; i.e., at least one buyer and seller agree on a price
The matching engine dequeues orders from this priority queue and runs what is called a ``continuous price-time matching'' algorithm~\cite{cptm}. It maintains two principal data structures: limit order books (Figure~\ref{fig-lob}) that store unmatched limit orders, and a portfolio matrix that tracks each market participant's assets and cash balance. The limit order book for each symbol stores the bids (buy orders) and asks (sell orders) for that symbol. The bids are sorted in order of decreasing limit price, and the asks sorted in order of increasing limit price. Incoming orders are matched to orders in the limit order books to produce trades. 
In our implementation, we shard the matching engine, with each shard connected to its own order priority queue and containing the limit order books of a subset of symbols. Orders are then routed to the shard corresponding to its symbol.
Orders are matched when either an incoming bid (ask) specifies a price greater (respectively, lesser) than or equal to the lowest ask (respectively, highest bid) in the order book. Limit orders that cannot be fully matched are added to the books.

After each order is processed, an order confirmation is generated and sent to the appropriate gateway's order handler (Figure~\ref{fig-order-lifecycle}). 
When a trade is executed, the portfolio matrix is updated and a record of the trade is generated. Trade records consist of the symbol that was traded, the number of shares traded, and the execution price, and are persisted in Google Bigtable~\cite{bigtable}. Traders are provided an API through which they can query for historical market data from Bigtable.

% Let $\{S_1,...,S_m\}$ denote the set of tradable symbols that the exchange supports, and let $\{P_1,...,P_n\}$ denote the set of market participants (traders). The matching engine maintains two principal data structures: limit order books $\{L_1,...,L_m\}$ that store unmatched limit orders \cite{limit-books}, and a portfolio matrix $P \in \mathbb{R}^{(m + 1) \times n}$ that stores the assets owned by each market participant. Specifically, $P_{ij}$ represents the number of units of symbol $S_i$ owned by participant $P_j$ for $i \in \{1,...,m\}$, while $P_{m+1,j}$ represents the cash balance of participant $P_j$. Limit order book $L_i$ stores the bids (buy orders) and asks (sell orders) for symbol $S_i$, the bids sorted in order of increasing limit price, and the asks sorted in order of decreasing limit price (see fig. \ref{fig-lob}). Orders are processed sequentially; after each order is processed, an order confirmation is generated and sent to the appropriate gateway's order handler (see fig. \ref{fig-order-lifecycle}). A trade is generated when either an incoming bid specifies a price point greater than or equal to the lowest ask in the order book or an incoming ask specifies a price point less than or equal to the highest bid in the order book, i.e., the buyer and the seller agree on a price). If an incoming order cannot be matched, it is considered unfilled and is placed in the appropriate limit order book where it awaits potential future matches.

% A limit-order trade is executed when either an incoming bid (ask) specifies a price greater (respectively, lesser) than or equal to the lowest ask (respectively, bid) in the order book; i.e., at least one buyer and seller agree on a price. If an incoming order cannot be matched, it is considered unfilled and is placed in the appropriate limit order book where it awaits potential future matches. Market order trades are executed immediately at the current price of the symbol, and unfulfilled portions of a market order are placed in the limit order book at a price specified in the market order.

%(cash is transferred from the buyer to the seller and shares are transferred from the seller to the buyer)

% \begin{subfigure}[t]{0.23\textwidth}
%      \centering
%      \includegraphics[width=\textwidth]{fig/exp02-downstream-fairness.png}
%      \caption{Market Data Unfairness}
%      \label{exp02-downstream-fairness}
% \end{subfigure}

% \as{Is third party important here? Third party with respect to what?}
% Vig - it is not particularly important.

The final function of the matching engine is to provide real-time market data streams to the traders via the H/R buffers. Market data consists of both trade records and periodic snapshots of the limit order books. Traders subscribe to this data on a per-symbol basis. Before trade records and limit order book snapshots are forwarded to the gateways, the matching engine assigns a release timestamp that specifies when the gateways ought to dispense each piece of market data to the traders (Figure~\ref{fig-order-lifecycle}).


\subsection{Dynamic Delay Parameters}
% - Introduce the method, how it works
%   - Scheduled Delivery queues
%   - Ordered Delivery queues
% - Describe the implementation, metrics observed and optimized

\subsubsection{Delay Parameters} From our description of ordered and synchronized delivery queues in Section \ref{sec:perimeters}, we introduced two delay parameters -- the ordered delivery and the synchronized delivery delay parameters -- that help determine how fair and fast information deliver will be. We first define the fairness metrics for fair and synchronized delivery and consequently introduce the delay parameters responsible for these metrics.

\textbf{Ordered delivery unfairness} Ordered delivery unfairness is defined as the percentage of total orders that are processed out of sequence. An order is considered to be processed out of sequence when its sender timestamp is earlier than that of the preceding processed order.

\textbf{Ordered delivery delay parameter, $d_{order}$.} To address order unfairness, a sequencing buffer is instructed to hold orders until the delay $d_f$ has elapsed relative to their sender timestamps. In other words, the sequencer dequeues an order $O$ if and only if $t_C - t_O \geq d_{order}$, where $t_C$ represents the current time and $t_O$ represents the sender timestamp of the order. This delay provides orders submitted before $O$ sufficient time to arrive at the processing server and be properly sequenced before order $O$ itself is dequeued.

\textbf{Synchronized delivery unfairness} Synchronized delivery unfairness is defined as the percentage of total pieces of market data that are unfairly disseminated. A piece of synchronized delivery data is considered to be unfairly disseminated if at least one of the receivers obtains the data at a time later than its designated release time.

\textbf{Synchronized delivery delay parameter, $d_{sync}$.} To address market data unfairness, we use hold/release buffers. Consider a piece of market data $M$, and let $t_M$ represent its creation time at the matching engine. The hold/release buffer at each gateway is instructed to release $M$ at time $t_R$, where $t_R = t_M + d_{sync}$. $d_{sync}$ is the maximum time that a piece of market data has to wait in the hold/release buffer before it can be released to the market participants. This delay provides all gateways enough time to receive $M$ from the matching engine before it is time to release $M$ to the traders. 

Determining how to set these two parameters is dependent, among other factors, on application requirements and network conditions. We present an algorithm  that time-sensitive queues use to optimize and dynamically adjust these delay parameters.

\subsubsection{Optimizing Delay Parameters}

We optimize $d_f$ and $d_s$ with Algorithm \ref{delayparamalgo}. In Section \ref{sec:cloudex} we detail the choice of the algorithm inputs for a sample application.

% Algorithms
\begin{algorithm}
\SetAlgoLined
\SetKwInOut{r}{}
 \textbf{Input}: \\ $r$ - target unfairness percent \\ $u_0$ - initial delay parameter \\ $W$ - window size \\ $S(e)$ - step size given an error \\ $f(W, u)$ - fairness given window and delay parameter \\
 \hrulefill \\
 $u \xleftarrow{} u_0$ \\
 \While{true}{
  $e \xleftarrow{} f(W, u) - r$ \;
  $u \xleftarrow{} u + S(e)$ \;
 }
 \caption{Delay Parameter Tuning}
 \label{delayparamalgo}
\end{algorithm}


\subsection{Multi-Gateway Message Submission}
% Intuition about the method (delay parameters adjust towards the tail latency).
% Reducing the tail latency allow us to reduce the delay needed to meet a desired unfairness $r$.
Based on the definitions of delay parameters, we can see that given some target unfairness $r$ we must tune our delay parameters to be at least as large the 100 - $r$ \% latency in expectation. Consequently, reducing tail latency across senders for fair delivery queues and receivers for synchronized delivery queues will allow us to achieve our target unfairness $r$ using smaller values for $d_f$ and $d_s$.

To reduce these tail latencies, we utilize a second technique -- Multi Gateway Message Submission. Simply stated, for fair delivery queues clients create multiple copies of their message and send each copy to one gateway. The fair delivery queue will enqueue the first copy of a message that it receives, thereby selecting the lowest latency transmission across these copies. On the synchronized delivery side, clients subscribe to multiple gateways and receive information from the first gateway which receives a copy of the published information.
% % $\epsilon_u$ (pertaining to upstream messages received from the traders)
% % $\epsilon_d$ (pertaining to downstream messages sent to the traders)

% %Unfairness can manifest itself as orders being processed out of sequence or market data not reaching participants simultaneously.\footnote{This notion of fairness based on latencies is distinct from the traditional notion of fairness in networking which is related to throughput~\cite{jain_fairness}.} 
% %, (2) clock synchronization error and (3) insufficient delay at the sequencer for upstream traffic or the H/R buffers for downstream traffic.

% In practice, it is impossible to build a perfectly fair exchange because of the difference in the propagation delays from the gateways to the matching engine. We quantify how unfair an exchange is through (1) an order unfairness score and (2) a market data unfairness score. In an ideal exchange, both should be zero. To remedy each source of unfairness, we introduce a compensating delay parameter. We explain the sources of unfairness and the delay parameters below.

% \Para{Order unfairness.} Order unfairness is defined as the percentage of total orders that are processed out of sequence. An order is considered to be processed out of sequence when its gateway arrival timestamp is earlier than that of the preceding processed order.

% \Para{Market data unfairness.} Market data unfairness is defined as the percentage of total pieces of market data that are unfairly disseminated. A piece of market data is considered to be unfairly disseminated if at least one of the gateways receives it at a time later than its designated release time. 

% \Para{Sequencer delay parameter, $d_s$.} To address order unfairness, the sequencing buffer is instructed to hold orders until the delay $d_s$ has elapsed relative to their gateway timestamps. In other words, the sequencer dequeues an order $O$ if and only if $t_C - t_O \geq d_s$, where $t_C$ represents the current time and $t_O$ represents the gateway timestamp of the order. This delay provides orders submitted before $O$ sufficient time to arrive at the central exchange server and be properly sequenced before order $O$ itself is dequeued.

% \Para{Hold/Release buffer delay parameter, $d_h$.} To address market data unfairness, we use hold/release buffers. Consider a piece of market data $M$, and let $t_M$ represent its creation time at the matching engine. The hold/release buffer at each gateway is instructed to release $M$ at time $t_R$, where $t_R = t_M + d_h$. $d_h$ is the maximum time that a piece of market data has to wait in the hold/release buffer before it can be released to the market participants. This delay provides all gateways enough time to receive $M$ from the matching engine before it is time to release $M$ to the traders. 

%\subsection{Configurable Exchange Parameters}\label{sec-configurable-ex-params}
% The sequencer and H/R buffers each have delay parameters that are configurable, and influence the fairness properties of the exchange. {\bf Sequencer Delay Parameter, $d_s$:} Consider some order $O$ that is sitting at the front of the sequencing queue, and let $t_O$ represent the gateway timestamp of this order. The sequencer dequeues $O$ if and only if $t_C - t_O \geq d_s$, where $t_C$ represents the current time. Intuitively, $d_s$ is the minimum time an order needs to take between gateway timestamping and being dequeued for processing at the matching engine (regardless of the gateway through which it arrived). To ensure fairness, $d_s$ is set large enough that orders submitted before order $O$ have enough time to arrive at the central exchange server before order $O$ itself is dequeued. {\bf Hold/Release Buffer Delay Parameter, $d_h$:} Consider some piece of market data $M$, and let $t_M$ represent its creation time at the matching engine. The hold/release buffer at each gateway is instructed to release $M$ at time $t_R$, where $t_R = t_M + d_h$. $d_h$ is the maximum time that a piece of market data has to wait in the hold/release buffer before it can be released to the market participants. To ensure fairness, $d_h$ is set large enough to ensure all gateways have received market data $M$ from the matching engine before $M$ is released to traders.

%\label{sec-network-jitter}
% \subsection{The Delay Parameters in Practice [REMOVE?]} 

% Since we run the various components of \sysname on Google Cloud, there is significant variation in the one-way delay (OWD) across the gateways and matching engine. 

% %As explained in Section \ref{sec-configurable-ex-params}, the Sequencer Delay Parameter and Hold/Release Buffer Delay Parameter mitigate the effects of the OWD variation by delaying data processing (in the upstream case) and data release (in the downstream case), respectively. The appropriate values for these delays can be configured by examining measurements of the upstream and downstream OWDs. 

% Table \ref{tb-owd} reveals the extent of the variation when we have 24 market participants and 8 gateways. The 99\textsuperscript{th} percentile OWD in the gateways-to-matching engine direction is \SI{355}{\micro\second}, which implies $d_s$ can be set to \SI{355}{\micro\second} in order to account for most of the OWD variation. Similarly, the 99\textsuperscript{th} percentile OWD in the matching engine-to-gateways direction is \SI{561}{\micro\second}, which gives the corresponding value for $d_h$.


% \newcolumntype{L}{>{\centering\arraybackslash}m{2.5cm}}
% \begin{table}[!t]
% \centering
% \begin{small}
%  \setlength{\tabcolsep}{1mm}
% \begin{tabular}{|l|c|c|c|c|c|}
% \hline
% \begin{tabular}{l} \textbf{One-Way Delay (\SI{}{\micro\second})}  \end{tabular} & 
% \begin{tabular}{l} \textbf{1p} \end{tabular} & 
% \begin{tabular}{l} \textbf{25p}  \end{tabular} & 
% \begin{tabular}{l} \textbf{50p} \end{tabular} &  
% \begin{tabular}{l} \textbf{75p}  \end{tabular} & 
% \begin{tabular}{l} \\ \textbf{99p}  \\ \\ \end{tabular} \\
% \hline

% \begin{tabular}{l}  \textbf{Upstream:}  Gateways $\xrightarrow{}$\\ Matching Engine  \\ \end{tabular} & 
% \begin{tabular}{l}    120 \end{tabular} & 
% \begin{tabular}{l} 153 \end{tabular} & 
% \begin{tabular}{l} 172 \end{tabular}& 
% \begin{tabular}{l}199 \end{tabular} & 
% \begin{tabular}{l} \\ 355 \\ \\ \end{tabular} \\ \hline 

% \begin{tabular}{l}
% \textbf{Downstream:} Matching \\ Engine $\xrightarrow{}$ Gateways \end{tabular} & 

% \begin{tabular}{l} 86 \end{tabular} & 
% \begin{tabular}{l} 124 \end{tabular}  & 
% \begin{tabular}{l} 146 \end{tabular} & 
% \begin{tabular}{l} 179 \end{tabular} & 
% \begin{tabular}{l} \\ 561 \\ \\ \end{tabular}  \\ \hline 
% \end{tabular}

% \end{small}
% \caption{OWD Measurements in \sysname Testbed}
% \label{tb-owd}
% \end{table}



% \as{Commenting out the equation because it seemed to suggest that the concept was more complicated than it actually is :) A figure might be helpful here though if we have space.}

%More precisely, let $t_1, t_2, ..., t_r$ respectively represent the timestamps of orders $O_1, O_2, ..., O_r$, where $O_i$ is pulled off the sequencing buffer just after order $O_{i-1}$. Then, the order (upstream) unfairness score $\epsilon_u$ is defined as follows:
%\begin{equation*}
%   \epsilon_u = \frac{\sum_{i=2}^r{1\{t_i < t_{i-1} \}}}{r}
%\end{equation*}

% measures the average release time discrepancy across all pieces of disseminated market data. For a given piece of market data, we define the release time discrepancy as the difference between the latest and earliest gateway release timestamps. 

%More precisely, in an exchange with $p$ gateways that releases $q$ atomic pieces of market data over its lifetime, let $T \in \mathbb{R}^{p \times q}$ denote the release time matrix. Specifically, $T_{ij}$ is the absolute time at which gateway $i$ released the $j^{th}$ piece of market data. Then, the market data (downstream) unfairness score $\epsilon_d$ is defined as follows:

%\begin{equation*}
%    \epsilon_d = \frac{1}{q}\sum_{j = 1}^q\left[\max(T_{1j},...,T_{pj}) - \min(T_{1j},...,T_{pj})\right]
%\end{equation*}

==> scratch/format_commands.tex <==
% Footnote settings
% \def\footnoterule{\kern-3\p
%   \hrule \kern 2.6\p} % the \hrule is .4pt high
% \makeatother

==> scratch/future_work.tex <==
\section{Future Work}
\label{ssec:futurework}
Currently, there is significant OWD variance across upstream and downstream paths because of multiple software layers in each path. The use of NIC hardware timestamps can reduce the variance in OWD by removing the latency variance associated with these layers. NIC timestamps are available on Azure (Accelerated Networking~\cite{azure-an}) and AWS (Enhanced Networking~\cite{aws-en}).  A reduction in OWD variance would enable us to reduce the delays at the sequencer and H/R buffers while maintaining fairness. 

There is also software stack latency in \sysname associated with zmq~\cite{zeromq}, a message passing library that offers a pub-sub abstraction on top of TCP. Replacing this with a lower-level interface like sockets will reduce order and market data latency. In turn, this would allow a smaller delay without unfairness.

\todo{open problems (applying this to games, lower latency through DPDK)}

  
  

==> scratch/hotnets_reviews.tex <==
Overall merit
-------------
1. Reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This paper attempts to address the requirements of time-sensitive
applications such autonomous cars, stock exchanges, and multiplayer
gaming. These requirements include jitter-free message delivery,
synchronized multicast and application-specific actions based on
global timestamps. Already existing proposals to address needs of such
applications include the Time-Sensitive Networking (TSN) framework
from IEEE and the DetNet proposal from IETF. These proposals take a
network-oriented approach and require the entire network to always
support stringent requirements such as clock synchronization without
considering the application's needs. This paper proposes an
abstraction called "time perimeter" which takes an application-aware
approach to time-sensitive applications. A time perimeter is a subset
of network nodes of two types: (i) Sensor nodes whose clocks are
synchronized to a reference clock and which apply timestamps to the
packets originating at or passing through them. (ii) Control nodes
which execute application-specific action based on the timestamps
applied by the sensor nodes. The paper presents a case study of using
time perimeters to build a stock exchange in public cloud. The paper
also claims time perimeter to have use cases in distributed systems,
networking and microservices monitoring.

Reasons to accept
-----------------
- None

Reasons to reject
-----------------
- Lack of a clear research contribution

- The claimed uses cases of time perimeter (section 3) are in fact use
  cases of the underlying time synchronization. Not clear what is the
  value of the proposed abstraction.

- Doesn't explain or quantify how time perimeter fares better than TSN
  or DetNet.

- CloudEx case study does not clearly explain the advantage of the
  proposed approach compared to bespoke solutions for real world stock
  exchanges.

Comments for author
-------------------
1. It is not clear to this reviewer what exactly is the research
   contribution. The proposed "abstraction" is pretty straightforward
   - use a highly accurate state-of-the-art time synchronization among
   a subset of nodes depending on the application. For the highly
   accurate and scalable time synchronization protocol, it is already
   available and is being used off-the-shelf. As for identifying a
   subset of nodes, it is pretty straightforward given a
   time-sensitive application e.g. for an autonomous car's central
   processing unit to be able to drop a delayed frame from an image
   sensor, it is pretty straightforward that the image sensor and the
   central processing unit are the subset of nodes to be
   synchronized. It is unclear what exactly is being *abstracted* by
   the "abstraction". There is only a brief mention of a control plane
   API to add and remove nodes from time perimeters and a data plane
   API to retrieve the node's current estimate of time wrt a time
   perimeter. Both APIs are pretty straightforward and the authors
   mention no challenges in providing these APIs.

2. Section 3 lists use cases of time perimeter. This reviewer is not
   convinced how these are the uses cases of the time perimeter
   abstraction and not that of the underlying time
   synchronization. What is it that time perimeter contributes to
   enable these use cases? Were these use cases not possible before
   the time perimeter abstraction? With a good clock synchronization
   mechanism, VMs at different locations can be snapshotted at a
   designated time without requiring coordination. The same applies
   for: (i) obtaining one-way delay in networking and its
   applications. (ii) using non-local timestamps for switch scheduling
   algorithms. (iii) correlating timestamps of logs across
   transactions in microservices. Claims like time perimeters
   providing a cheaper approach to implement Fastpass (SIGCOMM '14)
   are not substantiated with an explanation of how and why.

3. The paper introduces CloudEx as a case study to demonstrate how a
   time-sensitive application can be built in a public cloud using
   time perimeters.  First, no implementation details of CloudEx show
   how the timer perimeter "abstraction" is being used. Second, the
   case study doesn't quantify how time perimeter has fared better
   than TSN or DetNet approaches which are the closest related works
   and whose shortcomings were described as the motivation for an
   application-aware approach like the time perimeter. Third, the case
   study's purpose is to demonstrate that a stock exchange can be
   built in the public cloud. However, the evaluation of CloudEx fails
   to put the numbers in perspective of running a real world stock
   exchange. For example, is the throughput of 17.3k orders per second
   with 0.3% order unfairness good enough for a real world stock
   exchange? How does the 7.9% market data unfairness of CloudEx (72
   traders, 24 gateways) compare to today's stock exchanges that use
   bespoke solutions? Without this perspective, it is not possible to
   consider the presented results as promising or demonstrating of the
   claim that a time-sensitive application can be built in a public
   cloud using time perimeters.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #246B
===========================================================================

Overall merit
-------------
1. Reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
Time Perimeters is time synchronization approach proposed for
time-sensitive applications deployed in public cloud ecosystems. While
most of the paper is motivated by and discusses Cloud Exchange use
case, the authors attempt to generalize their proposal by discussing
Time Perimieter APIs. Using the Time Perimeters approach the authors have built a CloudExchange solution. This various fairness metrics have been studied using this application.

Reasons to accept
-----------------
It is difficult to figure out what the difference from prior work like virtual clocks, clock synchronization like Huygens referred to in the paper. The two key insights seem to be doing synchronization for a subset of nodes and artificially delaying the packets in the gateways to improve the fairness across various actors in the participating ecosystem.

Reasons to reject
-----------------
The proposed approach is most likely not going to be acceptable beyond
a selected use case. Prior studies have indicated reluctance from
online gamers towards addition of any sort of artificial delays for
fairness. Even the CloudExchange usecase will face similar issues it
real market was to be run on such an exchange. Setting of the delay
parameters seems sensitive to jitter in the system and difficult to
choose.

Comments for author
-------------------
While the authors focus on fairness in the system, fairness is not the primary metric for variety of time-sensitive application. In particular the online gamers prefer a better experience to fairness based on aritifically induced dealys.

The evaluation section primarily focusses on the sensitivity analysis of various configuration parameters of the system like Sequencer delay paramter or Hold/Release buffer delay parameter. The authors should show evaluation results in terms of fairness with global clock synchronization. As well as the reduction in synchronization overhead with their proposed approach of Time Perimeters.

It seems that the delay parameters have to be increased as the jitter in OWD increces (Table 1). As the size of the participants increase, so will the OWD jitter as well. Thus limiting the applicability space for the proposed approach.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #246C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper presents a cloud-based system for ensuring global FCFS ordering for trade exchange. The exchange gateway and central server are implemented in cloud VMs, that are time synchronized using existing Huygen software. The orders received by the gateways are time stamped at the gateways, and sent to central server where they are globally ordered.

Reasons to accept
-----------------
The paper talks about interesting applications of time-sensitive networks.

Reasons to reject
-----------------
I could not fully appreciate the technical contributions of the paper.

Comments for author
-------------------
I found the introduction of the paper to be very exciting, and felt that the paper is targeting a very interesting problem. As I read on, I found the rest of the paper to be a bit underwhelming. The idea of grouping servers that must be time synchronized seems very natural, and I wasn't sure what's new and interesting about the notion of time perimeters. The idea of synchronizing clocks is also not new, and the paper uses existing software for it. The system architecture for cloudex is interesting, but the central idea there seems straight out of a distributed system textbook, and is probably something that is implemented on bespoke networks in trade exchange anyway. So I could not fully appreciate the core technical contributions of this work. Perhaps providing more background on the state-of-the-art might help.

Also, if the key contribution lies in using the cloud for trade exchange instead of a bespoke network, that would require more justification that what the current paper provides. While ensuring global FCFS is one requirement in exchange servers that could be achieved via efficient clock synchronization in the cloud, from what I have heard, having extremely low latency is also very important for high frequency trading.

==> scratch/intro.tex <==
\section{Introduction}
\label{sec:introduction}

% Intro:

% 1. Stock exchanges are important: 10 M new investors in 2020, etc.

% 2. They have unique fairness requirements:
% 2a. orders must be processed in order of gateway timestamp due to the requirements of continuous price-time matching.
% 2b. market data must be released simultaneously.

% 3. Today, the predominant *technological* solution for this is bespoke infrastructure
% - Throw a quick forward pointer to related work for *economic/market/financial* solutions like batch auctions, libra, etc.

% 4. At the same time, stock exchanges are considering moving to the cloud for several reasons:
% - more scale,
% - reduced management burden and cost (https://www.nasdaq.com/articles/amazon-pilot-lifts-stock-exchanges-into-the-cloud-2020-11-20),
% - COVID-induced remote work
% - fewer outages (based on the same link above)
% - the cloud seems primetime ready in terms of security, performance, etc.

% 5. The cloud is great for elasticity but is a best-effort infrastructure without great/any(?) QoS guarantees.
% -  no control over path selection
% -  noisy neighbors

% 6. This paper proposes a solution to the technical challenges of running a stock exchange in the cloud.
% (much of the current last paragraph in the intro can be reused for this).

% Outline
% Move to the cloud -> Benefits, Proof of migration
% Move to the cloud -> Downsides (at a high level)
% https://www.wsj.com/articles/new-army-of-individual-investors-flexes-its-muscle-11609329600#:~:text=More%20than%2010%20million%20new,in%20to%20bet%20on%20stocks

Equity and cryptocurrency markets have broadened availability of financial services to more than 10 million new investors in 2020 \cite{army-investors}. 


This rapid growth and the pandemic have added urgency to the ambitions of deploying scalable cloud financial exchanges. One of the world's largest exchanges, Nasdaq, plans to migrate all markets to public cloud infrastructure in the next decade~\cite{nasdaq-cloud, nasdaq}. 

% Background -> Auction mechanisms, data retrieval mechanism
% FCFS expectation - time/speed is important
% Measurement of network links, etc.
% Cite budish, libra sources
Most exchanges process market transactions using a ``continuous price-time matching'' algorithm~\cite{cptm}, which means that incoming buy and sell orders are transacted in a ``first come, first served'' (FCFS) order, within a central matching engine. Those who can react to market mispricings, news, or other forms of arbitrage faster than others have an advantage over other participants~\cite{budish2015high, johnson2012financial, keim2012nanosecond, schneider2012microsecond, ye2013externalities}. 


While the migration of exchanges into a public cloud environment ostensibly removes or reduces the impact of many technological advantages currently exploited (e.g., custom hardware and limited co-location facilities), the network delays between participants and the matching engine can be uneven, varying in time due to both the workload of other tenants as well as VM placement. 

Relinquishing the carefully-constructed datacenter fabrics in which exchanges currently operate and adopting the noisy, best-effort environment of public clouds imposes new challenges. A major concern and a point of financial regulation lies in meeting the expectation of an exchange to operate \textit{as fairly as possible} \cite{sheridan2017mifid}. Fairness in this context refers to both (1) processing market transactions according to the order they enter the exchange system and (2) releasing market data uniformly in time to all market participants.

This variation in network delays is known as a source of unfairness, allowing some participants orders to overtake others en route to the central matching engine. A major body of work to address this variability lies in altering the matching engine algorithm to remove its strict dependence on order arrival time. We review these approaches, among others, in Section \ref{sec:related}.

We consider a new path towards tackling unfairness in financial exchanges. Specifically, we leverage high precision (nanosecond-level) software-based clock synchronization to measure and monitor the delays between a matching engine and market participants. Using these measurements, we develop techniques to compensate for uneven network delays directly in exchange software and describe in detail  \sysname -- a prototype for a cloud-native yet fair-access financial exchange.  We present results from controlled experiments describing two main techniques we adopt -- dynamic delay threshold (DDT) and replicated order submission (ROS) -- showing how they improve the latency-fairness trade-off and mitigate the latency variation of \sysname. Additionally, we discuss our experiences and lessons learned in running \sysname with student participants in a week-long summer high-school program and in a quarter-long graduate university course.


% The search for speed has spawned a technological "arms race"~\cite{budish2015high} among participants whereby software/hardware are implemented to often shave microseconds or even nanoseconds off the response or transmission time of orders to an exchange.

% Prior work -> Looked at using auction mechanisms to mitigate the downside
% Solutions - matching engine policies
% Citations
% \ag{moved the paragraph that was here to related work at the end. Shrink main idea there to one sentence and possible refer to related work section for more info}

% This work -> Consider how to directly compensate for the inequities. Name the technologies used to do so
% A new approach - using high precision time synchronization we can measure the delays and their unevenness.
% Can compensate directly for the delays through the use of dynamic resequencing buffers and multiple gateway submissions
% Arms race in pursuit of speed
% Dissemination latency is gamed
% A new world - delays unexpected, time varying

% Here, we consider the problem of building high-performance stock exchange infrastructure in the public cloud. We present our preliminary experience in building CloudEx, an infrastructure for trading market and limit orders in the cloud. We discuss how scalable software-based time synchronization in the public cloud can serve as a very competitive substitute for custom-engineered on-premise infrastructure. We discuss our experiences and lessons learned in running this stock exchange with student participants in a weeks-long summer high-school program and a quarter-long course. We also present results from controlled experiments showing the latency, latency variability, and throughput characteristics of CloudEx.

% This work -> Consider how to directly compensate for the inequities. Name the technologies used to do so
% A new approach - using high precision time synchronization we can measure the delays and their unevenness.
% Can compensate directly for the delays through the use of dynamic resequencing buffers and multiple gateway submissions

% Consequences of this work -> Experience in deploying the system in two courses, develop two techniques to improve fairness and provide results to demonstrate their effectiveness
% We implement an exchange tailored towards specifically addressing issues that emerge from cloud exchanges.
% Deployment in courses, key metrics (trading and system statistics)
% We experiment with two techniques -- under controlled experiments we can achieve ... 




% Electronic stock exchanges fulfill a vital role in the world economy. They allow businesses to raise capital and individuals or institutions to share in the economic progress of these companies. Facilitating these transactions at scale is a distinct and understudied problem in systems research. These systems are distinct in that maintaining a global order on transactions that reach an exchange to the microsecond level.
% Electronic stock exchanges (e.g., NASDAQ, NYSE) are an integral part of the world's economy. Viewed as a systems problem, today's electronic stock exchange infrastructure needs to satisfy several requirements. First, they must provide low latency from the stock exchange to the market participants. Second, they must ensure low latency variability across different market participants. Third, they must be able to support an average load of ABC orders per second and a peak load of XYZ orders per second.

% % Would be good to check this statement on "the co-location facility being owned by the exchange."
% Electronic exchanges go to great lengths to meet these requirements. For instance, to lower latency from the exchange to all market participants, market participants are located in the same co-location facility as the exchange. The co-location facility itself might be owned by the exchange. Further, to equalize latency across participants, participants are connected to the exchange by cables of equal length, up to a tolerance of XYZ mm~\cite{?}.

% Recently, electronic exchanges have been contemplating a move to public cloud services~\cite{nasdaq, forbes}. Moving to the cloud lowers capital expenditure, both in terms of real estate and equipment costs. It also allows an exchange to support a larger number of market participants, without being constrained by the small size of a co-location facility.
% However, the cloud is a best-effort environment without strong guarantees on performance. In particular, an operator of the stock exchange may have to share a physical machine with other tenants of the cloud, has no control over the network paths from market participants to the stock exchange, and has to contend with heterogeneity of both the underlying compute and network infrastructure. As an analogy, this transition of exchanges from a bespoke on-premise infrastructure to the public cloud mirrors the transition of networks from a homogeneous circuit-switched infrastructure for telephone networks to a heterogeneous packet-switched infrastructure for computer networks.

% Here, we consider the problem of building high-performance stock exchange infrastructure in the public cloud. We present our preliminary experience in building CloudEx, an infrastructure for trading market and limit orders in the cloud. We discuss how scalable software-based time synchronization in the public cloud can serve as a very competitive substitute for custom-engineered on-premise infrastructure. We discuss our experiences and lessons learned in running this stock exchange with student participants in a weeks-long summer high-school program and a quarter-long course. We also present results from controlled experiments showing the latency, latency variability, and throughput characteristics of CloudEx.

%TODO: Can uncomment if we end up doing this.
% While we have used CloudEx as a prototyping vehicle, the techniques developed in CloudEx have broader relevance to other forms of matching infrastructure (e.g., multiplayer game participants interacting with a game server or ad bidders interacting with an ad exchange). We conclude with a set of open research challenges to inform subsequent research in the area of systems support for such matching infrastructure.

==> scratch/intro_old.tex <==
\section{Introduction}
\label{sec:introduction}
This paper considers problems in distributed systems where wall-clock time plays an important role in real-time decision making and control. The following three applications illustrate the problems.  {\em Autonomous vehicles.}  Based on data from image sensors, a central processor in a self-driving car needs to urgently convey control signals to the brakes.  The time from sensing to control must be tightly bounded; stale signals are of no value. {\em Trading exchanges.} To ensure fairness in order execution, an exchange must execute transactions from market participants connected to exchange gateways in a global FCFS manner, i.e., in the temporal order in which transactions entered their respective gateways. {\em Multi-player games.} A game server must periodically update players of the state of the game. For fairness, these updates must reach all players simultaneously. This requires holding updates at gateways and releasing them to players at the same time.

We call the above applications {\em time-sensitive applications} to emphasize the central role of wall-clock time. In order to support such applications, the network infrastructure must provide new functions such as jitter-free or deterministic messaging (for cars), a global FCFS ordering of events (for exchanges) and synchronized multicast (for games).  This requires different network locations to synchronize to a common reference time so that timestamps taken at these locations can be sensibly compared.  Timestamps from synchronized clocks enable a unique total order of events (up to synchronization error), unlike approaches such as vector clocks~\cite{lamport_clocks}, which only provide a unique partial order. These applications also require control nodes which can interpret the timestamps to take application-specific actions, e.g., executing market orders in global FCFS fashion or prioritizing fresher images for controlling a car.

Recognizing the needs of such applications, the IEEE and IETF have, respectively, proposed the Time-Sensitive Networking (TSN) framework for layer 2 Ethernet~\cite{tsn_8021_as} and the DetNet proposal for layer 3 IP networks~\cite{detnet}. The TSN standard specifies the Precision-Time Protocol (PTP) for clock synchronization of {\em all} network nodes~\cite{tsn_ptp}, the ability to reserve bandwidth for virtual communication channels with deterministic bandwidth and latency guarantees for time-sensitive messages~\cite{tsn_8021_qbv}, and management interfaces to a TSN network~\cite{tsn_8021_qcc}. The DetNet proposal seeks to broaden TSN's goals from a single LAN to a layer 3 network with multiple independently administered LANs with different link layers.
%It proposes techniques for reserving bandwidth, buffer space, and routes for time-sensitive messages~\cite{detnet_dataplane}.

By working at layers 2 and 3, TSN and DetNet take a network-oriented view of time-sensitive applications. Specifically, this means clock synchronization, deterministic messaging and resource reservation are available all the time and everywhere in the network---regardless of the application's actual needs. Such an ``always-on-everywhere'' approach ignores application semantics and also sets too high a bar. It limits scalability (in network size and geographic distance) and hinders deployability, particularly in virtualized environments (e.g., the cloud) where customers run applications in VMs and cannot access switches. Finally, for accuracy, PTP is implemented in hardware, requiring hardware upgrades. 

In contrast, we take an {\em application-aware} approach to time-sensitive applications. Our approach is based on an abstraction we call {\em time perimeters}, formally defined in Section \ref{sec:perimeters}. Time perimeters allow applications to decide which subset of network nodes need to be synchronized and allows them to dynamically change this subset, providing ``just-where-needed'' clock synchronization which scales with network size and geographic distance. It can also be implemented in software on end-hosts, allowing it to work in virtualized environments and without hardware upgrades.  Further, unlike TSN and DetNet, time perimeters leverage application semantics; for instance, each perimeter includes control nodes that can execute application-specific logic such as the FCFS sequencer in the exchange.  These control nodes can optionally use programmable data planes~\cite{pensando, tofino}.

Time perimeters can go beyond deterministic messaging to enable a bigger suite of time-sensitive applications. In Section \ref{sec:usecases}, we discuss several applications from distributed systems and networking that had been previously designed under a ``clockless assumption,'' such as guaranteeing external consistency of databases, event ordering in distributed systems, distributed tracing, synchronized logging, and congestion control.

\noindent{\bf{\em \sysname.}}  In Section \ref{sec:cloudex} we present a detailed case study of using time perimeters to build a trading exchange called \sysname in a public cloud. Exchanges have been actively considering a move to the public cloud; e.g., see Nasdaq's recent announcement~\cite{nasdaq, forbes}.\footnote{"In five years, we expect to have multiple Nasdaq markets running in the cloud, and in 10 years they will likely all be in the cloud."}  By building an actual exchange, with a matching engine and APIs where traders can submit their transactions and receive market data, our goal is to demonstrate that an important time-sensitive application can be built in the heterogeneous environment of the public cloud using time perimeters.  In addition, \sysname is a teaching and research tool. We have run \sysname with 52 high school students as market participants submitting high-frequency trades using \sysname's APIs.  As a research tool, it provides researchers a testbed to understand the role of matching algorithms (e.g., continuous price-time matching vs batch auctions) and market microstructures, and a way to analyze market data at the price level as well as at the infrastructure level.

In Section \ref{sec:evaluation}, we evaluate \sysname.  We find that \sysname can process about 15--20k orders per second with a sweet spot at 17.3K when fairness is addressed (Figure~\ref{exp01-performance}) with a median latency of \SI{172}{\micro\second} for orders and \SI{146}{\micro\second} for market data (Table~\ref{tb-owd}). We quantify order unfairness by the fraction of orders that are executed out-of-sequence at the matching engine and market data unfairness by the fraction of late market data, i.e., data received after a deadline by at least one gateway. The global FCFS resequencer in the matching engine reduces the order unfairness from 22.9\% to 0.3\% (Figure~\ref{exp01-upstream-fairness}), while the hold-and-release buffer at gateways reduces market data unfairness from 78.8\% to 5.8\% with a release deadline of \SI{500}{\micro\second} and 0.6\% with a release deadline of \SI{750}{\micro\second} (Figure~\ref{exp01-downstream-fairness}). The previous numbers are when there are 24 traders and 8 gateways; numbers for the 48 and 72 trader cases have also been obtained. Finally, we discuss optimizations that we are implementing to improve the throughput, latency, and fairness of \sysname (Section~\ref{ssec:futurework}).

We note that time perimeters do give up some performance for wider applicability. A bespoke network can deliver much better performance because all nodes are designed for a particular application and the application is tightly coupled with layer 2 or 3 primitives. On the other hand, time-sensitive applications on commodity cloud networks are subject to the cloud's throughput and latency constraints.  But, cloud networks now provide abundant bandwidth (10s of Gbit/s) and low latency (10s of microseconds), making them increasingly attractive for many time-sensitive applications. Further, the cloud provides independent benefits (ubiquitous availability, cost, elasticity and security).
% Could remove the availability, cost, elasticity sentence if that's obvious at this point.

==> scratch/methods.tex <==
\section{Methods}
\label{sec:methods}

Given a fixed computational environment, the goals of fair and fast delivery are inherently at odds. 

For fair delivery, we are concerned with the ordered dequeue of messages into a consuming application. One has the ability to wait out the network variations from our senders at the cost of larger queueing delays. Similarly, in synchronized delivery we can instruct all receiver queues to hold messages for a longer period of time, increasing the likelihood that the message reaches all receivers before the scheduled release of information.

For applications such as financial/ad exchanges, massively multiplayer online games, and multi-agent control, information is generated frequently, the capabilities of constituent senders/receivers are heterogeneous, and actions granted at any time fully or partially determine the state of the system in the future. In these cases, fair processing determines the fate of many or even all end users.

These considerations motivate the optimization of the trade-off between fairness and speed through the use of time-sensitive queues. We present two techniques, dynamic delay parameters and multi-gateway message submission, which we further evaluate in the context of an archetype application, \sysname, in Section \ref{sec:cloudex}.




% \Para{Rethinking distributed systems.} Many distributed systems operate under a clockless assumption:  the assumption that nodes in the system are not synchronized to a common clock. In the absence of synchronized clocks to coordinate actions at different nodes, distributed systems have to either rely on a global coordinator or message passing to achieve goals such as event ordering, consensus, consistency, and snapshots. Time perimeters allow us to rethink these distributed systems and design simpler solutions by offering synchronized clocks as a service where needed~\cite{liskov_clock_sync}. For instance, event ordering in distributed systems becomes much simpler in the presence of accurately synchronized clocks~\cite{lamport_clocks}, VMs at different network locations can be simultaneously snapshotted at a designated time without requiring coordination, and external consistency can be achieved without the expense of GPS clocks~\cite{true_time}. In effect, time perimeters make the clock synchronization algorithm responsible for coordination, so that the coordination problem can be solved once and reused across different distributed applications.
% %that use clock synchronization.

% \Para{Rethinking networking.} If the sender and receiver of a message are part of the same time perimeter, the receiver's timestamp can be subtracted from the sender's timestamp to get the message's one-way delay (OWD). 
% With enough such OWD measurements, and knowledge of the network topology, we can infer queueing delays in the network using network tomography from the edge~\cite{simon}. These measurements can also be used as a congestion signal in delay-based congestion control~\cite{vegas, fast}. Today, such protocols rely on inaccurate techniques to estimate OWD (e.g., dividing RTT by 2) or settle for RTT instead, which conflates forward and backward path congestion. Time perimeters also enable centralized control of small-scale clusters. An example is Fastpass~\cite{fastpass}, which used PTP for clock synchronization. Time perimeters provide a cheaper approach to implementing Fastpass. Finally, by separating control nodes and sensor nodes, time perimeters allow programmable packet scheduling at the control nodes~\cite{PIFO} based on non-local timestamps; e.g., the global FCFS resequencer in Section~\ref{sec:cloudex}. This contrasts with current scheduling algorithms, which can only use the node's own local time to make scheduling decisions.

% \Para{Monitoring microservices.} In a microservice architecture, different microservices within an application naturally run on different VMs, perhaps even at different locations. Synchronizing time at these nodes is critical to monitoring these applications. For instance, distributed tracing~\cite{dapper} tracks caller-callee relationships between a parent microservice and a child microservice called by that parent.  While this allows temporal ordering of events {\em in a single transaction} based on causality and work-arounds like clock-skew adjustment~\cite{clockskew_jaeger}, it does not allow comparison of events {\em across transactions}. Time perimeters would permit such inter-transaction comparisons.  Similarly, when logging statements~\cite{loggly} or tracking metrics~\cite{prometheus}, it is important to be able to correlate timestamps of logs and metrics across different locations, failing which logs and metrics become less useful~\cite{stackify_logging}.

==> scratch/time-sensitive-queues.tex <==
\section{Time-sensitive Queues}
\label{sec:perimeters}

Time-sensitive queues are distributed queues that rely on accurate clock synchronization across network nodes to provide time-related guarantees to message deliveries. In this section, we discuss two such guarantees: \textit{ordered delivery} (\S\ref{sub-sec:ordered-delivery}) and \textit{synchronized delivery} (\S\ref{sub-sec:sync-delivery}), explaining their definitions and use cases. These guarantees have to be maintained even if the underlying physical network suffers from latency variations both across sender-receiver pairs and across time for the same sender-receiver pair.

Many systems today rely on such guarantees for \textit{correct} behaviour, where correctness is dictated for example by user expectations (e.g., in multiplayer games \cite{xx}), or even by legal requirements (e.g., in financial exchanges \cite{xx}). In Section \ref{sec:cloudex}, we discuss our implementation of a fair cloud-native financial exchange (\sysname), explaining how we employ time-sensitive queues to provide necessary functionality for \sysname.

Time-sensitive queues are enabled by two key ideas: (1) accurately synchronized clocks that put senders and receivers on a common time axis, and (2) artificial delay applied at the receivers, which compensate for latency variations between different network paths. In Section \ref{sec:methods}, we further describe some techniques we devised to improve the performance of our time-sensitive queue implementation, especially as it relates to the existing trade-offs. 

% For clock synchronization, we use the recently 

\subsection{Ordered Delivery}
\label{sub-sec:ordered-delivery}
In \textit{ordered delivery}, we want to ensure that messages transmitted from multiple senders to some receiver are dequeued at the receiver in the same order as their \textit{transmission} order. 

To determine the transmission order, we timestamp the message at the sender before transmission. Then, at the receiver we use a priority queue outputting messages in the increasing order of their transmission timestamps. Moreover, to compensate for the latency variations across the network paths from the senders to the receiver, we add artificial delay at the receiver. We call this delay the ordered delivery delay parameter, $d_{order}$.
%[AG] More explanation here?

In many applications, ordered delivery is desired because it implies fairness. It does not allow a sender to transmit a message \textit{after} the other senders transmit theirs, yet also have the receiver process that message \textit{before} the other senders' messages. Such a behaviour would give that sender an unfair advantage in scenarios where senders compete on rewards by being the first to react to an event, e.g., reacting to market data in financial trading, or to state changes in multiplayer gaming.

\subsection{Synchronized Delivery}
\label{sub-sec:sync-delivery}
The goal of \textit{synchronized delivery} is to ensure that a message from a sender to a group of receivers gets released \textit{synchronously} by a specified deadline at all receivers. 

Similar to the ordered delivery case, we add artificial delay to deal with latency variations across the network paths from the sender to the receivers. We call this delay the synchronized delivery delay parameter, $d_{sync}$.
%[AG] More explanation here?

The synchronized delivery guarantee is often required by the same applications that also require the ordered delivery guarantee discussed above. Events that contain valuable information (e.g., financial market data or multiplayer game state changes) should be disseminated synchronously to the receivers so that no receiver can have unfair early access to such valuable information.

